Automatic and Efficient Customization of Neural Networks for ML Applications

ML APIs have greatly relieved application developers of the burden to design and train their own neural network models -- classifying objects in an image can now be as simple as one line of Python code to call an API. However, these APIs offer the same pre-trained models regardless of how their output is used by different applications. This can be suboptimal as not all ML inference errors can cause application failures, and the distinction between inference errors that can or cannot cause failures varies greatly across applications. To tackle this problem, we first study 77 real-world applications, which collectively use six ML APIs from two providers, to reveal common patterns of how ML API output affects applications' decision processes. Inspired by the findings, we propose ChameleonAPI, an optimization framework for ML APIs, which takes effect without changing the application source code. ChameleonAPI provides application developers with a parser that automatically analyzes the application to produce an abstract of its decision process, which is then used to devise an application-specific loss function that only penalizes API output errors critical to the application. ChameleonAPI uses the loss function to efficiently train a neural network model customized for each application and deploys it to serve API invocations from the respective application via existing interface. Compared to a baseline that selects the best-of-all commercial ML API, we show that ChameleonAPI reduces incorrect application decisions by 43%.

==> bk/0-abstract_0525.tex <==
ML-as-a-Service has greatly relieved application developers of the burden to train and run ML models---classifying objects in an image can now be as simple as one line of Python code to call an ML API. However, these APIs run the same ML models {\em regardless} of how their output is used by different applications. This can be suboptimal as not all ML inference errors can cause application failures, and the distinction between inference errors that can or cannot cause application failures varies greatly across applications.

To tackle this problem, we first study 77 real-world applications, which collectively use six ML APIs from two MLaaS providers, to reveal common patterns of {\em how ML API output affects applications' decision processes}. Inspired by the findings, we propose {\em \tool}, an optimization framework for ML APIs, which takes effect without changing the application source code. \tool provides application developers with a parser that automatically analyzes the application to produce an abstract of its decision process, which is then used to devise an application-specific loss function that only penalizes API output errors critical to the application. \tool uses the loss function to efficiently train a DNN model customized for each application and deploys it to serve API invocations from the respective application via existing API interface. Compared to a baseline that selects the best-of-all commercial ML API, we show that \tool reduces incorrect application decisions by  41\%.

==> bk/1-introduction_0523.tex <==
\label{sec:intro}

% \cc{Intro outline:

% - ml apis are popular. clean runtime interface is a key

% - however, currently same model is used for all applications. two issues: 

% ---- similar errors affect the same app differently
   
% ---- same error affects different apps differently
   
% ---- show the example here
   
% - this suggests room for improvement by customizing ml model

% ---- many similar prior attempts, but they dont fit the runtime interface or must change app code
   
% - our goal: without changing api runtime interface or app code, train ml to minimize wrong app decisions. we make two contributions.

% - 1. an empirical study to reveal common ways real apps use ml api (i.e., software context)

% ---- brag the breath of our study and highlight the key dimensions
     
% - 2. a new optimization framework that 

% ----(a) extracts common patterns from user code

% ----(b) autocreate a new loss function for training
     
% - putting our solution in the context: e.g., shares the goal with blazeit, but tailored to ml api setting, etc

% - eval highlight
% }

% \subsection{Motivation}





The landscape of ML applications has greatly changed, with the rise of ML-as-a-service (MLaaS) significantly lowering the barrier of application developers.
Traditionally, ML application developers manage ML models via standard libraries (\eg TensorFlow, PyTorch).
In contrast, MLaaS providers, including Google, Microsoft and Amazon, offer generic cloud-based ML APIs that simplify common ML tasks (\eg object detection, facial emotion analysis) to just one invocation of an ML API within a single line of code. 
These APIs thus give rise to a variety of ML applications on smartphones, tablets, sensors, personal assistants~\cite{9778241,9453402,10.1145/3555802,wan2021machine}.
% There have been an increasing number of software applications with the need of deploying deep neural networks (DNNs) to understand what is present in the input. Due to the heavy burden of designing and training such DNNs, many cloud service providers (\eg Google, Microsoft, Amazon) offer off-the-shelf machine learning (ML) APIs with clean and simple interfaces for software developers (\eg simply inputting an image and outputting a list of classes recognized by the ML models) to easily incorporate ML models into their software applications. 

These generic APIs ease the integration with applications;
% While the generic interface provided by these APIs eases their integration with  applications, 
however, it is suboptimal that they run the same ML models to serve all applications because different applications can use the same API in different ways.
% each application may use the same API in different ways.
This difference is particularly striking when applications use the ML API's inference result to make control-flow decisions (also referred to as \textit{application decisions} in this paper). 
Different applications may check 
the result of the same ML API using different control-flow code structures and different condition predicates, a process that we refer to as 
the application's {\em decision process} (see \S\ref{sec:empirical} for the formal definition).
% \hank{Can we change this to be specific about the problem we address?  I am thinking something about application control flow rather than just application decision making.  I worry that decision making sounds too vague, but control flow gets right to the technical matter. Alternatively, maybe we just say that application decision processes refers to control flow.}\shan{I am afraid it is too late to remove ``decision making'' :'-(, because it is mentioned like 1000 times in later sections. It definitely makes sense to find a place early in the Introduction to connect decision making with control flow.} \hank{Yeah, I think just saying at this point that application decision making refers to what ML API outputs are used in the branch conditions and how those branches are related to each other (or whatever is appropriate).}
Due to the heterogeneity across applications' decision processes, we make two observations.
% which are agnostic to how the API output may affect individual application's decisions (see \S\ref{sec:empirical} for the formal definition). 
% \hank{I don't think I know what agnostic means in this context.  Certainly our tool is going to extract the decision making process (control flow) from the application.  That feels like the opposite of agnostic---rather than say the control flow is unknowable, we are proposing to exactly categorize it.  And the two cases below are about distinguishing how the decision making process is affected by the ML API output.}
%\shan{Hank, can you proofread this paragraph?}
\begin{packeditemize}
\item First, some incorrect API outputs may still lead to correct application decisions, with only certain {\em critical errors} of API output affecting the application's decision.
% First, similar errors of ML API output (\eg misclassifying an image with different labels) may affect an application's decisions {\em differently}, with only specific errors being critical to each application's decisions.
% \shan{``Similar errors'' is not well defined -- what errors are similar; what are different? But I don't have good suggestion here.}
% \hank{Again, I think this becomes much clearer if this is application control flow rather than decisions.}
\item  Second, among all possible output errors of an API, which ones are critical {\em vary} significantly across applications that use this API. That is, the same API output error may have a much {\em greater} effect on one application than on another. 
%\hank{There are two types of errors that need to be distinguighsed and I think should be explicitly defined: application  control flow errors and ML API output errors.  I beleive the first point is that some ML API errors do not affect application control flow and thus do not manifest as application errors.  However, the same ML API error can have different affects on different applications, causing no error in one and a critical failure in another. }
\end{packeditemize}
%\jc{rephrased per Hank's comment to emphasize critical errors are different from (a subset of all) API output errors. Hank, pls proofread}
% However, nowadays, the ML models behind the ML APIs are the same across all software applications.

% In particular, we make two observations. 
% % Since all ML models make mistakes from time to time on cognitive tasks, including the ones adopted by ML APIs, using unifying ML models across applications can bring issues. 
% \begin{packeditemize}
% \item First, similar errors of ML API output (\eg misclassifying an image with different labels) may affect an application's decisions {\em differently}, with only specific errors being critical to each application's decisions.
% \shan{``Similar errors'' is not well defined -- what errors are similar; what are different? But I don't have good suggestion here.}

% \item  Second, these critical errors of ML API {\em vary} significantly across applications, so the same error may have a much {\em greater} affect on one application than on another.
% \end{packeditemize}

Figure~\ref{fig:input_example} illustrates the decision process of a garbage-classification application \code{Heapsortcypher}~\cite{heapsort}.
It first applies Google's classification API upon a garbage image. Then, based on the returned labels, a simple logic assigns the image to one of the pre-defined categories (\code{Recycle}, \code{Compost}, and \code{Donate}) or \code{others}. 
For this application, the assigned category is the {\em application decision}.
For an input image whose ground-truth label is \code{``Shirt''}, the correct application is \code{Donate}.
Figure~\ref{fig:input_example} (c) and (d) show two possible output label lists of the ML API, both of which have the {\em same} number of mis-classified labels, but have {\em different} impacts on the application decision. 
If the output is \code{``Paper''}, the application will choose the wrong decision, but if the output is \code{``Jacket''}, the application will choose the correct decision (\code{Donate}) despite not matching the ground-truth label.



% However, the generic ML APIs misalign with the software context, where a tiny ML API mistake could lead to severe software misbehavior. Thus, a solution is needed to adapt generic ML models behind ML API to fit the software's needs.
% \shan{This sentence needs rewording. Not clearly what it tries to deliver.}


% many software developers use off-the-shelf machine learning (ML) APIs  provided by many cloud service providers (\eg Google, Microsoft, Amazon) to reduce their development effort~\cite{wan2021machine}. 




% \yh{All ML models will make mistakes, but some errors made by the ML models will not change software behaviors. 

% Change the example 
% }

% \yh{
% For the same app, one error can have zero impact on its control flow, but some other errors can greatly change the control flow. Across apps, one error might have zero impact on its control flow, but for other apps, it might lead to wrong control flow 
% }

% To illustrate why some errors  made by the ML models may not lead the software executing wrong software components and vice versa

% \shan{This opening sentence is a bit odd: it seems to fit our OOPSLA submission better, don't you think so? Furthermore, even with your tool and ML APIs with increased accuracy, the software may still misbehave, right?}
% To illustrate how similar errors made by the ML models might have different impacts on a software application, we take a garbage classification application \emph{Heapsortcypher} in Figure~\ref{fig:app_example} as an example. It takes a trash image as input, and invokes \code{label\_detection}, Google's multi-label classification API, to get the labels describing image content. It then post-processes ML APIs' outputs into categories of garbage with three pre-defined lists, \code{Recycle}, \code{Compost}, and \code{Donate}. It examines the ML APIs' output classes, ranked with descending order of confidence scores, and searches for the first label that matches any of the labels in the three pre-defined lists. Finally, it executes the branch edge that corresponds to the found pre-defined list. Unless otherwise specified, the remaining paper refers to the decision of executing which ML-API-related if-branch edge as control flow decisions. 
% % \cc{How about this ``Unless otherwise specified, the remaining paper refers to the decision of ML-API-related if-branches as control flow decisions.''}

% Figure~\ref{fig:top_label_example} shows two types of errors that have different impacts on the software's control flow decisions. Given an image with a glowing jacket, whose human-labeled ground-truth class is ``Jacket'', the software is supposed to execute Line 12, as ``Jacket'' belongs to the corresponding \emph{Donate} list. We refer to the control flow decisions led by the human-labeled ground-truth as \emph{ground-truth control flow decisions}. Both of the errors mis-classifies the input image into a wrong class. On one hand, if ML API mis-classifies the jacket as ``Metal'', the software makes a wrong control flow decision of executing Line 8. On the other hand, if the ML API mis-classifies wrongly outputs ``Shirt'', the corresponding control flow decision still matches the ground-truth control flow decision.



% \shan{After I finished reading the above two paragraphs, I finally saw what you are trying to tell the readers. I guess you are trying to say that not all mistakes of an ML API are equally important for a software application. Is that what you are trying to say? You need to clearly present what messages you want to deliver BEFORE you present examples. You cannot ask readers to summarize/infer what you mean AFTER they read the example.}



% \kt{I would expect you saying this type of error is a common error. People do not directly care about the common usage pattern of ML API.}

% \cc{The old opening sentence seems duplicate to P2. Following is another version}
% Actually, such misaligning between ML API and the software is common in software applications querying ML APIs.

% The reason is that the ML APIs are optimized for generic accuracy over a large number of classes, and are unaware of which errors will change the control flow decisions of the software. 

As we can see, for a specific application, some errors of an ML API may be critical, like mis-classifying the shirt to \code{Paper} in the example above, and yet some errors may be non-critical, like mis-classifying the shirt image as \code{Jacket} in the example above.
Which errors are critical varies, depending on the application's decision process. 
For instance, if another application differentiates \code{``Jacket''} vs. \code{``Shirt''}, the API output of \code{``Jacket''} will still induce a wrong decision.
% \shan{I added this paragraph. Good?}\jc{looks great. did some minor twists}

These observations regarding the critical errors specific to each application suggest substantial room for improvement by customizing the ML API backend for individual application's decision process.
%\hank{Somewhere, perhaps here, I think we should mention that this is a natural tension.  Of course, skilled application developers would be able to design and train an ML model that works for just there application.  However, MLaaS exists because designing and training those models is beyond reach for many application developers.  So, this work keeps the accessibility of MLaaS while getting closer to the performance of a custom model. Could we add something like that?}
In particular, for a given application, the new backend can trade errors less critical to the application for fewer critical errors that cause wrong application decisions.
% errors made by the ML models have different levels of severity: some errors may lead to a different control flow decision than the ground-truth control flow decisions, while others may not. Also, the same error might have different impacts on different software's control flow decisions depending on how the software is specifically written. 
% Thus, this offers 
% an opportunity for the cloud service provider to take advantage of the software which reveals the different levels of severity of the errors, and adapt the ML models behind the API such that the errors that lead to incorrect control flow decisions can be greatly reduced. 

Thus, our goal is a solution for MLaaS that given an application, can {\em automatically} extract the application's decision process and customize the ML API backend to {\em minimize} incorrect application decisions {\em without} 
% offering the ML APIs to \textit{automatically} adapt the DNNs behind the ML API, so as to greatly reduce wrong application decisions led by ML APIs' predictions, \textit{without 
changing the application's source code or the interface of the ML API exposed to the developers.  This way, application developers who do not have the expertise 
to design and train customized ML models can still
enjoy the accessibility of MLaaS while getting closer to the accuracy of an ML model customized for the application. 
% \shan{I added the last sentence based on Hank's ``tension'' comment, which I like. How about it now?} \hank{I like it.}


% Failing to realize the issue that some errors may lead to incorrect control flow decisions might unavoidably include 

% Thus, instead of providing a generic ML API that could be applied to all software, an ideal solution is for the cloud service providers to adapt the ML models behind the APIs, while still remaining the API interface. In this way, the adapted application-specific ML models can be aware of the different levels of severity for their errors, and thus improve the rate at which the control flow decisions led by ML APIs' prediction match with those led by human-labeled ground-truth without any modifications on the  application's side. 
% the ML APIs are optimized for generic accuracy over a large number of classes, but the ML software has a different focus and priority. Particularly, software only cares about whether the ML API can produce outputs leading the software to making correct control flow decisions

% \shan{I think it is a bit too early to mention control flow here. Please think and rephrase.}

% The way the ML software is typically written 
%  \shan{?????What? Am I in the wrong paper? This sentence seems to fit our OOPSLA submission but does NOT fit here AT ALL. Your example so far is about wrong API result; it is NOT about accurate API result that leads to software failure. I am very confused.}. Specifically,  developers usually specify a subset of labels that they care about, such as \code{Recycle}, \code{Compost}, and \emph{Donate} lists, and how they use the labels, such as these three lists correspond to three software branches. Under such code patterns, ML API mis-predictions have different levels of severity: errors that lead to wrong software behaviors are more damaging than others\shan{No, it is not about which one is more damaging. Some mis-prediction simply has NO damage at all. Right?}. For example, in Heapsortcypher, the confusion within the lists, such as misclassifying a ``Food'' image to ``Produce'', is less damaging \shan{Again, when you say ``less damaging'', you are implying there exists some damage. But, that is not true here. mis-classifying food to produce has no damage to the software at all!} than across the list, such as misclassifying a ``Food'' image to ``Glass'', as only the latter would lead to a wrong control flow decision.


% to customize the DNNs behind ML API for each software, while keeping the same interface\shan{How do you define interface? If you really keep the same interface, how do you collect the software control flow information for the API provider?}. In this way, the ML API is aware of how the ML APIs' outputs affect the software behavior and is optimized to provide outputs that ensure\shan{no way you can ensure} software behaves as if the ground-truth of the input is returned by the ML APIs. Meanwhile, the developers would not be bothered to modify their software to fit the adaptation. 

% Existing work proposes solutions to improve the performance or accuracy of ML models in software applications. However, they either do not fit the interface of the ML API or introduce extra burdens for software developers. 

No prior work shares the same goal as us.
The closest line of prior work specializes DNN models for given queries~\cite{kang2018blazeit,kang2017noscope,koudas2020video,figo,cao2021thia}, but they require application developers to use a domain specific language (\eg in SQL~\cite{kang2018blazeit}) instead of general programming languages, like Java and Python, and mostly focus on reducing the DNN's size.
%The other line of work keeps current MLaaS interface, but unlike this work, they make no change to the backend implementation of ML API based on each application's decision process~\cite{chen2020frugalml,chen2022frugalmct,wan2021machine, wan2022automated}.
% Another line of work keeps the ML API interface, but either fails to incorporate application-specific software context~\cite{chen2020frugalml,chen2022frugalmct} or performs offline correction 
% % of API output on the user device in addition 
% to application source code~\cite{wan2021machine, wan2022automated}. 
In contrast, we keep both the ML API interface and the application source code intact while avoiding incorrect decisions for ML applications.

% \shan{Rewrote this paragraph. pls proofread.} \hank{Two minor fixes, otherwise good.}





% \jc{yuhan, does the above para convey what you wanted to say?} \yh{Yes}

% \shan{I find this argument very weak: the change required sounds very minimal and can be easily wrapped inside a library call. More importantly, I feel there are much more fundamental differences between your work and this previous work and yet you didn't mention.}


% \shan{Just like my comments in the abstract, I feel you still didn't make it very clear about your assumption. What is your assumption about what you have access to and what you can change? This assumption is VERY different from our OOPSLA submission, right? That is why you need to clearly explain your problem statement and assumption here.}

% In this work, we present \tool, which guides the cloud service provider to design the implementation of ML APIs that adapt DNNs behind, such that when the applications query the ML APIs, the incorrect application decisions can be greatly reduced. Automatic DNN adaptation to software context faces several challenges. 



% \emph{Firstly}, automatic model adaptation is hard. As software developers are typically non-experts in ML, we should not require the software developers to manually specify how to adapt the DNNs. An automatic way to construct the training dataset without  
% % To achieve such automatic adaptation, we need to understand how software uses ML API output label and the severity of different types of mis-predictions. We also need to translate this information to a DNN-understandable format for adaptation, such as a loss function, which is inherently hard due to rich code syntax. Furthermore, it is hard for software developers to provide training data for model adaptation


% \emph{Secondly}, model adaptation needs to be very efficient. 
% Since we need to re-train the ML model for each software application and software applications may change from time to time during the development procedure, model adaptation should be fast. 
% \shan{I guess we also assume that we cannot obtain new training data from application developers.}\cc{Agree with Shan. I think this could be put in first challenge, saying that we lack information of dataset and severity, due to the automation requirement}


% \begin{figure}
% \begin{subfigure}{0.45\textwidth}    
%          \centering
%          \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% Recycle = ['Plastic', 'Wood', 'Glass', 'Paper', 'Cardboard', 'Metal', 'Aluminum', 'Tin', 'Carton']
% Compost = ['Food', 'Produce', 'Snack']
% Donate = ['Clothing', 'Jacket', 'Shirt', 'Pants', 'Footwear', 'Shoe']
% image = types.Image(content=trash_image)
% response = client.label_detection(image=image)
% for obj in response.label_annotations:
%   if obj.name in Recycle:
%     return recycle(trash_image)
%   elif obj.name in Compost:
%     return compost(trash_image)
%   elif obj.name in Donate:
%     return donate(trash_image)
% return 'It is others.'
% \end{lstlisting}
% %          \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % Recycle = ['Plastic', 'Wood', 'Glass', 'Paper', 'Cardboard', 'Metal', 'Aluminum', 'Tin', 'Carton']
% % Compost = ['Food', 'Produce', 'Snack']
% % Donate = ['Clothing', 'Jacket', 'Shirt', 'Pants', 'Footwear', 'Shoe']
% % image = types.Image(content=trash_image)
% % response = client.label_detection(image=image)
% % Predictions = []
% % for obj in response.label_annotations:
% %   Predictions.append(obj.name)
% % if any([label in Recycle for label in Predictions]):
% %   return 'It is recyclable.'
% % elif any([label in Compost for label in Predictions]):
% %   return 'It is compostable.'
% % elif any([label in Donate for label in Predictions]):
% %   return 'It is donatable.'
% %     \end{lstlisting}
% \subcaption{The software implementation}
% \label{fig:app_example}
%     \end{subfigure}
%  \hfill
%  \begin{subfigure}{0.45\textwidth}  
%         \includegraphics[width=\linewidth]{figs/top_label_example.pdf}
%         \subcaption[]{Mis-classifying the class ``Plastic'' does not change the control flow decision. }
%         \label{fig:top_label_example}
%     \end{subfigure}
% \caption{HeapsortCypher, an application that classifies a garbage image. \cc{Maybe ajust the width and vertical position of the whitelist box} }
% \label{fig:app_example_entire}
% \end{figure}


% \subsection{Contributions} 
\begin{figure}
    % \includegraphics[width=1.3\linewidth]{figs/input_example.pdf}
    \includegraphics[width=0.9\linewidth]{figs/input_example_new.pdf}
    \tightcaption{An example ML application whose decision depends on the output of ML API (multi-label classification), but not all errors of ML API output have the same effect.
    % Heapsortcypher: a garbage classification application that uses Google's multi-label classification API to make application decisions. 
    }
    \label{fig:input_example}
\end{figure}

With the aforementioned goal, this paper makes two contributions.
% \begin{packeditemize}
%     \item We run an empirical study to reveal the common application-specific context, which makes it feasible to automate context extraction and ML model customization. 
%     \item We present a concrete solution to automate the process
% \end{packeditemize}
First, we run an empirical study over 77 real-world applications that collectively use six ML APIs to reveal several common patterns of how the outputs of ML APIs 
% to understand several common patterns of how the ML APIs' outputs 
affect the application decisions (\S\ref{sec:empirical}). 
% \shan{This opening sentence is toooo generic. I could have used it in all recent papers from our group. If I am a reviewer, I would wonder ``haven't people already conducted tons of study to understand how applications use ML APIs? Why do you need to study again?????''. What EXACTLY was not understood before and hence you want to understand?}
% we conduct an empirical study on a recently published ML software benchmark suite~\cite{wan2021machine}. 

Our study identifies two types of ML API output that are used by applications
to make {control-flow} decisions (categorical labels and sentiment
scores), and three types of decision types (True-False, Multi-Choice, and
Multi-Selection) with different implications regarding
which ML API output errors are critical to the application. 

Our study also
quantitatively reveals opportunities of model customization. (1) Although
popular image-classification models are trained to recognize as many as 
19.8K different labels, the largest number used by any one application for
decision making is only 54. Consequently, mis-classification among
the remaining tens of thousands of labels are completely irrelevant to an application. 
(2) More importantly,
% Apart from those irrelevant labels, 
applications tend to treat multiple labels (4.7 on average)
as one equivalence class in their decision making, such as labels
\code{Plastic}, \code{Wood}, \code{Glass}, \code{Paper}, and \code{Cardboard}
in Figure \ref{fig:input_example}(a).
Mis-classification among those labels inside one
equivalence class does not matter. (3) Which labels are relevant to an
application's decision making vary greatly
across applications, with only 12\% of application pairs share any labels used for their decision making.
% \shan{I have rewritten the above two paragraphs. Pls proofread.} \hank{Minor changes like equivalent--->equivalence}

%For instance, with a list of detected labels returned by ML API, the critical errors differ between two programs:
%{\em (i)} one matches the first label against a list of pre-defined ``whitelists'' (such as those in Figure~\ref{fig:input_example}(a)) and moves on to match the next label if the first label does not match any whitelist, and 
%{\em (ii)} the other matches the first whitelist against all returned labels and before moving on the match the next whitelist.
% We find four different code structure patterns of how ML software uses ML APIs' outputs to make control flow decisions, such that the same errors affect the decisions differently under these patterns (details are in Section~\ref{sec:empirical})\shan{Again, why isn't this already covered by previous work?}.  


Second, inspired by the empirical study, we propose \tool, which customizes and serves ML models behind the ML API for each given application's decision process, without any change to the existing ML API or the application source code (\S\ref{sec:method}). 
%\hank{Software context has not been defined yet.  If we stick with application decision making then we should use it again here.  or we replace it with control flow.  No need to introduce a new term here, though, unless we are using context to mean more than just the control flow information (including structure and labels).}\shan{Good catch! This should be decision making, not software context. Yuhan, can you search the paper for ``context''? This paper should not contain any ``context'' or ``software context'' phrase, a term that we decided not to use.} \yh{Removed software context. }
% , so as to increase the rate of correct software control flow decisions. 
\tool works in three steps.
First, it provides a simple parser that analyzes application source code to extract information about how ML inference results are used in the application's decision process. 
Based on the analysis result, \tool then constructs the loss function to reflect which API output is more relevant to the given application as well as the different severity of ML inference errors on the application decisions. 
The ML model will be retrained accordingly using the new loss function. 
Finally, when a query of the ML API is received in runtime, \tool dynamically redirects the query to the customized ML models based on the existing meta data in the query.
% Tackling the efficiency challenge, \tool adopts a fine-tuning approach to adapt the ML model behind ML API with minimum training costs.
% \shan{I like this paragraph, but clearer than earlier paragraphs.}


% We share similar goals with existing work performing model adaptation~\cite{kang2018blazeit,kang2017noscope}: constructing a specialized model that fits a specific context. However, they train specialized models that achieve much simpler tasks, expressed directly through their defined syntax, with compressed model sizes, while we aim at automatically extracting the context from the applications' source code and re-training the DNNs behind the ML APIs without changing DNN model architecture. 
% 

We evaluate \tool on 44 real-world open-source applications that use Google and Amazon's vision and language APIs.
We show that \tool's re-trained models reduce  51\% of incorrect decisions compared to the off-the-shelf ML models and 53\% compared to the commercial ML APIs. Even compared with a baseline that selects the best-of-all commercial ML API, \tool reduces 41\% of incorrect decisions. \tool only takes up to 21 minutes on a  GeForce RTX 3080 GPU to re-train the ML model.
% \shan{mention which machine you use to get this 21 minute result. 
% Using a super computer for 21 minute is different from 21 minute on a phone :P}
% \yh{updated this paragraph to make it more clear.}
% select the correct application decisions on XXX\% more input compared to the pre-trained models, and XXX\% more input compared to model trained on \tool's training data. 


==> bk/2-2-empirical_0525.tex <==
\label{sec:empirical}


We conduct an empirical study to understand how MLaaS applications
make decisions based on ML APIs (\S\ref{subsec:study-mech}), and how this
decision making logic implies the different severity of
ML inference errors (\S\ref{subsec:study-imp}).
This study will reveal why and how to customize the ML API backend for 
each application.



\tightsubsection{Definitions}
\label{sec:definitions}
% In addition, ML APIs are only loosely integrated into these applications, e.g., not interacting with other software components. We believe they do not represent the future direction of ML software.

% The 40 applications come from two sources: (1) 19 applications, which post-process the ML APIs' outputs to make control flow decisions, come from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}\shan{Why do you pick these 19?}; and (2) 21 applications come from GitHub by random checking around 60 applications\shan{What exactly are you looking for when you randomly check? Why don't you use all these 60?}.
% Among these applications, 29 use Google \code{label\_detection} API, and 11 use Amazon \code{detect\_labels} API.

% \cc{Maybe also add some statistics}



% \subsubsection{Test data selection}
% TO-DO
% \cc{It is weird to have a subsection that only has one subsubsection. How about we also introduce the open image data and ground-truth label?}


% \begin{figure}
%      \includegraphics[width=.95\linewidth]{figs/motivate_2examples.pdf}
%     \caption{Code snippets from two example applications. Branch conditions influenced by API output and the structures over the conditional branches are highlighted.}
% \label{fig:2examples}
% \end{figure}

% \jc{agreed with hank. moved the preamble to footnote1}
% \hank{It is extremely abrupt to go from this to just some definitions.  I think this concept of equally critical needs to be defined a bit more clearly and then there needs to be some transition sentence into definitions (maybe to better understand the class of applications that we do care about.}
% and hence there is little room for improvement by customizing the model for each application.

\mypara{Preliminaries} We begin with basic definitions.
% We first define the terminologies used in our paper.



% \begin{itemize}
%     \item \emph{Application decision}: the control flow decision of  which ML-API-related branch edge to execute
%     \item \emph{Conditional branches}: the lists of classes the application pre-defines in their source code, such that classes in these lists will lead to the same application decision. \yh{needs polish}
%     \item Selecting a whitelist $A$: the process of executing the branch edge corresponding to whitelist A
%     \item Selecting \code{others}: the process of executing the branch edge for not selecting any \wls
%     \item \emph{Ground-truth decision}: the application decision led by the human-labeled ground-truth of the input
% \end{itemize}


\begin{packeditemize}
    % \item {\em ML API output:} the output of the MLaaS in response to the invocation of a single input, \eg a list of classes describing the content of an input image or the scores indicating the sentiment of the input text.\shan{Junchen, can we remove this definition? Seems unnecessary.}
    % \item \emph{Conditional branches}: the branch conditioned on the API outputs 
    % \item \emph{Branch conditions:} once the application receives the API output, it uses the branch conditions to decide which branch or branches to execute based on the API outputs. \hank{Note that this is not a definition of branch conditions.  }\shan{I suggest we remove this definition. I see no point of defining what are ``branch conditions'' :'-).}
    % \item \emph{Target-edge:} the branch edge that is executed when the API outputs fulfill a branch condition.%predicate of containing certain values. It typically is the edge following \code{then} statement.
    % \item \emph{A-edge}: for applications that compare API outputs with arrays of classes (\eg \code{A, B, C}), we refer to the Target-edge that is executed when the branch condition using array \code{A} is fulfilled as \emph{A-edge}.
    % \item \emph{Otherwise-edge}: the edge that is executed when none of the Target-edge is executed. 
    % \item \emph{Fall-through edge}: The non-target edge of a branch.
    % \item \emph{Path}: A feasible combination of edges of all conditional branches.
    % \item \emph{Target-path}: A path that contains at least one target edge.
    
    % % \item \emph{Whitelist}: A whitelist is a set of all ML API outputs that lead software to execute its corresponding whitelist-path.
    % \item \emph{Otherwise-path}: A path without any target edge. \cc{Please feel free to remove any concepts that are needed}
    \item \emph{Application decision}: 
    the collective control-flow decisions (i.e., which branch(es) are taken) made by the application under the
    influence of a particular ML API output.
    \shan{I rewrote this definition, as in the old version, ``branch'' seems
    a bit come out of blue.}
    %the branch or branches whose branch conditions are satisfied.
    % \footnote{Here, it is implicitly assumed that an application decision only depends on the ML API output on the current input, not previous API output. While this may not be universally true, it holds for all the applications that we have studied. \hank{I don't follow what is going on in this clarification. What is a current input versus a previous input?  It seems like there are some unstated assumptions here.}}
    % \item {\em Target class:} a set of ML API outputs that lead to the same application decision. \jc{need to revisit after Shan makes a pass in 3.1/3.2}
    % the decision of which \emph{Target-edge} or \emph{Otherwise-edge} to execute. 
    % \item Selecting a whitelist $A$: the process of executing the branch edge corresponding to whitelist A
    % \item \emph{ML API error}: 
    \item {\em Incorrect ML API output:} 
    a situation when the API output differs from the API input's human-labeled ground truth.
    We refer to such ML API outputs as {\em API output errors}.
    
    
    \item \emph{Correct decision}: the application decision if the API output is the same as the human-labeled ground-truth of the input. 
    
    \item \emph{Application decision failure}: a situation when the application decision is different from the correct decision, also referred to as \textit{application failure} for short in this paper.
    % \item \emph{Critical errors}: the errors that lead the application to execute edges different from the ground-truth decisions.
\end{packeditemize}


\mypara{\Process}
Given these definitions, an application's {\em \process} (or decision process for short) is the logic that maps an ML API output to an application decision. 
The code snippet in Figure~\ref{fig:input_example} shows an example decision process, which maps the output of a classification ML API on an image to the image's recycling categorization specific to this application.

\mypara{Critical and non-critical errors}
For a given decision process, some API output errors will still lead to a correct decision, whereas some API output errors will lead to an incorrect decision and hence an application failure.
We refer to the former as {\em non-critical errors}, and the latter as {\em critical errors}.
%\jc{rephrased. Hank, pls proofread}
% Importantly, each software decision process decides whether an ML API error is critical or not. When an erroneous ML API output leads to 
% the ground-truth decision (defined above), this error is 
% {\em non-critical}; when it leads to a decision different from the correct decision (\ie an application decision failure), it is {\em critical}. 
%\hank{I found this a little confusing.  The text seems to imply that the application makes this distinction between critical and non-critical errors, but that is not the case right?  Does our tool do this or is it just a philosophical distiniction?}




% As we will see, the key is that {\em not} all errors are critical and that the critical errors {\em vary} across applications (using the same ML API) due to their different application decision processes.
% %Thus, each application's decision process, if used carefully, could be leveraged to improve ML API output to reduce wrong application decisions. 
% In the remainder of the section, we first present a systematic taxonomy of application decision processes and then apply the taxonomy to analyze a range of real-world applications using commercial MLaaS ML APIs.
% %However, to unleash such potential in practice, we first need a deep understanding on the software contexts of various applications using real MLaaS {\em in the wild}.
% In this empirical analysis, we focus on two central questions:
% \begin{packeditemize}
% \item Among applications using the same ML API, how much they differ in their application decision processes, and 
% \item Despite the application heterogeneity, whether common patterns emerge which might allow extraction of information regarding an application's decision process.
% \end{packeditemize}



% \begin{figure}
%      \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
%     \caption{Key dimensions that differentiate the code structures. The decision nodes (in blue) are key dimensions. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
% \label{fig:hierarchy}
% \end{figure}



% \begin{figure*}
%      \includegraphics[width=\linewidth]{figs/code.pdf}
%     \caption{Code snippets from four example applications. Branch conditions influenced by API output and the structures over the conditional branches are highlighted.\cc{TODO: fix citation}}
% \label{fig:code}
% \end{figure*}




%\tightsubsection{\hspace{-0.2cm} How ML API affects conditional branches}
\tightsubsection{Methodology}
\label{sec:methodology}
%\tightsubsection{Taxonomy on how ML APIs affect application decision process}
 
\begin{table}[]
\begin{footnotesize}
   \begin{tabular}{@{}lllr@{}}
\toprule
ML API name          & ML task              & Provider & \# of apps \\ \midrule
label\_detection     & Vision::Image classification & Google           & 29         \\
detect\_labels       & Vision::Image classification & Amazon           & 11         \\
object\_localization & Vision::Object detection     & Google           & 8          \\
analyze\_sentiment   & Language::Sentiment analysis   & Google           & 14         \\
analyze\_entities    & Language::Entity recognition   & Google           & 6          \\
classify\_text       & Language::Text classification  & Google           & 9          \\ \bottomrule
\end{tabular} 
\end{footnotesize}
\tightcaption{Summary of applications used in our empirical study. }
\label{tab:all_stats}
\end{table}

Our work focuses on applications that use ML API output to make control-flow decisions. 
To this end, we look at 77 open-source applications which collectively use six widely used vision and language APIs~\cite{wan2021machine, chen2021did} offered by two popular MLaaS providers, as summarized in Table~\ref{tab:all_stats}. 

These applications come from two sources. First, we study all  50 applications that use vision and language APIs from a recently published benchmark suite of open-source ML applications~\cite{wan2022automated}. Second, given the popularity of image classification APIs~\cite{chen2020frugalml,chen2022frugalmct}, we additionally sample 27 applications from GitHub 
that use Google and Amazon image classification APIs
(16 for the former and 11 for the latter). We obtain these 27 by checking close to 100 applications that use image classification APIs and filtering out those that directly print out or store the API output.
Every application in our benchmark suite uses exactly one ML API for decision making. 

\mypara{Threats to validity} 
While many applications use the APIs listed in Table~\ref{tab:all_stats}, there are a few other APIs not covered in our study. 
Speech APIs are not covered, because their outputs are rarely used to affect application control flow based on our checking of open-source applications.
%\footnote{A recent empirical study~\cite{wan2021machine} shows 93\% of their studied applications that use speech APIs only use the API outputs to affect data flow.}
% Speech APIs are not covered in our study, as speech applications tend to only use ML API to affect software data flow (around 93\% in a recent empirical study~\cite{wan2021machine}\shan{How do you get this number? Unless this is from a previous work, you have to explain what is the denominator and how you get it.}\cc{Done}).\jc{93\% over what? also does ``data flow'' mean displaying or storing results?} \cc{93\% of applications that uses Speech API in this empirical study. Data flow means that API output value affect the values of other variables in the software. It is slightly larger than the scope of directly displaying and storing}
A few other vision and language-related APIs (\eg face recognition and syntax analysis) are not covered in our study, and neither are applications that use APIs similar to those in Table~\ref{tab:all_stats} but provided by other MLaaS providers (\eg Microsoft Cognitive Service and  IBM Cloud Watson).
We leave it to future work to extend our methodology to other ML tasks and API providers.

\begin{comment}


% they account for less than 14\% of the applications in
% and API providers (\eg Microsoft Cognitive Service and IBM Cloud Watson).
There are also vision and language APIs that are not 
covered in our study, including text recognition, face detection, and syntax analysis\shan{why not?}\cc{Done}. 
Our methodology of analysis could also be applied to other ML tasks (\eg face recognition) and API providers (\eg Microsoft Cognitive Service and  IBM Cloud Watson). We leave that to future research.
% We omit them as they either are a specialized version of the studied ones \cc{face detection could be regarded as a special case of object detection}, or do not provide categorical results\jc{didn't we handle more than categorical results (e.g., emotion analysis)?}, or are less frequently used by developers. Finally, there are ML APIs offered by other providers like Microsoft Cognitive Service and  IBM Cloud Watson. These APIs are used
% not as often as Google and Amazon APIs in GitHub while having similar interface and functionality~\cite{wan2021machine, chen2021did}.
% \jc{isn't Microsoft API included in the evaluation? please update the text} \yh{The apps are using Google API, though we add Microsoft API to test their accuracy for comparison}

\end{comment}

\tightsubsection{Understanding the decision mechanism}
\label{subsec:study-mech}

\begin{figure*}
\centering
     \includegraphics[width=0.99\linewidth]{figs/code-v4.pdf}
    \tightcaption{Code snippets from five example applications where ML API output affects control flow decisions in different ways.}
\label{fig:code}
\end{figure*}

% \begin{figure}
% \centering
%      \includegraphics[width=0.99\linewidth]{figs/code-v5.pdf}
%     \caption{Code snippets from five example applications where ML API output affects control flow decisions in different ways.}
% \label{fig:code}
% \end{figure}


% For example, image classification and text classification APIs output categorical labels, and confidence scores for the predictions, to describe the inputs. Sentiment analysis API outputs a sentiment score and a magnitude\footnote{The magnitude is used to disambiguate mixed emotions when the sentiment score is close to 0. } to indicate the sentiment of the input. Object detection API output a label, a confidence score, together with the bounding boxes coordinates, to describe the detected objects.  


\emph{\textbf{Q1}: {What types of ML API outputs are typically used by applications to make decisions? } }



ML APIs produce output of a variety of types.
The sentiment analysis API outputs a list of floating-point value pairs (\code{score} and 
\code{magnitude}), describing the sentiment of the whole document and every individual sentence; the other five APIs in Table \ref{tab:all_stats} each 
produces a list of categorical labels ranked in {descending} order of their confidence scores, which is also part of the output. Some APIs' output also 
contains other information, like coordinates of bounding boxes, 
entity names, links to Wikipedia URLs, and so on.
%associated with each label.The entity recognition API (\code{analyze\_entities}) outputs a set of information for each entity identified from the input text, including the entity type in the form of a categorical label, the entity name, a salience score indicating the importance, and some meta-data (\eg link to Wikipedia URL). 
Among all these, only two types have been used in application decision processes of our studied application: the floating-point pair (\code{score} and \code{magnitude})
and the categorical labels.
%(\code{label\_detection}, \code{detect\_labels}, \code{classify\_text}, \code{object\_localization}, \code{analyze\_entities}).
%Other types
%such as confidence scores, bounding box coordinates, salience score and meta-data information
%are \textit{never} used.

For the 63 applications that use categorical-label output from the five APIs (all except \code{analyze\_sentiment} in Table \ref{tab:all_stats}), they each define one or more {\em label lists} and check which label list(s) an API output label belongs to. 
The code snippet of a landmark classification application in Figure~\ref{fig:code}(a) is an example of this. 
It calls MLaaS with a sight-seeing image and checks the output labels to see if the image might contain \code{Landmark}, or just ordinary \code{Building}, or \code{Person}.
% \jc{i moved the label-based api upfront, since it's what most ensuing discussions use}

For the 14 applications that use the \code{analyze\_sentiment} API, they each define several \emph{value ranges} and check which range the sentiment
\code{score} and/or \code{magnitude} falls in. 
The code snippet of  \code{FoodDelivery}~\cite{food-delivery}
in Figure~\ref{fig:code}(b) is an example.
This application calls \code{analyze\_sentiment} with a restaurant review text, and then checks the returned
sentiment \texttt{score} to judge if the review is negative, positive, or neutral.
% This application calls MLaaS with a text sentence and receives a sentiment score as the ML API output. 
% It uses three branch conditions, each checking if the API output score lies in a certain range.  



  
\emph{\textbf{Q2}: What type of decisions do applications make?} %\term{True-False}, \term{Multi-Choice}, or \term{Multi-Select}?}

We observe three categories of ML-based decision making, 
which
%depending on how many choices are presented and how many selections are allowed. 
we name following common question types in exams:

(1) \term{True-False} decision, where a single label list or value range
% \shan{TODO: terminology} 
is defined and one selection is allowed: either the ML API output belongs to this  list/range or not.
This type occurs in about one third of the applications in our study. 
For example, the plant management application \code{Plant-watcher}~\cite{plant-watcher} (Figure~\ref{fig:code}(c)) checks to see if the image contains plants or not.


(2) \term{Multi-Choice} decision, where 
multiple
lists of labels or value ranges are defined, and one selection is allowed.
The ML API output will be assigned to \emph{at most one} list or range; the application's decision making logic determines which of these lists/ranges the output belongs to, or determines that the output belongs to none of them.
This type of decision is the most common, occurring in about 45\% of benchmark applications.
%, with 3 being the median number of \targets.
% 3.0 target classes on average (3 as the median)
% \shan{``Other'' is not counted as a target class, right?} \yh{No, we don't count other as a target class.}. 
The garbage classification application discussed in \S\ref{sec:intro} makes such a \term{Multi-Choice} decision. 
It decides which one of the following classes the input image belongs to:
\code{Recycle}, \code{Compost}, \code{Donate}, or none of them. 
% The code snippet of this \term{Multi-Choice} decision making is shown in . 


(3) \term{Multi-Select} decision, where multiple label lists or value ranges are defined, and {\em multiple} selections are allowed about which label lists or value ranges the ML API output belongs to. 
This type of decisions occur in close to a quarter of the applications.
%, with two being the median number of \targets (3.0 being the average).
% 3.0 target classes on average (2 as the median).
Figure~\ref{fig:code}(d) illustrates such an example
from the nutrition advisor application \code{The-Coding-Kid}~\cite{coding-kid}. 
This application defines three  label lists to represent nutrition types: \code{Protein}, \code{Grain}, and \code{Fruit}, and it checks to find all the nutrition types present in the input image.

In the remainder of the paper, we will use {\bf \target} to refer to a label list (or a value range) that is used to match against a categorical label (or a value). 
For instance, the code snippet in Figure~\ref{fig:code}(a) has three label lists as its \targets (\code{[Landmark, Sculpture]}, \code{[Building, Estate, Mansion]}, and \code{[Person, Lady]}), and the code snippet in Figure~\ref{fig:code}(b) has three value ranges as its \targets (\code{<0.3}, \code{>0.6}, and in between).



%Across these three types of decisions, an ML inference error (\eg misclassifying an image) naturally might affect the application decision (and is thus more critical) if the error involves some \target. For instance, the ground-truth labels of an image overlaps with some \target but such overlap is not present in the detected labels. Or the ground-truth labels have no overlap with any \target, but some overlap is present in the detected labels.
% \jc{is this number repetitive?}. 
%Alternatively, if an inference error on an image does not involve a label in any \targets), the error 
% If an image's ground-truth labels do not belong to those non-target ones, an inference error 
%is unlikely to change the application decision. 
% On the contrary, if an image's ground-truth label belongs to a target class, an inference error is much more likely to change the application decision.


%\emph{\textbf{Implication}:} Given these observations, it is possible to build automated tools that extract this information and then pass that on to the MLaaS infrastructure for customization of ML models---all without any additional user input. \jc{replaced it with Hank's suggested text, pls proofread}

\begin{comment}
There are great opportunities to improve application decision accuracy by customizing ML models behind MLaaS APIs, as long as we know what type of decision and what target classes are there in an application. 
\end{comment}
%\hank{Again, slight rephrasing might make the point much stronger.  This study implies that there are a relatively small and well-defined set of patterns that are present in software that calls ML APIs.  Given these observations, it is possibl to build automated tools that extract this information and then pass that on to the MLaaS infrastructure for customization---all without any additional user input. In other words, "we" don't need to know the type of decision---our tools do and those tools can get the info automatically.  }


\emph{\textbf{Q3}: How do applications reach \term{Multi-Choice} decisions?
}

When the ML API outputs multiple labels, the outcome of a \term{Multi-Choice} decision varies depending on which {\em matching order} is used.
First, the matching order can be determined by the API output. 
For example, the garbage classification application
(Figure~\ref{fig:input_example})
%matches the API-output labels in the descending order of their associated confidence score. 
%It 
first checks whether the first label in the API output matches any \target. 
If so, later API output labels will be skipped, even if they might match with a different class. 
If there is no match for the first label, the second output label is checked, and so on. These labels are ranked by the API in the descending order of
their associated confidence scores, so we refer to such a matching order as
\term{API-order}. It is used by 80\% of applications that make \term{Multi-Choice} decisions.

The matching order can also be specified by the application, referred to as \term{App-order}.
For instance, 
%examine each element one by one against the conditional branches (\ie examining the $1^{\textrm{st}}$ element in API output against all branch conditions before moving to the $2^{\textrm{nd}}$ element, and so forth) or examine all elements against each conditional branch (\ie examining all elements against the $1^{\textrm{st}}$ branch condition, then all elements against the $2^{\textrm{nd}}$ condition, and so forth). 
% For instance, the land-mark application \code{Aander-ETL} uses \term{application-choice} order. As shown inin Figure~\ref{fig:code}(a), 
regardless the API output, application \code{Aander-ETL}~\cite{aander-etl} (Figure~\ref{fig:code}(a)) always first checks if the \code{Landmark} class matches with \emph{any} output label.
If there is a match, the decision is made. Only when it fails to match
\code{Landmark}, will it move on to check the next choice, \code{Building}, and so on.
This matching order is used by 20\% of applications that make \term{Multi-Choice} decisions.



%\emph{\textbf{Implication}:} 
%To best customize ML models for an application that makes \term{Multi-Choice} decision, one also needs to know the order in which the branch conditions are checked against ML API output.
% decision making mechanism underneath. 

 

\tightsubsection{Understanding the decision implication}
\label{subsec:study-imp}

%\shan{I will work on this sub-section tomorrow.}

\emph{\textbf{Q4}: Does an application need ML APIs that can accurately identify thousands of labels?}

ML models in MLaaS are well trained to serve different applications. For example, Google and Microsoft's image-classification APIs are capable of identifying more than 10000 labels \cite{openimages}, while
Amazon's image-classification API can identify 2580 labels \cite{amazon-label}. However, 
for each individual application, its decision making only
requires classifying the input image into a handful of \targets: 7 at most
in our benchmark applications. The largest
number of image-classification labels checked by an application is 54, a tiny
portion of all the labels an image-classification API could output.

Clearly, for any application, a customized ML model that focuses on those
\targets used by the application's decision process has the potentially to
out-perform the big and generic ML model behind ML APIs. How to accomplish the
customization without damaging the accessibility of MLaaS will be the goal of \tool.

%These three types of decisions show similar potential to benefit from ML model customization: they all only define a handful of \targets (7 at most across all applications in our study), 
%The average number of decision classes in Multi-Choice and Multi-Select decisions is 2.7, with the median being 2\shan{Please fill. I refer to a conditional branch as one class. For example, the four applications in Figure 2 all have 3 choice classes.}\cc{Done}. much smaller than the number of classes in a typical classification training dataset (\eg 19.8K classes in Open  Images V4~\cite{openimages} or 1K classes in ImageNet~\cite{5206848}). 
% For example, image-classification and object-detection APIs each can output 19.8K and 600 different categorical labels~\cite{openimages}.
% \jc{won't reviewer question if google api really uses openimages classes?}
%In contrast, at most 54 categorical labels are included in the \targets across all benchmark applications.


\emph{\textbf{Q5}: Are there equivalence classes among ML API outputs in the context of application decision making?}




For the 63 applications that make decisions based on API output of categorical labels, they present 121 \targets in total, each containing 4.7 labels on average (3 being the median). Only 35 \targets in 22 applications contain a single label.
% \shan{TODO: terminology}
For the 14 applications that make decisions based on floating-point sentiment \code{score} and \code{magnitude}, their \targets \emph{all} contain an infinite number of \code{score} or \code{magnitude} values. In other word, no class contains just a single value. 

Clearly, the wide presence of multi-value \targets creates equivalence classes among output returned by the API---errors within one equivalence class are \emph{not} critical to the corresponding application. This offers another opportunity for ML customization. 

%\emph{\textbf{Q5}: How many decision classes (i.e., choices) are presented?} 
 



\emph{\textbf{Q6}: How much difference is there between different applications' \targets?} 
 
Overall, the difference is significant. We have conducted pair-wise comparison
between any two applications in our benchmark suit, and found that 88\% of 
application pairs share \emph{no} common labels in any of their \targets. 
%Note that, we did not pair applications that use vision APIs with applications that use language APIs together for fair counting.
%Specifically, among all 826 pairs\footnote{We separately count the pairs for the 40 Vision tasks and 5 NLP entity recognition task, and 9 NLP text classification tasks as they do not share label sets.} of applications with branch conditions based on categorical label output of ML APIs, 88\% of them share no common labels
%in their branch conditions (723 out of 826 pairs). \hank{Maybe it is my covid brain, but it took me a while to figure out why we suddenly have application pairs.  I think that needs some more explanation assuming my brain fog is equivalent to a distracted reviewer.}
%71 of them overlap by more than one label between their target-class lists\shan{how many has one label overlap?} \yh{103 has one label overlap}. 
Similarly, among the 381 labels that appear in at least one application's 
\targets, 88\% of them appear in only one application
(\ie 335 out of 381 labels).
%only 16 of them appear in more than three applications\shan{how many appear in two applications?} \yh{46}.

Clearly, there is {\em little overlap} among the \targets of different applications, again making a case for {\em per-application} customization of the ML models used by the ML APIs. 
%\hank{Is it overlap between branch conditions or the targets (or label sets or something)?  I would htink there is no overlap between branch conditions, but that is not the point, it is the overlap between the labels that matters for this point.}


\emph{\textbf{Q7}: Do different decision mechanisms imply different sensitivity to output errors of ML APIs?}

Even for two applications that have the same \targets, if they try to make
different types of decisions,
they will have different sensitivity to ML API output errors---some 
 API errors might be critical to one application, but not to the other.
For example, errors that affect the selection of different \targets are equally critical to \term{Multi-Select} decisions. 
However, this is not true for \term{Multi-Choice}, where only the first matched \target matters.
% only one target class can be matched. 
%We will dig deeper into this phenomenon for \term{Multi-Choice} decisions next in our study of Q3. Furthermore, only inference errors related to the single target class in \term{True-False} decisions are critical. %\shan{anything else?} 
% As we can see, the exact implementation of 
Furthermore, the matching order of a \term{Multi-Choice} decision affects which errors are critical.
When the \term{API-output} order is used (\eg \code{HeapsortCypher} in Figure~\ref{fig:input_example}), an error on the first label in the API output is more likely to be critical than an error on other labels in the output.
However, when \term{App-order} order is used (\eg \code{Aander-ETL} in Figure~\ref{fig:code}(a)), errors related to labels in the first \target (\eg \code{Landmark}) are more likely to be critical than those related to labels in later \targets (\eg \code{Person}). 
%\hank{How can an error be more or less critical?  Critical typically implies binary: either critical or not, I am not sure what it means to be more critical.  Do we need a notion of error priority?}
%\shan{Good point. Indeed, actually our definition of ``critical errors'' meant to be binary as well. Maybe, we can say ``more likely to be critical'', 
%instead of ``more critical''?}
%\jc{fixed. pls proofread}

Clearly, to customize ML models for each application, we need to take into account what is the decision type and what is the matching order (for \term{Multi-Choice} decisions). 

% \jc{TODO: add a summary of the observations}

%Similarly, the structure over the conditional branches also varies greatly across applications, though four common patterns are enough to cover them. Out of the applications we study, 32\% of applications are T-or-F, 23\% of them fall into the pattern of M-to-N-set, 8\% of them are Priority-list, and the rest of them are Top-label.
% \jc{a few words on this}
%\end{packeditemize}



% \mypara{An empirical study over real MLaaS applications}
% % Given the rich syntax that can be expressed by Python, critical errors for applications in the wild can be very different.
% % To understand common types of software context that affect the application decisions, we first perform 
% To this end, in the remainder of this section, we run an empirical study over 78 open-source applications  whose application decisions 
% % control flow decisions 
% which collectively use \fillme ML APIs.
% These applications are from a recently published benchmark suite~\cite{wan2021machine}~\footnote{
% We ignore applications that directly print out the ML API outputs or store these outputs without post-processing, and thus by definition any errors of API output will be critical.
% % The tasks that these applications perform are the same as the task of ML API. Therefore, there is no need to adapt APIs to software. 
% }. 
% These applications cover a wide range of use cases, from \fillme to \fillme. 



% % Google (benchmark, search), AWS (search)

% % \begin{definition}[Application decision]\label{def:app_decision}
        
% % \end{definition}

% % These applications compare the ML API's output classes with the applications' pre-defined lists of classes, and decide which if-branch edge to execute. We refer to this process as making \textit{application decisions} and the pre-defined lists of class as \wls. 


%%%%%COMMENT OUT%%%%%%%%
%\end{packeditemize}

%We summarize the aforementioned structures of the branch conditions into the following four application categories. 

%For each of these applications in our study, its software context is determined along two dimensions
% An application decision process can be characterized in two dimensions:
% Two application decision processes may differ along one (or both) of the following dimensions:
% {\em (i)} how each branch condition uses ML API output, and
% {\em (ii)} how the conditional branches are structured.


% \yh{be more precise about the titles, ask questions, define it and measure it }

% \mypara{Two types of API output-based branch conditions}
% % We identify two types of conditional branches
% Figure~\ref{fig:2examples} shows an illustrative example for each.
% %\item{\em Class lists:} 
% The first type is used when the API output is a label or a list of labels, and several pre-defined {\em class lists} are then used to check if the API output labels belong to which list.
% The code snippet of \code{Heapsortcypher}~\cite{heapsort} in Figure~\ref{fig:2examples}(a), for example, calls MLaaS with an image and receives class labels as ML API output.
% It then checks if the API output belongs to three lists of classes, \code{Recycle}, \code{Compost}, \code{Donate} as the branch conditions to decide which branch to execute.
% For an input with ground-truth class \code{``Shirt''}, the ground-truth decision is to execute the \code{Donate} branch.
% If the ML API output is \code{``Paper''}, it will be a critical error, because the application decision (the \code{Recycle} branch) deviates from the ground-truth decision, whereas, if the ML API output is \code{``Jacket''}, it is not a critical error since the application's decision remains the same as the ground-truth decision.
%For example, the branch conditions in the \code{Heapsortcypher} application check if each API output class belongs to one of the three pre-defined lists. 
% \shan{This example is already discussed in the Introduction.}

%\item{\em Value ranges:}



% The second type of branch condition is used when the API output is a score, and several pre-defined {\em value ranges} are then used to check if the API output scores fall in which range. 
% The code snippet of \code{FoodDelivery}~\cite{food-delivery} in Figure~\ref{fig:2examples}(b), for example, calls MLaaS with a text sentence and receives a sentiment score as the ML API output. 
% It uses three branch conditions, each checking if the API output score lies in a certain range. 
% Given an input sentence whose ground-truth label is ``positive'', the ground-truth decision will print \code{It's a positive sentence}, and a critical error in this case will be when the API outputs a score lower than 0.6 on this sentence. 

% \shan{I am not totally sure about this arrangement. We already motivated somewhat in Introduction. How about we put any extra examples to a bit later when we discuss our empirical study result? It will also help move the pace faster into the empirical study.}
%As shown in the \code{FoodDelivery} application in Figure~\ref{fig:input_example}(b), it calls Google's \code{analyze\_sentiment} API to output a score indicating the emotional opinion of the input text. 
%The branch condition checks whether the score is over 0.6 (\ie the text is positive) or below 0.3 (\ie the text is negative), or otherwise (neutral). 
%\end{packeditemize}



%While these concepts may sound high-level, let us make them more concrete using two real-world applications, \code{Heapsortcypher} (Figure~\ref{fig:input_example}(a)) and \code{Food-delivery} (Figure~\ref{fig:input_example}(b)).
%
%\begin{packeditemize}
%\item 
%
%%\shan{This example is already discussed in the Introduction.}
%
%\item 
%%\shan{I am not totally sure about this arrangement. We already motivated somewhat in Introduction. How about we put any extra examples to a bit later when we discuss our empirical study result? It will also help move the pace faster into the empirical study.}
%\end{packeditemize}




% \mypara{Common structures over conditional branches}
% Given the conditional branches, the way these branches are structured can also greatly affects the application decision process.
% The structures over conditional branches differ along three key dimensions.
% (1) the {\em number of conditional branches}; 
% (2) the {\em number of executed branches} (for applications with several conditional branches, the application can either execute the first satisfied branch or all branches that satisfy the branch conditions); and finally
% (3) the {\em order of examination}---when there are multiple elements in an ML API output {\em and} multiple conditional branches, an application can choose to examine each element one by one against the conditional branches (\ie examining the $1^{\textrm{st}}$ element in API output against all branch conditions before moving to the $2^{\textrm{nd}}$ element, and so forth) or examine all elements against each conditional branch (\ie examining all elements against the $1^{\textrm{st}}$ branch condition, then all elements against the $2^{\textrm{nd}}$ condition, and so forth). 
%\begin{packeditemize}
%\item {\em Number of conditional branches:} The applications may define one or several branch conditions. 
%\item {\em Number of executed branches:} For applications with several conditional branches, the application can either execute the first satisfied branch or all branches that satisify the branch conditions. 
%\item {\em Order of examination:}  
%When there are multiple elements in an ML API output {\em and} multiple conditional branches, an application can choose to examine each element one by one against the conditional branches (\ie examining the $1^{\textrm{st}}$ element in API output against all branch conditions before moving to the $2^{\textrm{nd}}$ element, and so forth) or examine all elements against each conditional branch (\ie examining all elements against the $1^{\textrm{st}}$ branch condition, then all elements against the $2^{\textrm{nd}}$ condition, and so forth). 
%%Applications that execute at most one branch  may either iterate through branch conditions first or the API outputs first in a two-level for loop. 
%\end{packeditemize}

% With these dimensions, we identify four structures over conditional branches (Figure~\ref{fig:hierarchy}). 
% Figure~\ref{fig:code} depicts a simple illustrative example of each structure.
% \jc{we need to replace these names with macros. they will definitely be changed.}
% \jc{yuhan, can you explain these categories using the three dimensions just introduced? what's the point of introducing the dimensions without actually using them?}
%\begin{packeditemize}
%\item {\em T-or-F:} This type of applications make binary decision based on only one branch condition, such as checking if the API outputs intersect with a class list. 
%\item {\em M-to-N-set:}  This type of applications, such as the \code{The-Coding-Kid} application in Figure~\ref{fig:code}(b), define several branch conditions, and make multi-select decisions based on API outputs. All the branches whose conditions are fulfilled will be executed. 
%\item 

%\item 
%{\em Priority-list:} This type of applications define several branch conditions, and make multi-choice decision by examining all elements against each branch condition one-by-one, such as the \code{Aander-ETL} application in Figure~\ref{fig:code}(c). 


% \begin{figure*}
%      \includegraphics[width=\linewidth]{figs/variation.pdf}
%     \caption{Code snippets of variations in structures of branch conditions of the garbage classification application \code{Heapsortcypher}. \shan{Do we really need this?} \yh{Not necessarily, I put there because i was worried about whether people can understand why differentiating between multi-select/API-output order/app-choice order. but if we explain clearly enough in text, it's not necessary}}
% \label{fig:variations}
% \end{figure*}


%\shan{Do we really need this example???}
%Take the code snippets in Figure~\ref{fig:variations} as examples, which are variants of the garbage classification application. All of them use the \emph{same} class lists in branch conditions (\code{Recycle}, \code{Compost}, and \code{Donate}), though the structures of the branch conditions lead to different application decision processes. Figure~\ref{fig:variations}(a) is the original implementation of the application, which falls into the Top-label category. Figure~\ref{fig:variations}(b) and Figure~\ref{fig:variations}(c) write the application in different structures of condition branches, M-to-N-set and Priority-list respectively. Given an image with ground-truth label \code{``Paper''}, the MLaaS outputs [\code{``Shirt''}, \code{``Paper''}] to describe the image. In the case of a Top-label structure, this API output is a critical error because the wrong prediction  \code{``Shirt''} ranks higher in the output classes, leading the application to execute the branch \code{return ``donate''}. However, in the case of a Priority-list structure, this API output is a non-critical error because it overlaps with the highest ranked class list, \code{Recycle}, and executes the correct branch \code{return ``reycle''}. As for M-to-N-set, this also becomes a critical error because it adds an extra string \code{``donate''} into the set. 
 
 


% \mypara{Software context}
% Given these definitions, we define the software context of an application as the {\em critical errors} on the ML API output that will lead to different application decisions than the ground-truth decisions\shan{???I don't quite get it}.
% While these applications may sound high-level, let us make them more concrete using two real-world applications, \code{Heapsortcypher} (Figure~\ref{fig:input_example}(a)) and \code{Food-delivery} (Figure~\ref{fig:input_example}(b)).

% \begin{packeditemize}
% \item 
% The code snippet of \code{Heapsortcypher} in Figure~\ref{fig:input_example}(a) calls MLaaS with an image and receives class labels as ML API output.
% It then checks if the API output belongs to three lists of classes, \code{Recycle}, \code{Compost}, \code{Donate} as the branch conditions to decide which branch to execute.
% % , so that 
% % % s. Each of the branch conditions 
% % checks if the API output belongs to the list of classes associated with the branch. 
% For an input with ground-truth class \code{``Shirt''}, the ground-truth decision is to execute the \code{Donate} branch.
% % \emph{Target-edge} associated with the \code{Donate} list. 
% If the ML API output is \code{``Paper''}, it will be a critical error, because the application decision will be the \code{Recycle} branch, deviating from the ground-truth decision.
% % is executing the \emph{Target-edge} associated with the \code{Recycle} list. This application decision deviates from the ground-truth decision, thus forming a critical error. 
% Nevertheless, if the ML API output is 
% % mis-classifies the Shirt image to 
% \code{``Jacket''}, it is not a critical error since the application's decision remains the same as the ground-truth decision.
% % is still executing the \emph{Target-edge} associated with the \code{Donate} edge.
% \shan{This example is already discussed in the Introduction.}

% \item The code snippet of \code{FoodDelivery} in Figure~\ref{fig:input_example}(b) calls MLaaS with a sentence and receives a sentiment score as the ML API output. 
% It uses three branch conditions, each checking
% % . Each branch condition checks 
% if the API output score lies in a range. Given an input sentence whose ground-truth label is ``positive'', the ground-truth decision will execute the branch that prints \code{It's a positive sentence}, and a critical error in this case will be when the API outputs a score lower than 0.6 on this sentence. 
% \shan{I am not totally sure about this arrangement. We already motivated somewhat in Introduction. How about we put any extra examples to a bit later when we discuss our empirical study result? It will also help move the pace faster into the empirical study.}
% \end{packeditemize}

% Importantly, these examples show that {\em not} all errors are critical errors, and thus such per-application software context, if used carefully, could improve ML API output to reduce wrong application decisions. 
% However, to unleash such potential in practice, we first need a deep understanding on the software contexts of various applications using real MLaaS {\em in the wild}.


% \mypara{An empirical study over real MLaaS applications}
% To this end, in the remainder of this section, we run an empirical study over 77 open-source applications which collectively use 6 ML APIs.
% These applications are selected from a recently published benchmark suite~\cite{wan2021machine}.
% We keep all applications except those that directly print out or store the ML API outputs without post-processing (for these applications, by definition any errors of API output will be critical).

% Our empirical analysis focuses two central questions:
% (1) among applications using the same ML API, how much they differ in their software context (critical errors), and 
% (2) despite the application heterogeneity, whether common patterns emerge which might allow automatic extraction of software context.  



% \tightsubsection{\hspace{-0.2cm} Use of API output in conditional branches}


% For each of these applications in our study, its software context is determined along two dimensions
% {\em (i)} the branch conditions that use API output, and
% {\em (ii)} the structure over the branch conditions.Two applications' software contexts can differ along either or both dimensions. 

% \mypara{Use of API output in branch conditions}
% Depending on the API output, we identify two types of conditional branches. 
% \begin{packeditemize}
% \item{\em Class lists:} The first type is used when the API output is a label or a list of labels, and it checks if the API output labels belong to several pre-defined lists of classes.
% For example, the branch conditions in the \code{Heapsortcypher} application check if each API output class belongs to one of the three pre-defined lists. 
% \item{\em Value ranges:}
% The second type of branch condition is used when the API output is a score, and it  then checks if the API output scores fall in several pre-defined value ranges. 
% As shown in the \code{FoodDelivery} application in Figure~\ref{fig:input_example}(b), it calls Google's \code{analyze\_sentiment} API to output a score indicating the emotional opinion of the input text. 
% The branch condition checks whether the score is over 0.6 (\ie the text is positive) or below 0.3 (\ie the text is negative), or otherwise (neutral). 
% \end{packeditemize}


% \mypara{Structures of conditional branches}
% Given the API output and conditional branches, the way these conditional branches are structured can also greatly affect the application decision.
% The structures of conditional branches differ along three key dimensions, shown in Figure~\ref{fig:hierarchy}:
% \begin{packeditemize}
% \item Number of branch conditions: The applications may define one or several branch conditions. 
% \item Number of executed branches: For applications that define several branch conditions, the application can either execute at most one branch or execute a set of branches that fulfill the branch conditions. 
% \item Order of examination:  Applications that execute at most one branch  may either iterate through branch conditions first or the API outputs first in a two-level for loop. 
% \end{packeditemize}

% Along these dimensions, we carefully categorize the conditional branch structure of each application in our study.
% Four common structures emerge.
% \begin{packeditemize}
% \item T-or-F: As shown in Figure~\ref{fig:code}(a), the application defines one branch condition to check if the API outputs intersect with the list \code{A}. If so, it executes the branch \code{return "branch 1"}, otherwise, the branch \code{return "branch 2"} is executed. 
% \item M-to-N-set: As shown in Figure~\ref{fig:code}(b), the application defines two branch conditions in the for loop. If any of the branch conditions are fulfilled, the branch will be executed (\ie adding the message corresponding to the branch to the final output set). 
% \item Priority-list: This type of applications define several class lists, and check the class lists in order until finding the first one that intersects with the API outputs. Figure~\ref{fig:code}(c) is an example of this code structure.  
% \item Top-label: This type of applications iterate over the API outputs until finding one that intersects with any of the defined class lists, as shown in Figure~\ref{fig:code}(d). 
% \end{packeditemize}















% {\em As a consequence of the application decision processes, not all errors are critical.
% And because each application has unique conditional branches and its structure over these branches, their critical errors are greatly different. 
% }

% % \mypara{An empirical study over real MLaaS applications}
% % To this end, in the remainder of this section, we run an empirical study over 77 open-source applications which collectively use 6 ML APIs.
% % These applications are selected from a recently published benchmark suite~\cite{wan2021machine}.
% % We keep all applications except those that directly print out or store the ML API outputs without post-processing (for these applications, by definition, any errors of API output will be equally critical, so there is little room for improvement by customizing the model based on critical errors.)

% \mypara{How code structures affect critical errors of API output}
% If a misclassification occurs within a class list associated to the same conditional branch, then it is not a critical error. 
% But it would be a critical error, if an image is misclassified with a label in the class list of a different conditional branch than the ground-truth label.

% Even with the same branch conditions, the critical errors can differ depending on the structure of the conditional branches.

% Take the code structures in Figure~\ref{fig:code} as an example. Figure~\ref{fig:code}(b)(c)(d) defines two same class lists. Given an input  with ground-truth class \code{c1} and API outputs \code{[c3, c1]}. The ground-truth decision is execute the branch corresponding to \code{A}. For M-to-N-set, this API output leads the execution of branches corresponding to class lists \code{A} and \code{B}, thus forming a critical error. However, for Priority-list, this API output correctly leads the application to execute the branch corresponding to \code{A}. On the other hand, Top-label iterates over the outputs and breaks at the branch corresponding to \code{B}, which is also a critical error for the application. 


% \jc{Yuhan, please fill in}

% \mypara{Empirical observations on application heterogeneity}

==> bk/3-method_0525.tex <==
\label{sec:method}

Inspired by the study of \S\ref{sec:empirical}, we now present \tool which automatically customizes ML models for applications.


% \tightsubsection{High-level workflow and key components}
\tightsubsection{Problem formulation}
\label{sec:overall}


\begin{figure}
    \centering
    % \includegraphics[width=\linewidth]{figs/workflow.pdf}
    \includegraphics[width=0.99\linewidth]{figs/workflow-v2.pdf}
    \tightcaption{The logical steps of how \tool customizes DNNs of MLaaS for individual applications.
    % \jc{(1) "code" => "app source code"; "loss function" => "app-specific loss function"
    % (2) this might mislead people to think we use the same loss function for all apps. let's just use one code, not multiple.
    % (3) annotate the top part by "creation of app-specific loss function for a given application", and the bottom part "training DNN based on the app-specific loss function"}
    }
    \label{fig:steps}
\end{figure}
\mypara{Goal}
For an application that uses MLaaS, our goal is to efficiently train an ML model (in the form of DNN) run by the MLaaS backend, to {\bf minimize critical errors} in the API outputs for this application (\S\ref{sec:definitions}); our approach stands in contrast to typical approaches that minimize {\em all} inference errors.
In other words, the new ML model should return outputs that lead the application process to the same decision as if the ground-truth of the input is returned by the ML API. 
\jc{added the last sentence to provide more intuition of the formalism. Hank, pls proofread}
\hank{I like it  I did reword the first sentence.  I still don't love it, though. I was even thinking about changing it to say minimize the loss over all infernce errors.}

To formally state this objective, we denote how an application makes a decision by $\Appdecision(\API(\x))$, where $\x$ is the input to the ML API and $\API(\x)$ is the API output. 
Then for a given application decision process of $\Appdecision(\cdot)$ and an input set $\X$\footnote{A careful reader might notice that the formulation in Eq.~\ref{eq:goal} also depends on the input set.
Though the input set should ideally follow the same distribution of real user inputs of the application, this distribution is hard to obtain in advance and may also vary over time and across users.
Instead, we focus our discussion on training the ML model to minimize Eq.~\ref{eq:goal} with an assumed input distribution. Our evaluation (\S\ref{sec:evaluation}) will test the resulting model's performance over different input distributions.}, our goal is to train an ML model $\DNN(\cdot)$ such that 
\begin{align}
    \min_{\x_\InputId \in \X} \left|\{\x_\InputId | \Appdecision(\API(\x_\InputId)) \neq \Appdecision(\widehat{\API}(\x_\InputId))\}\right|, \nonumber \\
    \textrm{where }\API(\x_\InputId)=\Filter(\DNN(\x_\InputId))
    \label{eq:goal}
\end{align}

% Then for a given decision process of $\Appdecision(\cdot)$ and input set $\X$, our goal is an ML model $\DNN(\cdot)$ such that the number of wrong decisions are minimized:\footnote{A careful reader might notice that the formulation in Eq.~\ref{eq:goal} also depends on the input set $\X$.
% Though the input set should ideally follow the same distribution of real user inputs of the application, this distribution is hard to obtain in advance and may also vary over time and across users.
% Instead, we focus our discussion on training the ML model to minimize Eq.~\ref{eq:goal} with an assumed input distribution. Our evaluation (\S\ref{sec:evaluation}) will test the resulting model's performance over different input distributions.}
% We should clarify that this formulation keeps the ML API between user application and MLaaS intact. 
% \jc{Shan, do the last few sentences address the original comments?}


% \jc{NEED TO UPDATE THE DEFINITION AND TEXT AROUND IT}

Here, $\widehat{\API}(\x_\InputId)$ is a hypothetical API function that always returns the ground truth of input $\x_\InputId$, and $\Filter(\cdot)$ represents the postprocessing used by the API backend to translate a DNN output to an API output.
For instance, 
% In practice, the DNN output $\DNN(\x)$ may not be directly returned to user applications.
% For instance, 
an image classification model's output is a vector of confidence scores between 0 and 1 (each for a label),
% (with the $\LabelId^{th}$ score indicating how confident the model is about if the $\LabelId^{th}$ label exists in the image), 
but the ML API backend will use a threshold $\theta$ to filter and return only labels with scores higher than $\theta$, or the
%Another example is when the ML API returns the 
top $k$ labels with the highest confidence scores. 
\hank{I would suggest that we add one sentence to this paragraph before the formal definition that provides the intuition. I believe the idea is that we want to train an ML model such that the application decision process is as close as possible to what it woudl be with the ground truth.  Maybe this seems obvious, but as a reviewer I first make sure that I understand the intuition behind a formalism and then dive into the formal part.  If I don't think I can understand what the formalism is about, I won't invest the time to deep dive further. I guess the other issue here, is that it is not obvious why this formalism is different than just making the model as accurate as possible.  Certainly, in the limit if the model is 100\% accurate, then the two are equivalent, so we need to make sure people understand the magic of focusing on the application decision process---it only requires improving the accuracy of the labels that affect the application.}
\jc{tried to address it in end of the 1st para of 3.1 and the new text in the next para.}


Our goal in Eq~\ref{eq:goal} differs from the traditional goal of an ML model, which minimizes any errors in the API output, \ie 
\begin{align}
\min_{\x_\InputId \in \X} \left|\{\x_\InputId | \API(\x_\InputId) \neq \widehat{\API}(\x_\InputId)\}\right|.
\label{eq:goal_old}
\end{align}
Given that it is hard to obtain a DNN with 100\% accuracy, the difference between the two formulations is crucial, since not  all API output errors in Eq.~\ref{eq:goal_old} will cause incorrect application decisions in Eq.~\ref{eq:goal}.
Thus, compared to optimizing Eq.~\ref{eq:goal_old}, optimizing Eq.~\ref{eq:goal} is more likely to focus the DNN training on reducing the critical errors for the application.
\jc{the last few sentences to address Hank's comment on why the old formulation less suitable, which i believe is generally missing. Pls proofread.} \hank{I think this is super helpful to people's intuitive understanding.  Question: in the first sentence, should that be all errors instead of any errors?}
% \hank{Again, need to say why this difference is significant.  In the limit they are the same.  }

\begin{comment}
    


\begin{equation}
    \min_{\x_\InputId \in \X} \left|\{\x_\InputId | \Appdecision(\y_\InputId) \neq \Appdecision(\hat{\y_\InputId})\}\right|, \textrm{where }\y_\InputId=\DNN(\x_\InputId)
    \label{eq:goal}
\end{equation}
\noindent
Here, $\hat{\y_\InputId}$ is the inference ground truth under input $\x_\InputId$.


% Because this post-processing (\eg thresholding) will not be optimized as part of DNN training, it is captured as part of $\Appdecision(\cdot)$ in the formulation of Eq~\ref{eq:goal}.
\end{comment}



% Given our goal of optimizing Eq.~\ref{eq:goal}, we break it down to three logical steps (Figure~\ref{fig:steps}).
To train a DNN that optimizes Eq.~\ref{eq:goal}, the MLaaS backend must be able to efficiently determine if a DNN inference output $\DNN(\x)$ is a critical error or not (\ie $\Appdecision(\DNN(\x))\neq\Appdecision(\widehat{\API}(\x))$) at the end of \textit{every} training iteration.
If we assume $\Appdecision(\cdot)$ to be the whole application source code, the MLaaS backend must either repeatedly run the entire ML application, or let the developers run the application and send the results to the backend; neither is ideal as they could arbitrarily slow down the MLaaS's backend training procedure. %\yh{Junchen, please proof read}
% If we assume $\Appdecision(\cdot)$ to be the whole application source code, this means the MLaaS backend must repeatedly run the entire ML application,which  could arbitrarily slow down the MLaaS backend.
% \item First, we need to determine if a DNN inference output $\DNN(\x)$ will lead $\Appdecision(\cdot)$ to make an incorrect decision (\ie critical errors) without running the entire application, which could drastically slow down the
% training process and may not be feasible for the MLaaS backend
% for security concerns or application-dependency issues\shan{JC, we may need to discuss about this.}.
%only be accessible by developers/users.

\mypara{Logical steps of \tool}
To customize and deploy the DNN for an application, \tool takes three logical steps (Figure~\ref{fig:steps}).
First, \tool extracts from an application's source code a \emph{\summary} (explained shortly), a succinct representation of the application's decision process, which will be used to determine if a DNN inference error is critical (details in \S\ref{sec:extract}). 
Second, \tool converts a \summary to a {\em loss function}, which can be directly used to train a DNN (details in \S\ref{sec:loss}).
This loss function only penalizes DNN outputs that lead to critical errors with respect to a given application. 
Finally, the loss function will be used to train a customized DNN to be run by MLaaS for this particular application's requests (\S\ref{sec:runtime}). 
\jc{i split the text in two paras to address hanks comment. pls check} \hank{looks good.  My only question ifs if we can replace the train a customized model in the last bit to efficiently fine-tune or efficiently re-train or something similar soto emphasize the efficiency and the fact that we are not starting from scratch.}
% \hank{This paragraph promises three logical steps, but the steps are not clearly identified.  I think the problem is that the sentence after promising three steps starts with "First," which makes it sound like the first step, but then the actual first step comes much later.  Also, the sentence that lists the three steps and really refers back to the figure doesn't reference the figure.}

% (1) how to judge the correctness of $\Appdecision(\DNN(\x))$ without running the application in MLaaS backend, which is both slow and in-secure

%how to automatically extract function $\Appdecision(\cdot)$ from application source code, 
% (2) how to train the ML model $\DNN(\cdot)$ to optimize Eq.~\ref{eq:goal}.

\begin{comment}
Given our problem setting, the formulation of Eq.~\ref{eq:goal} implies two high-level challenges: 
(1) how to judge the correctness of $\Appdecision(\DNN(\x))$ without running
the application in MLaaS backend, which is both slow and in-secure\shan{The original text says ``how to automatically extract $\Appdecision(\cdot)$''. I feel
there was a logical gap in the original text, and hence made a change here. Please proofread.},
%how to automatically extract function $\Appdecision(\cdot)$ from application source code, 
and 
(2) how to train the ML model $\DNN(\cdot)$ to optimize Eq.~\ref{eq:goal}.


% \smallskip
% \noindent
\mypara{Logical workflow of \tool}To solve the aforementioned two problems, \tool has two logical steps, as depicted in Figure~\ref{fig:general_description}.
It first extracts a \emph{\summary} (explained shortly) from an application's source code to characterize how decisions are made by the application based on ML API output (details in \S\ref{sec:extract}).
Based on the \summary, \tool creates an application-specific loss function used for DNN training, through separating the ML API's critical errors that leads to incorrect application decisions from non-critical errors (details in \S\ref{sec:loss}). 
The loss function will then be used to train a customized DNN to be run by MLaaS for this particular application's queries (details in \S\ref{sec:runtime}).
% uses general framework to describe the application's decision process. 
% The general framework can identify critical errors for the application, and then be used to construct a new \emph{app-specific loss function} to train the DNN. 
% First, a \emph{decision-process summary} of the application is extracted from an application \App's source code.
% Secondly, application \App's decision process is viewed in a general framework of the \summary, which can identify critical errors of \App. 
% The critical errors are then used to create an \emph{app-specific loss function}, which is then used to train the DNN in order to minimize the critical errors. 
\end{comment}

\myparashort{A \summary}is 
% At a high-level, a {\bf \summary} extracted from an application is 
a succinct abstraction of the application that contains enough information to determine if a DNN inference output causes a critical error or not. 
% uniquely specifies\shan{JC, I have concerns with ``uniquely specifies''. I still think this is an abstraction. \summary actually throws away some details of an application-decision process, and only keeps the ones that help determine
% criticality of an error. I would prefer that we say ``a \summary extracted from an application offers an abstraction of $\Appdecision(\cdot)$ that can be used to determine if a DNN inference ....''} $\Appdecision(\cdot)$, which can be used to determine if a DNN inference output is a critical error or not.
% \shan{We need to discuss this. 
% With $\Appdecision$, we can infer which errors are critical, but the former
% does not equal the latter.
% To me, a \summary is an abstraction of $\Appdecision(\cdot)$. It allows 
% us to precisely judge which errors are critical without running application code.
% }
Specifically, it includes three pieces of information (defined in \S\ref{subsec:study-mech}): 
\begin{packeditemize}
\item \emph{Composition of \targets:} 
% \shan{``Value type'' is ambiguous, because ``string'' and ``floating point'' are also value types. I would recommend saying ``Composition of \targets''} \yh{sounds good}: 
the label list or value range of each \target; 
\item {\em Decision type:} \term{True-False}, \term{Multi-Choice}, or \term{Multi-Select};
\item {\em Matching order:} over the target classes, \term{API-order} or \term{App-order}, if the application makes a \term{Multi-Choice} decision.
\end{packeditemize}
For a concrete example, the \summary of the garbage classification application in Figure~\ref{fig:code}(a) contains
(1) three label lists representing three \targets: \code{Recycle}, \code{Compost}, and \code{Donate}; 
(2) the \term{Multi-Choice} type of decision; and 
(3) the matching order of \term{API-order}.  

% These three pieces of information uniquely describe which errors are critical and which are non-critical to the application, and they will be used to customize the ML model for the application, as elaborated in \S\ref{sec:loss}. 


\mypara{What is changed, what is not}
\tool does {\em not} change the ML API or the application source code.
Unlike recent work that aims to shrink the size of DNNs or speed them up~\cite{mullapudi2019online,kang2018blazeit,kang2017noscope}, we do not change the DNN architecture (shape and input/output interface); 
instead, we train the DNN to minimize critical errors.
That said, deploying \tool has two requirements.
%\hank{The first thing is not a change, though, right? That is just a thing that users need to do.}
%\jc{how about "deploying \tool has two requirements"}
First, the application developers need to run \tool's parser script to automatically extract the \summary, without MLaaS needing access to the application source code.
Second, \tool modifies the MLaaS backend to re-train an ML model per application, instead of serving the same model to all applications, and selects the right ML model to serve each query.
\S\ref{sec:extract} and \ref{sec:runtime} will explain why these changes are practical.


The remainder of this section will begin with the design of the application-specific loss function based on \summary,
% , ( critical component in training/customizing the ML model $\DNN(\cdot)$ to optimize Eq.~\ref{eq:goal}, 
followed by how to extract the \summary from the application, and finally, how the customized ML models are used to serve ML API queries.



\tightsubsection{Application-specific loss function}
\label{sec:loss}

% \tool solves Eq~\ref{eq:goal} 
% \shan{Eq1 already included a 
% ``min''. We cannot say minimize a ``min(...)'' expression. Can we?} 

Given Eq~\ref{eq:goal}, \tool trains a DNN model with a {\em new loss function}, which only penalizes critical errors of an application, rather than all DNN inference errors.
Since decision processes vary greatly across applications (\S\ref{subsec:study-imp}), we first explain how to conceptually capture different decision processes in a generic description, which allows us to derive the mathematical form of \tool's loss function later.

% At a high level, our loss function expresses a \summary in a continuous, differentiable form that can be used to train neural networks.
% \shan{sorry, what does ``differentiable form'' mean?}\jc{shan, let me know if it's still unclear. it should be a common knowledge that loss function must be differentiable.}
% that penalizes critical errors (which cause different decisions than the correct ones).


\begin{figure}
\centering
     \includegraphics[width=0.94\linewidth]{figs/loss-v2.pdf}
    \tightcaption{The generic description (shown in (c)) of an application (whose source code is shown in (a) and \summary in (b)) on a DNN inference output $\y$.
%     A decision process can be equivalently converted to a generic description. 
% (a) shows an example application, and (b) shows the generic description of its decision process on DNN inference output $\y$, 
% goes through several conditional checks, and each check is matched if certain label belongs to the \target and has a high enough (over $\theta$) score in $\y$.
% As we will elaborate, such generic description helps \tool to categorize critical errors and derive loss function.
}
\label{fig:loss}
\end{figure}

\mypara{Generalization of decision processes}
For each application in our study (\S\ref{sec:methodology}), our insight is that its decision process can always be viewed as traversing a sequence of conditional {\em checks} until an {\em end-of-decision} ({\em EOD}) occurs:
% \shan{``break'' is a widely used term/key-word in programming. I suggest that you use a different phrase, like end-of-decision, short as EOD.} 
\vspace{-0.4cm}

% {\footnotesize
% \begin{align*}
% 1^{\textrm{st}}\textrm{ check:} &<\textrm{MaskedOutput}^{(1)},\textrm{TargetClass}^{(1)}>\rightarrow\textrm{Matched?}^{(1)}&\\
% &\dots&\\
% \TraverseId^{\textrm{th}}\textrm{ check:} &<\textrm{MaskedOutput}^{(\TraverseId)},\textrm{TargetClass}^{(\TraverseId)}>\rightarrow\textrm{Matched?}^{(\TraverseId)}&\Leftarrow \textrm{break}\\
% &\dots&
% \vspace{-0.2cm}
% \end{align*}
% }
{\small
\begin{align*}
1^{\textrm{st}}\textrm{ check:} &<\y,\ClassId^{(1)}>\rightarrow\Match^{(1)}&\\
&\dots&\\
\TraverseId^{\textrm{th}}\textrm{ check:} &<\y,\ClassId^{(\TraverseId)}>\rightarrow\Match^{(\TraverseId)}& \Leftarrow \textrm{\bf EOD}\\
&\dots&
\vspace{-0.4cm}
\end{align*}
}
\noindent
% where the $\TraverseId$-th conditional check takes as input a masked output (\eg a masked vector of DNN output $\y$ with only score of certain label left) and one \target, and returns as output a binary indicating whether the masked output {\em matches} the condition of the \target, and a binary decision whether this check happens before the break.
% The set of \targets of checks with $\Match^{(\TraverseId)}=True$ before the break will be the decision.
where the $\TraverseId$-th check takes as input the DNN output $\y$ and one of \targets $\ClassId^{(\TraverseId)}$, 
% where the $\TraverseId$-th check takes as input a masked output \shan{I suggest that we don't introduce this term here. I feel just saying $y$ is the output of ML API doesn't hurt your explanation here. I think you will need to explain how DNN output is masked into the API output using threshold at a later place.}\jc{let's discuss this}$\y^{(\TraverseId)}$ (\eg a masked vector of DNN output $\y$ with only score of certain label left) and one of \targets $\ClassId^{(\TraverseId)}$, 
and returns a binary $\Match^{(\TraverseId)}$ indicating whether $\y^{(\TraverseId)}$ {\em matches} the condition of $\ClassId^{(\TraverseId)}$ and a binary decision whether this check happens before the EOD.
The set of \targets successfully matched before the EOD will be those selected by the application.
 % $\{\ClassId^{(j)} | \Match^{(\TraverseId)}=True\}$.

Figure~\ref{fig:loss} shows (a) an example application, (b) the decision-process summary,  and (c) the generic description for this application's decision process and a DNN output.  

This generic description (\eg the traversal order of the \targets, how a match is determined in a check, and when the EOD occurs) will depend on the information in the \summary and the DNN output $\y$. 
%\jc{good point! fixed}
%\hank{Again, it is slightly awkward to refer to the specifics of a generic description.  Can we just delete the first three words of the previous sentence?}
We stress that this generic description may {\em not} apply to all applications, but it does apply to all applications in our study (\S\ref{sec:methodology}). 

\hank{This sentence really confused me.  The figure shows three things, but the description only lists two. Also, just from a syntax point of view it is a bit jarring to refer to a generic description of a particular decision process (since those words are opposites). Maybe replace it with the generic description of this application's decision process. }
\jc{thanks Hank. fixed the text and the caption} \hank{I added a bit to the first sentence, please double check.}


\mypara{Categorization of critical errors}
Importantly, this generic description helps to categorize critical errors:
\begin{packeditemize}
\item {\em Type-1 Critical Errors:} A correct \target $\ClassId$ is not matched before EOD, but will be so if EOD occurs later. 
% matched only after the EOD. 
\hank{I don't understand how this one occurs.  EOD implies to me that the decision has been made, so it is unclear to me how the target gets matched after the decision is made.}
\jc{this is a good point. Hank, is the new text clearer?} \hank{I feel like I am missing something silly, but I just don't get it.  I keep reading EOD as ent of the control flow that is influenced by the ML API output.  Not reaching EOD feels like an inifinite loop or that somehow the code manages to exit out of the control flow that involves the ML output. I am probably missing something obvious but I would guess reviewers will too.}
\item {\em Type-2 Critical Errors:} A correct \target $\ClassId$ is never matched, before or after the EOD.
\item {\em Type-3 Critical Errors:} An incorrect \target $\ClassId$ is matched before EOD. 
\end{packeditemize}
A useful property of this categorization is that any wrong decision (a correct \target not being picked, or an incorrect \target being picked) falls in a unique category, and non-critical errors do not belong to any category. 
\hank{replace "nice" in the previous with a more descriptive word: "useful" or something.  It seems like this is technically important so this property might be essential for updating the loss fucntion (if that is true, that is a much stronger claim than just nice).  } \jc{done! that's a good point!}
In other words, as long as the loss function penalizes the occurrences of each category, it will only capture critical errors. 
%\hank{I fixed something in the previous sentence (which seemed to have an editing error) but someone needs to verify that I did not change the meaning.}\jc{good catch. that was an editing error. thanks!}

% \jc{before this point, use API output. transition to DNN output here!!}



% \footnote{A careful reader might notice that the formulation in Eq.~\ref{eq:goal} also depends on the input set $\X$.
% Though the input set should ideally follow the same distribution of real user inputs of the application, this distribution is hard to obtain in advance and may also vary over time and across users.
% Instead, we focus our discussion on training the ML model to minimize Eq.~\ref{eq:goal} with an assumed input distribution. Our evaluation (\S\ref{sec:evaluation}) will test the resulting model's performance over different input distributions.}
% We should notice that in Eq~\ref{eq:goal}, the ML model output $\DNN(\x)$ may not be directly returned to user applications.
% For instance, an image classification model's output is a vector of confidence scores between 0 and 1 (with the $\LabelId^{th}$ score indicating how confident the model is about if the $\LabelId^{th}$ label exists in the image), but the ML API backend will use a threshold $\theta$ to filter and return only labels with scores higher than $\theta$.
% Because this post-processing (\eg thresholding) will not be optimized as part of DNN training, it is captured as part of $\Appdecision(\cdot)$ in the formulation of Eq~\ref{eq:goal}.
% % We should clarify that this formulation keeps the ML API between user application and MLaaS intact. 
% \jc{Shan, do the last few sentences address the original comments?}

% In Eq~\ref{eq:goal}, such post-processing is viewed as part of the decision process $\Appdecision$\shan{???this seems counter-intuitive.}.
% This way\shan{??Why do we need the earlier claim to not need to modify ...?}, we do not need to modify the input/output of the ML model $\DNN(\cdot)$ or its training process, except using a different loss function.
% So \emph{how to design a loss function that can achieve our customization goal?}


\mypara{\tool's first attempt of a new loss function}
To understand why it is difficult to penalize critical errors and critical errors {\em only}, we first consider the common practice of assigning a higher weight to the loss of a DNN output if the ground-truth of the input will lead to a selection of some \targets (\eg~\cite{mcdnn,jung2015joint,vasan2020imcfn}).
% For instance, when training an image classifier, a traditional loss (\eg sum of cross-entropy) can be calculated for the DNN output on each input image, and higher weight can be given to input whose ground-truth labels lead the application to the selection of some \targets.
Henceforth, we refer to this basic design of loss function as \toolbasic.

At best, \toolbasic might improve the DNN's {\em label-wise} accuracy on inputs whose ground-truth decision selects some \targets.
% on all labels belonging to any \targets.
However, as elaborated in \S\ref{subsec:study-mech}, we also need to consider which labels belong to the same \target, the decision type, and the matching order of an application decision process in order to capture the three types of critical errors.
% First, all categories of critical errors requires to knowledge of which labels belong to the same \target, which \toolbasic fails to capture.
% This is because it misses two crucial aspects of a decision process.
% \jc{all CEs need to express the grouping of labels in a \target but this one doesn't capture it, and CE 1 and 3 need to capture the traversal order, but \toolbasic doesn't do that either.}
% {\em (i)} It fails to capture which the values (labels or values) belong to the same \target and which do not.
For instance, in the garbage-classification application (Figure~\ref{fig:input_example}), without knowing the label lists of each \target, \toolbasic will give an equal penalty to a critical error of mis-classifying a \code{Paper} image to \code{Wood} and a non-critical error of mis-classifying a \code{Paper} image to \code{Shirt}.
Similarly, without knowing the matching order, \toolbasic will equally penalize the output of [\code{Plastic}, \code{Jacket}] and [\code{Jacket}, \code{Plastic}], but only the latter leads to correct output because \code{Jacket} is matched first. 






\hank{I have to admit I had to read these two paragraphs multple times to figure out what was going on.  I would say that this descritpion of common practice is too vague---isn't htat also a description of what we are doing?  As I see it the only difference is how to determine the cost of errors.  So, I think this parapraph is trying to say that the problem with common practice is that the cost does not factor in the affect on application decision processes.  If so, just say that.  It might be saying something stronger, though, which is that even if you had a list of the labels that the app cares about, just focusing on those is not enough because the order in which the labels appear in branches is also important.  Anyway, I am not sure we need two paragraphs.  I think this could just be replaced with common proactice is to assign higher weight to an input sample if its error has higher cost and then we follow that practice.  Our unique insight is to factor the application decision making process into the assignment of these costs.  }
\jc{good suggestion. rewrote the last para. pls proofread}

% incrementally changes the traditional loss function following the common practice 
% \toolbasic also uses information in \summary.
% but it only considers which labels are in target classes and which are not. 
% Specifically, \toolbasic 
% % With the observation that applications typically heavily cluster on a small subset of labels appearing in the target classes(\S\ref{sec:empirical}), we naively come up with a \emph{strawman} of loss function design: 
% assigns a higher penalty to errors of the ML model on inputs whose correct decisions are one or multiple of the target classes. 

\begin{comment}

\mypara{\tool's first attempt of a new loss function}
% \myparaq{}
To understand {\em why penalizing critical errors is difficult},
% \shan{Why don't we just move the footnote 5 here as a reason: A typical approach to customize loss function is too xxx, so in our first attempt, we xxx. And, how about we move the content inside parentheses out to explain what is the traditional loss function?}, 
we first consider a simple loss function, \toolbasic, which follows the common practice of modifying the classic loss function by assigning higher weight to an input sample if its error has a higher ``cost'' (\eg~\cite{mcdnn}). 

For instance, when training an image classifier, \toolbasic still calculates the traditional loss for individual input (\ie a sum over cross-entropy losses that penalize the error on each label), and it penalizes the loss on inputs whose ground-truth labels lead the given application to match some \targets (rather than not matching any \target), which improves the DNN's {\em label-level} accuracy on input images that should match some \targets.
% \footnote{Indeed, it is a typical modification to loss function, when the cost of errors on certain labels is higher than those on other labels (\eg~\cite{mcdnn}).}

% \shan{Since we now have a categorization of critical errors. Can we discuss its limitation in regard to the three types of critical errors?}\jc{i planned to do exactly that, but it became extremely complicated, and instead, \toolbasic's problem can be explained much more easily without the CE categorization (whose purpose is to explain \tool's loss function). so i'm in favor of reverting to the original order of \toolbasic -> CE categorization -> \tool. let's discuss this!}
Unfortunately, \toolbasic fundamentally {\em cannot} distinct critical errors from other errors.
First, all categories of critical errors requires to knowladge of which labels belong to the same \target, which \toolbasic fails to capture.
% This is because it misses two crucial aspects of a decision process.
% \jc{all CEs need to express the grouping of labels in a \target but this one doesn't capture it, and CE 1 and 3 need to capture the traversal order, but \toolbasic doesn't do that either.}
% {\em (i)} It fails to capture which the values (labels or values) belong to the same \target and which do not.
For instance, in the garbage-classification application (Figure~\ref{fig:code}(a)), \toolbasic will give an equal penalty to a critical error of mis-classifying a \code{Paper} image to \code{Wood} and a non-critical error of mis-classifying a \code{Paper} image to \code{Shirt}.
% \shan{Do you have a quick example that explains point (ii) as well?}
Second, Type-1 and Type-2 critical errors are sensitive to the exact matching order, which is not captured by \toolbasic either. 
% {\em (ii)} It fails to capture the traversal order of conditional checks that matches DNN output with the \targets one by one. 
In the garbage-classification application (Figure~\ref{fig:code}(a)), given a \code{Jacket} image, two DNN outputs, [\code{Plastic}, \code{Jacket}] and [\code{Jacket}, \code{Plastic}], both misclassify \code{Jacket} to \code{Plastic}, and thus \toolbasic will penalize them equally, but  the latter leads to correct output because \code{Jacket} is matched first. 

\end{comment}



% For instance, when training a classifier, the traditional loss function on a DNN inference output is the sum of cross-entropy's, each penalizing the error on a label (\ie if a correct label has a low confidence score, or an incorrect label has a high confidence score).
% Based on this, \toolbasic gives the loss on the input a high weight, if the input's ground truth leads an application to the match of some \targets (rather than not matching any \target).

% , 
% Take image classification as an example.
% The loss function on an input image is the binary cross entropy between the confidence-score vector of $\DNN(\x)$ and the ground-truth binary vector ($\hat{\y}$) with each correct label having a 1\shan{???}.
% % Take the classification task  as an example to illustrate this idea. 
% % For an image, an ML model returns a vector of confidence scores ($\API(\x)=\y$), each score for one of a label, and the ground truth is a vector of binary scores ($\hat{\y}$) with each ground-truth label getting a score of 1.
% % The loss function is the cross entropy between the two vectors.
% If the ground truth leads to the selection of a target class, \toolbasic will penalize the cross-entropy value by multiplying it with a high weight. 


% The ground truth is a list, where the $j^{th}$ element is 1 if the $j^{th}$ label exists in the input, and 0 otherwise. 
% The pre-trained model is trained to reduce the \emph{average} errors between the probabilities and the ground truth across a wide range of labels (\eg 9605 labels in Open Images~\cite{ASL}).
% On the other hand, 

% \jc{shouldn't we use ``confidence scores'' as opposed to ``probability''? probably ``probability'' is used in some context, but it's confusing --- no one uses these scores as probability to draw values..} \yh{Sure}

% \myparaq{Why not \toolbasic}
% Although \toolbasic also uses \summary to determine which inputs lead to \targets, 



% \shan{Make sense, but the writing needs to be sharpened.}.
% Therefore, \toolbasic cannot separate critical errors (that yield different application decisions) from non-critical errors.



% we first introduce a general description of different decision processes and the \tool's design based on this general description, before detailing the loss function design case-by-case.
% Specifically, \tool's loss function expresses the target classes and matching orders in a {\em differentiable} form, such that it can be plugged into model training.
% To handle the critical errors of various applications, we first introduce a general description of different decision processes.
% , and this type of errors are non-critical to the application.
% because the strawman is unaware that different applications may make different decisions given the same output (\eg \emph{True-False}, \emph{Multi-select}, and \emph{Multi-choice}) and how these decisions affect the severity of ML model errors
% \shan{This last sentence is not clear.}. 



% \begin{equation}
% L(y_i) = w_i \cdot T_i \cdot L_{BCE}(y_i) + (1-T_i) \cdot L_{BCE}(y_i)
% \end{equation}
% where $w_i$ is a large weight (\eg $w_i = 20$), and $T_i = 1$ if the ground-truth labels of the $i^{th}$ sample overlap with the applications' target classes, and 0 otherwise. 


% Intuitively, this \emph{strawman} loss function is compatible with our goal since it prioritizes the reduction of the loss on the samples belonging to the target classes than the non-target ones. 






% We propose a new loss function directly constructed from the \summary.
% \yh{Why they fails and we do not fail }
% \yh{add general recipe }


% \begin{figure*}
%      \includegraphics[width=\linewidth]{figs/loss.pdf}
%     \caption{Decision processes of applications under our study (\S\ref{sec:empirical}) can be equivalently described in a general framework. 
% %     Here is an example of using the general formula to describe a decision process (top) on the DNN output $\y$ (bottom-left).
% % The \score $\M_\ClassId(\y)$ of \target $\ClassId$ is the highest confidence score in $\y$ associated with any label in the \target, because the labels in \code{detection\_labels} are sorted in descending order of their confidence scores, so the highest-score label in each \target is always matched first.
% % It then goes through the three \targets in the order of $\M_{Landmark}(\y)$, $\M_{Building}(\y)$, and $\M_{Person}(\y)$ (\ie following the if-else statements in the code), and in this case, the break occurs after matching the \target of \code{Building}.
% % This is because this is a \term{Multi-Choice application choice} process (\ie return on the first match), and the \score of the first \target ($\M_{Landmark}(\y)$) is below the threshold $\theta=0.5$. \jc{Yuhan, let's discuss an alternative of fig 4. i think the current fig (in a simplified form) serves well for the case study, but doesn't help much for people to understand the general idea of code -> abstract framework -> critical errors -> loss function. we need a more direct illustration of this thought process. ping me when you get a chance. thanks!
% Here is an example of using the general formula to describe a decision process (right) on the DNN output $\y$ (left). 
% % \yh{TODO: more explanation on penalization on critical errors}
% }
% % only labels with confidence scores over $\theta=0.5$ can be matched with \target, and $\M_{Building}(\y)$ is the first to exceed $\theta$.
%     % at a high level, the process first calculates the effective score of each target class (??), ranks them in an order (??), and traverse the target classes until a break (??). \tool's loss function for a \term{Multi-Select} example. \yh{Other, don't }
    
% \label{fig:loss}
% \end{figure*}

% \shan{We need to change the tone a bit. The writing sounds really like \tool versus \tool-basic, which is the wrong tone.}

% In contrast, \tool's loss function only penalizes critical errors specific to each application's decision process, rather than all errors in the DNN output. 
% At a high level, our loss function converts the logic of an application's decision process to a differentiable form that penalizes critical errors (which cause different decisions than the correct ones).





% \begin{packeditemize}
% \item {\em Type-1 Critical Errors:} A correct \target $\ClassId$ is never traversed in any conditional checks before the break.
% \item {\em Type-2 Critical Errors:} A correct \target $\ClassId$ is traversed 
% before the break, but each time (\eg at the $\TraverseId^{th}$ check) the score vector $\y^{(\TraverseId)}$ used does not match $\ClassId$'s condition.
% \item {\em Type-3 Critical Errors:} An incorrect \target $\ClassId$ is traversed in some check (\eg at the $\TraverseId^{th}$ check) before the break, and the score vector $\y^{(\TraverseId)}$ used match $\ClassId$'s condition.
% \end{packeditemize}


\mypara{\tool's loss function} 
\tool leverages the categorization of critical errors to systematically derive a loss function that penalizes each type of critical error.
To make it concrete, we explain \tool's loss function of ``label-based API, \term{Multi-Choice} type of decision, and \term{App-order}'' (\eg Figure~\ref{fig:loss}).
% , which is one of the most common types of decision processes in our study.
% (defined in \S\ref{subsec:observations}).  
\S\ref{sec:loss_appendix} will detail the loss functions of other decision processes.
The loss function of such applications has three terms, each penalizing one type of critical error:

\vspace{-0.3cm}
{\small
\begin{align}
     L(\y) &=   
 % \overbrace{ \sum_{\ClassId\leq\hat{\ClassId}} \textrm{Sigmoid}\left(\max_{\LabelId\in\TargetSet_{\ClassId}}\y[\LabelId]-\theta\right)}^{\substack{\text{\sf \footnotesize {{\bf Type-1} Critical Errors}} }} +
  \overbrace{ \textrm{Sigmoid}\left(\min\left(\max_{\LabelId \in \cup_{\ClassId < \hat{\ClassId}}\TargetSet_{\ClassId}}\y[\LabelId],\max_{\LabelId\in\TargetSet_{\hat{\ClassId}}}\y[\LabelId]\right)-\theta\right)}^{\substack{\text{\sf \footnotesize {{\bf Type-1} Critical Errors}} }} \label{eq:loss_app} \\&+
 \overbrace{ \textrm{Sigmoid}\left(\theta-\max_{\LabelId\in\TargetSet_{\hat{\ClassId}}}\y[\LabelId]\right)}^{\substack{\text{\sf \footnotesize {{\bf Type-2} Critical Errors}} }} + 
 \overbrace{ \sum_{\ClassId<\hat{\ClassId}}\textrm{Sigmoid}\left(\max_{\LabelId\in\TargetSet_{\ClassId}}\y[\LabelId]-\theta\right)}^{\substack{\text{\sf \footnotesize {{\bf Type-3} Critical Errors}} }}\nonumber
\end{align}
}
Here, $\y[\LabelId]$ denotes the score of the label $\LabelId$, $\TargetSet_\ClassId$ denotes the set of labels of \target $\ClassId$, $\hat{\ClassId}$ denotes the correct (\ie ground-truth) \target, and the sigmoid function $\textrm{Sigmoid}(x)=\frac{1}{1+e^{x}}$ will incur a higher penalty on a greater positive value.

% \jc{Yuhan, we need to explain why such a confidence threshold $\theta$ exists. i understand dnns commonly use thresholds like this, but we need to remind people that. also, any evidence that real APIs do threshold DNN output? did we pick threshold 0.3 for some reason? maybe it leads to similar DNN output as real API output?} 

{\em Why does it capture the critical errors?} 
% Here, we intuitively explain why Eq~\ref{eq:loss_app} captures each type of error 
% (see \S\ref{sec:loss_appendix} for formal proofs). 
Given this application is \term{Multi-Choice}, the EOD will occur right after the first match of a \target, \ie the first check with a $\ClassId$ such that $\max_{\LabelId \in \TargetSet_{\ClassId}}\y[\LabelId]\geq\theta$.
% Intuitively (see \S\ref{sec:loss_appendix} for formal proofs), because this is a \term{multi-choice} application (break at the first match) and it goes through labels in \code{detection\_labels} in descending order of their confidence scores, $\MaxScore$ is the score of the first matching label and is also when the break occurs.
\begin{packeditemize}
\item A Type-1 critical error occurs, if (1) the correct \target $\hat{\ClassId}$ is matched {\em and} (2) it is matched after the EOD.
First, the correct \target $\hat{\ClassId}$ is matched, if and only if at least one of its labels has a score above the confidence threshold, so $\max_{\LabelId\in\TargetSet_{\hat{\ClassId}}}\y[\LabelId]\geq\theta$).
Second, this match happens after the break, if and only if some \target $\ClassId$ before $\hat{\ClassId}$ (\ie $\ClassId<\hat{\ClassId}$) is matched, so $\max_{\LabelId \in \TargetSet_{\ClassId}}\y[\LabelId]\geq\theta$).
Put together, the first term of Eq~\ref{eq:loss_app} penalizes any occurrence of these conditions. 
\item A Type-2 critical error occurs, if no label in the correct \target $\hat{\ClassId}$ has a score high enough for $\hat{\ClassId}$ to be matched, \ie $\max_{\LabelId\in\TargetSet_{\hat{\ClassId}}}\y[\LabelId] < \theta$, so the second term of Eq~\ref{eq:loss_app} penalizes any occurrence of this condition.
\item A Type-3 critical error occurs, if any incorrect \target $\ClassId$ before $\hat{\ClassId}$ (\ie $\ClassId<\hat{\ClassId}$) has a label with a score high enough for $\ClassId$ to be matched, \ie $\max_{\LabelId\in\TargetSet_{\ClassId}}\y[\LabelId]-\theta$, so the third term of Eq~\ref{eq:loss_app} penalizes any occurrence of this condition.
\end{packeditemize}






To train a DNN, the loss function must be differentiable with respect to the DNN ouput $\y$. 
% It is important to note that optimizers used in ML(\eg Adam)
% % \jc{you tend to add references on non-essential terms, } 
% to train  models are gradient-based. 
% Thus, the loss function (\ie every function in the composite function) needs to be differentiable in order to calculate the gradient of the loss value with respect to the DNN output. 
Eq~\ref{eq:loss_app} uses the $\max$ function several times. 
Though $\max$ is not naturally differentiable, it can be closely approximated in well-known differentiable forms provided by PyTorch's differentiable operators~\cite{paszke2017automatic}).


\tightsubsection{Extracting applications' decision process}
\label{sec:extract}
 

% How we use sym-ex to get info, and which info 
% \yh{Change all the whitelists}
%\tool automatically extracts the \summary from an application.

The current prototype of \tool program analysis supports Python applications that make decisions based on categorical label output or floating point output of ML APIs. We first discuss how it works for ML APIs with categorical label output, 
like all the APIs in Table \ref{tab:all_stats} except for \code{analyze\_sentiment}. We will then discuss a variant of it that works for most use cases of \code{analyze\_sentiment}.
%, which produces floating point output.


 
Given application source code, \tool first identifies all the invocations of ML APIs. For every invocation $I$ in a function $f$, \tool then identifies all the branches whose conditions have a data dependency upon the ML API's label output. We will refer to these branches as $I$-branches. If there is no such branch in $f$, \tool then checks the call graph, and analyzes up to 2 levels of callers and up to 5 levels of callees of $f$ until such a branch is identified. If no such branch is identified after this, \tool considers the ML API invocation $I$ to not affect application decisions and hence does not consider any optimization for it. If some $I$-branches are identified, \tool records the top-level function analyzed, $F$,
%(\ie $f$ itself or one of its ancestors on the call graph), 
and moves on to extract the \summary in following steps.

%\tool tracks along the control-flow graph to see how its output is used to make control flow decisions. \tool is inter-procedural and checks the callee functions that take ML API output as input and caller functions that invoke current functions to get ML API output. \tool stops either when (1) it reaches a function that uses ML API output in branch conditions, as described in Section~\ref{sec:empirical}; or (2) it tracks a threshold number of functions, configured as 5. \tool then analyzes these tracked functions to obtain the application decision process. 

\myparashort{What are the \targets?} 
\tool figures out all the \targets and their composition in two steps.

The first step leverages symbolic execution and constraint solving to identify all the labels that belong to \textit{any} \targets. Specifically, \tool 
applies symbolic execution to function $F$, treating the parameters of $F$ and the
label output of $I$ as symbolic (\ie the symbolic execution skips the ML API invocation $I$ and directly uses $I$'s symbolic output in the remaining execution of $F$)\footnote{{Recall that an API output contains several fields not used to influence 
control flow in any applications. We set them with pre-defined dummy values.}}. 
{
Since applications typically match only one label in API output at a time (as observed in \S\ref{subsec:study-mech}), we set the label array returned by $I$ to contain one element (label) and use a symbolic string to represent it. 
}
Through symbolic execution, \tool obtains constraints for every path that involves an $I$-branch, solving which tells \tool which labels need to be in the 
output of the ML API in order to execute each unique path, essentially all the labels that belong to any \target.


%\jc{the original paragraph was commented, as it reads like API output always only contains one label. feel free to revert.}

\begin{comment}

To simplify the above analysis, 
although the output object of an ML API contains many fields, 
\tool uses pre-defined dummy values for all but
the array of categorical labels, as only the latter affects control flow.
\tool also assumes the label array to contain just one element.
Take the code in Figure \ref{fig:code}(e) as an example. \tool focuses on 
the \code{response.label\_annotations[..].name} array. \tool assumes this
array to contain only one element, and uses 
a symbolic string to represent it.

\end{comment}

One potential concern is that a solver may only output one instead of all values that satisfy a constraint.
%, which could prevent us from identifying 
%\textit{all} the labels that belong to any \target. 
Fortunately, the symbolic execution engine used by \tool, NICE~\cite{irlbeck2015deconstructing}, turns Python code into an intermediate representation where each branch is in a simplest form. Take Figure \ref{fig:code}(d) as an example, the source-code branch 
\code{if obj.name in Protein} is transformed into three branches where \code{obj.name}
is compared with \code{``Hamburger''}, \code{``Meat''}, and \code{``Patty''} separately, allowing us to capture all three labels by solving three separate path constraints.

The second step groups these labels into \targets by comparing their respective
paths: 
%they each corresponds to: 
{if two API output, each with one label, lead}
% if two label outputs of an ML API allow 
the program to follow the same execution path at the source-code level, these two labels belong to the same \target.
For example, in Figure \ref{fig:code}(d), the execution path is exactly the same when the \code{label\_detection}
API returns \code{[``Hamburger'']}, comparing with when it returns \code{[``Meat'']}, with
all function parameters and other API output fields being the same. Consequently, we can know that 
label \code{Hamburger} and label \code{Meat} belong to the same \target.
 To figure out the path, \tool simply executes function $F$ using each input produced by the constraint solver and traces the source-code execution path using the Python trace module.

One final challenge is that \tool needs to identify and exclude the path where none of the \targets are matched (\eg the \code{``It is others.''} path in Figure \ref{fig:code}(a)).
We achieve this by carefully setting the default solution in the constraint solver to be an empty string, 
%Given a constraint, the solver first checks whether the pre-configured default value can satisfy the constraint. If so, this default value is output as the solution.
%We sets this default value to be an empty string, 
which
is impossible to output for any ML APIs in this paper. This way, whenever this default solution is output, \tool knows that the corresponding path 
matches no \target.
%\shan{TODO: -1 for float value}




\myparashort{What is the type of decision?}
% Now that \tool knows all the \targets, it further 
%Next, \tool analyzes the type of decision.
When only one \target is identified, \tool reports a \term{True-False} decision type. Otherwise, \tool decides whether the decision type is 
\term{Multi-Choice} or \term{Multi-Select} by checking the source-code execution path associated with every \target label obtained above. 
%Specifically, \tool checks 
If any execution evaluates an $I$-branch \textit{after} another $I$-branch
is already evaluated to be true, \tool reports a 
\term{Multi-Select} decision type; otherwise, \tool reports a \term{Multi-Choice}
decision type.

%To decide whether the decision type is \term\tool analyzes all the statements inside the basic block following the if-branch that compares ML API output with \targets. If the software bypasses other comparisons between API output after making a selection\shan{it is better, but still unclear.} (\eg a break statement inside the loop and a return statement inside a function body), \tool regards it as a \term{Multi-Choice} and further examines the order. 
%If there is no such bypass, \tool determines it as \term{Multi-Select} structure. 

\myparashort{What is the matching order over the \targets?}
%For applications that make \term{Multi-Choice} decisions, \tool wants to figure out whether the application iterates through the API's label array output until one output label is matched with a \target (\ie \term{API-Order} like in Figure~\ref{fig:code}(d)), or the application iterates through the \targets in whatever order determined by the application until one \target is matched (\ie \term{App-Order} like in Figure~\ref{fig:code}(a)).
To tell whether a \term{Multi-Choice} decision is made
through \term{API-Order} like in Figure \ref{fig:input_example} or 
\term{App-Order} like in Figure \ref{fig:code}(a), \tool first identifies all the \code{for} loops that
iterate through the label array output by the ML API and have control-dependency
with $I$-branches, \eg 
% These are the control structures where \target matching
% occurs, like 
the \code{for l in labels} in Figure~\ref{fig:code}(a)
and the \code{for obj in response.label\_annotations} in Figure~\ref{fig:input_example}.


\tool then checks how many such output-iterating loops there are.
If there is only one and this loop is not inside another loop, 
like that in Figure \ref{fig:input_example}, \tool considers the matching order to be
\term{API-Order}, as the application only iterates through
each output label once, with the matching order determined
by the output array arranged by the ML API. Otherwise, \tool considers
the matching order to be \term{App-Order}. This is the case for the example
shown in Figure \ref{fig:code}(a), where three output-iterating loops are
identified, each of which matches with one \target in an order determined by the
application: the \code{Landmark} \target, followed by the 
\code{Building}, and
finally the \code{Person}.

%In rare cases when \tool cannot find any such output-iterating loops, \term{App-Order} is reported, as it happens when developers configure the ML API to only output one label. or when all the output labels are concatenated into one string.
%In these cases, the \term{Multi-Choice} mapping order would be determined by the application.

% The current prototype of \tool uses a Python byte-code analysis framework XXX\shan{CC, please fill in}
% to implement the above analysis. Particularly, \tool identifies the object 
% that is iterated
% through by a \code{for}-loop through the \code{GET\_ITER} instruction  in each for-loop header. 

%\jc{i merged the last para to sec 4}
\begin{comment}
The current prototype of \tool uses Python static analysis framework Pyan \cite{pyan} and Jedi \cite{jedi} to implement the above analysis. Particularly, \tool identifies the object that is iterated through by a \code{for}-loop through the \code{iter} expression in each for-loop header. 
\shan{Is this a byte-code instruction?}\cc{It is a byte-code instruction. But I did it at source code level: the \code{iter} expression between keyword \code{for} and \code{in}. I changed the description.}
\end{comment}

%If the inner (outer) loop iterates through the ML API's output label array and the outer (inner) loop iterates through the application choices\cc{Then how about ``iterates through a variable that have control dependency with $I$-branches while not having data dependency on ML API's output''?}\shan{What exactly is your implementation? I am confused here.}\cc{I will first find the $I$-branches, and find the loops whose iterator affect the $I$-branch decisions. Then I further checks the iterated object and classified it into two categories based on whether have data dependency with ML API output: ML-API-related and Application-choice-related. During this process, I also treat \code{if obj.name in Recycle} as alternative way of \code{for r in Recycle: if obj.name==r}, and therefore counts as a loop.
%Next I make judgement based on the nesting level of these for-loops and if-branches.}, \tool regards it as pattern \term{Application-choice} order (\term{API-output order}). 

%If the software does not contain any for-loop iterating through ML API's output or \targets, \tool stops analysis and reports an unknown code pattern\shan{what would happen after this? Do you abort the optimization plan? Can you offer some reasoning about why such a case should or should not occur?}\cc{I checked the implementation details again. It actually will be treated as \term{Application-choice} order. If there is no for-loop, it means the software is doing set intersection over API output and target class. This prioritizes the \targets.}\shan{hah? Can you elaborate? I don't understand.}\cc{A typical implementation is to iterate both API output and \targets to compare each individual output label and elements in \targets. However, for applications as Figure 2.a and 2.c, the syntax only contains iteration of  API output. \tool  treats \code{if element in list} as alternative way of iterating \targets. If there is no nesting loop, the only possible implementation would be a variant of figure 2.c, \code{if len(Landmark.intersect(detected\_labels))>0}, which is \term{Application-choice} order}.

\myparashort{How to handle floating-point output of ML APIs?}
Recall in \S\ref{subsec:study-mech} that some ML APIs, \eg \code{analyze\_sentiment}, have floating-point output and the application defines several value ranges to put each floating-point output into one category. To handle this type of API, \tool needs to identify the value
range of each \target, which is not supported by NICE and other popular constraint solvers. Fortunately, many applications directly compare API output with constant values in $I$-branches, giving \tool a chance to infer the
value range. For these applications, \tool first extracts those constant values that are compared with API output in $I$-branches, 
\eg 0.3 and 0.6 in Figure \ref{fig:code}(b).
\tool then forms tentative value ranges using these numbers, like -1 -- 0.3, 0.3 -- 0.6, and 0.6 -- 1 for Figure \ref{fig:code}(b) (-1 and 1 are the smallest and biggest possible \code{score} output of \code{analyze\_sentiment} based on the API manual). To confirm these value ranges and figure out the boundary situation, \tool then
executes function $F$ with all the boundary values, as well as some values in the middle of each range. By comparing which values lead to the same execution path, \tool finalizes the value ranges. For the example in Figure \ref{fig:code}(b), after executing with \code{score} set to -0.35, 0.3, 0.45, 0.6, and 0.8, \tool settles down on the final value ranges to be: (-1,0.3), [0.3,0.6), and [0.6,1). %\shan{what about -1 and 1? They are impossible output?}\cc{The official document just mention `` ranges between -1.0 (negative) and 1.0 (positive) ''. Based on my experience, I never saw any output reaching these two values. So I guess the range is (-1, 1)}


\myparashort{Limitation}
The static analysis in \tool does not handle the iterated object of while loops, unfolded loops, and recursive functions. For complexity concerns, \tool only checks caller and
callee functions with limited levels, and hence may miss some $I$-branches
far away from the API invocation. \tool's ability of identifying \targets is limited by the constraint solver. \tool assumes different source-code paths correspond to different target classes, which in theory could be wrong 
if the application behaves exactly the same under different execution paths.
% \tool is only able to handle the decision types and mapping orders described in Section~\ref{sec:empirical}.  



\tightsubsection{Putting them together}
\label{sec:runtime}


\begin{figure}
     \includegraphics[width=.99\linewidth]{figs/system.pdf}
    \tightcaption{Workflow of \tool.
    % \jc{the overall flow looks ok, but there are so many minor issues in this figure. just to name a few: 
    % (1) where is "cloud service" coming from? 
    % (2) (a) and (b) shouldn't be distinguished (see comment in 3.1).
    % (3) i thought we decided to drop the arrow of giving the parser to developer?
    % (4) why "software context" is still used?
    % (5) user is not running python code! they run real apps
    % (6) why calling it "prediction" instead of API output?
    % (7) what's "model inference code"? if it's simply selecting the right model to run, we shouldn't introduce a new term.
    % (8) the three customized models should be put side by side (either all vertically or horizontally),
    % (9) why calling them "adapted" ML model? if the term we always use is "customized", then stick to that.}
    % \jc{in general, EVERY word must be picked very carefully, which you clearly didn't do :)}
    % \yh{fixed comments, I'm calling it ML model outputs instead of API outputs because the outputs comes before the ``output interface'', thus it's not API outputs yet}
    % \jc{sorry i disagree. again, don't introduce new terms unless really necessary, which i don't think is the case. why dont you change the figure, to move the output and input the left of the model output interface, which should also be changed to "ML API"?}
    % \jc{and don't let arrows overlap with arrows or lines (e.g., Model pool, Select)}
    }
\label{fig:system}
\end{figure}


% Naturally, these two problems drive \tool's workflow, as depicted in Figure~\ref{fig:system}. 
% When developers publish an application (\App), they first run a parser script provided by \tool on \App's source code to extract its {\em \summary} (explained in\S\ref{sec:overall}) and then upload the summary to \tool's MLaaS backend (details in \S\ref{sec:extract}). 
% The backend uses the received \summary to construct a new {\em app-specific loss function} (details in \S\ref{sec:loss}), such that when the ML model is trained using the new loss function, it will produce inference results that yield fewer application decision failures for the application \App.
% \tool then adds the new ML model to a pool of customized ML models. 
% When a user of application \App queries \tool's MLaaS backend with an input via the existing ML API, the backend will select the ML model customized for \App and return the inference result of the selected ML model (details in \S\ref{sec:runtime}).

% \jc{let's move the workflow and fig 3 to the end of 3 as a "let's put them together" type of subsection and merge with existing 3.4}

Finally, we put these components together in the workflow shown in Figure~\ref{fig:system}. 
First, when an application (\App) is developed, the developers run a parser (described in \S\ref{sec:extract}) provided by \tool on \App's source code to extract the \summary for \App.
% (introduced in \S\ref{sec:overall}).
The developers can then upload the \summary to \tool's backend together with a unique application ID (which will later be used to identify queries from the same application). 
% Developers upload the summary to \tool's MLaaS backend through . 

\tool's backend then uses the received \summary to construct a new  application-specific loss function (described in \S\ref{sec:loss}). 
When a DNN is trained using the new loss function, its inference results will lead to fewer critical errors (\ie incorrect application decisions) for application \App.
In our prototype, \tool uses the new loss function to re-train an off-the-shelf pre-trained DNN, rather than training the DNN from scratch. 
This is a common practice to save training time (see \S\ref{sec:evaluation} for quantification).
The DNN re-training will use 
an application-specific dataset sampled from the dataset  (see Table~\ref{tab:datasets} and \S\ref{sec:implement}). 
\tool samples the data so that each target/non-target class is selected by ground-truth decisions of the same number of inputs.
% We will discuss training data in \S\ref{sec:implement}.
% \footnote{Model re-training is a common ML approach~\cite{sharif2014cnn,devlin2018bert,sun2019fine,ekya} used to save training time with a much smaller training dataset.}, where the DNN's parameters are updated based on a pre-trained model. 


% \tool re-trains the ML model based on the \summary, and maintains a model pool with a key-value database that maps the application ID to the customized ML model. 


To serve different applications, the backend maintains a set of DNN models, each of which is customized for an application and is keyed by its application ID. 
Before an application \App queries \tool's MLaaS backend, they will first use existing APIs to create a connection to the MLaaS service with a credential that includes the application ID of \App.\footnote{In many MLaaS offerings~\cite{google-cloud,amazon-ai}, a connection between the application and the MLaaS backend is commonly created before the application issues any queries. 
% existing APIs to set up such connections 
Existing MLaaS
already allows applications to specify the application ID via the connection between the application and backend.}
% Before a user of application \App queries \tool's MLaaS, he/she first needs to establish connection to the cloud service using a credential (associated with \App's application ID), same as the existing querying procedure. 
Then the application uses existing ML API to query \tool's backend with an input.
The backend will use the application ID associated with this connection to identify the DNN model customized for \App, run the DNN on the input, and return the inference result of the selected model.

% When a user of the application queries MLaaS via the ML API, the same ML API querying procedure is followed as in existing MLaaS. 
% The user needs to establish connection to the cloud service using a credential. 
% \tool then uses this credential to select the corresponding customized ML model from the model pool.  
% Later on, when the user queries the ML API to perform prediction, the backend will run inference on the selected ML model and returns the result. 


% MLaaS provides an additional API for developers to upload the \summary together with a credential that associated with an unique application ID.
% In the backend, \tool re-trains the ML model based on the \summary, and maintains a model pool with a key-value database that maps the application ID to the customized ML model. 

% xxx


% During application run-time, it follows same API querying procedure as original MLaaS. The user needs to establish connection to the cloud service using a credential. \tool then uses this credential to select the corresponding customized ML model from the model pool.  
% Later on, when the user queries the ML API to perform prediction, the backend will run inference on the selected ML model and returns the result. 













==> bk/4-implement_0525.tex <==
\label{sec:implement}

% We implemented our prototype of \tool in Python 3.8. It contains these key components.
% For ML model training and inference, we use PyTorch v1.10~\cite{paszke2017automatic} and CUDA 11.1. 

% \jc{chengcheng, please doublecheck the following paragraph}
% \cc{We take the source code as input. We will identify all the ML API invocations and customize for each of them. The developer could decide to turn-off the customization for any of them.}

\mypara{Extractor of \summary}
The current prototype of \tool is implemented for Python applications that use Google or Amazon ML APIs.
It takes as input the application source code and returns as output the \summary in the JSON format.
It uses NICE symbolic execution engine~\cite{irlbeck2015deconstructing} and CVC5 constraint solver~\cite{cvc5} to identify \targets, and uses Python static analysis framework Pyan \cite{pyan} and Jedi \cite{jedi} to identify the decision type and the matching order. 
Particularly, it identifies the object that is iterated through by a \code{for}-loop through the \code{iter} expression in each for-loop header, which is used to distinguish \term{Multi-Choice} and \term{Multi-Select} decisions and the matching order.
% \shan{Is this a byte-code instruction?}\cc{It is a byte-code instruction. But I did it at source code level: the \code{iter} expression between keyword \code{for} and \code{in}. I changed the description.}

% \mypara{Software decision process extractor} It is implemented for Python applications that use Google or Amazon ML APIs. It takes a code location of ML API invocation as input and outputs software decision process in JSON file format. \tool adopts NICE symbolic execution engine~\cite{irlbeck2015deconstructing}, CVC5 constraint solver~\cite{cvc5} to extract \wls content. It use Pyan \cite{pyan} and Jedi \cite{jedi} library to analysis other decision processes.

\mypara{ML re-training} 
The re-training module is implemented in PyTorch v1.10 and CUDA 11.1.
It uses a \summary to construct a new loss function (see \S\ref{sec:loss}), and then 
% The module parses the output of the software decision process extractor as input, and the re-training module constructs a loss function for the specific type of application. The re-training module then 
replaces the builtin loss function in Pytorch with the new loss function, and uses the common forward and backward propagation procedure to re-train an off-the-shelf pre-trained DNN model (explained next).

% Table~\ref{tab:datasets} summarizes the pre-trained model for each ML task.
% \cc{Maybe we could directly say it takes the output of extractor as its input}


% As described in \S~\ref{sec:method}, we want to achieve the effect of assigning higher penalties on errors in the target classes. One approach is to use the original training dataset, but assign a larger weight  in the loss function for those training samples belonging to target classes. we adopt a more efficient approach of re-sampling the training dataset so that the target classes weigh more than the original dataset. 


% To achieve the effect of assigning higher penalties on errors in the target classes, as described in \S~\ref{sec:method}, we adopt a more efficient approach of 
% \cc{No need to describe other methods}



\mypara{Pre-trained models} 
Without access to commercial MLaaS' DNNs and their training data, we use open-sourced pre-trained DNNs and their training datasets
% \shan{there are too many pre-trained models in the world. Please comment a bit on why you choose these specific models. I guess they are popular for some reasons?}\cc{These are classic network design with high accuracy. Explained in in next sentence} 
as a proxy, which are summarized in Table~\ref{tab:datasets}. 
These DNNs are trained on the ``training'' portion of their respective datasets.
They are trained to achieve good accuracy over a wide range of labels, and we have confirmed that their accuracies in terms of application decisions are similar to the real ML APIs (\S\ref{subsec:results}). 
% They are popular DNN designs with high accuracy. 
% We use the TResNet-L model~\cite{ASL}, is a variation of the ResNet model~\cite{he2016deep} pre-trained on Open Images~\cite{openimages}, as a proxy for the image classification API backend. 
% For object detection, we use the Faster-RCNN model~\cite{NIPS2015_14bfa6bb} pre-trained on COCO dataset~\cite{coco}. 
% For the three APIs performing NLP tasks, we use the BERT~\cite{devlin2018bert} model fine-tuned on the corresponding datasets. %, as listed in Table~\ref{tab:datasets}.

\mypara{Training data}
We make sure that the labels included in these datasets cover the labels used in the decision processes of the applications in our study.
An exception is text classification: to our best knowledge, there is no open-source dataset that covers the classes in Google's text classification API. 
% There lacks an open-source dataset that covers the classes in Google's text classification API. 
Instead, we use the Yahoo Question topic classification dataset~\cite{yahoo}, whose classes are similar to those used in the applications. 


Instead of training DNNs on all training data, most of which do not match any \targets of an application, we create a downsampled training set for \tool and \toolbasic.
For each application, we randomly sample (without replacement) its training data such that each \target and the non-target class (not matching any \target) is the correct decision for the same number of training inputs, which depending on applications, ranges from 12K to 40K.
With such training set, \toolbasic 
%(which assigns higher weight to loss on inputs whose correct decisions are \targets) 
will be equivalently implemented by training on the downsampled training set using the conventional loss function (\ie cross-entropy loss for classification tasks). 
Moreover, the downsampled training set significantly speedups DNN re-training (\S\ref{subsec:results}).

% Note that the loss function used by \toolbasic (\S\ref{sec:loss}) assigns a higher weight to inputs whose ground truth leads to the selection of some \targets than in the original training dataset associated with the pre-trained model. 
% This is effectively the same as training with a new dataset where inputs whose ground truth leads to the selection of \targets have a higher portion than in the one associated with the pre-trained model. 
% Thus, in the evaluation, we adopt a more efficient way of implementing \toolbasic's loss function: re-training the DNN with a downsampled dataset, where data whose ground-truth decision selects some \targets has a higher portion than the one associated with the pre-trained model.

% \jc{yuhan, please move the training data discussion to the next para}
% \shan{I am also confused that shouldn't the pre-trained model already be associated with a fixed data set? And, shouldn't the classes/labels already determined by the pre-trained model? Furthermore, if there is concerns for all but one API, then you should explicitly say so, instead of saying ``most of the classes''.} \yh{I merged pre-trained models/datasets into one paragraph, would this be better? }
% In the evaluation, we will also show that the pre-trained models we use can achieve similar performance on our metric, indicating that the pre-trained models are good proxies for the ML APIs. \cc{no need to say this}

==> bk/5-evaluation_0525.tex <==
\label{sec:evaluation}
% We apply \tool on 44 real-world open-source applications using Google, Amazon's ML APIs, which cover vision and natural language processing tasks, to answer the following questions:
Our evaluation aims to answer following questions:
% \yh{Several TODOs as suggested by JC: 1. put case study in overall results; 2. change OOD figures to show the difference between \tool and \modeld DO NOT change with distribution 3. move cost of re-training to after overall results; 4. add two another bars for the overall results}
%\begin{packeditemize}
%\item 
How much can \tool reduce incorrect application decisions? 
How long does it take \tool to customize DNN models for applications? 
% \tool's re-training cost?
and Why does \tool reduce incorrect application decisions where \toolbasic falls short?
% How robust are the benefits in reduction of incorrect decisions brought by \tool are? \jc{this is subject to change}
%\end{packeditemize}

% The key findings are: \cc{Actually I am a little bit nervous about puttign all the conclusions at the beginning. How about we put research questions here?}

% \begin{packeditemize}
%     \item Across 44 \cc{What about the others?} applications, 6 ML APIs, and 2 MLaaS providers, \tool's re-trained model selects incorrect application decisions on \fillme-\fillme\% less input compared to the pre-trained model, and \fillme-\fillme\% less input compared to the model trained on \tool's training data. 
%     \item \tool's retrained model can still achieve more reduction in the rate of incorrect application decisions, when the testing data distribution deviates from the training data distribution.
    
% \end{packeditemize}

\tightsubsection{Setup}


\begin{table}[]
\centering
\begin{footnotesize}

\begin{tabular}{llll}
\hline
                         & Dataset       & Pre-trained model \\ \hline
{\begin{tabular}[l]{@{}l@{}}Image Classification\end{tabular}}       &  OpenImages~\cite{openimages}    & TResNet-L~\cite{ASL}        \\ \hline
{\begin{tabular}[l]{@{}l@{}}Object Detection\end{tabular}}     &  COCO~\cite{coco}          & Faster-RCNN~\cite{NIPS2015_14bfa6bb}      \\ \hline
{\begin{tabular}[l]{@{}l@{}}Sentiment Analysis\end{tabular}}   &  Amazon review~\cite{marc_reviews} & BERT~\cite{devlin2018bert}              \\ \hline
{\begin{tabular}[l]{@{}l@{}}Text Classification\end{tabular}}  &  Yahoo~\cite{yahoo}  & BERT~\cite{devlin2018bert}             \\ \hline
{\begin{tabular}[l]{@{}l@{}}Entity Recognition\end{tabular}}   & conll2003 ~\cite{tjong-kim-sang-de-meulder-2003-introduction}      & BERT~\cite{devlin2018bert}               \\ \hline
\end{tabular}
\tightcaption{The ML APIs and datasets  in evaluation. }
\label{tab:datasets}
\end{footnotesize}
\end{table}
% \yh{testing / training data don't overlap}

% \begin{figure*}
%     \centering
%      \includegraphics[width=.97\linewidth]{figs/google.pdf}
%     \caption{ Overall results on 29 applications using Google's image classification API. }
% \label{fig:overall}
% \end{figure*}

% \yh{change y axis to incorrect decision rate (IDR)}
\begin{figure*}
\centering
    \subfloat[][Applications making \term{True-False} decisions.]
    {
        \includegraphics[width=0.99\textwidth]{figs/tf.pdf} 
        \label{fig:tf}
    }
    
    % \caption{Overall results on applications making \code{True-False} decisions.}
    
    \subfloat[][Applications making \term{Multi-Choice} decisions.]
    {
        \includegraphics[width=0.95\textwidth]{figs/multi_choice.pdf} 
        \label{fig:multi_choice}
    }

    \subfloat[][Applications making \term{Multi-Select} decisions.]
    {
        \includegraphics[width=0.52\textwidth]{figs/multi_select.pdf} 
        \label{fig:multi_select}
    }
    \subfloat[][Case studies on other Google's APIs. ]
    {
        \includegraphics[width=0.39\textwidth]{figs/nlp.pdf} 
        \label{fig:case_study}
    }
    \tightcaption{\tool reduces the incorrect decision rate (\Rate) on the 44 applications that use Google's or Amazon's image-classification APIs (a-c) and four applications using another four Google APIs (d). 
    For each application, \Rate is measured with the output of real APIs (even though the application source code uses a specific API) and the output of other schemes.
    % Note that the names for the applications are abbreviated. \code{PlantWat}
    % \jc{swap best api and pre-trained models}
    % \jc{yuhan, can shrink the space on the two sides of a and b?}\yh{Better now?}
    }
    % \cc{1. The font of (c) is much larger than the others. The figure should be smaller. 2. The hatch makes the figure hard to read when the bars are small. Since we have very different colors, maybe we could simply remove hatches? 3. These three figures shares same legend. We may only keep the first one. 4. Can we add a line break at y-axis title? Then we could save some space  5. Would it possible that we use abbreviation for the app names? E.g., ``Ingredient.'' or ``IngrePred'' to replace ``IngredientPrediction''. Then the x-axis labels would only take 1 line}}
    \label{fig:overall}
\end{figure*}

% \yh{put all in one figure }
% \yh{7b xticks write app names}
% \yh{Put 2-colmns table  averaging the results, 7 rows  }

% \cc{I feel this subsection is too long. I've shrinked it. Still wondering how to futher simplify it}

\mypara{Applications} We test \tool on all the 40 applications in our empirical study (\S\ref{sec:methodology}) that use image classification APIs provided by Google (\code{label\_detection}) and Amazon (\code{detect\_labels}).
% , which are all the applications in our empirical study that uses Google \code{label\_detection} and Amazon \code{detect\_labels} API.
We also perform case studies on 4 other applications, covering object detection, sentiment analysis, text classification, entity recognition APIs, 
randomly selected from our empirical study. 
% \cc{You need to explain what are the 45 applications, as they are not exactly the same as the ones in empirical study}. These applications use five ML API provided by Google and Amazon, covering ML tasks from image classification, object detection, sentiment analysis, text classification, entity recognition.


% \mypara{ML APIs} We evaluate \tool across five ML API, provided by Google and Amazon, covering ML tasks from image classification, object detection, sentiment analysis, text classification, entity recognition. Since we do not have access to the ML models in the MLaaS backend, we use pre-trained models as a proxy of the ML model supported in the MLaaS backend. Table~\ref{tab:datasets} summarizes the pre-trained models we use as proxies of the ML models in the MLaaS backend. We use the TResNet-L model~\cite{ASL}, which is a variation of the ResNet model, as a proxy for the ML model in the image classification API backend. For object detection, we use the Faster-RCNN model. For the three APIs performing NLP tasks, we use the BERT model re-trained on the corresponding Downstream tasks to approximate the ML model in the MLaaS backend. In the evaluation, we will also show that the pre-trained models we use can achieve similar performance on our metric, indicating that the pre-trained models are good proxies for the ML APIs.


% \mypara{Dataset} 
% Table~\ref{tab:datasets} summarizes the datasets we use to evaluate \tool. Again, we do not have access to the datasets the MLaaS provider uses to train their models. Instead, we use datasets that cover all the classes\shan{this makes me concerned. Can you offer more details? } \yh{The datasets we use cover all classes in all apps studied in Evaluation  \emph{except} the text classification task. because we didn't find a dataset that can cover all classes used in Google's API. The app we use to study text classification API defines two target classes, one about sensitive subjects (we approximate this with ``Politics and Government'' in our dataset), another about identity relations (we approximate this with ``Family and relationships'') }\cc{They actually are associated. We first decide the dataset, and then find pre-trained models based on them} that are used in the applications in our study, except for text-classification API. 
% We use the OpenImages dataset~\cite{openimages} for imag



% \cc{Please feel to revise the scheme name. Yuhan, if you feel good with these names, please change the other places accordingly} \yh{let's make them macros :) }
% In the evaluation, we show the results of (1) the real ML API provided by the MLaaS providers;  (2) the pre-trained model; (3) the model re-trained with rebalanced training data, where the number of ground-truth decisions for executing each branch is the same; (4) the model re-trained with rebalanced training data with the loss function constructed from the extracted \emph{software decision process}, which we refer to as the model re-trained with our solution. 



% Specifically, $K$ is determined by the minimum number
% Specifically, $K$ is determined by the smallest number of times a \target is selected by the ground-truth 
% denote the number of times a \target  $\ClassId$ is selected by ground-truth decisions in the original training as $S_\ClassId$, $K=\min_{\ClassId}S_j$ for all \targets defined in the application. 

% \shan{Is this the sampling setting for re-training or accuracy evaluation or both?} 
% \shan{How much training data do you use during re-training? Is there a setting here, like you take $K$ amount of training data for each class? I am asking this because I feel, without this information, it is difficult to assess your re-training time result.} \yh{Modified text}
% In the evaluation section, unless specified, we assume that the extent to which the application cares about each of the branches and \code{Others} is the same, as mentioned in Section~\ref{sec:method}. 

% % \cc{Would this assumption be mentioned at method sections? If so, we could simply refer to that section}
% Thus, we construct our dataset by sampling an equal number of data points from each of the branch conditions and \code{Others} (re-balancing to the smallest number of data points across all the branch conditions). 
 % We randomly split the data into training, validation, and testing sets, following standard DNN training approaches and previous work~\cite{kang2017noscope}.

% \shan{Have you explained the source of testing data? } \cc{Usually the dataset includes a training split, a testing split. Sometimes, there is an additional validation split. So I guess we do not need to explicit mention training and testing }





\mypara{Metrics} 
For each scheme (explained shortly) and each application, we calculate the \emph{incorrect decision rate} ({\em \Rate}): the fraction of testing inputs whose application decisions do not match the correct application decisions (\ie decisions based on human-annotated ground truth).
%\yh{rate of incorrect decisions = 1-accuracy, it's common to report the numbers either way. }
% , where the application decisions led by the DNN's predictions do not match with the decisions led by ground truth.
% We use the metric of the rate at which ground-truth application decisions do not match with the decisions led by the ML models' predictions, denoted as \emph{rate of incorrect decisions}. 
% \cc{Yuhan, please use error rate, instead of a long explaination in the later sections}
% For classification tasks, we count the incorrectness at the granularity of each testing input. 
% % judge the incorrectness for each input. 
% For entity recognition and object detection that include multiple  instances in one input, we count the incorrectness at the granularity of each instance. 


\mypara{Schemes}We compare the results of five schemes:
\begin{packeditemize}
    \item \emph{Various commercial ML APIs}: the results returned by the real ML APIs of three MLaaS providers (Google~\cite{google-cloud}, Amazon~\cite{amazon-ai} and Microsoft~\cite{ms-azure}).
    We do not have access to the ML models behind these APIs. 
    \item \emph{\bestapi}: 
    % \jc{yuhan, i changed the term to "Best Commercial API*". can you update the figures?}
    a hypothetical method that queries all three real ML APIs on each input and picks the best output based on the classic definitions of accuracy: label-wise recall for classification tasks and mean-square-error of floating-point output for sentiment analysis.
    This serves as an idealized reference of recent work~\cite{chen2020frugalml,chen2022frugalmct}, which tries to select the best API output with high label-wise accuracy.
    % Previous work~\cite{chen2020frugalml,chen2022frugalmct} adaptively invokes APIs from different service providers within a resource budget. We use an ``idealized'' version where we select the most accurate API among the three real ML APIs  (based on the traditional accuracy metric\footnote{We use Mean Squared Error for DNNs outputting floating point values as the metrics, and label-wise recall for DNNs outputting categorical labels. }) on each input in the testing data;
    \item \emph{Pre-trained models}: the open-sourced pre-trained model from which \tool and \toolbasic are re-trained. They serve as a reference without customization and achieve similar accuracy as the real APIs. % initialize re-training from; 
    \item \modeld: the model re-trained with \tool's training data with the conventional loss function.
    This can be seen as a baseline that uses the \summary but not our application-specific loss function.
    % with the loss function used to train the pre-trained model; 
    \item \tool (our solution): the model re-trained with our training data and loss function.
\end{packeditemize}
% Note that the pre-trained models are not necessarily the same models used by the three real ML APIs, but we have confirmed that they attain similar \Rate as the real ML APIs (Figure~\ref{fig:overall}).

\mypara{Testing data} 
For the same application, all schemes are tested against the same testing input set.
The testing set of an application is randomly sampled from the ``testing'' portion of the dataset associated with the application's pre-trained model (Table~\ref{tab:datasets}). 
We make sure that {\em no} testing input appears in the training data. 
Like the creation of training data of \tool (\S\ref{sec:implement}), by default, we randomly sample the testing data such that each \target and the non-target class (not matching any \target) appear as the correct decision for the same number of testing inputs, which ranges from 1.2K to 4K.
% By default, we randomly sample the testing data such that each \target and the non-target class (not matching any \target) appear as the correct decision for the same number $\TestNum$ of testing inputs.
% Depending on applications, $\TestNum$ ranges from 1.2K to 4K, which is 
This is similar to the testing sets used in related work on ML API (\eg~\cite{kang2018blazeit,kang2017noscope,wan2022automated, chen2022frugalmct}).
Such data downsampling is commonly used in ML~\cite{elrafey2017recent,liu2020study}
Other than Figure~\ref{fig:ood}, we will use this as the default testing dataset.
% will use different testing data distributions.
% We ensure each \target and non-target class are selected roughly equal number of times ($T$). 
% This default class-level testing distribution is identical with that of the class-level training data explained in \S\ref{sec:implement}.\jc{yuhan, doublecheck after you've added the text there}

\begin{comment}
\mypara{Testing data} In the evaluation section, unless specified, \modeld and \tool use testing data randomly sampled from the testing dataset used by the pre-trained model. 
We ensure each \target and non-target class are selected roughly equal number of times ($T$). 
For instance, given two \targets, each being selected by 2K, 5K times in the dataset used to train the pre-trained model. 
$T$ will be 2K in this case \footnote{This is a data down-sampling approach commonly adopted in ML.}.  
The training data we use to re-train \modeld and \tool is created in the same way (\S\ref{sec:runtime}), and we ensure there is no overlap between the training data and testing data.

\end{comment}



\mypara{Hardware setting}
We evaluate \tool and other approaches on a GeForce RTX 3080 GPU, and an Intel(R) Xeon(R) E5-2667 v4 CPU, with 62GB memory. 
% \cc{what about the CPU? memory? disk? Also, I think we could explain this latter when we talk about training time}

% \begin{table}[]
% \centering
% \begin{tabular}{@{}llll@{}}
% \toprule
%                   & Type-1 & Type-2 & Type-3 \\ \midrule
% Pre-trained model & 0.12   & 0.07   & 0.10   \\
% $TOOL_{basic}$   & 0.09   & 0.06   & 0.08   \\
% TOOL              & 0.06   & 0.03   & 0.05   \\ \bottomrule
% \end{tabular}
% \caption{Critical error rate for different types for \code{Aander-ETL}. 
% \label{tab:source}
% \end{table}


% \begin{figure*}
%     \centering
%      \includegraphics[width=.6\linewidth]{figs/amazon.pdf}
%     \caption{ Overall results on applications using Amazon's image classification API. }
% \label{fig:amazon}
% \end{figure*}




\begin{table}[]
\setlength\tabcolsep{5pt}
\centering
\begin{tabular}{@{}rccc@{}}
\toprule
                  & \term{True-False} & \term{Multi-Choice} & \term{Multi-Select} \\ \midrule
Google API        & 0.29       & 0.32         & 0.35         \\
Microsoft API     & 0.30       & 0.33         & 0.32         \\
Amazon API        & 0.31       & 0.33         & 0.36         \\
Pre-trained model & 0.28       & 0.30         & 0.34         \\
\bestapi         & 0.22       & 0.27         & 0.30         \\
\toolbasic  & 0.18       & 0.19         & 0.23         \\
{\bf \tool}              & {\bf 0.13}       & {\bf 0.14}        & {\bf 0.18}         \\ \bottomrule
\end{tabular}
\tightcaption{Average incorrect decision rate (\Rate) among applications that make different types of decisions using image classification APIs. The lower the better. 
% \jc{todo: highlight the last row in color}
% \cc{There is a * at best API. What is this for? Are you going to add an explaination like ``(* xxxx)''?}
}
\label{tab:overall}
\end{table}


% \tightsubsection{Overall results }

\tightsubsection{Results}
\label{subsec:results}

% ML APIs (Google, Amazon, and Microsoft, \bestapi, pre-trained models, and \toolbasic. 

% Previous work~\cite{chen2020frugalml,chen2022frugalmct} adaptively invokes several APIs from different service providers to achieve better accuracy or save cost within a resource budget. 
% To 

\mypara{Overall gains}
We start with \tool's overall reduction in \Rate over the other four schemes.
Figure~\ref{fig:overall}(a-c) summarize the average \Rate for all 40
% \cc{Please put number here} 
applications that invoke image classification APIs. 
Note that we show the abbreviations of application names in Figure~\ref{fig:overall}, where applications  in Figure~\ref{fig:code}, and the application in Figure~\ref{fig:input_example} are abbreviated as ``AanETL'', ``FoodDelivery'', ``PlantWat'', ``CodeKid'', and ``HeapSo'' respectively. 
% Among these applications, 14 make \term{True-False} decisions, 18 make \term{Multi-Choice}, and 8 make \term{Multi-Select} decisions. 
% Detailed results on each application are shown in Figure~\ref{fig:overall}. 
Compared to the real ML APIs, \tool reduces \Rate from 0.32 to 0.14 (a reduction of 56\% in the number of incorrect decisions).
\tool reduces the rate of incorrect decisions from 0.30 to 0.14 (a reduction of 53\% in number of incorrect decisions) compared to the pre-trained model.
Even compared to the \bestapi, \tool also reduces \Rate from 0.25 to 0.14 (a reduction of 44\% in the number of incorrect decisions).
As a reference, \toolbasic reduces \Rate from 0.25 to 0.19 compared to \bestapi (a reduction of 24\% in the number of incorrect decisions), which is about half the improvement by \tool.
% \jc{yuhan, please check the numbers (rate vs number) this para}
Table~\ref{tab:overall} groups the results by the three high-level decision types: \term{True-False} (14 applications), \term{Multi-Choice} (18 applications), and \term{Multi-Select} (8 applications).
The reduction in \Rate by \tool is roughly consistent across the three decision types. 

% Overall, compared to the three commercial ML APIs, \toolbasic reduces the number of incorrect decisions by 33\%-42\%, and \tool reduces the number of incorrect decisions by 48\%-58\%. 
% Compared to \bestapi, \toolbasic can reduce the rate of incorrect decisions by 15\%-25\%, while \tool can reduce the rate of incorrect decisions by 34\%-44\%.
% Compared to the pre-trained model, \toolbasic reduces the rate of incorrect decisions by 27\%-39\%, and \tool reduces the rate of incorrect decisions by 48\%-55\%. 



% Among the three types, \tool shows the greatest reduction in the rate of incorrect decisions on \term{Multi-Choice}.
% \jc{yuhan, this needs to be rephrased.} The reason is that the traversal order of the conditional checks (captured by \tool's loss function) has the most influence on \term{Multi-Choice}'s decision process (\eg the critical errors are most likely to happen on the first conditional check). 

% Note that the rate of incorrect decisions is the highest for \term{Multi-Select} applications, because a correct decision needs to select every correct \target, which is fundamentally harder than others. 

% \cc{This sentence should be put earlier. That is, you first describe how much improvement \tool and \toolbasic achieve compared to pre-trained model. Then talk about achievement over APIs. And then put all the detailed analysis (``Note that...'', ``among three types...'')} 

% \begin{figure}
%     \centering
%      \includegraphics[width=\linewidth]{figs/nlp.pdf}
%     \caption{ Overall results on applications using Amazon's image classification API. }
% \label{fig:case_study}
% \end{figure}



\mypara{Case studies on other APIs}
% To test \tool on more ML APIs, 
% To show the generalizability of \modeld, and \tool, 
Figure~\ref{fig:overall}(d) tests the other four ML APIs in Table~\ref{tab:datasets}, each with one example application that uses the API.
Across the four APIs, \tool achieves sizable reduction in \Rate compared to the baseline schemes\footnote{Amazon and Microsoft do not provide APIs for text-classification task, thus their results for text classification are not included.}.
\code{FoodDelivery} is the only application with a marginal improvement (relative to other applications).
This is because its \targets (three value ranges) roughly evenly split the full range of sentiment-analysis API output (a floating value), so any error on API output might affect the selection of a \target, so there is limited room to improve DNN.
Yet, \tool still has decent improvement as it captures other aspects of code structures, such as the decision type.
% \fillme\jc{write down the reason why the inherent room for improvement is limited}
% On the application of \fillme\jc{API name}, for instance, \tool reduces the \Rate from \fillme of the pre-trained model to \fillme.

Across \emph{all} applications, \tool reduces 53\% and 51\% of incorrect decisions, compared to the commercial ML APIs and pre-trained models, respectively.
Furthermore, even compared with the \bestapi, \tool reduces the number of incorrect decisions by 41\%.

\begin{comment}
    

\tool reduces \Rate from 0.36, 0.25, 0.30 and 0.29, to 0.30, 0.13, 0.22 and 0.21 on the four applications respectively (a reduction in number of incorrect decisions by xxx, xxx, xxx, and xxx\% respectively) compared with the pre-trained models. 
Compared with the real ML APIs, \tool reduces \Rate from 0.38, 0.24, 0.31 and 0.32 to 0.30, 0.13, 0.22 and 0.21 on the four applications respectively (a reduction in number of incorrect decisions by 21\%, 46\%, 29\%, and 34\% respectively). 
Even compared with \bestapi, \tool reduces \Rate from 
% \jc{yuhan, reduction of rate or number. rewrite the next four sentences.} \yh{updated}
% Compared with the commercial ML APIs and pre-trained models, \tool reduces the \Rate from  () on average across the four tasks. 
% Furthermore, compared with \bestapi, \tool achieves 15\%-40\% reduction in the number of incorrect decisions. 

% Lastly, compared with the pre-trained models, \modeld achieves 10\%-25\% reduction in the number of incorrect  decisions. 
% Furthermore, \tool achieves 21\%-46\% reduction in the number of incorrect decisions.
\end{comment}

% \jc{this para needs to be updated!}


\begin{comment}
    

In the image classification task, \toolbasic can reduce the label-wise errors on inputs involving \targets, where the label-wise errors are defined as the labels missed by the DNN predictions out of all the ground-truth labels for an image. 
As a concrete example, in the landmark detection application \code{Aander-ETL} (Figure~\ref{fig:code}(a)), \toolbasic reduces the number of label-wise errors by 35\% compared to the pre-trained model. 
However, because of \toolbasic's inability of identifying critical errors, which lead to incorrect decisions, it is only able to reduce the number of incorrect decisions by 28\%, going down from 0.36 to 0.26. 
\tool, on the other hand, although only able to reduce the number of label-wise errors by 26\%, it can reduce the number of incorrect decisions by 45\%. 
% In summary, compared to the pre-trained model which minimizes average errors (\eg binary cross-entropy errors for classification tasks) on a wide range of labels/scores, \modeld can prioritize the reduction of average errors on inputs involving \targets.
% Take the landmark classification application \code{Aander-ETL} (Figure~\ref{fig:code})(a)
% % \cc{Please refer to the experiment result image. Do we have a macro for application name? If so, maybe also use it}
% as an example to illustrate. 
% Compared with the pre-trained model, \toolbasic is able to reduce the label-wise errors\footnote{We define the label-wise errors for an input as the number of missing labels divided by the number of ground-truth labels.} in the testing dataset  by 35\%.
% % \cc{35\% more than pre-trained model? 35\% error of pre-trained model?}.
% However, more than 80\% of the label-wise errors reduced by \toolbasic are non-critical errors. 
% % \toolbasic spares a lot of energy \cc{I guess you are not mentioning the machine power... Maybe use another word?} reducing non-critical errors as only 18\% of the reduced label-wise errors are critical.  
% On the other hand, \tool is able to only penalize critical errors, thus leading to far more reduction (66\% more) in the rate of incorrect decisions, compared to \modeld. 
% Furthermore, the \bestapi, which also cannot distinguish between non-critical errors and critical errors, can reduce label-wise errors by 30\% compared to the actual APIs on average in the testing data. 
% However, it is only able to reduce the critical errors by 13\% compared to the actual APIs because its incapability of identifying them. 
% % \mypara{Compare with the pre-trained model}


\end{comment}

% \mypara{Google's image classification API}Figure~\ref{fig:overall} summarizes the rate of incorrect decisions of the four schemes on applications using Google’s image classification API.
% Overall, compared to the pre-trained model, \modeld reduces the rate of incorrect decisions by 35\%, going down from 0.31 to 0.20 on average across 29 applications. 
% \tool reduces the rate of incorrect decisions by 51\%, going down from 0.31 to 0.15 on average, compared to the pre-trained model.
% Compared with the actual ML APIs, \modeld and \tool reduce the rate of incorrect decisions by 39\% and 55\% on average across the three APIs. 
% % \yh{Say a few more words on this} \shan{I feel the percentage point is still a bit confusing, can be mixed with rate. How about we say increase the accuracy by how many times, or reduce the inaccuracy by how many times?} 

% \mypara{Amazon's image classification API}In addition, we apply \tool on 11 applications that use Amazon image classification API, and achieve similar reduction in the rate of incorrect decisions.  As shown in Figure~\ref{fig:amazon}, \modeld reduces rate of incorrect decisions by 28\%, going down from 0.29 to 0.21
% % \shan{What exactly is percentage point? Maybe we can just say what is one scheme's incorrectness rate and what is the other scheme's incorrectness rate?} 
% compared with the pre-trained model on average across the 11 applications. 
% The model re-trained with \tool reduces the rate of incorrect decisions by 41\%, going down from 0.29 to 0.17. 
% Furthermore,  \modeld and \tool reduce the rate of incorrect decisions by 32\% and 45\%, compared to the three actual ML APIs on average. 

% \mypara{Other Google's APIs}To show the generalizability of \modeld, and \tool, we conduct case studies on four other common ML tasks and summarize in Table~\ref{tab:datasets}. 
% As shown in Figure~\ref{fig:case_study}, \modeld achieves 10\%-25\% reduction in the rate of incorrect application decisions compared to the pre-trained model. 
% Furthermore, \tool achieves 21\%-46\% reduction in rate of incorrect decisions, compared to the pre-trained models. 
% Compared with the actual ML APIs, \modeld and \tool achieve 10-26\% and 19-43\% reduction in the rate of incorrect decisions. 




% These label-wise errors include some critical errors (\eg mis-classifying \code{Shirt} to \code{Paper} in the garbage classification application in Figure~\ref{fig:code}(a)). 
% However, \modeld fundamen83\al83864ly cannot distinguish non-critical errors and critical errors, thus may spare energy reducing  hard-to-distinguish non-critical errors (\eg mis-classifying \code{Shirt} to \code{Jacket}).
% On the other hand, \tool will only reduce the critical errors, leading to reducing 10-25\% more critical errors than \modeld.

% \yh{TODO: update this paragraph on Friday}


% \myparashort{Source of improvement} \yh{TODO: rewrite this part, show how many non-critical errors/ critical errors can \modeld / \tool reduce}
% The pre-trained model is trained to reduce average label-wise errors on a wide range of labels (\eg 9605 labels in Open Images~\cite{ASL})\footnote{Traditionally, the loss function minimizes the average error between the predicted probability and ground-truth labels for every class, which we refer to as average label-wise errors. }. 
% However, the labels included in the \targets are a very small subset of the whole label set, as we have seen in \S\ref{sec:empirical}, and errors made on the \targets only have a small impact on the overall label-wise errors. 
% As a result, it is highly possible for the pre-trained model to lead to critical errors of the applications. 
% Take the landmark classification in Figure~\ref{fig:code}(b) as an example to illustrate the source of improvement for \modeld and \tool. 
% This application makes  \term{Multi-Choice Application Choice order} decisions. 
% Three types of critical errors may occur:
% (1) Type-1: A correct \target is not matched because its \score is lower than detection threshold $\theta$. A lower-priority \target is matched, or none of the \targets is matched because of this;
% (2) Type-2: The \score for a higher-priority incorrect \target is higher than $\theta$, thus it is matched and the decision process breaks;
% (3) Type-3: Any one of the \targets is matched when the ground-truth decision selects the non-target class. 

% Table~\ref{tab:source} shows the breakdown of the three types of critical errors as described in \S\ref{sec:loss} for the pre-trained model, \modeld, and \tool. 
% The pre-trained model is trained to reduce average label-wise errors on a wide range of labels (\eg 9605 labels in Open Images~\cite{ASL})\footnote{Traditionally, the loss function minimizes the average error between the predicted probability and ground-truth labels for every class, which we refer to as average label-wise errors. }. 
% However, the labels included in the \targets are a very small subset of the whole label set, as we have seen in \S\ref{sec:empirical}, and errors made on the \targets only have a small impact on the overall label-wise errors. 
% % As a result, it is highly possible for the pre-trained model to lead to critical errors of the applications. 
% \modeld can reduce average label-wise errors on the labels appearing in the \targets, and that leads to 25\%, 14\%, 20\% reduction in each type of critical errors respectively.
% On the other hand, \tool directly minimizes the critical errors, leading to 50\%, 57\%, 50\% reduction in each type of critical errors compared to the pre-trained model. 
% It is important to note that type-2 critical errors would be inherently hard to minimize.
% When any higher-priority incorrect \target exceeds $\theta$, no matter if the correct \target is included in the output or not, this becomes a critical error. 
% We can see that \tool can reduce much more on type-2 critical errors than \modeld since it directly minimizes the critical errors. 

% \modeld can reduce the label-wise errors for labels in the \targets, but failing to include the 
% The major source of improvement for \modeld comes from its ability to include classes  defined in branch conditions in the top predictions. For example, in the nutrition advisor application in Figure~\ref{fig:code}(b), by re-training the model with rebalanced training data, the incorrect application decisions caused by missing relevant classes are reduced by 15\%. However, since the model re-trained with rebalanced training data is unaware of the critical errors\shan{This phrase seems not precise. Knowing which labels are relevant is already being aware of some of the critical errors. }, it can only reduce other types of critical errors (\eg mis-classifying grain foods into fruit, or mis-classifying an image with both grain foods and fruit to only grain foods)\shan{I really don't get this. What exactly are ``other types of critical errors''????} by 2\% compared to the pre-trained model. However, the model re-trained with \tool's loss function incorporates the critical errors, thus able to reduce both errors of missing relevant classes by 26\%, and other types of critical errors by 21\% compared to the pre-trained model\shan{It would be better if you have figures or tables or something that can show where these 26\%, 21\%, 2\%, 15\% come from.}. 
% \cc{We typically write in this way: 1) First give an overall description. 2) Then go details. 3) Explain why we are good and why others are bad. 4) If space allows, take one app together with a certain type of images as an example to explain}


% \yh{explain why the Google API's app accuracy is low, and add Google API's original accuracy}

\begin{figure}
    \centering
     \includegraphics[width=.86\linewidth]{figs/google_time.pdf}
    \tightcaption{ Re-training time for applications in Figure~\ref{fig:overall}(a). 
    % \jc{how about we only show the bars of 6(a), and make it single-column?} \cc{Maybe we do not need to show the app name, just out a title like ``Applications (in alphabetical order)''} 
    }
\label{fig:google_time}
\end{figure}

% \tightsubsection{\tool's re-training overhead}

\mypara{Customization delay}
The delay for \tool to customize the ML model for an application includes 
(1) extracting its \summary from source code, and 
(2) re-training the ML model using an application-specific loss function.
On an Intel(R) Xeon(R) E5-2667 v4 CPU machine, for all applications, our parser can always  extract the \summary from an application within 10 seconds.

Figure~\ref{fig:google_time} shows the delay of re-training DNNs for the 14 applications in Figure~\ref{fig:overall}(a) on a single RTX 3080 GPU, until the validation loss increases (\ie the model has converged). 
% Other applications have similar training delays.
% the delay of the second step. 
% the re-training time for \tool. 
The re-training delay is around 9 to 21 minutes (similar to other applications).
This is much faster 
% The re-training time for \tool is around 9 to 21 minutes to re-train the models.
% The re-training time is much smaller 
than training the DNN from scratch.
% (\eg 400+ hours on a single GPU like ours based on their training epochs~\cite{ASL}). 
We attribute \tool's faster training speed to fewer training data (40K) than the pre-trained models (540K in Open Images~\cite{openimages}), and thus fewer iterations to converge.
\tool needs fewer training data to cover the labels belonging to the \targets, and these labels account for a small fraction of all possible labels (\S\ref{subsec:study-imp}). 
This re-training overhead is likely acceptable to MLaaS; \eg a V100 GPU (with similar processing GFLOPS as our RTX 3080 GPU) only costs \$2.38 per hour on Google Cloud, so re-training an ML model for one application will incur less than \$1 on the MLaaS provider side. 

% \shan{I feel some explanation is needed to help me interpret this result. Is the re-training time short because we are not using much data for re-training? Or is it because re-training converge fast?} \yh{Added some explanation in the next sentence}. 

% \tool's re-training overhead is low due to quick convergence with a much smaller amount of training data, compared to the one used to train a ML model from scratch.
% % \yh{Pre-training time. lowerend compared with other papers }
% For instance,  \tool uses less than 40K images to re-train the DNN for image classification applications, which is much smaller than the one used to train the DNN from scratch (\ie 540K images).
% Given that \tool's solution lies in the MLaaS backend side, this re-training cost is acceptable. 
% To justify, a V100 GPU (with similar processing GFLOPS as RTX 3080 GPU) only costs \$2.38 per hour on Google Cloud Computing platform. 
% Thus, \tool's re-training procedure will only incur less than \$1 on the MLaaS provider side. 




% \tightsubsection{In-depth analysis}
% We next perform in-depth analysis  to study how robust is \tool, and the precision and recall trade-off of \tool. 



\begin{comment}
    


% \yh{Sensitivity test }
% \yh{In terms of precision / recall trade-off. we are still better than baselines  }
\mypara{Sensitivity test on \tool's improvement}\tool can outperform \toolbasic more on \targets whose correctness greatly depends on the order of conditional checks. 
For instance, for applications making \term{Multi-Choice App-Order} decisions, \targets examined later would benefit more from \tool's loss function. 
% The reason is that critical errors like outputting labels in \targets examined earlier (\eg \code{Landmark} in Figure~\ref{fig:code}(a)) for inputs whose ground truth selects \targets examined later (\eg \code{Building}) are hard to reduce without knowing the order of the conditional checks.
The reason is that without knowing the order of the conditional checks,  the DNN is likely to lead to critical errors like outputting labels in \targets examined earlier (\eg \code{Landmark} in Figure~\ref{fig:code}(a)) for inputs whose ground-truth decision selects \targets examined later on(\eg \code{Building}). 
Figure~\ref{fig:ood} shows the difference in the rate of incorrect decisions between \tool and \toolbasic for the landmark classification application \code{Aander-ETL} in Figure~\ref{fig:code}(a), where the higher the difference is, the more benefit of \tool over \toolbasic is. 
Each of the three plots increases the fraction of each \target, where the testing distribution deviates more from the default (which is also the training data distribution) moving further to the right.
As we can see, the benefit of \tool over \toolbasic increases when the fraction of later-examined \targets (\eg \code{Building} or \code{Person}) increases.

\end{comment}

% \tool's ability to distinguish between non-critical and critical errors does not change with respect to testing data distributions. 
% The reason is that no matter how testing data distribution changes, which errors are critical (\eg mis-classifying a \code{Paper} image to \code{Shirt} in the garbage classification application) will not change.
% This complies with our observation. 
% In
% Figure~\ref{fig:ood}, we vary the testing data distribution to deviate from the default distribution (which is also the training data distribution), and show the difference in the rate of incorrect decisions between \modeld and \tool.
% The left most bar is the result under the default setting of testing data distribution, and the bars further to the right show the results when testing distributions deviate further from the default one.
% % The figures illustrate the difference in the rate of incorrect decisions between \modeld and \tool. 
% % \yh{First explain reason}
% We can see that the benefits brought by \tool over \modeld (\ie identifying the critical errors in application decision processes) remain nearly constant when the testing data distribution deviates further from default. 
% % This is because the critical errors are not related 

% The benefits brought by \tool that identifies  critical errors in the  decision processes only vary slightly when the testing data distribution deviates further from the training data distribution. 



% decisions when the testing data distribution deviates from the training data distribution. The axis is the testing distribution ordered by the deviation from the training distribution, where the left most group shows the results without data distribution difference.


% We can see that \tool's re-trained model can still provide reduction in incorrect  decisions even when the testing data distribution deviates from the training data's. The rate of incorrect  decisions for the model re-trained with rebalanced training data increases when the testing data distribution deviates further from the testing data distribution. The intuition behind this trend is that the extra information seen by the model re-trained with rebalanced dataset is the class distribution used in the testing phase (\ie equally distributed across branch conditions), and it is only able to reduce incorrect  decisions for classes that are less dominant in the original dataset, but have a larger portion in the rebalanced dataset. As a result, deviating from this specific distribution will lead to worse performance. 

% The rate of incorrect application decisions for the model re-trained with our solution also increases when the testing distribution deviates from the training distribution, while it increases at a slower rate compared with the model re-trained with rebalanced training data. The reason is that other than the rebalanced data distribution, \tool's proposed loss functions also take the critical errors for the applications into consideration, thus not biasing towards reducing incorrect application decisions for certain classes like the model re-trained with rebalanced datset.  


% \begin{figure}
%     \centering
%      \includegraphics[width=.8\linewidth]{figs/ood_hot.pdf}
%     \caption{ Robustness analysis for \code{Foodier} \cc{Is Foodier introduced some where? Similar problems with other images. Please make sure that you introduced them some where. If it is introduced earlier, please refer to the section or the image}. }
% \label{fig:ood2}
% \end{figure}






\begin{figure}
    \centering
     \includegraphics[width=.99\linewidth]{figs/pr_garbage.pdf}
    \tightcaption{ Precision-recall trade-off for \code{HeapsortCypher}. }
\label{fig:pr}
\end{figure}
\mypara{Precision-recall tradeoffs}
Traditionally, for a trained ML model, it is common to vary the confidence-score thresholds in order to find the best precision-recall tradeoff of a trained model. 
Thus, it is important that \tool also achieves better precision-recall tradeoffs.
% than the baselines of pre-traiend model and \toolbasic. 
Figure~\ref{fig:pr} shows the precision-recall results in each  \target of a particular application,
% \mypara{Understanding the effect of different detection thresholds $\theta$}An ML model in the MLaaS backend may perform well by trading-off the precision of one \target with the recall of another \target. 
% To see \tool's re-trained model does not, we plotted the precision and recall trade-off of each \target for the garbage classification application (Figure~\ref{fig:code}(b)) for the pre-trained model, \toolbasic, and \tool, 
by varying the detection threshold $\theta$ (defined in \S\ref{sec:loss}) of two baselines (real APIs are excluded, because we cannot change their thresholds and their \Rate is not as low as \toolbasic). 
\tool's tradeoffs are better than both baselines (and we observe similar results in other applications).
Note that since \tool's loss function uses an assumed $\theta$, we do not vary the $\theta$ when testing it; instead, we re-train five DNNs of \tool, each with a different $\theta$ and test them with their respective thresholds.

% for each point corresponding  to \tool, we re-train the model with a different $\theta$. 
% As we can see, for each \target, \tool performs better in terms of precision and recall trade-off than the pre-trained model and \toolbasic. 




\mypara{Understanding the improvement}
\tool's unique advantage is that it factors in the decision process of an application (its \targets, decision type, matching order), rather than which labels in \targets (\S\ref{sec:loss}).
% So far, we have only seen the effect of such advantage manifested in the reduction of overall \Rate. 
Next, we use two case studies to reveal the underlying tradeoffs made by \tool to achieve its improvement.

First, given a decision process, some \targets are naturally more important, so \tool should learn to reduce more of critical errors related to these \targets (\S\ref{subsec:study-mech}).
This effect is particularly striking in \term{Multi-Choice} applications with the matching order of \term{App-Order}, where the first \target is always matched against API output.
% so if the correct \target is not the first one, misclassifying a label within the first \target will .
Thus, when the correct \target is not the first one, falsely including a label that belongs to the first \target will more likely be a critical error than other mis-classifications, because it will block the match of other \targets.
% To show \tool does reduce more critical errors related to the first \target in such application, 
To illustrate this, we consider the \term{Multi-Choice} application of \code{Aander-ETL}.
We increase the percentage of testing inputs whose correct action is the first \target or the last \target.
Figure~\ref{fig:ood} shows that increasing the portion of inputs of the first \target (\code{Landmark}) generally leads to smaller gains of \tool, whereas increasing the portion of the last \target (\code{Person}) does the opposite. 
This shows that \tool has learned to prevent critical errors when the correct \target is not the first \target.
% , suggesting that \tool is sensitive to structures in a decision process.

% , the matching order, between the \targets and the API output labels, dictates that the first \target

\begin{figure}
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-overall-1.pdf}
    % \subfloat[][\centering{Object detection\\~~~~(Dashcam)}]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/detection_dashcam_FPN.pdf}
    %     \label{subfig:1}
    % }
        \includegraphics[width=0.44\textwidth]{figs/ood_landmark.pdf} 
    % \subfloat[][Smart wardrobe application \code{roblab-hslu}]
    % {
    %     \includegraphics[width=0.33\textwidth]{figs/ood_coat.pdf} 
    %     \label{fig:ood_coat}
    % }
    % \subfloat[][Landmark classification application \code{Aander-ETL}]
    % {
    %     \includegraphics[width=0.33\textwidth]{figs/ood_landmarks.pdf} 
    %     \label{subfig:3}
    % \yh{y-axis: (\Rate(\toolbasic)-\Rate(\tool))}
    % }
    \tightcaption{How the accuracy advantage of \tool changes with different input distribution.
    %. X-axis is the fraction of input on \code{Landmark} (the first \target), and \code{Person} (the last \target), and y-axis is the difference in the rate of incorrect decisions between \tool and the pre-trained model. 
    % \vspace{0.1cm}
    }
    \label{fig:ood}
\end{figure}
% \mypara{Understanding the gain of \tool}
% Recall that the advantage of \tool over \toolbasic is its awareness of the \targets and decision process of an application, rather than simply what labels are in any \target (\S\ref{sec:loss}).

Second, recall from \S\ref{sec:loss} that our loss function helps to minimize critical errors, even at the cost of missing labels that do not affect application decisions (\ie non-critical errors). 
To show this, we define {\em label missing rate} on an image as the fraction of the image's ground-truth labels that are missed by the DNN output (a label list). 
We consider \code{IoTWor} (explained in Table~\ref{tab:stats}), which similar to \code{Anander-ETL} makes \term{Multi-Choice} decisions with \term{App-Order} matching order.
The average label missing rate of \tool on our testing images is 0.21, which is slightly higher than \toolbasic's 0.18. This means \tool makes more label-level mistakes than \toolbasic. 
However, our \Rate (0.17) is 44\% lower than \toolbasic, which means \tool makes far fewer critical errors.

==> bk/7-related_works_0525.tex <==
\label{sec:related}

Due to space constraints, we discuss related papers that have not been discussed earlier in the paper.
% P1: Network Adaptation
% P2: ML-related runtime techniques (System and DNN)
% P3: Cloud service runtime techniques

% \jc{can i suggest the following flow. just a slightly different organization of the same substance.

% \begin{packeditemize}
% \item {\bf techniques that optimizes delay, storage, or throughput.} this include smart distillation, model prunning, scheduling, etc. instead, \tool minimizes inaccurate application decisions
% \item {\bf techniques that require changes to ML API.} this includes those based on sql, etc. instead, \tool doesn't require changes to existing APIs
% \item {\bf techniques that changes the user-side application.} this includes chengcheng's work, frugal, etc. instead, \tool only changes the MLaaS backend.
% \item {\bf others:}
% % like measurements of commercial MLaaS, academic MLaaS systems (including serving and training), and we are orthorgonal to them
% \end{packeditemize}}
% % \yh{last point: TVM/Clipper etc. }

% \mypara{Techniques that optimize delay, storage, or throughput}
\mypara{Optimizing storage and throughput of DNN serving}
Various techniques have been proposed to optimize the delay, throughput, and storage of ML models via model distillation~\cite{mullapudi2019online,shen2017fast,poe}, pruning~\cite{mcdnn} or cascading~\cite{cao2021thia,anderson2019physical}. 
This line of work explores a different design space than \tool: they design ML models with higher inference speed or smaller model size with minimum loss in accuracy. 
\tool focuses on re-training existing ML models such that the rate of incorrect decisions of a given application is reduced. 

%\mypara{New interface for ML serving} Several recent efforts propose new query interfaces that allow applications to specify their intent (\eg counting average number of cars in a specific video clip), and train models to serve the intent. For instance, a line of recent work trains specialized ML models to answer queries specified in SQL~\cite{kang2018blazeit,kang2017noscope,koudas2020video,figo,cao2021thia}.
%In contrast, our work keeps the existing generic ML APIs (\eg those in Table~\ref{tab:all_stats}) and automatically extracts the application decision processes from applications' source code, without needing users to provide extra information other than the query input.
% , and does not require 
% users provide any extra information other than the querying input.  

% \mypara{Techniques that require changes to application source code}
\mypara{Application-side optimization}
Recent work also proposes to change the applications to better leverage existing MLaaS and ML APIs.
One line of work~\cite{chen2020frugalml,chen2022frugalmct,xie2022cost} invokes ML APIs from different service providers to achieve high accuracy within a query cost budget. 
Another line of work aims to eliminate  misuse of ML APIs in applications~\cite{wan2021machine,wan2022automated}. 
They require changes to the application source code (\eg changing the API input preparation, switching from image-classification API to object-detectin API, etc.).
They are complementary to our work, because we customize the MLaaS backend DNN and do not require changes on the application's source code. 

% \mypara{Neural Network adaptation} Much work has been proposed to adapt neural network to achieve higher inference accuracy.
% Several work~\cite{tajbakhsh2016convolutional, yanai2015food, kading2016fine,vasan2020imcfn,jung2015joint} fine-tunes existing neural network model to apply on a slightly different problem domain.
% Other work~\cite{royer2015classifier, zintgraf2019fast, wang2021tent, chen2022contrastive, li2021faster} studies domain adaptation to generalize neural networks to solve data unseen during its training procedure. 
% However, these work only improves neural network itself, without the knowledge of software decision process. 
% % \cc{yuhan, please add some more categories. These are two types of adaptation I have in mind}

% Another line of work aims to reduce latency by compressing DNNs to perform a specialized task defined by a subset of SQL syntax~\cite{kang2018blazeit, kang2017noscope,cao2021thia,figo}. 
% They cannot improve inference accuracy and thus are not able to eliminate software misbehaviors. 


% \mypara{ML Software}
% Several work aim to improve software that uses ML APIs. One line of work optimizes inference accuracy by adaptively invoking several APIs from different service providers within a resource budget~\cite{chen2020frugalml, chen2022frugalmct,xie2022cost}. Another line of work aims to eliminate software misuse of ML APIs~\cite{wan2021machine,wan2022automated}. These work aims to improve client-side and requires developers to modify their implementation. They are orthogonal to our work.





% \mypara{ML-as-a-Service and inference/training  system}Other line of work studies the quality of ML-as-a-Service platform, including 
\mypara{Measurement work on MLaaS}
For their rising popularity, ML-as-a-Service platforms have also attracted many measurement studies to understand 
accuracy~\cite{chen2021did}, performance~\cite{yao2017complexity}, robustness~\cite{hosseini2017google}, and fairness~\cite{koenecke2020racial}. 
However, they have so far not taken in account the ML applications that use ML APIs, and is thus different from our empirical study of ML applications in \S\ref{sec:empirical}. Previous work that studies ML applications \cite{wan2021machine} did not look
into the decision making process and how ML API errors might affect 
different applications differently.
% However, they ignore the applications invoking ML APIs and do not provide customized solutions.

Finally, a myriad of techniques have been studied to better manage and schedule GPU resources in ML training/serving systems (\eg~\cite{clipper,infaas,inferline,mlaasinthewild,zhang2018deepcpu,grnn,zhang2019mark,parity,shen2019nexus,gujarati2020serving,lee2018pretzel,mohan2022looking,8980322,han2022microsecond,choi2022serving}).
They aim for different goals than \tool, but these techniques can be used to help \tool train and serve the application-specific ML models. 

% Another line of work~\cite{clipper,infaas,inferline,mlaasinthewild,zhang2018deepcpu,grnn,zhang2019mark,parity,shen2019nexus,gujarati2020serving,lee2018pretzel,mohan2022looking,8980322,han2022microsecond,choi2022serving} focuses on the scheduling algorithm and resource management in inference serving system, aiming to improve model inference throughput with a latency SLO. 

% Other proposals design efficient training systems aiming at accelerating the DNN training with model or data parallelism~\cite{pipedream,zheng2022alpa,park2020hetpipe,unger2022unity}, or managing resources in GPU clusters~\cite{qiao2021pollux,xiao2020antman,xiao2018gandiva,gu2019tiresias}.

% \tool differs in that it aims at reducing the rate of incorrect  decisions for applications invoking ML APIs by re-training the DNN in the MLaaS backend. 



% Existing work proposes solutions to improve the performance or accuracy of ML models without the knowledge of the software. However, we are tackling a different problem than these prior work. 
% One line of work optimizes the ML APIs' query accuracy or cost by adaptively choosing a sequential strategy to invoke available APIs within a resource budget ~\cite{chen2020frugalml, chen2022frugalmct}. 
% These work requires modifications on the developers' side, such as changing the code to apply the most accurate API. 

% Another line of work trains specialized models performing the tasks specified through a subset of SQL queries, such as aggregation and limit, such that the inference delay is reduced ~\cite{kang2018blazeit, kang2017noscope}. 
% The problem we are targeting at is different from this line of work for the following reasons. Firstly, these approaches cannot guide the ML APIs to produce outputs that lead to correct software behaviors, as they only optimize for inference delay instead of improving the model. Secondly, a great number of existing applications on GitHub calling ML APIs are written in Python~\cite{wan2021machine} instead of SQL. Thirdly, the operations that can be expressed in SQL queries that the prior work optimizes for are limited. For example, the SQL queries that are optimized by these work can only count average number of objects among all the video frames, or selecting limited number of frames that meet several constraints. Nevertheless, there are a wider range of operations that can be expressed by Python. For example, aggregation or limit queries cannot specify subsets of labels can have the same effects on the final program behaviors. 
% Lastly, in order to use the these systems that optimize for SQL queries, users need to translate their code into SQL queries, which incurs an extra development burden for the users.


% Existing work proposes solutions to improve the performance or accuracy of ML models in software applications.
% However, we found that existing solutions are not desirable as they add extra burden on the developers.
% Specifically, one line of works focus on improving accuracy of ML task itself by modifying the software call to the ML APIs~\cite{chen2020frugalml, chen2022frugalmct}. 
% Given a resource budget, they adaptively invokes several ML APIs from different cloud providers and ensemble their results. 
% However, this approach require changing the software implementation in order to call different ML APIs, thus creating extra burden to the developers\shan{I find this argument very weak: the change required sounds very minimal and can be easily wrapped inside a library call. More importantly, I feel there are much more fundamental differences between your work and this previous work and yet you didn't mention.}.
% Another line of work aims to reduce latency by compressing DNNs to perform a specialized task defined by a subset of SQL syntax~\cite{kang2018blazeit, kang2017noscope}. 
% However, this approach cannot correct the software misbehavior triggered by wrong DNN output (as the DNN compression reduces the DNN latency while keeping the DNN ouput the same). 
% Besides, this approach adds extra developer effort to reimplement their software logic (which is typically written in Python~\cite{wan2021machine}) using SQL syntax.

==> bk/8-conclusion_0525.tex <==
\label{sec:conclusion}

MLaaS is popular for its accessibility to application developers who do not have the expertise to design and train their own ML models. In this paper, we study how the generic MLaaS APIs might affect different applications' control-flow decisions in different ways, and how some API output errors may or may not be critical due to the application decision making logic. Guided by this study, we have designed \tool that offers both the accuracy advantage of a custom ML model and the accessibility of the traditional MLaaS. 

==> bk/backups_before_fist_submission/1-introduction-0927.tex <==
\label{sec:intro}

\subsection{Motivation}
Nowadays, there have been an increasing number of software applications with the need of deploying deep neural networks (DNNs) to understand what is present in the images. Due to the heavy burden of designing and training such DNNs, many software developers use off-the-shelf machine learning (ML) APIs provided by many cloud service providers (\eg Google, Microsoft, Amazon) to reduce their development effort~\cite{wan2021machine}. However, the generic ML APIs might not be able to solve the tasks that the software intends to perform. 

When the service providers design the ML APIs, their goal is mainly to improve traditional class-wise accuracy metrics (\ie high average recall and precision)~\cite{wang2020multi} over all classes for large-scale datasets. However, when developers employ the ML APIs in their software, they care about whether ML APIs' outputs match their expectations (\ie as if the ML APIs' outputs are exactly the ground-truth labels). This gap in service providers' and software developers' purposes can lead to many software mis-behaviors, thus model adaptation is needed to provide a customized model that reduces software mis-behaviors as much as possible.





% Therefore, there is a need to adapt the ML APIs to directly optimize for producing correct software behaviors \cc{``ML APIs are xxx, while software are xxxx. Therefore, there is a need to adapt xxx''} 

To understand how and why optimizing class-wise accuracy does not necessarily lead to the correct software behaviors, we take the software application Smart can in Figure~\ref{fig:app_example} as an example. This application defines three lists to classify trash into categories. It calls Google's multi-label classification API to get the labels that describe the content in the image. The application then compares the output labels, ranked with descending order of confidence scores, with the three lists and returns the corresponding judgment if the outputs intersect with one of the lists. 
% goes through the output labels, and executes a branch if an output label is included in its corresponding pre-defined list. 

% and 
% then performs a post-processing step which executes one of \emph{Recycle, Compost, } and \emph{Donate} branches if the output labels contain any of the keywords specified in the pre-defined list \code{Recycle, Compost, Donate} \cc{``the pre-defined list'', you need to explain what is recycle, as it means a branch in the last reference} .


This simple post-processing step incurs potential software mis-behaviors even with a highly reliable ML API. For example, consider an input image (trash\_image) with ground-truth labels specified in the figure. The multi-label classification API returns an ordered list of labels, ranked in descending order of confidence scores. If we measure the outputs according to traditional recall and precision, this output yields a recall of 100\% and a precision of 80\%. Nevertheless, this output is completely wrong from the view of the software.  
According to the ground-truth labels, the correct branch to be executed is the one that returns ``This belongs to Compost'', since the only intersection between the ground-truth labels and the three lists is the one associated with the \emph{Compost} branch. However, the API's outputs lead to the program executing the branch which returns ``This belongs to Recycle. ''

% where its ground-truth labels include \emph{['Alcoholic beverage', \textcolor{red}{``Glass''}, 'Cocktail', 'Liqueur', 'Stemware'] }, and the API outputs are \emph{['Stemware', \textcolor{cyan}{``Food''}, 'Cocktail', 'Alcoholic beverage', 'Liqueur', 'Wine', \textcolor{red}{``Glass''}]}\cc{Maybe create a figure with a concrete image example and show the list (use color to show overlaps). 
% \yh{}
% Reader have to work hard to understand what is going on here }. This output yields a per-example recall of 100\% and precision of 71.5\%, while this prediction will be considered completely wrong from the view of the software. To be more specific, the correct branch to be executed, according to the ground-truth labels, should be \textcolor{red}{Recycle}. However, the labels generated by the ML API will lead to executing the branch which returns Compost. 
% \cc{This is not reason, but a detailed version of ``software considers it wrong''. Maybe use another way to describe this fact. Also, ``human-labeled ground-truth label'' and ``expected'' seem come out of blue. Suddenly human appears, and there is an expectation. You may just say the correct branch is xxx, according the ground-truth label} 

% This example demonstrates a common pattern of the mismatch between the generic tasks that the ML APIs are designed for and the specific tasks the software intends to perform. 
This is not the only case where the ML APIs' outputs lead to wrong software behaviors. When the software developers use the ML APIs in specific scenarios (\eg performing garbage classification), errors made by the ML APIs have different levels of severity: errors that lead to wrong software behaviors are more damaging than others. For example, false positives that lead to the program executing the wrong program branches, such as the ``Glass'' prediction that leads to the Recycle branch, are more devastating than false positives that are not included in the pre-defined lists associated with wrong program branches. 
Thus, an ideal solution for using ML APIs in the software is to customize the DNNs behind the ML APIs to reduce the errors that lead to wrong software behaviors. 
% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

Automatically adapting the ML APIs has many challenges. 

\begin{itemize}

\item First, automatic model adaptation is hard. We need to infer the software-specific task from the software. The software developers did not explicitly specify the specific tasks they are performing and are not able to specify the specific tasks in the format that can be directly used to optimize the DNNs behind the ML APIs. 

% from the software about the specific task. 
% why infer? Users didn't explicitly specify the tasks, and they are non-experts, so they are not able to specify the tasks in the form that can be directly used to optimize for DNNs' accuracy 
% It is unrealistic to provide extra input for model adaptation (\eg manuals for performing model re-training) at the software developers' end. The main reason is that the software developers who call the ML APIs are typically non-experts in ML, thus it is hard for them to provide an effective model adaptation strategy. 


\item Secondly, model adaptation needs to be very efficient. As the software developers typically lack the computation resources to perform model training, model adaptation has to happen on the cloud service providers' side. Thus, it is important to provide a quick way of adapting models which reduces errors leading to wrong software behaviors with minimum training cost. 


% such that the number of damaging errors leading to incorrect software behaviors can be reduced most effectively (\ie incurring minimal training cost).  

% \item We performed empirical study on the applications that use ML APIs performing image classification tasks to affect the control flow of the software. We found that a common pattern 


% \item Machine Learning (ML) offers effective ML APIs to a wide range of cognition tasks. Many cloud providers offer ML APIs, supported by underlying Deep Neural Networks (DNNs), that perform well on generic tasks (\eg image classification). These ML APIs are utilized in a wide range of software applications for different specific tasks. However, the ML APIs are not adapted to achieve the application specific tasks, leading to many software misbehaviors.
    % \item List an application such that why/how high class-wise accuracy does not lead to correct software behavior or vice versa and cite~\cite{wan2022automated} to illustrate that there are many such applications. 
    % \ref{fig:app_example} is an example software that incorporates Google \code{label\_detection} API, which outputs all the existing labels in the input image. If we consider traditional class-wise F1 score of the application, the ML API can achieve 
    % \item Here we define the software achieving correct behaviors if the outputs of the ML APIs lead to the same software behavior as if the ground-truth is returned.  
    % \item Explain why the accuracy of the software would be low: the service providers train the ML models aiming to maximize class-wise accuracy, while the software developers need to ensure correct software behavior given the ML API outputs.  
    % \begin{itemize}
    %     \item the service providers pre-train the ML models that support the ML APIs with large-scale datasets (\eg Open Images dataset), aiming at providing good class-wise accuracy. \cc{Do you want to emphasis that they have different optimization goals?}
    %     \item When software developers use the ML APIs in their software, they expect the ML APIs to output classes that lead to the correct software behavior (\ie same software behavior as what the ground-truth leads to) \cc{What's the different between point2 \& 3?} 
    %     \item The pre-trained ML models may make mistakes that lead to the wrong software behavior
    % \end{itemize}
    

    % \item Automatically adapting the ML APIs to the software is important: (1) The developers who use the ML APIs are usually not experts in ML, thus may not know how to adapt the models (2) The developers do not have an affordable way to support model adaptation. 
    % \yh{mention why automation is important}
    % \yh{Emphasize that the problem is important}
    
    
    
    % \item However, when the developers use the ML APIs in their software, they are either unaware of the mismatch between ML APIs' accuracy and software's accuracy, or they do not have an affordable way to adapt the ML APIs to fit the software application they are writing.  \yh{Define affordable: 1. developers do not need to provide training data 2. they do not need to specify what are the context that can be digested by the DNNs to improve accuracy. }
    % \item Automatically adapting the ML APIs to the software is challenging. 
    % \begin{itemize}
    %     \item No existing benchmark has shown that there is a discrepancy between the outputs resulting in high class-wise accuracies and the ones leading to the correct software behaviors

    %     % (prior works either (1) only study ML APIs themselves (2) realize the low accuracy of ML APIs in the software~\cite{wan2021machine} (3) do not understand why the ML APIs do not work when applying to the software (SW only cares about branch prediction are correct) )
    %     % \item Need to transform cognition task into math expression 
    %     % create the template 
    %     \item Need to extract software specific cognitive task automatically and transform the extracted software context into mathematical expression that enables ML API adaptation
    %     \item Need to adapt the ML APIs efficiently 
       
    % \end{itemize}
    
    
    
    
    
    % \yh{To adapt the ML solutions to the software, software developers face many issues... (or accuracy decrease) or say adaptation is very important}
    % \yh{why do adaptation ? if not, will cause accuracy decrease. }
    
    % \yh{Developers did not realize this issue or they do not have an affordable way to adapt}
    
    % \yh{List an example}
    
    
    % \yh{Automatically adapt to the software is challenging. }
    

   
\end{itemize}
Existing works have performed model customization in different scenarios. 
They either directly input (\eg the classes that need to be classified)~\cite{kim2021pool, cao2021thia} or specify the specific tasks through a fixed program interface (\eg SQL)~\cite{kang2018blazeit}, and adjust the models, by training specialized models or reorganize different pre-trained model components, based on the specific tasks. Another line of work observes run-time data distribution and customizes the model to fit the specific content in the data. 

\begin{figure}
   \centering
\begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Recycle = ['plastic', 'wood', 'glass', 'paper', 'cardboard', 'metal', 'aluminum', 'tin', 'carton']
Compost = ['food', 'produce', 'snack']
Donate = ['clothing', 'jacket', 'shirt', 'pants', 'footwear', 'shoe']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Recycle:
    return 'It is recyclable.'
  if obj.name in Compost:
    return 'It is compostable.'
  if obj.name in Donate:
    return 'It is donatable.'
\end{lstlisting}
\includegraphics[width=.99\linewidth]{figs/app_example2.pdf}
    \caption{Heapsortcypher, a smart can application \cite{xxx} using Google Cloud API.}
    \label{fig:app_example}
    
\end{figure}
\subsection{Contributions} 
\begin{itemize}
%  \item We present \tool, which is an end-to-end system which automatically extracts software context from the applications that incorporate ML APIs, and adapt the ML models to improve the software accuracy. 
\item Studied a wide range of software applications that incorporate image classification APIs, and identified that one of the common software-specific tasks is mapping fine-grained ML API output classes to program branches. 
\item Automatically extracts the software-specific task from the code the software developers write, and transforms it into a mathematical expression that can adapt the ML APIs to the software. 
% Defined a template to automatically transform the code that the software developers write into mathematical expression that can adapt the ML APIs to the software. 
% \item defined the template and the transformation to math expression 
\item Leveraged two ways of model adaptation with the defined software context that (1) changes the training data distribution to reflect the subset of classes that the users care about; (2) modifies training loss function to directly optimize for the software-specific task. 
% \item Compared the ways of model adaptation in terms of accuracy improvement and training cost on \todo{X} real applications using ML APIs.

% defined two types of software context that can improve the accuracy of the software: (1) Data distribution context; (2) Subset of classes context. 

% \item Developed a tool to automatically extract the defined context from the Python code written by software developers 


\end{itemize}

==> bk/backups_before_fist_submission/1-introduction-1004.tex <==
\label{sec:intro}

% \subsection{Motivation}

% \kt{It is not common to put subsections inside introduction (I'm not sure if it is common in SE community though)}
Nowadays, there have been an increasing number of software applications with the need of deploying deep neural networks (DNNs) to understand what is present in the input. Due to the heavy burden of designing and training such DNNs
% \kt{need citations here}
, many software developers use off-the-shelf machine learning (ML) APIs provided by many cloud service providers (\eg Google, Microsoft, Amazon) to reduce their development effort~\cite{wan2021machine}.  However, the generic ML APIs with good accuracy might lead to misbehaviors when applied to the software.
% \kt{The argument ``the software misbehavior is because that APIs are agnostic to software'' is an important argument and it directly leads to your key contribution. You bring this point too quick without much support, making this argument sounds trivial. I would suggest we postpone the mentioning of this point and just say a general ML API with good performance can lead to a lot of software behavior.}
% \yh{example: use the figure 1 example }
% \yh{existing works cost reduction by leveraging e.g., model compression 

% correct software misbehaviors by improving the ml models  =>  }

To illustrate how ML APIs with good accuracy may lead to software misbehaviors,
% how and why optimizing class-wise accuracy does not necessarily lead to the correct software behaviors,
% \kt{Maybe discribe the software behavior following the processing order of the software, like input -> API -> labels -> list -> output}
we take the software application \emph{Heapsortcypher} in Figure~\ref{fig:app_example} as an example. The application takes an image as input, and calls Google's multi-label classification API to get the labels that describe the content in the image. This application then goes through a post-processing step which classifies the ML APIs' outputs into categories of garbage. The application pre-defines three lists, \emph{Recycle, Compost, and Donate}. It then checks the output labels (\eg [Glass, Candy, Snack, Confectionery, Lollipop]), ranked with descending order of confidence scores, and searches for the first label (\eg Glass) that matches any of the labels in the three pre-defined lists. Then it executes the branch that corresponds to the found pre-defined list (\eg the one that outputs returns ``It is recyclable. '').
% the corresponding judgment if the outputs intersect with one of the lists. 

% and 
% then performs a post-processing step which executes one of \emph{Recycle, Compost, } and \emph{Donate} branches if the output labels contain any of the keywords specified in the pre-defined list \code{Recycle, Compost, Donate} \cc{``the pre-defined list'', you need to explain what is recycle, as it means a branch in the last reference} .


This simple post-processing step incurs potential software mis-behaviors even with an ML API that is able to correctly identify most of the classes.
% \kt{80\% recall does not sound like highly reliable. Also, ``highly reliable'' is vague. Maybe just say ``even when the ML API correctly identifies most of the classes''.} 
 Figure~\ref{fig:app_example2} shows a concrete example of how \emph{Heapsortcypher} works.  
% \cc{Maybe directly say that ``the bottom of Figure 1 shows a concrete example'', instead repeating what we have introduced earlier} 
 Given the outputs of the ML API, if we use traditional recall and precision as the metrics~\cite{wang2020multi}, this output yields a recall of 100\% and a precision of 80\%. Nevertheless, this output is completely wrong from the view of the software. 
According to the ground-truth labels, the correct branch to be executed is the one that returns ``It is compostable. '', since the only intersection between the ground-truth labels and the three lists is the one associated with the \emph{Compost} branch. However, the API's outputs lead to the program executing the branch which returns ``It is recyclable. '' \kt{From a system guy's perspective, I guess it is better  to highlight the cost of such software misbehavior. I'm not sure if this is needed in SE conference though.}
% \cc{P4 \& 5 have duplicate description}
%\cc{Maybe create a figure with a concrete image example and show the list (use color to show overlaps). 
% \yh{}
% Reader have to work hard to understand what is going on here }. This output yields a per-example recall of 100\% and precision of 71.5\%, while this prediction will be considered completely wrong from the view of the software. To be more specific, the correct branch to be executed, according to the ground-truth labels, should be \textcolor{red}{Recycle}. However, the labels generated by the ML API will lead to executing the branch which returns Compost. 
% \cc{This is not reason, but a detailed version of ``software considers it wrong''. Maybe use another way to describe this fact. Also, ``human-labeled ground-truth label'' and ``expected'' seem come out of blue. Suddenly human appears, and there is an expectation. You may just say the correct branch is xxx, according the ground-truth label} 

% This example demonstrates a common pattern of the mismatch between the generic tasks that the ML APIs are designed for and the specific tasks the software intends to perform. 
\kt{It is a cool empirical finding. The current way of giving this point is a bit too direct, and unintentionally trigger the reader to downplay the importance of this finding. Maybe back this finding up with more empirical evidence.} \yh{systematically find on Github}
This example represents a common usage pattern of ML APIs in software: developers specify a subset of labels that they care about in the specific application, such as the classes in different garbage categories, and how they plan to use the labels, such as which sets of labels trigger the same program branches. Under such usage patterns, ML API mis-predictions can have different levels of severity: errors that lead to wrong software behaviors are more damaging than others.\kt{You are somewhat downplaying an important new point (errors have different severity) by ``hiding'' it inside the para that seems to introducing the common usage pattern of ML API. Make this point clear by giving it a new paragraph.}  
% \cc{need connection. This example represents a common usage pattern of ML API:xxxx. Under such usage pattern, ML API mis-prediction have different level of damages to the software. xxx (not all API errors would lead to failure)}
For example, when the developer write the code as shown in Figure~\ref{fig:app_example}, false positives that lead to the program executing the wrong program branches, such as the ``Glass'' prediction that leads to the Recycle branch, are more devastating than false positives that do not affect the behavior of the software. 


\kt{Maybe contrast this design point with the one-size-fit-for-all design point.}Thus, an ideal solution for using ML APIs in the software is to customize the DNNs such that they are aware of the errors that lead to software misbehaviors. On this front, we want to 
% \cc{``we want''. It's still the motivation section, not contribution} 
re-train the DNNs behind the ML APIs with a re-constructed loss function that reflects the subset of labels the software cares about and the most damaging errors. For example, given the code structure in Figure~\ref{fig:app_example}, the re-constructed loss function will incur penalty only if the DNN makes mistakes that lead to wrong program branch (\eg ``Glass'' appearing in the outputs), and ignores any other types of errors that do not affect the software behavior(\eg the DNNs being confused between ``Snack'' and ``Food'', both belonging to the pre-defined list associated with \emph{Compost} branch).  
% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

% \kt{As I learned from Junchen, in general, when introducing related works, it is better to suggest what we are going to do, but do not say it directly.}
Existing work proposes solutions to improve ML models on specific tasks without the knowledge of the software. 
% \kt{Adapting ML models sounds a bit abrupt. Maybe say ``existing work improves the performance of ML API by adapting the ML model.}
% \kt{Also, for me it feels early for us to mention ``optimizing without the knowledge of the software'' as the definition and importance of software knowledge is unclear here.}
% One line of work customizes the DNNs based on run-time data statistics and still optimizes for the same tasks (\eg image classification)~\cite{kim2021pool, cao2021thia, anderson2019physical}. Another line of work trains specialized models performing the tasks specified through a subset of SQL queries, such as aggregation and limit ~\cite{kang2018blazeit, kang2017noscope}.

\kt{Saying that we are targeting a different problem sounds like we are not picking the correct related work for our problem. Maybe try to say previous work are solving the same problem with the wrong assumption.}
However, we are tackling a different problem than these prior work. Firstly, as software developers typically write Python code to use the ML APIs, instead of declarative\kt{declarative is a ``noise'' here. It's better for us to focus on the popularity of the language here.} languages such as SQL.\kt{Previous work use SQL is not immediately clear to the reader.}
Second of all, the operations that can be expressed in SQL queries that the prior work optimizes for are limited (\eg aggregation, limit)\kt{People tend to not directly care about the limit of operations. Maybe link to what people care, like SQL limits what the \textbf{software can do}, and give a real (at least seemingly real) example to convince people a true need of software cannot be expressed by SQL.}, while there are a wider range of operations that can be expressed by Python. For example, aggregation or limit queries cannot specify subsets of labels can have the same effects on the final program behaviors. Thirdly, in order to use the these systems that optimize for SQL queries, users need to translate their code into SQL queries, which incurs an extra development burden for the users.\kt{For me, this point is essentially the same as the first point. The effect of choosing a programming language that people don't use is forcing the user to ``tranlate'' their code to another language.} Lastly, these approaches cannot guide the ML APIs to produce outputs that lead to correct software behaviors\kt{Personally I feel like this is the most fundamental reason. Putting it at the last is kind of downplaying this point.}\kt{I guess maybe you are referring that these works cannot fix the misbehavior of the software as they are just compressing the model, not improving the model. ``Software behavior'' and ``ground-truth labels'' are noise.} (\ie as if the ground-truth labels are returned), as they only optimize for inference delay. 

% When the service providers design the ML APIs, their goal is mainly to improve traditional class-wise accuracy metrics (\ie high average recall and precision)~\cite{wang2020multi} over all classes for large-scale datasets. However, when developers employ the ML APIs in their software, they care about whether ML APIs' outputs match their expectations (\ie as if the ML APIs' outputs are exactly the ground-truth labels). This gap in service providers' and software developers' purposes can lead to many software mis-behaviors, thus model adaptation is needed to provide a customized model that reduces software mis-behaviors as much as possible.


\kt{Maybe contrast this design point with the one-size-fit-for-all design point.}Thus, an ideal solution for using ML APIs in the software is to customize the DNNs such that they are aware of the errors that lead to software misbehaviors. On this front, we want to 
% \cc{``we want''. It's still the motivation section, not contribution} 
re-train the DNNs behind the ML APIs with a re-constructed loss function that reflects the subset of labels the software cares about and the most damaging errors. For example, given the code structure in Figure~\ref{fig:app_example}, the re-constructed loss function will incur penalty only if the DNN makes mistakes that lead to wrong program branch (\eg ``Glass'' appearing in the outputs), and ignores any other types of errors that do not affect the software behavior(\eg the DNNs being confused between ``Snack'' and ``Food'', both belonging to the pre-defined list associated with \emph{Compost} branch).  
% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

Automatically adapting the DNNs behind ML APIs to fit the software's need has many challenges. 

\begin{itemize}

\item First, automatic model adaptation is hard. We need to automatically extract information embedded in the code structure that indicates how the software plans to use the labels. We also need to transform the information extracted from the software into loss functions that can directly be applied to optimize the DNNs. 


% from the software about the specific task. 
% why infer? Users didn't explicitly specify the tasks, and they are non-experts, so they are not able to specify the tasks in the form that can be directly used to optimize for DNNs' accuracy 
% It is unrealistic to provide extra input for model adaptation (\eg manuals for performing model re-training) at the software developers' end. The main reason is that the software developers who call the ML APIs are typically non-experts in ML, thus it is hard for them to provide an effective model adaptation strategy. 


\item Secondly, model adaptation needs to be very efficient. Given how the interface of the ML APIs is designed, the software developers who call the ML APIs are not able to adapt the DNNs behind the ML APIs. Thus, model adaptation has to happen on the cloud service providers' side, and it is important to provide a quick way of adapting models which reduces errors leading to wrong software behaviors with minimum training cost. 


% such that the number of damaging errors leading to incorrect software behaviors can be reduced most effectively (\ie incurring minimal training cost).  

% \item We performed empirical study on the applications that use ML APIs performing image classification tasks to affect the control flow of the software. We found that a common pattern 


% \item Machine Learning (ML) offers effective ML APIs to a wide range of cognition tasks. Many cloud providers offer ML APIs, supported by underlying Deep Neural Networks (DNNs), that perform well on generic tasks (\eg image classification). These ML APIs are utilized in a wide range of software applications for different specific tasks. However, the ML APIs are not adapted to achieve the application specific tasks, leading to many software misbehaviors.
    % \item List an application such that why/how high class-wise accuracy does not lead to correct software behavior or vice versa and cite~\cite{wan2022automated} to illustrate that there are many such applications. 
    % \ref{fig:app_example} is an example software that incorporates Google \code{label\_detection} API, which outputs all the existing labels in the input image. If we consider traditional class-wise F1 score of the application, the ML API can achieve 
    % \item Here we define the software achieving correct behaviors if the outputs of the ML APIs lead to the same software behavior as if the ground-truth is returned.  
    % \item Explain why the accuracy of the software would be low: the service providers train the ML models aiming to maximize class-wise accuracy, while the software developers need to ensure correct software behavior given the ML API outputs.  
    % \begin{itemize}
    %     \item the service providers pre-train the ML models that support the ML APIs with large-scale datasets (\eg Open Images dataset), aiming at providing good class-wise accuracy. \cc{Do you want to emphasis that they have different optimization goals?}
    %     \item When software developers use the ML APIs in their software, they expect the ML APIs to output classes that lead to the correct software behavior (\ie same software behavior as what the ground-truth leads to) \cc{What's the different between point2 \& 3?} 
    %     \item The pre-trained ML models may make mistakes that lead to the wrong software behavior
    % \end{itemize}
    

    % \item Automatically adapting the ML APIs to the software is important: (1) The developers who use the ML APIs are usually not experts in ML, thus may not know how to adapt the models (2) The developers do not have an affordable way to support model adaptation. 
    % \yh{mention why automation is important}
    % \yh{Emphasize that the problem is important}
    
    
    
    % \item However, when the developers use the ML APIs in their software, they are either unaware of the mismatch between ML APIs' accuracy and software's accuracy, or they do not have an affordable way to adapt the ML APIs to fit the software application they are writing.  \yh{Define affordable: 1. developers do not need to provide training data 2. they do not need to specify what are the context that can be digested by the DNNs to improve accuracy. }
    % \item Automatically adapting the ML APIs to the software is challenging. 
    % \begin{itemize}
    %     \item No existing benchmark has shown that there is a discrepancy between the outputs resulting in high class-wise accuracies and the ones leading to the correct software behaviors

    %     % (prior works either (1) only study ML APIs themselves (2) realize the low accuracy of ML APIs in the software~\cite{wan2021machine} (3) do not understand why the ML APIs do not work when applying to the software (SW only cares about branch prediction are correct) )
    %     % \item Need to transform cognition task into math expression 
    %     % create the template 
    %     \item Need to extract software specific cognitive task automatically and transform the extracted software context into mathematical expression that enables ML API adaptation
    %     \item Need to adapt the ML APIs efficiently 
       
    % \end{itemize}
    
    
    
    
    
    % \yh{To adapt the ML solutions to the software, software developers face many issues... (or accuracy decrease) or say adaptation is very important}
    % \yh{why do adaptation ? if not, will cause accuracy decrease. }
    
    % \yh{Developers did not realize this issue or they do not have an affordable way to adapt}
    
    % \yh{List an example}
    
    
    % \yh{Automatically adapt to the software is challenging. }
    

   
\end{itemize}
% Existing works have performed model customization in different scenarios. 
% They either directly input (\eg the classes that need to be classified)~\cite{kim2021pool, cao2021thia} or specify the specific tasks through a fixed program interface (\eg SQL)~\cite{kang2018blazeit}, and adjust the models, by training specialized models or reorganize different pre-trained model components, based on the specific tasks. Another line of work observes run-time data distribution and customizes the model to fit the specific content in the data. 

\begin{figure}
\begin{subfigure}{0.45\textwidth}    
         \centering
         \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Recycle = ['plastic', 'wood', 'glass', 'paper', 'cardboard', 'metal', 'aluminum', 'tin', 'carton']
Compost = ['food', 'produce', 'snack']
Donate = ['clothing', 'jacket', 'shirt', 'pants', 'footwear', 'shoe']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Recycle:
    return 'It is recyclable.'
    if obj.name in Compost:
    return 'It is compostable.'
  if obj.name in Donate:
    return 'It is donatable.'
    \end{lstlisting}
\subcaption{The software implementation}
\label{fig:app_example}
% \includegraphics[width=.99\linewidth]{figs/app_example2.pdf}
    \end{subfigure}
 \hfill
    \begin{subfigure}{0.45\textwidth}  
        \includegraphics[width=\linewidth]{figs/app_example2.pdf}
        \subcaption[]{A concrete example. }
        \label{fig:app_example2}
    \end{subfigure}
    \caption{Heapsortcypher, a garbage classification application \cite{heapsort} using Google Cloud API.}
\end{figure}

\subsection{Contributions} 
 We present \tool, which helps the cloud service providers, who offer the ML APIs, to automatically adapt the ML APIs to the applications the developers write. 

To understand common tasks software developers intend to perform, we conduct an empirical study on the applications using Google's \code{label\_detection} in a recently published benchmark suite studying ML software~\cite{wan2021machine}, a multi-label image classification API. We focus on 19 applications whose control flow decisions are affected by ML APIs' outputs, for example, the software will print out a warning if the outputs contain ``Gun'' or ``Fire'', and do nothing otherwise. We found that a common pattern of the code structures for these applications is triggering the same program actions for sets of labels, such as returning the same message for labels specified in the same pre-defined list. For example, labels specified in the \emph{Compost} list, including ``Food'', ``Produce'', and ``Snack'', triggers the same program behavior (\ie returning the message ``This is recyclable''). However, different applications have different specific ways of triggering program behaviors based on pre-defined lists. We generalized three levels of abstraction from the code structures of the applications in the benchmark suite: (1) labels that will trigger the same program behaviors; (2) whether the final program output is exclusively 
 
\begin{itemize}

\item Perform program analysis to extract the information needed to perform model adaptation, including the subset of labels that the software cares about, and the sets of labels that are considered equivalent by the software. We also re-constructed loss functions using the extracted information to directly reflect the damaging errors that are not acceptable by the software. 
% Defined a template to automatically transform the code that the software developers write into mathematical expression that can adapt the ML APIs to the software. 
% \item defined the template and the transformation to math expression 
\item Re-train the DNNs behind the ML APIs with the re-constructed loss function, and systematically measure the improvement in the rate of software mis-behaviors on \todo{X} open-source applications invoking ML APIs. 
% \item Compared the ways of model adaptation in terms of accuracy improvement and training cost on \todo{X} real applications using ML APIs.

% defined two types of software context that can improve the accuracy of the software: (1) Data distribution context; (2) Subset of classes context. 

% \item Developed a tool to automatically extract the defined context from the Python code written by software developers 


\end{itemize}

==> bk/backups_before_fist_submission/1-introduction-1106.tex <==
\label{sec:intro}

\subsection{Motivation}
\kt{I would suggest listing the first sentence of each para as bullet points here. It is important to iterate on the structure and the logic (instead of the language details) first.}

% \kt{It is not common to put subsections inside introduction (I'm not sure if it is common in SE community though)}
% \begin{itemize}
%     \item increasing number of software applications use off-the-shelf ML APIs to understand what is present in the input. However, the generic ML APIs with good accuracy might make small mistakes leading to software misbehaviors
%     \item Illustrate how small mistakes could lead to software misbehaviors with the application example 
%     \item This 
% \end{itemize}
There have been an increasing number of software applications with the need of deploying deep neural networks (DNNs) to understand what is present in the input. Due to the heavy burden of designing and training such DNNs
% \kt{need citations here}
, many software developers use off-the-shelf machine learning (ML) APIs provided by many cloud service providers (\eg Google, Microsoft, Amazon) to reduce their development effort~\cite{wan2021machine}.  However, the accuracy of generic ML APIs misaligns with software correctness\shan{This sentence needs rewording. Not clearly what it tries to deliver.}. 
% \kt{The argument ``the software misbehavior is because that APIs are agnostic to software'' is an important argument and it directly leads to your key contribution. You bring this point too quick without much support, making this argument sounds trivial. I would suggest we postpone the mentioning of this point and just say a general ML API with good performance can lead to a lot of software behavior.}
% \yh{example: use the figure 1 example }
% \yh{existing works cost reduction by leveraging e.g., model compression 

% correct software misbehaviors by improving the ml models  =>  }

To illustrate how ML APIs with good accuracy may lead to software misbehaviors\shan{This opening sentence is a bit odd: it seems to fit our OOPSLA submission better, don't you think so? Furthermore, even with your tool and ML APIs with increased accuracy, the software may still misbehave, right?},
% how and why optimizing class-wise accuracy does not necessarily lead to the correct software behaviors,
% \kt{Maybe discribe the software behavior following the processing order of the software, like input -> API -> labels -> list -> output}
we take the software application \emph{Heapsortcypher} in Figure~\ref{fig:app_example} as an example. It takes a trash image as input, and invokes \code{label\_detection}, Google's multi-label classification API, to get the labels that describe the content in the image. It then goes through a post-processing step which classifies the ML APIs' outputs into categories of garbage. Heapsortcypher pre-defines three lists, \emph{Recycle, Compost, and Donate}. It checks the output labels (\eg [Glass, Candy, Snack, Confectionery, Lollipop]), ranked with descending order of confidence scores, and searches for the first label (\eg Glass) that matches any of the labels in the three pre-defined lists. Finally it executes the branch that corresponds to the found pre-defined list (\eg the one that outputs returns ``It is recyclable. '').
% the corresponding judgment if the outputs intersect with one of the lists. 

% and 
% then performs a post-processing step which executes one of \emph{Recycle, Compost, } and \emph{Donate} branches if the output labels contain any of the keywords specified in the pre-defined list \code{Recycle, Compost, Donate} \cc{``the pre-defined list'', you need to explain what is recycle, as it means a branch in the last reference} .


This simple post-processing step incurs potential software mis-behaviors even with an ML API that only mis-classifies one class, as shown in Figure~\ref{fig:input_example_top_wrong}.
% \kt{80\% recall does not sound like highly reliable. Also, ``highly reliable'' is vague. Maybe just say ``even when the ML API correctly identifies most of the classes''.} 
% Figure~\ref{fig:app_example2} shows a concrete example of how \emph{Heapsortcypher} works.  
% \cc{Maybe directly say that ``the bottom of Figure 1 shows a concrete example'', instead repeating what we have introduced earlier} 
% Given the outputs of the ML API, if we use traditional recall and precision as the metrics~\cite{wang2020multi}, this output yields a recall of 100\% and a precision of 80\%. Nevertheless, this output is completely wrong from the view of the software. 
% According to the ground-truth labels, the correct branch to be executed is the one that returns ``It is compostable. '', since the only intersection between the ground-truth labels and the three lists is the one associated with the \emph{Compost} branch. However, the API's outputs lead to the program executing the branch which returns ``It is recyclable. '' 
Given a candy image, the ML API wrongly returns the label ``Glass''. This mistake is minor in terms of the multi-label classification task~\cite{wang2020multi}: it  finds all the objects in the input image while recognizing an extra wrong object ``Glass'', providing a recall of 100\% and a precision of 80\%\shan{I don't understand how you get these numbers: 100\% and 80\%.}. However, it leads to a completely wrong software behavior. While this image belongs to \emph{compostable} branch, the software wrongly executes the \emph{recyclable} branch as \code{Recycle} list contains the first API output label ``Glass''.

\shan{After I finished reading the above two paragraphs, I finally saw what you are trying to tell the readers. I guess you are trying to say that not all mistakes of an ML API are equally important for a software application. Is that what you are trying to say? You need to clearly present what messages you want to deliver BEFORE you present examples. You cannot ask readers to summarize/infer what you mean AFTER they read the example.}


% \cc{I changed the description. Please proof read}

% \kt{From a system guy's perspective, I guess it is better  to highlight the cost of such software misbehavior. I'm not sure if this is needed in SE conference though.}
% \cc{P4 \& 5 have duplicate description}
%\cc{Maybe create a figure with a concrete image example and show the list (use color to show overlaps). 
% \yh{}

% \kt{It is a cool empirical finding. The current way of giving this point is a bit too direct, and unintentionally trigger the reader to downplay the importance of this finding. Maybe back this finding up with more empirical evidence.}
\kt{I would expect you saying this type of error is a common error. People do not directly care about the common usage pattern of ML API.}
% This example represents a common error pattern of applying ML APIs in software: developers specify a subset of labels that they care about, such as \code{Recycle}, \code{Compost}, and \emph{Donate} lists, and how they use the labels, such as these three lists correspond to three software branches. 
% We perform an empirical study to study the common patterns of the applications in the benchmark suite~\cite{wan2021machine}, focusing on the applications whose program behaviors are affected by the ML APIs' outputs\footnote{We study these applications as they reflect non-trivial ways of using ML APIs. If the applications directly return the APIs' outputs, they do not provide extra information for us to perform adaptation. }. We find that it is common for applications to pre-define one or more lists of labels, and execute different branches by comparing the output labels with the lists. \kt{People may wonder what happened to the remaining 40\% applications.} 
% \kt{It would be better to separate these two important points {\footnotesize (This pattern is common \& mispredictions have different levels of severity)} into two paragraphs.}
This example represents a common phenomenon in ML software. The reason is that the ML APIs are optimized for generic accuracy over a large number of classes, but the ML software has a different focus and priority: it cares about whether the ML API can produce outputs leading to correct control flow decisions\shan{I think it is a bit too early to mention control flow here. Please think and rephrase.}. 

The way the ML software is typically written can cause accurate ML APIs' outputs to lead to wrong control flow decisions\shan{?????What? Am I in the wrong paper? This sentence seems to fit our OOPSLA submission but does NOT fit here AT ALL. Your example so far is about wrong API result; it is NOT about accurate API result that leads to software failure. I am very confused.}. Specifically,  developers usually specify a subset of labels that they care about, such as \code{Recycle}, \code{Compost}, and \emph{Donate} lists, and how they use the labels, such as these three lists correspond to three software branches. Under such code patterns, ML API mis-predictions have different levels of severity: errors that lead to wrong software behaviors are more damaging than others\shan{No, it is not about which one is more damaging. Some mis-prediction simply has NO damage at all. Right?}. For example, in Heapsortcypher, the confusion within the lists, such as misclassifying a ``Food'' image to ``Produce'', is less damaging \shan{Again, when you say ``less damaging'', you are implying there exists some damage. But, that is not true here. mis-classifying food to produce has no damage to the software at all!} than across the list, such as misclassifying a ``Food'' image to ``Glass'', as only the latter would lead to a wrong control flow decision.



% Under such code patterns, ML API mis-predictions have different levels of severity: errors that lead to wrong software behaviors are more damaging than others. For example, in Heapsortcypher, the confusion within the lists, such as misclassifying a ``Food'' image to ``Produce'', is less damaging than across the list, such as misclassifying a ``Food'' image to ``Glass'', as only the latter would lead to a wrong execution path.
% \cc{Please explain the effect of mis-classification inside list and outside list} \yh{Done}
% \kt{You are somewhat downplaying an important new point (errors have different severity) by ``hiding'' it inside the para that seems to introducing the common usage pattern of ML API. Make this point clear by giving it a new paragraph.}  
% For example, when the developer write the code as shown in Figure~\ref{fig:app_example}, false positives that lead to the program executing the wrong program branches, such as the ``Glass'' prediction that leads to the Recycle branch, are more devastating than false positives that do not affect the behavior of the software. 


% \kt{Maybe contrast this design point with the one-size-fit-for-all design point.}
% \kt{``customize the DNNs'' is a surprise. Maybe give more rationales to justify why customizing DNN instead of something like redesigning the API interface.}
% \cc{Be aware of software behavior? aim to improve software correctness?} \yh{Done} \kt{This issue is not solved yet. I guess Chengcheng questions these two things because they are vague. Maybe try to answer what kind of concrete software behavior are you aim to improving/what is software correctness/what kind of software correctness are you trying to improve.}

Thus, instead of providing a generic ML API that could be applied to all software, an ideal solution is to customize the DNNs behind ML API for each software, while keeping the same interface\shan{How do you define interface? If you really keep the same interface, how do you collect the software control flow information for the API provider?}. In this way, the ML API is aware of how the ML APIs' outputs affect the software behavior and is optimized to provide outputs that ensure\shan{no way you can ensure} software behaves as if the ground-truth of the input is returned by the ML APIs. Meanwhile, the developers would not be bothered to modify their software to fit the adaptation. 
% On this front, we want to re-train these DNNs behind the ML APIs with a re-constructed loss function\kt{Justify this design choice.} that reflects the subset of labels the software cares about and the most damaging errors. For example, given the code structure in Figure~\ref{fig:app_example}, the re-constructed loss function will incur penalty only if the DNN makes mistakes that lead to wrong program branch (\eg ``Glass'' appearing in the outputs), and ignores any other types of errors that do not affect the software behavior(\eg the DNNs being confused between ``Snack'' and ``Food'', both belonging to the pre-defined list associated with \emph{Compost} branch).   \cc{This is solution. So I comment it out. I'll put them in Section 1.2}

% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

% \kt{As I learned from Junchen, in general, when introducing related works, it is better to suggest what we are going to do, but do not say it directly.}
% \kt{This paragraph is tooooo long. Maybe illustrate these two line of works in two paragraphs?}
% \cc{``To the best of our knowledge, we are the first to study xxx problem.'' Can we claim something like this? If not, maybe starts with ``Existing work cannot tackle our problem. They improve xxxx without the knowledge of software.'' } \yh{I mentioned we are tackling a different problem, is this ok? }
% \kt{Adapting ML models sounds a bit abrupt. Maybe say ``existing work improves the performance of ML API by adapting the ML model.}
% \kt{Also, for me it feels early for us to mention ``optimizing without the knowledge of the software'' as the definition and importance of software knowledge is unclear here.}

% Existing work proposes solutions to improve the performance or accuracy of ML models without the knowledge of the software. However, we are tackling a different problem than these prior work. 
% One line of work optimizes the ML APIs' query accuracy or cost by adaptively choosing a sequential strategy to invoke available APIs within a resource budget ~\cite{chen2020frugalml, chen2022frugalmct}. 
% These work requires modifications on the developers' side, such as changing the code to apply the most accurate API. 

% Another line of work trains specialized models performing the tasks specified through a subset of SQL queries, such as aggregation and limit, such that the inference delay is reduced ~\cite{kang2018blazeit, kang2017noscope}. 
% The problem we are targeting at is different from this line of work for the following reasons. Firstly, these approaches cannot guide the ML APIs to produce outputs that lead to correct software behaviors, as they only optimize for inference delay instead of improving the model. Secondly, a great number of existing applications on GitHub calling ML APIs are written in Python~\cite{wan2021machine} instead of SQL. Thirdly, the operations that can be expressed in SQL queries that the prior work optimizes for are limited. For example, the SQL queries that are optimized by these work can only count average number of objects among all the video frames, or selecting limited number of frames that meet several constraints. Nevertheless, there are a wider range of operations that can be expressed by Python. For example, aggregation or limit queries cannot specify subsets of labels can have the same effects on the final program behaviors. 
% Lastly, in order to use the these systems that optimize for SQL queries, users need to translate their code into SQL queries, which incurs an extra development burden for the users.


Existing work proposes solutions to improve the performance or accuracy of ML models in software applications.
However, we found that existing solutions are not desirable as they add extra burden on the developers.
Specifically, one line of works focus on improving accuracy of ML task itself by modifying the software call to the ML APIs~\cite{chen2020frugalml, chen2022frugalmct}. 
Given a resource budget, they adaptively invokes several ML APIs from different cloud providers and ensemble their results. 
However, this approach require changing the software implementation in order to call different ML APIs, thus creating extra burden to the developers\shan{I find this argument very weak: the change required sounds very minimal and can be easily wrapped inside a library call. More importantly, I feel there are much more fundamental differences between your work and this previous work and yet you didn't mention.}.
Another line of work aims to reduce latency by compressing DNNs to perform a specialized task defined by a subset of SQL syntax~\cite{kang2018blazeit, kang2017noscope}. 
However, this approach cannot correct the software misbehavior triggered by wrong DNN output (as the DNN compression reduces the DNN latency while keeping the DNN ouput the same). 
Besides, this approach adds extra developer effort to reimplement their software logic (which is typically written in Python~\cite{wan2021machine}) using SQL syntax.
% In addition, they focus on SQL, while we study real-world applications written in general purpose language like Python~\cite{wan2021machine}, which supports much more operations.

Our goal is to \textit{automatically} adapting the DNNs behind the ML API \textit{without extra developer effort}.
\shan{Just like my comments in the abstract, I feel you still didn't make it very clear about your assumption. What is your assumption about what you have access to and what you can change? This assumption is VERY different from our OOPSLA submission, right? That is why you need to clearly explain your problem statement and assumption here.}

% \kt{Saying that we are targeting a different problem sounds like we are not picking the correct related work for our problem. Maybe try to say previous work are solving the same problem with the wrong assumption.}


% as software developers typically write Python code to use the ML APIs, instead of declarative\kt{declarative is a ``noise'' here. It's better for us to focus on the popularity of the language here.} languages such as SQL.\kt{Previous work use SQL is not immediately clear to the reader.}
% \kt{People tend to not directly care about the limit of operations. Maybe link to what people care, like SQL limits what the \textbf{software can do}, and give a real (at least seemingly real) example to convince people a true need of software cannot be expressed by SQL.}, 
% \kt{For me, this point is essentially the same as the first point. The effect of choosing a programming language that people don't use is forcing the user to ``tranlate'' their code to another language.}  \kt{Personally I feel like this is the most fundamental reason. Putting it at the last is kind of downplaying this point.}\kt{I guess maybe you are referring that these works cannot fix the misbehavior of the software as they are just compressing the model, not improving the model. ``Software behavior'' and ``ground-truth labels'' are noise.} 


% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

% As a result, we need an approach that automatically adapts the ML models behind ML APIs such that they are aware of the damaging errors that will lead to software misbehaviors\cc{This sentence belongs to P5. It also looks like a repletion of P5-sentence1}.

Automatically adapting the ML models faces several challenges. 



\emph{Firstly}, automatic model adaptation is hard. Aiming to help non-expert developers, an automatic approach that minimizes developer effort is desired. To achieve such automatic adaptation, we need to understand how software uses ML API output label and the severity of different types of mis-predictions. We also need to translate these information to a DNN-understandable format for adaptation, such as a loss function, which is inherently hard due to rich code syntax. 
% \cc{Yuhan, please proof read}

% Automation is necessary because the application developers using the ML APIs typically lack expertise in ML, thus may not be able to efficiently perform model adaptation. We need to automatically extract information\kt{vague} embedded in the code structure that indicates how the software plans to use ML APIs' output labels. We also need to transform the information extracted from the software into loss functions that can directly be applied to optimize the DNNs.  
% \cc{why automation? please explain} \yh{added. }


% from the software about the specific task. 
% why infer? Users didn't explicitly specify the tasks, and they are non-experts, so they are not able to specify the tasks in the form that can be directly used to optimize for DNNs' accuracy 
% It is unrealistic to provide extra input for model adaptation (\eg manuals for performing model re-training) at the software developers' end. The main reason is that the software developers who call the ML APIs are typically non-experts in ML, thus it is hard for them to provide an effective model adaptation strategy. 


\emph{Secondly}, model adaptation needs to be very efficient. 
 Since we need to re-train the ML model for each software application, model adaptation should be fast. Moreover, software applications may change time to time during the development procedure, thus adapting the ML models quickly can greatly save the time and operation cost of re-training. 
 \shan{I guess we also assume that we cannot obtain new training data from application developers.}
 % \kt{Another reason is that your approach needs to train different DNNs for different softwares, so the training need to be cheap.}
% Given how the interface of the ML APIs is designed, the software developers who call the ML APIs are not able to adapt the DNNs behind the ML APIs. Thus, model adaptation has to happen on the cloud service providers' side, and it is important to provide a quick way of adapting models which reduces errors leading to wrong software behaviors with minimum training cost. \cc{It does not matter whether developer or service provider pay the training cost. Actually, service providers could charge more on developer if training takes more time. You may say (1) software may change time by time during development (2) a fast adaptation could save time and operation cost} 


% such that the number of damaging errors leading to incorrect software behaviors can be reduced most effectively (\ie incurring minimal training cost).  

% \item We performed empirical study on the applications that use ML APIs performing image classification tasks to affect the control flow of the software. We found that a common pattern 


% \item Machine Learning (ML) offers effective ML APIs to a wide range of cognition tasks. Many cloud providers offer ML APIs, supported by underlying Deep Neural Networks (DNNs), that perform well on generic tasks (\eg image classification). These ML APIs are utilized in a wide range of software applications for different specific tasks. However, the ML APIs are not adapted to achieve the application specific tasks, leading to many software misbehaviors.
    % \item List an application such that why/how high class-wise accuracy does not lead to correct software behavior or vice versa and cite~\cite{wan2022automated} to illustrate that there are many such applications. 
    % \ref{fig:app_example} is an example software that incorporates Google \code{label\_detection} API, which outputs all the existing labels in the input image. If we consider traditional class-wise F1 score of the application, the ML API can achieve 
    % \item Here we define the software achieving correct behaviors if the outputs of the ML APIs lead to the same software behavior as if the ground-truth is returned.  
    % \item Explain why the accuracy of the software would be low: the service providers train the ML models aiming to maximize class-wise accuracy, while the software developers need to ensure correct software behavior given the ML API outputs.  
    % \begin{itemize}
    %     \item the service providers pre-train the ML models that support the ML APIs with large-scale datasets (\eg Open Images dataset), aiming at providing good class-wise accuracy. \cc{Do you want to emphasis that they have different optimization goals?}
    %     \item When software developers use the ML APIs in their software, they expect the ML APIs to output classes that lead to the correct software behavior (\ie same software behavior as what the ground-truth leads to) \cc{What's the different between point2 \& 3?} 
    %     \item The pre-trained ML models may make mistakes that lead to the wrong software behavior
    % \end{itemize}
    

    % \item Automatically adapting the ML APIs to the software is important: (1) The developers who use the ML APIs are usually not experts in ML, thus may not know how to adapt the models (2) The developers do not have an affordable way to support model adaptation. 
    % \yh{mention why automation is important}
    % \yh{Emphasize that the problem is important}
    
    
    
    % \item However, when the developers use the ML APIs in their software, they are either unaware of the mismatch between ML APIs' accuracy and software's accuracy, or they do not have an affordable way to adapt the ML APIs to fit the software application they are writing.  \yh{Define affordable: 1. developers do not need to provide training data 2. they do not need to specify what are the context that can be digested by the DNNs to improve accuracy. }
    % \item Automatically adapting the ML APIs to the software is challenging. 
    % \begin{itemize}
    %     \item No existing benchmark has shown that there is a discrepancy between the outputs resulting in high class-wise accuracies and the ones leading to the correct software behaviors

    %     % (prior works either (1) only study ML APIs themselves (2) realize the low accuracy of ML APIs in the software~\cite{wan2021machine} (3) do not understand why the ML APIs do not work when applying to the software (SW only cares about branch prediction are correct) )
    %     % \item Need to transform cognition task into math expression 
    %     % create the template 
    %     \item Need to extract software specific cognitive task automatically and transform the extracted software context into mathematical expression that enables ML API adaptation
    %     \item Need to adapt the ML APIs efficiently 
       
    % \end{itemize}
    
    
    
    
    
    % \yh{To adapt the ML solutions to the software, software developers face many issues... (or accuracy decrease) or say adaptation is very important}
    % \yh{why do adaptation ? if not, will cause accuracy decrease. }
    
    % \yh{Developers did not realize this issue or they do not have an affordable way to adapt}
    
    % \yh{List an example}
    
    
    % \yh{Automatically adapt to the software is challenging. }
    

   

% Existing works have performed model customization in different scenarios. 
% They either directly input (\eg the classes that need to be classified)~\cite{kim2021pool, cao2021thia} or specify the specific tasks through a fixed program interface (\eg SQL)~\cite{kang2018blazeit}, and adjust the models, by training specialized models or reorganize different pre-trained model components, based on the specific tasks. Another line of work observes run-time data distribution and customizes the model to fit the specific content in the data. 

\begin{figure}
\begin{subfigure}{0.45\textwidth}    
         \centering
         \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Recycle = ['Plastic', 'Wood', 'Glass', 'Paper', 'Cardboard', 'Metal', 'Aluminum', 'Tin', 'Carton']
Compost = ['Food', 'Produce', 'Snack']
Donate = ['Clothing', 'Jacket', 'Shirt', 'Pants', 'Footwear', 'Shoe']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Recycle:
    return 'It is recyclable.'
  elif obj.name in Compost:
    return 'It is compostable.'
  elif obj.name in Donate:
    return 'It is donatable.'
return 'It is others.'
\end{lstlisting}
%          \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% Recycle = ['Plastic', 'Wood', 'Glass', 'Paper', 'Cardboard', 'Metal', 'Aluminum', 'Tin', 'Carton']
% Compost = ['Food', 'Produce', 'Snack']
% Donate = ['Clothing', 'Jacket', 'Shirt', 'Pants', 'Footwear', 'Shoe']
% image = types.Image(content=trash_image)
% response = client.label_detection(image=image)
% Predictions = []
% for obj in response.label_annotations:
%   Predictions.append(obj.name)
% if any([label in Recycle for label in Predictions]):
%   return 'It is recyclable.'
% elif any([label in Compost for label in Predictions]):
%   return 'It is compostable.'
% elif any([label in Donate for label in Predictions]):
%   return 'It is donatable.'
%     \end{lstlisting}
\subcaption{The software implementation}
\label{fig:app_example}
% \includegraphics[width=.99\linewidth]{figs/app_example2.pdf}
    \end{subfigure}
 \hfill
    \begin{subfigure}{0.45\textwidth}  
        \includegraphics[width=\linewidth]{figs/app_example2.pdf}
        \subcaption[]{Including an extra wrong\shan{???What do you mean by missing???} recognition ``Glass'' leads to software mis-behavior. The arrows starting from the Ground-truth labels are the correct software control flow decision (\ie as if the ground-truth labels are output by the ML API). In this example, the correct control flow is executing the branch associated with the Compost list, because the ground-truth labels only have an intersection with the Compost list. \shan{This caption is very difficult for readers to understand.}}
        \label{fig:input_example_top_wrong}
    \end{subfigure}
    %     \begin{subfigure}{0.45\textwidth}  
    %     \includegraphics[width=\linewidth]{figs/input_example_top_label_correct.pdf}
    %     \subcaption[]{Mis-classifying the label ``Wood'' does not lead to software mis-behavior. }
    %     \label{fig:input_example_top_correct}
    % \end{subfigure}
    % \caption{Heapsortcypher, a garbage classification application \cite{heapsort} using Google Cloud API. 
    % \kt{The key in this figure is the contrast between highly accurate API output and wrong software misbehavior. Maybe not calling the ideal API output as ``ground-truth''? It is better for your point to come across without letting the reader to parse what does ``ground-truth'' means, and realize that this image comes from your dataset and it is an image annotated with ground-truth label.}\cc{It's fine. We just take it literally: the correct answer.}
    % }
\label{fig:app_example_entire}
\end{figure}


\subsection{Contributions} 
%\kt{I would expect contributions to be some short and condensed bullet points.}\cc{Let's first make a long version and then decide how to compress it.}


% We present \tool, which helps the cloud service providers to automatically re-train the ML models behind the ML APIs to the applications the developers write, so as to reduce the software mis-behaviors incurred by the ML APIs' outputs.
% \cc{I changed the description. Please proof read} \yh{we are not helping developers, our solution happens on the cloud service providers' side. }

% We find that the code structures reflect the severity of different API mis-predictions.
% For example, in Figure~\ref{fig:app_example}, labels in the \emph{Recycle} list and labels in the \emph{Compost} list trigger different program behaviors. Therefore, given an input image only containing labels in the \emph{Recycle} list, it is a severe error if the ML API outputs labels in the \emph{Compost} list. \cc{This paragraph should belong to empirical study} 

To understand how real world applications use ML APIs\shan{This opening sentence is toooo generic. I could have used it in all recent papers from our group. If I am a reviewer, I would wonder ``haven't people already conducted tons of study to understand how applications use ML APIs? Why do you need to study again?????''. What EXACTLY was not understood before and hence you want to understand?}, we conduct an empirical study on a recently published ML software benchmark suite~\cite{wan2021machine}. We found five code structure patterns of how ML software post-process ML APIs' outputs, and derived three types of abstractions to characterize how the control flows are affected by ML APIs' outputs (details are in Section~\ref{sec:empirical})\shan{Again, why isn't this already covered by previous work?}.  
% We focus on 19 applications which invokes Google \code{label\_detection} API to make control flow decisions. These applications use the ML APIs' outputs to determine which program branch to be executed, like Heapsortcypher in Figure~\ref{fig:app_example}. They typically define several lists of labels and program branches the application should execute when the ML APIs' output labels intersect with their associated pre-defined list. 

% To characterize the application's post-processing step of ML API outputs, we defined three types of abstraction: (1) the sets of labels that have equivalent effects on the control flow;  (2) whether the final output of the software is exclusively associated with only one program branch; and (3) whether errors made in some sets of labels can be disguised by correct predictions in other sets of labels.


% \cc{Do we want to mention mutually exclusive?}. 
% Specifying the values of the abstractions can uniquely identify how the applications are going to post-process the ML APIs' outputs. 

Guided by the empirical study, we propose \tool, an automated framework that adapts ML models behind the ML API to the software implementation while keeping the same API interface, so as to reduce software misbehaviors. Tackling automation challenge, it first perform static analysis on the Python source code to extract the abstractions from the software. \tool then re-constructed the loss function to reflect the different severity of mis-predictions on software correctness. Tackling efficiency challenge, \tool adopts fine-tuning approach to adapt the ML model behind ML API with minimum training costs.
\shan{I like this paragraph, but clearer than earlier paragraphs.}
% \cc{Can you map these solutions to challenges?} \yh{i put the second challenge in the evaluation part}
% \cc{The second half of sentence are evaluation} 



% We systematically measure the improvement in the rate of software mis-behaviors on 19 open-source applications that call multi-label image classification API.
We systematically evaluate \tool on 19 open-source applications that use multi-label image classification API to make control flow decision.
Our evaluation shows that the re-constructed loss function provides up to \todo{X\%} improvements in reduction of software mis-behaviors, whereas alternative approach only improves rate of software mis-behaviors by \todo{Y\%}. Our evaluation also shows that performing model adaptation with the re-constructed loss function can finish within \todo{Z} minutes.  \yh{Will update the numbers after I finish the evaluation section. }
% (1) labels that will trigger the same program behaviors; (2) whether the final software output is exclusively associated with only one program branch, for example, in the application example shown in Figure~\ref{fig:app_example}, the final output of the software is the message specified in one of the program branches; (3) whether different sets of labels triggering same program behaviors have different priority levels. 


==> bk/backups_before_fist_submission/2-1-background.tex <==
\label{sec:background}

\subsection{ML Cloud API}
Many cloud service providers \cite{google-cloud, amazon-ai, ibm-watson, ms-azure} have offered ML APIs covering a wide range of vision, natural language, and speech tasks. For example, Google offers 


\subsection{ML-enabled Software}
Increasing number of software applications using ML APIs. 
Cite ICSE'21 \cite{wan2021machine} paper

% \subsection{Terminologies}

\yh{NLP / speech / object detection}




==> bk/backups_before_fist_submission/2-2-empirical-1025.tex <==
\label{sec:empirical}

To understand how developers use ML API in real-world applications, we conduct an empirical study on ML software that invokes  ML APIs to make control flow decisions. \cc{I weakly remember that you plan to study Amazon APIs. Please revise it if I'm wrong}

% We observe that there are different ways for developers to specify how they plan to use the ML APIs' outputs to affect the control flow of ML software. 
% In order to understand the common patterns of the control flows of the ML software, we conduct an empirical study on ML software using Google's \code{label\_detection} API, which performs multi-label image classification.  
% From the case study, we summarize three types of abstractions for the code structures of the ML software. 



% \yh{ML API on OI or pretrained on OI}
\subsection{Methodology}

\subsubsection{Application selection}



% Google (benchmark, search), AWS (search)
We study 40 open-source ML software applications  whose control flows are affected by the output of a multi-label image classification API. These applications comes from two sources: (1) 19 applications come from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}; and (2) 21 applications comes from GitHub by random checking around 60 applications.
Among these applications, 29 of them use Google \code{label\_detection} API and 11 use Amazon \code{detect\_labels} API.

\yh{select applications using multi-label classification and object-detection APIs, because that's representative of the ML software }

% \cc{Maybe also add some statistics}


We do not study the applications that directly print out the ML APIs' outputs or store these outputs without post-processing. The tasks that these applications perform are the same as the task of ML API. Therefore, there is no need to adapt APIs to software. In addition, ML APIs are only loosely integrated into these applications, e.g., not interacting with other software components. We believe they do not represent the future direction of ML software.

\subsubsection{Test data selection}
TO-DO
\cc{It is weird to have a subsection that only has one subsubsection. How about we also introduce the open image data and ground-truth label?}




% We study the open-source applications from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}. We focus on applications whose control flows are affected by the ML APIs' outputs. We focus on 19 applications which invoke Google \code{label\_detection} API to make control flow decisions. These applications use the ML APIs' outputs to determine which program branch to be executed. For example, in the application example in Figure~\ref{fig:app_example}, the API output labels in Figure~\ref{fig:app_example2} will lead the software executing \code{return 'Recycle'} on line 8 because ``Glass'' is included in the \code{Recycle} list. We refer to the branch being executed, such as \code{return  `Recycle'}, when the if condition is satisfied, as \emph{if/then branch}. 
% To characterize the application's post-processing step of ML API outputs, we defined three types of abstraction: (1) the sets of labels that have equivalent effects on the control flow;  (2) whether the final output of the software is exclusively associated with only one program branch; and (3) whether errors made in some sets of labels can be disguised by correct predictions in other sets of labels.
% We do not study the applications that directly print out the ML APIs' outputs or store all the outputs in the databases, because these applications do not have mismatch between ML APIs' outputs and software's output thus do not have room for improvement. 




% \subsection{Common patterns of code structure of software utilizing ML APIs}
\subsection{Result summary}
Across all applications we studied, 48\% of them defines several whitelists and compares ML API output labels with them. 

Take Heapsortcypher (Figure~\ref{fig:app_example_entire}) as an example. It executes Line 8 when given a candy image, as the API output ``Glass'' is included in the \code{Recycle} list and thus fulfills the statement in Line 7. We refer to this executed branch as \emph{if/then branch}. Correspondingly, we refer to another branch that  not executes Line 8 as \emph{if/else branch}.
We refer to a list of labels (or classification category) leading to the same control flow decision as a \emph{whitelist}. \code{Recycle}, \code{Compost}, and \code{Donate} are the three whitelists, taking Heapsortcypher as an example.

% \cc{yuhan, please put terminologies (those used in Section 3) here. Make sure that you are only using the Heapsortcypher as an example}

While these applications typically uses whitelists to post-process ML API results, they vary in the way of using whitelists to make control flow decisions. Even with same whitelists and API inputs, the applications would behave differently according to its code structure. Next, we will introduce the common patterns observed in the studied applications.


% We find that these software typically pre-defines one or several lists of labels as branch conditions, and then maps the original output labels to the pre-defined lists which intersect with the labels. Then the software executes one or more \ifts that correspond to those mapped pre-defined lists. 
% In other words, all the labels specified in one list will lead to the same control flow decision. 

% We refer to the lists of labels leading to the same control flow decisions as \emph{whitelists} in the rest of the paper. For example, in the application example shown in Figure~\ref{fig:app_example}, the software defines three \emph{whitelists}, Recycle, Compost, and Donate. 



% They typically define several lists of labels and which one or more program branches the application should execute by comparing the API output labels and these lists. 
% They typically define several lists of labels and which one or more program branches the application should execute when the ML APIs' output labels intersect with their associated pre-defined list. 


\begin{figure}
    \centering
     \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}

\end{lstlisting}
    \caption{Software implementation. }
    \label{fig:app_example_non_mut}
\end{figure}


\subsection{Abstractions}
\label{sec:abstractions}
As summarized in Figure~\ref{fig:hierarchy} we define four types of abstractions to characterize the code structure. We will use several minimal templates to illustrate the four types of abstractions. 


\textbf{1) Number of whitelists.} The software specifies one \wl or multiple \wls. Particularly, as shown in Figure~\ref{fig:template1}, each whitelist is related to a particular software branch: the software will execute the corresponding \ift when the ML APIs' outputs intersect with the labels in the \wl. In the rest of the paper, we will refer to executing a branch as mapping API outputs to its corresponding whitelist.

\textbf{2) Type of mapping.} For the software specifying multiple \wls, there are two types of mapping from ML API outputs to whitelists: (i) the software executes all the \ifts when the API's outputs intersect with the \wls associated with the branch condition. In other words, the original output labels are mapped to several \wls; (ii) the software checks whitelists in a specific order, and only executes the lower-ranked \ifts when API outputs do not intersect with any higher-ranked whitelist, leading to at most one \ift to be executed. In other words, the original output labels are mapped to at most one \wl. 
% \cc{I changed it from multiple to several, so that it means 0 to N}

% For the software specifying multiple \wls, when the software checks if the output labels intersect with the \wls, there are two possible ways of checking: (i) the software executes all the \ifts when the API's outputs intersect with the \wls associated with the branch condition. In other words, the original output labels may be mapped to multiple \wls; (ii) the software checks the branch conditions in a specific order, and only executes the lower-ranked \ifts if the higher-ranked branch conditions are false, leading to at most one \ift to be executed. In other words, the original output labels are mapped to at most one \wl. 
% (i) the software executes at most one if/then branch when the API's outputs intersect with the \wl associated with the branch condition; (ii) the software executes all the if/then branches when the API's outputs intersect with the \wls associated with the branch condition. 
% For the software that specifies several \wls, some software will compare the ML APIs' outputs with the \wls, and break at a program branch once the outputs intersect with the \wl associated with the branch. In other words, the final output of the software is the message corresponding to with only one program branch. Other software compares the ML APIs' outputs with the \wls, and outputs all the messages 

\textbf{3)Type of output.} For the software which maps original output labels of the ML API to several \wls, it either construct the final output in a format of (i) set or (ii) list. In the latter, the final output is affected by the order of examination.
% For the software which maps original output labels of the ML API to several \wls, there are two possible ways for software to construct the final output:  (1) the software checks the output labels one by one, and add a \wl to a list if the output labels intersect with the \wl. Finally, the software outputs the list containing all the matched \wls. In this case, the order at which the \wls intersect with the output labels does matter; (2) the software checks the output labels one by one, and add a \wl to a set if the output labels intersect with the \wl. Finally, the software outputs the set containing all the matched \wls. In this case, the order at which the \wls intersect with the output labels does not matter.

\textbf{4) Order of examination.}  For the software specifying multiple \wls, the order of examining intersections between \wls and ML API outputs determines software behavior. If we reconstruct the examination into a two-level nested loop that iterates through \wls and API outputs, there naturally arises two types of loop structure: prioritize the specified \wls or the API output labels.
% For the software which executes at most one \ift, the order at which the software performs the checking on the branch conditions may either prioritize the specified \wls or the output labels. 
% As a result, for the software that prioritizes the order of the output labels, mis-classifications happened on the lower-ranked output labels do not matter, as long as the higher-ranked output labels can lead to the correct control flow decisions. Similarly, for the software that prioritizes \wls, mis-classifications happened on the lower-ranked \wl do not matter, as long as the . 

\begin{figure}
     \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
    \caption{Common code patterns of ML software. The decision nodes (in blue) are abstractions defined in Section~\ref{sec:abstractions}. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
\label{fig:hierarchy}
\end{figure}



\subsection{Common Code Patterns}
\label{sec:examples}
\yh{TODO: add connection to the abstractions} \cc{Also add how many applications belongs to each category}
Based on these four types of abstractions, Figure~\ref{fig:hierarchy} summarized all the possible code patterns in a structure of decision tree. Each decision nodes represent an abstraction. Each leaf node represents a code pattern constructed with the sequences of different decisions made at each decision node. While Figure~\ref{fig:hierarchy} illustrates six possibilities, our studied applications only contain four of them (green box in solid lines).

% Based on these four types of abstractions, we can characterize the common code structures as shown in Figure~\ref{fig:hierarchy}. Each decision node in the decision tree represents an abstraction as described in Section~\ref{sec:abstractions}. Each leaf node in the decision tree represents a type of code structure constructed with the sequences of different decisions made at each decision node. The leaf nodes are all the possible code structures constructed with the abstractions. However, we only found a subset of all the possible code structures in the benchmark suite. The existing types of code structures are shown in the leaf nodes with edges marked with solid lines, whereas the non-exisiting code structures are the leaf nodes with edges marked with dashed lines in Figure~\ref{fig:hierarchy}. We list four patterns of ML software. 
% software examples to illustrate the common patterns of how ML APIs' outputs affect ML software's control flow decisions. 

\subsubsection{Software pattern 1: T-or-F} This type of software only specifies one \wl which includes multiple labels, such that labels in the \wl have an equivalent effect on the software's control flow decisions. Around 35\% applications in our benchmark suite belongs to this category.

Figure~\ref{fig:app_example_level1} shows a carnivore identification application. It goes through all the predicted labels of an input photo, and executes the \ift \code{ return `It is an animal. '} if the predicted labels intersect with the pre-defined \wl Animal. In this example, mis-classifications within the pre-defined \wl Animal (\ie mis-classifying a dog image as ``Wolf'') do not lead to software misbehavior. Instead, the ML API only needs to guarantee that the input images that should lead the software executing the \ift corresponding to \wl Animal (\ie having ground-truth labels that intersect with the \wl Animal), are classified into at least one of labels specified in \wl  Animal. On the contrary, if an image contains a carnivore, while the API output do not include any label in the \wl (Figure~\ref{fig:input_example_tf_wrong}). 


To quantify the difference in the metrics of the ML API and the correctness of this software, the traditional F1 score of the ML API on the test dataset is 58\%, while only 43\% of the data correctly identified classes in the \code{Dog} \wl, leading to software behaviors as human expected. 


% percentage of data such that the software behaves as human expected is 43\%. 

% \cc{I found it awkward to say groud-truth label contains xxxx. Can we just say the image contains a carnivore?} 

% For example, in Figure~\ref{fig:app_example_level1}, the software goes through all the predicted labels of an input image, and executes the \ift \code{return `It is an animal. '} if the predicted labels intersect with the pre-defined \wl Animal. In this example, we can see that mis-classifications within the pre-defined \wl Animal do not matter, such as mis-classifying an input image with ground-truth label `Dog' to `Wolf'. Instead, the ML API only needs to guarantee that the input images that should lead the software executing the \ift corresponding to \wl Animal (\ie having ground-truth labels that intersect with the \wl Animal), are classified into at least one of labels specified in \wl  Animal. 

% For example, in Figure~\ref{fig:input_example_tf_wrong}, the ML API's output labels lead to incorrect control flow decision because the ground-truth of the input image include a label in the pre-defined \wl (\ie ``Carnivore''), while the output labels do not include any label in the \wl. 

\subsubsection{Software pattern 2: M-to-N-set} In our benchmark, 25\% software defines multiple \wls, and the \wls themselves are parallel to each other. In other words, all the \wls have equivalent priority and all the \wls that have an intersection with the output labels will be reflected in the final output of the software. In Figure~\ref{fig:app_example_non_mut}, the food classifier application invokes ML API to determine the existence of protein, fruit, and grain in a food image\cc{Yuhan, please make sure you introduce what this app is doing before talking about its code structure}. It iterates through the predicted labels of an input image, and executes all the \ifts whose corresponding branch conditions are satisfied. In this example, we can see that mis-classifications within any of the \wls could still lead to correct software behavior.

As shown in Figure~\ref{fig:input_example_mton_correct}, for an input image that includes pasta with meat,  mis-classifying ``Pasta'' to ``Noodle'' does not matter, because the ML API's outputs lead the software to correctly set \code{protein} and \code{grain} variables to \code{True}.
% \cc{Please directly say misclassify which label as which label. The same description already exists in the previous paragraph}. 
However, if an input image has ground-truth labels covering all of the \wls, the correct software behavior is setting \code{protein}, \code{fruit} and \code{grain} to \code{True}. Missing ``Bread'' in the output leads to wrong software behavior: only setting \code{protein} and \code{fruit} variables to \code{True}. 
% \cc{Same here, please describe the example. By looking at this paragraph, it could be applied to any example}.  
% \cc{yuhan, please make the format consistent. Some whitelist names are in code format, some are not}

We also quantitatively measure the difference in the metrics for the ML API and this ML Software's correctness after invoking the ML API. We see that the ML API's F1 score on the food classifier application is 73.88\%. However, only 54.72\% of the input images in which the ML API's output labels lead the software executing all the corresponding \ifts as human expected. 

\subsubsection{Software pattern 3: Priority-list} Around 10\% software defines multiple \wls, and checks the \wls one by one until finding the first one that intersects with output labels. For example, Aander-ETL (Figure~\ref{fig:priority_input_example}) specifies three \wls (\code{Monument, Construction, Person}) to classify tourist photos. It first checks if the output labels have an intersection with the \code{Monument} \wl, and executes the corresponding \ift if having an intersection. If the output labels do not intersect with \code{Monument}, the software compares the output labels with \code{Construction} and \code{Person} in a similar way. Under such software pattern, we can see that mis-classifications for labels inside any of the lower-ranked \wl will not lead to wrong control flow decisions if ML API correctly recognizes the existence of labels in the hig her-ranked \wls. 

In Figure~\ref{fig:input_example_priority_correct}, the software behaves correctly even when the API recognizes an extra incorrect label ``Mansion'' in the \wl \code{ Construction}, as API correctly recognize ``Ancient history'', which belongs to the highest-ranked \wl \code{ Monument}. However, in Figure~\ref{fig:input_example_priority_wrong},  only missing the label ``Landmark'' in the \wl \code{  Monument} can lead to completely incorrect software behavior: the software wrongly executes the \ift corresponding to the second-highest ranked \wl \code{ Construction} since it is the first \wl that intersects with the API's output labels.

We observe that the ML API's overall F1 score for the Anander-ETL software is 61\%, while only 54\% of API's output labels lead to the software executing the \ift corresponding to the highest-ranked \wl included in the input images. 

% for an input image with ground-truth labels that intersect with all the three \wls, the ML API's output labels lead to incorrect control flow decision because missing the label ``Landmark'' in the highest-ranked \wl makes the software executing the \ift corresponding to the second-highest ranked \wl. 


\subsubsection{Software pattern 4: Top-label} For APIs that produce multiple output labels, some software maps the output labels to control flow decisions in a specific order. Around 30\% applications fall in this category.
For example, Heapsortcypher (Figure~\ref{fig:app_example}) iterates through the API output labels that are ranked in descending order of their confidence scores and finds the first output label that intersects with any of the specified \wls. Then the software executes the corresponding \ift associated with the found \wl. Therefore, mis-classification for lower-ranked output labels will not lead to software misbehavior if the higher-ranked output intersects with \wls. 

As shown in Figure~\ref{fig:input_example_top_correct}, API correctly recognizes ``Produce'' for an image of apple on table, which intersects with \wl Compost. Therefore, even it wrongly outputs a lower-ranked label``Wood'' which belongs to another \wl, the software still makes a correct control flow decision. 






\begin{figure}
\begin{subfigure}{0.45\textwidth}    
    \centering
\begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Dog = ['Dog','Mammal','Carnivore','Wolf']
image = types.Image(content=dog_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Dog:
    return 'It is a animal.'
return 'It belongs to others.'
\end{lstlisting}
    \caption{Code pattern: T-or-F. }
    \label{fig:app_example_level1}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_tf_wrong.pdf}
    \caption{Failing recognize the carnivore leads to software failure. }
    \label{fig:input_example_tf_wrong}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/app_input_example_level1.pdf}
    \caption{Mis-classifying a dog as wolf does not trigger software failure. }
    \label{fig:input_example_tf_correct}
\end{subfigure}
\caption{Dogecoin~\cite{food}, an application that classifies carnivore images.  }
\label{fig:tf_example}
\end{figure}



\begin{figure}
\begin{subfigure}{0.45\textwidth}    

    \centering
             \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
proteinfoods = ['Hamburger', 'Meat', 'Patty']
fruitfoods = ['Apple', 'Fruit', 'Orange']
grainfoods = ['Noodle', 'Pasta', 'Al dente']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
protein, fruit, grain = False, False, False
for obj in response.label_annotations:
  if obj.name in proteinfoods:
    protein = True
  if obj.name in fruitfoods:
    fruit = True
  if obj.name in grainfoods:
    grain = True
RENDER_TEMPLATE(protein, fruit, grain)
\end{lstlisting}
    \caption{Software implementation. }
    \label{fig:app_example_non_mut}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_mton_wrong.pdf}
    \caption{Failing to recognize ``Cheese'' leads to software mis-behavior. }
    \label{fig:input_example_mton_wrong}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_mton_correct.pdf}
    \caption{Mis-classifying ``Pasta'' to ``Noodle'' still leads to correct software behavior. }
    \label{fig:input_example_mton_correct}
\end{subfigure}
\caption{Food classifier~\cite{food}, an application that classifies food images.}
\end{figure}


\begin{figure}
    \centering
             \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
proteinfoods = ['Hamburger', 'Meat', 'Patty']
fruitfoods = ['Apple', 'Fruit', 'Orange']
grainfoods = ['Noodle', 'Pasta', 'Al dente']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
food_list = []
for obj in response.label_annotations:
  if obj.name in proteinfoods:
    food_list.append('protein')
  if obj.name in fruitfoods:
    food_list.append('fruit')
  if obj.name in grainfoods:
    food_list.append('grain')
return food_list
\end{lstlisting}
    \caption{An example software that maps original output labels of the ML APIs to a list of \wls.  }
    \label{fig:app_example_non_mut}
\end{figure}



\begin{figure}
\begin{subfigure}{0.45\textwidth}
        \centering
             \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Monument = ['Landmark', 'Sculpture', 'Monument']
Construction = ['Building', 'Estate', 'Mansion']
Person = ['Human','Person',  'Lady']
image = types.Image(content=landmark_image)
response = client.label_detection(image=image)
Predictions = []
for obj in response.label_annotations:
  Predictions.append(obj.name)
if any([label in Monument for label in Predictions]):
  return 'It belongs to monument.'
elif any([label in Construction for label in Predictions]):
  return 'It is construction.'
elif any([label in Person for label in Predictions]):
  return 'It is person.'
\end{lstlisting}
    \caption{Software implementation. }
    \label{fig:app_example_priority}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_priority_wrong.pdf}
    \caption{Missing a label ``Landmark'' leads to software mis-behavior. }
    \label{fig:input_example_priority_wrong}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_priority_correct.pdf}
    \caption{Recognizing an extra wrong label ``Mansion'' still leads to correct software behavior. }
\label{fig:input_example_priority_correct}
\end{subfigure}
\caption{Aander-ETL~\cite{etl}, an application that classifies landmark images.  }
\label{fig:priority_input_example}
\end{figure}

\cc{Do we want to introduce the accuracy difference between API and software? And the room for improvement?}

==> bk/backups_before_fist_submission/2-2-empirical-1110.tex <==
\label{sec:empirical}

To understand how developers use ML API in real-world applications\shan{As I commented in Introduction, this opening sentence has to be more precise. It is tooooo generic now.}, we conduct an empirical study on ML software that invokes  ML APIs to make control flow decisions. 

\shan{The overall feeling of this section is lack of motivation. As a reader, I keep asking myself: why do I care how many applications use whitelists? Why do I care how many types of abstraction you use to characterize code structure? Or, why do I care about the whatever code structure? It is not clear to me, as a reader, why any of these have ANYTHING to do with software correctness, with how to customize ML APIs for software. This is related to my comments of your over-general opening sentences. Please keep in mind that readers do NOT necessarily want to ``understand how developers use ML API''. In other words, there are many more readers who want to understand how to customize an ML API to improve software correctness than readers who want to know how many whitelists a software defines. As a reader and an (impatient) reviewer, I skip paragraphs and sections that do not motivate me.}

% \yh{ML API on OI or pretrained on OI}
\subsection{Methodology}

\subsubsection{Application selection}



% Google (benchmark, search), AWS (search)
We study 40 open-source ML software applications  whose control flows are affected by the output of \emph{a multi-label image classification API}. 

We do not study the applications that directly print out the ML APIs' outputs or store these outputs without post-processing. The tasks that these applications perform are the same as the task of ML API. Therefore, there is no need to adapt APIs to software. In addition, ML APIs are only loosely integrated into these applications, e.g., not interacting with other software components. We believe they do not represent the future direction of ML software.

The 40 applications come from two sources: (1) 19 applications, which post-process the ML APIs' outputs to make control flow decisions, come from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}\shan{Why do you pick these 19?}; and (2) 21 applications come from GitHub by random checking around 60 applications\shan{What exactly are you looking for when you randomly check? Why don't you use all these 60?}.
Among these applications, 29 use Google \code{label\_detection} API, and 11 use Amazon \code{detect\_labels} API.

% \cc{Maybe also add some statistics}



\subsubsection{Test data selection}
TO-DO
\cc{It is weird to have a subsection that only has one subsubsection. How about we also introduce the open image data and ground-truth label?}







% \subsection{Common patterns of code structure of software utilizing ML APIs}
\subsection{Result summary}
The 40 applications whose control flow decisions are affected by the ML APIs' outputs pre-define several \wls, and compare ML APIs' outputs with them to decide which if-branch edge to execute, which we refer to as making application decision. 


\shan{Without knowing your application selection criteria, I cannot interpret what this ``48\%'' implies. What does the remaining 52\% applications do? If all applications in your bencharmk suite use ML API output to affect control flow, how can there be no whitelist? Can you offer more explanation here about what exactly this 48\% mean?} \yh{Sorry 48\% was an out-dated number. All the 40 apps whose control flow are affected by the ML APIs' outputs do specify whitelists. }

Take Heapsortcypher (Figure~\ref{fig:app_example}) as an example. It executes Line 8 when given a garbage image, as the API output ``Glass'' is included in the \code{Recycle} list and thus fulfills the statement in Line 7. 
% We refer to this executed branch as \emph{if/then branch}. Correspondingly, we refer to another branch that  not executes Line 8 as \emph{if/else branch}\shan{what if there is if-elsif-then?}.
We refer to a list of classes (or classification category) defined in the code\shan{what labels? you mean outputs of an ML API?} leading to the same control flow decision as a \emph{whitelist}. \code{Recycle}, \code{Compost}, and \code{Donate} are the three whitelists, taking Heapsortcypher as an example\shan{This definition has a lot of flaws.
One quick question: based on your definition, aren't all labels minus those in Recycle, Compost, and Donate also a white list? Are they?
}.

% \cc{yuhan, please put terminologies (those used in Section 3) here. Make sure that you are only using the Heapsortcypher as an example}

While these applications typically use \wls to post-process ML API results, they vary in the way of using whitelists to make application decisions. Even with the same whitelists and API outputs, the applications would behave differently according to their code structure. Next, we will introduce the common patterns observed in the studied applications.


% We find that these software typically pre-defines one or several lists of labels as branch conditions, and then maps the original output labels to the pre-defined lists which intersect with the labels. Then the software executes one or more \ifts that correspond to those mapped pre-defined lists. 
% In other words, all the labels specified in one list will lead to the same control flow decision. 

% We refer to the lists of labels leading to the same control flow decisions as \emph{whitelists} in the rest of the paper. For example, in the application example shown in Figure~\ref{fig:app_example}, the software defines three \emph{whitelists}, Recycle, Compost, and Donate. 



% They typically define several lists of labels and which one or more program branches the application should execute by comparing the API output labels and these lists. 
% They typically define several lists of labels and which one or more program branches the application should execute when the ML APIs' output labels intersect with their associated pre-defined list. 


% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X]
% if X == C1: 
%     return "B1"
% elif X == C2: 
%     return "B2"
% elif X == C3: 
%     return "B3"
% elif X == C4: 
%     return "B4"
% \end{lstlisting}
%     \caption{Minimal example showing an application without any post-processing on the ML API's output labels.  }
%     \label{fig:template_0}
% \end{figure}

% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X]
% A = [C1, C2]
% if X in A: 
%     return "X"
% else:
%     return "Y"
% \end{lstlisting}
%     \caption{Minimal example showing an application that defines a single \wl.}
%     \label{fig:template_1}
% \end{figure}


% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X1, X2]
% A = [c1, c2]
% B = [c3, c4]
% count = 1
% for W in [A, B]:
%     for x in [x1, x2, ...]:



% for x in [x1, x2, ...]:
%     for W in [A, B]:


% for W in [A, B]:
%     if x1 in W or x2 in W:
%         return "branch " + str(count)
%     if X2 in W:
%         return "branch " + str(count)
%     count += 1
% return "branch 3"
% \end{lstlisting}
%     \caption{Minimal example showing an application that defines a single \wl.}
%     \label{fig:template_2}
% \end{figure}

% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X1, X2]
% A = [C1, C2]
% B = [C3, C4]
% for X in [X1, X2]:
%     if X in A:
%         return "branch 1"
%     if X in B:
%         return "branch 2"
% return "branch 3"
% \end{lstlisting}
%     \caption{Minimal example showing an application that defines a single \wl.}
%     \label{fig:template_3}
% \end{figure}




% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X1, X2]
% W1 = [C1, C2]
% W2 = [C3]
% output = set()
% for X in ML_API_outputs:
%     if X in W1:
%         output.add("B1")
%     elif X in W2:
%         output.add("B2")
% return output 
% \end{lstlisting}
%     \caption{Minimal example showing an application that defines a single \wl.}
%     \label{fig:template_4}
% \end{figure}


\subsection{Abstractions}
\label{sec:abstractions}
As summarized in Figure~\ref{fig:hierarchy} we define four types of abstractions to characterize the code structure. 

% We denote the whole set of classes that the DNN behind the ML API is able to classify as $C=\{C_1, C_2, C_3, C_4, C_5, C_6\}$, and the labels that the input images contain as $G$. To start with, Figure~\ref{fig:template_0} shows a minimal example application without any post-processing of the ML APIs' output labels (\eg directly prints out the output labels). The application simply returns the direct output of the ML API. In other words, any one of the ML API's output classes will lead to the software executing its corresponding \ift. In the following section, we will use several minimal templates to illustrate four types of abstractions. 


% Applications may specify a \wl candidate, such that when the API's output labels intersect with the \wl, then the corresponding \ift will be executed, \code{return "B1"} in Figure~\ref{fig:template_1}. In the rest of the paper, we will refer to executing a \ift as mapping the API outputs to its corresponding \wl. In this case, mis-classifications inside the \wl do not matter, as long as the ML API output labels intersect with the \wl for images containing labels in \wl. 

% Applications may specify multiple \wls candidates, and check these whitelists one by one to find the first one that intersects with API result as shown in Figure~\ref{fig:template_2}. In this case, mis-classifications for lower-ranked \wls do not matter, as long as the output labels in higher-ranked whitelists lead to the correct control flow decision. 


\textbf{1) How many \wl candidates does the software define? } The software may specify one or several \wls candidates. Each \wl candidate is related to a particular software branch: the software will execute the corresponding \ift when the ML APIs' outputs intersect with the labels in the \wls candidates. In the rest of the paper, we will refer to executing the \ift as selecting its associated \wl.

\textbf{2) How are the \wls selected? } For the software specifying several \wls, there are three ways such that the \wls are selected: (1) the software checks the \wls in a specific order, and selects at most one \wl when the API outputs intersect with the \wl; (2) the software selects a set of \wls which intersect with API outputs; (3) the software selects an ordered list of \wls which intersect with API outputs. In this case, the order in which the API outputs appear and intersect with the \wls matters. 
 
% (i) the software executes all the \ifts when the API's outputs intersect with the \wls associated with the branch condition. In other words, the original output labels are mapped to several \wls; (ii) the software checks whitelists in a specific order, and only executes the lower-ranked \ifts when API outputs do not intersect with any higher-ranked whitelist, leading to at most one \ift to be executed. In other words, the original output labels are mapped to at most one \wl. 
% \cc{I changed it from multiple to several, so that it means 0 to N}

% For the software specifying multiple \wls, when the software checks if the output labels intersect with the \wls, there are two possible ways of checking: (i) the software executes all the \ifts when the API's outputs intersect with the \wls associated with the branch condition. In other words, the original output labels may be mapped to multiple \wls; (ii) the software checks the branch conditions in a specific order, and only executes the lower-ranked \ifts if the higher-ranked branch conditions are false, leading to at most one \ift to be executed. In other words, the original output labels are mapped to at most one \wl. 
% (i) the software executes at most one if/then branch when the API's outputs intersect with the \wl associated with the branch condition; (ii) the software executes all the if/then branches when the API's outputs intersect with the \wls associated with the branch condition. 
% For the software that specifies several \wls, some software will compare the ML APIs' outputs with the \wls, and break at a program branch once the outputs intersect with the \wl associated with the branch. In other words, the final output of the software is the message corresponding to with only one program branch. Other software compares the ML APIs' outputs with the \wls, and outputs all the messages 


\textbf{3) How is the order determined?}  For the software specifying multiple \wls, the order of examining intersections between \wls and ML API outputs determines software behavior. If we reconstruct the examination into a two-level nested loop that iterates through \wls and API outputs, there naturally arises two types of loop structure: prioritize the specified \wls or the API output labels.




\begin{figure}
     \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
    \caption{Abstractions that characterize the code structure. The decision nodes (in blue) are abstractions defined in Section~\ref{sec:abstractions}. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
\label{fig:hierarchy}
\end{figure}




\begin{figure*}
     \includegraphics[width=\linewidth]{figs/code.pdf}
    \caption{Examples of software such that the ML APIs' outputs affect the control flow decisions. }
\label{fig:code}
\end{figure*}



\subsection{Common Code Patterns}
\label{sec:examples}
\yh{Currently re-writing this section}
Based on these four types of abstractions, Figure~\ref{fig:hierarchy} summarized all the possible code patterns in a structure of a decision tree. Each decision nodes represent an abstraction. Each leaf node represents a code pattern constructed with the sequences of different decisions made at each decision node. While Figure~\ref{fig:hierarchy} illustrates six possibilities, our studied applications only contain four of them (green box in solid lines).

% Based on these four types of abstractions, we can characterize the common code structures as shown in Figure~\ref{fig:hierarchy}. Each decision node in the decision tree represents an abstraction as described in Section~\ref{sec:abstractions}. Each leaf node in the decision tree represents a type of code structure constructed with the sequences of different decisions made at each decision node. The leaf nodes are all the possible code structures constructed with the abstractions. However, we only found a subset of all the possible code structures in the benchmark suite. The existing types of code structures are shown in the leaf nodes with edges marked with solid lines, whereas the non-exisiting code structures are the leaf nodes with edges marked with dashed lines in Figure~\ref{fig:hierarchy}. We list four patterns of ML software. 
% software examples to illustrate the common patterns of how ML APIs' outputs affect ML software's control flow decisions. 

\subsubsection{Software pattern 1: T-or-F} This type of software only specifies one \wl which includes multiple labels, such that labels in the \wl have an equivalent effect on the software's control flow decisions. Around 35\% of applications in our benchmark suite belong to this category.

As shown in Figure~\ref{fig:code}(a), the application defines a \wl \code{A = [c1, c2]}, and goes through the outputs of the ML API. It  executes the if-branch edge \code{return "branch 1"} when it finds an output class belonging to \code{A}. We refer to executing the if-branch edge as selecting the \wl \code{ A} in the rest of the paper.  If none of the output classes belongs to \code{A}, the application executes the code \code{return "branch 2"}. We refer to executing the code when the ML API's outputs do not match any of the \wls as selecting \code{others}. 

In this application pattern, mis-classifications within the pre-defined \wl do not matter, as long as samples with ground-truth 
% shows a carnivore identification application. It goes through all the predicted labels of an input photo, and executes the \ift \code{ return `It is an animal. '} if the predicted labels intersect with the pre-defined \wl Animal. In this example, mis-classifications within the pre-defined \wl Animal (\ie mis-classifying a dog image as ``Wolf'') do not lead to software misbehavior. Instead, the ML API only needs to guarantee that the input images that should lead the software executing the \ift corresponding to \wl Animal (\ie having ground-truth labels that intersect with the \wl Animal), are classified into at least one of labels specified in \wl  Animal. On the contrary, if an image contains a carnivore, while the API output do not include any label in the \wl (Figure~\ref{fig:input_example_tf_wrong}). 


% To quantify the difference in the metrics of the ML API and the correctness of this software, the traditional F1 score of the ML API on the test dataset is 58\%, while only 43\% of the data correctly identified classes in the \code{Dog} \wl, leading to software behaviors as human expected. 


% percentage of data such that the software behaves as human expected is 43\%. 

% \cc{I found it awkward to say groud-truth label contains xxxx. Can we just say the image contains a carnivore?} 

% For example, in Figure~\ref{fig:app_example_level1}, the software goes through all the predicted labels of an input image, and executes the \ift \code{return `It is an animal. '} if the predicted labels intersect with the pre-defined \wl Animal. In this example, we can see that mis-classifications within the pre-defined \wl Animal do not matter, such as mis-classifying an input image with ground-truth label `Dog' to `Wolf'. Instead, the ML API only needs to guarantee that the input images that should lead the software executing the \ift corresponding to \wl Animal (\ie having ground-truth labels that intersect with the \wl Animal), are classified into at least one of labels specified in \wl  Animal. 

% For example, in Figure~\ref{fig:input_example_tf_wrong}, the ML API's output labels lead to incorrect control flow decision because the ground-truth of the input image include a label in the pre-defined \wl (\ie ``Carnivore''), while the output labels do not include any label in the \wl. 

\subsubsection{Software pattern 2: M-to-N-set} In our benchmark, 25\% software defines multiple \wls, and the \wls themselves are parallel to each other. In other words, all the \wls have equivalent priority and all the \wls that have an intersection with the output labels will be reflected in the final output of the software. In Figure~\ref{fig:app_example_non_mut}, the food classifier application invokes ML API to determine the existence of protein, fruit, and grain in a food image\cc{Yuhan, please make sure you introduce what this app is doing before talking about its code structure}. It iterates through the predicted labels of an input image, and executes all the \ifts whose corresponding branch conditions are satisfied. In this example, we can see that mis-classifications within any of the \wls could still lead to correct software behavior.

As shown in Figure~\ref{fig:input_example_mton_correct}, for an input image that includes pasta with meat,  mis-classifying ``Pasta'' to ``Noodle'' does not matter, because the ML API's outputs lead the software to correctly set \code{protein} and \code{grain} variables to \code{True}.
% \cc{Please directly say misclassify which label as which label. The same description already exists in the previous paragraph}. 
However, if an input image has ground-truth labels covering all of the \wls, the correct software behavior is setting \code{protein}, \code{fruit} and \code{grain} to \code{True}. Missing ``Bread'' in the output leads to wrong software behavior: only setting \code{protein} and \code{fruit} variables to \code{True}. 
\shan{This example's discussion is confusing. The phenomenon of mis-classifying pasta to noodle does not matter is not unique to this pattern; it applies to the first T-of-F pattern as well. I also don't understand why you emphasize 
``if an input ... has ground-truth labels covering all ...''. Even if the ground truth labels do not cover all but
instead only cover fruit and grain, wouldn't missing bread still a problem? None of your discussion here sounds 
unique to this pattern to me.}
% \cc{Same here, please describe the example. By looking at this paragraph, it could be applied to any example}.  
% \cc{yuhan, please make the format consistent. Some whitelist names are in code format, some are not}

% We also quantitatively measure the difference in the metrics for the ML API and this ML Software's correctness after invoking the ML API. We see that the ML API's F1 score on the food classifier application is 73.88\%. However, only 54.72\% of the input images in which the ML API's output labels lead the software executing all the corresponding \ifts as human expected. 

\subsubsection{Software pattern 3: Priority-list} Around 10\% software defines multiple \wls, and checks the \wls one by one until finding the first one that intersects with output labels. 



% For example, Aander-ETL (Figure~\ref{fig:priority_input_example}) specifies three \wls (\code{Monument, Construction, Person}) to classify tourist photos. It first checks if the output labels have an intersection with the \code{Monument} \wl, and executes the corresponding \ift if having an intersection. If the output labels do not intersect with \code{Monument}, the software compares the output labels with \code{Construction} and \code{Person} in a similar way. Under such software pattern, we can see that mis-classifications for labels inside any of the lower-ranked \wl will not lead to wrong control flow decisions if ML API correctly recognizes the existence of labels in the higher-ranked \wls. 

% In Figure~\ref{fig:input_example_priority_correct}, the software behaves correctly even when the API recognizes an extra incorrect label ``Mansion'' in the \wl \code{ Construction}, as API correctly recognize ``Ancient history'', which belongs to the highest-ranked \wl \code{ Monument}. However, in Figure~\ref{fig:input_example_priority_wrong},  only missing the label ``Landmark'' in the \wl \code{  Monument} can lead to completely incorrect software behavior: the software wrongly executes the \ift corresponding to the second-highest ranked \wl \code{ Construction} since it is the first \wl that intersects with the API's output labels.

% We observe that the ML API's overall F1 score for the Anander-ETL software is 61\%, while only 54\% of API's output labels lead to the software executing the \ift corresponding to the highest-ranked \wl included in the input images. 

% for an input image with ground-truth labels that intersect with all the three \wls, the ML API's output labels lead to incorrect control flow decision because missing the label ``Landmark'' in the highest-ranked \wl makes the software executing the \ift corresponding to the second-highest ranked \wl. 


\subsubsection{Software pattern 4: Top-label} For APIs that produce multiple output labels, some software maps the output labels to control flow decisions in a specific order\shan{???In pattern 3, software maps ... ``in a specific order'' as well.}. Around 30\% applications fall in this category.
For example, Heapsortcypher (Figure~\ref{fig:app_example}) iterates through the API output labels that are ranked in descending order of their confidence scores and finds the first output label that intersects with any of the specified \wls. Then the software executes the corresponding \ift associated with the found \wl. Therefore, mis-classification for lower-ranked output labels will not lead to software misbehavior if the higher-ranked output intersects with \wls. 

As shown in Figure~\ref{fig:input_example_top_correct}, API correctly recognizes ``Produce'' for an image of apple on table, which intersects with \wl Compost. Therefore, even it wrongly outputs a lower-ranked label``Wood'' which belongs to another \wl, the software still makes a correct control flow decision. 

\shan{What is the F1 score drop for this category?}






% \begin{figure}
% \begin{subfigure}{0.45\textwidth}    
%     \centering
% \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% Dog = ['Dog','Mammal','Carnivore','Wolf']
% image = types.Image(content=dog_image)
% response = client.label_detection(image=image)
% for obj in response.label_annotations:
%   if obj.name in Dog:
%     return 'It is a animal.'
% return 'It belongs to others.'
% \end{lstlisting}
%     \caption{Code pattern: T-or-F. }
%     \label{fig:app_example_level1}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_tf_wrong.pdf}
%     \caption{Failing recognize the carnivore leads to software failure. }
%     \label{fig:input_example_tf_wrong}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/app_input_example_level1.pdf}
%     \caption{Mis-classifying a dog as wolf does not trigger software failure. }
%     \label{fig:input_example_tf_correct}
% \end{subfigure}
% \caption{Dogecoin~\cite{food}, an application that classifies carnivore images.  }
% \label{fig:tf_example}
% \end{figure}



% \begin{figure}
% \begin{subfigure}{0.45\textwidth}    

%     \centering
%              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% proteinfoods = ['Hamburger', 'Meat', 'Patty']
% fruitfoods = ['Apple', 'Fruit', 'Orange']
% grainfoods = ['Noodle', 'Pasta', 'Al dente']
% image = types.Image(content=trash_image)
% response = client.label_detection(image=image)
% protein, fruit, grain = False, False, False
% for obj in response.label_annotations:
%   if obj.name in proteinfoods:
%     protein = True
%   if obj.name in fruitfoods:
%     fruit = True
%   if obj.name in grainfoods:
%     grain = True
% RENDER_TEMPLATE(protein, fruit, grain)
% \end{lstlisting}
%     \caption{Software implementation. }
%     \label{fig:app_example_non_mut}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_mton_wrong.pdf}
%     \caption{Failing to recognize ``Cheese'' leads to software mis-behavior. }
%     \label{fig:input_example_mton_wrong}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_mton_correct.pdf}
%     \caption{Mis-classifying ``Pasta'' to ``Noodle'' still leads to correct software behavior. }
%     \label{fig:input_example_mton_correct}
% \end{subfigure}
% \caption{Food classifier~\cite{food}, an application that classifies food images.}
% \end{figure}


% \begin{figure}
%     \centering
%              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% proteinfoods = ['Hamburger', 'Meat', 'Patty']
% fruitfoods = ['Apple', 'Fruit', 'Orange']
% grainfoods = ['Noodle', 'Pasta', 'Al dente']
% image = types.Image(content=trash_image)
% response = client.label_detection(image=image)
% food_list = []
% for obj in response.label_annotations:
%   if obj.name in proteinfoods:
%     food_list.append('protein')
%   if obj.name in fruitfoods:
%     food_list.append('fruit')
%   if obj.name in grainfoods:
%     food_list.append('grain')
% return food_list
% \end{lstlisting}
%     \caption{An example software that maps original output labels of the ML APIs to a list of \wls.  }
%     \label{fig:app_example_non_mut}
% \end{figure}



% \begin{figure}
% \begin{subfigure}{0.45\textwidth}
%         \centering
%              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% Monument = ['Landmark', 'Sculpture', 'Monument']
% Construction = ['Building', 'Estate', 'Mansion']
% Person = ['Human','Person',  'Lady']
% image = types.Image(content=landmark_image)
% response = client.label_detection(image=image)
% Predictions = []
% for obj in response.label_annotations:
%   Predictions.append(obj.name)
% if any([label in Monument for label in Predictions]):
%   return 'It belongs to monument.'
% elif any([label in Construction for label in Predictions]):
%   return 'It is construction.'
% elif any([label in Person for label in Predictions]):
%   return 'It is person.'
% \end{lstlisting}
%     \caption{Software implementation. }
%     \label{fig:app_example_priority}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_priority_wrong.pdf}
%     \caption{Missing a label ``Landmark'' leads to software mis-behavior. }
%     \label{fig:input_example_priority_wrong}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_priority_correct.pdf}
%     \caption{Recognizing an extra wrong label ``Mansion'' still leads to correct software behavior. }
% \label{fig:input_example_priority_correct}
% \end{subfigure}
% \caption{Aander-ETL~\cite{etl}, an application that classifies landmark images.  }
% \label{fig:priority_input_example}
% \end{figure}

% \cc{Do we want to introduce the accuracy difference between API and software? And the room for improvement?}

==> bk/backups_before_fist_submission/2-2-empirical-1117.tex <==
\label{sec:empirical}

This section introduces how ML API influences the behavior of MLaaS applications and then motivates:  
(1) the need to customize the ML API backend for each application, and 
(2) common patterns in which ML API output affects an application's decision process.
\subsection{Definitions}

% In addition, ML APIs are only loosely integrated into these applications, e.g., not interacting with other software components. We believe they do not represent the future direction of ML software.

% The 40 applications come from two sources: (1) 19 applications, which post-process the ML APIs' outputs to make control flow decisions, come from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}\shan{Why do you pick these 19?}; and (2) 21 applications come from GitHub by random checking around 60 applications\shan{What exactly are you looking for when you randomly check? Why don't you use all these 60?}.
% Among these applications, 29 use Google \code{label\_detection} API, and 11 use Amazon \code{detect\_labels} API.

% \cc{Maybe also add some statistics}



% \subsubsection{Test data selection}
% TO-DO
% \cc{It is weird to have a subsection that only has one subsubsection. How about we also introduce the open image data and ground-truth label?}


\begin{figure}
     \includegraphics[width=.95\linewidth]{figs/motivate_2examples.pdf}
    \caption{Code snippets from two example applications. Branch conditions influenced by API output and the structures over the conditional branches are highlighted.}
\label{fig:2examples}
\end{figure}

\mypara{Preliminaries} We begin with basic definitions.
% We first define the terminologies used in our paper.



% \begin{itemize}
%     \item \emph{Application decision}: the control flow decision of  which ML-API-related branch edge to execute
%     \item \emph{Conditional branches}: the lists of classes the application pre-defines in their source code, such that classes in these lists will lead to the same application decision. \yh{needs polish}
%     \item Selecting a whitelist $A$: the process of executing the branch edge corresponding to whitelist A
%     \item Selecting \code{others}: the process of executing the branch edge for not selecting any \wls
%     \item \emph{Ground-truth decision}: the application decision led by the human-labeled ground-truth of the input
% \end{itemize}


\begin{packeditemize}
    \item {\em ML API output:} the output of the MLaaS in response to the invocation of a single input, \eg a list of classes describing the content of an input image or the scores indicating the sentiment of the input text.
    % \item \emph{Conditional branches}: the branch conditioned on the API outputs 
    \item \emph{Branch conditions:} once the application receives the API output, it uses the branch conditions to decide which branch or branches to execute based on the API outputs.
    % \item \emph{Target-edge:} the branch edge that is executed when the API outputs fulfill a branch condition.%predicate of containing certain values. It typically is the edge following \code{then} statement.
    % \item \emph{A-edge}: for applications that compare API outputs with arrays of classes (\eg \code{A, B, C}), we refer to the Target-edge that is executed when the branch condition using array \code{A} is fulfilled as \emph{A-edge}.
    % \item \emph{Otherwise-edge}: the edge that is executed when none of the Target-edge is executed. 
    % \item \emph{Fall-through edge}: The non-target edge of a branch.
    % \item \emph{Path}: A feasible combination of edges of all conditional branches.
    % \item \emph{Target-path}: A path that contains at least one target edge.
    
    % % \item \emph{Whitelist}: A whitelist is a set of all ML API outputs that lead software to execute its corresponding whitelist-path.
    % \item \emph{Otherwise-path}: A path without any target edge. \cc{Please feel free to remove any concepts that are needed}
    \item \emph{Application decision}: given particular ML API output, the branch or branches whose branch conditions are satisfied.\footnote{Here, it is implicitly assumed that the application decision is affected only by the ML API output on the current input, not previous API output. While this may not be universally true, it holds for all the real-world applications that we have studied.}
    % the decision of which \emph{Target-edge} or \emph{Otherwise-edge} to execute. 
    % \item Selecting a whitelist $A$: the process of executing the branch edge corresponding to whitelist A
    \item \emph{Ground-truth decision}: the application decision if the API output is  human-labeled ground-truth of the input. 
    % \item \emph{Critical errors}: the errors that lead the application to execute edges different from the ground-truth decisions.
\end{packeditemize}


\mypara{Software decision process}
Given these definitions, an application's {\em software decision process} is the logic that maps an ML API output to an application decision. 
The code snippet in Figure~\ref{fig:input_example} shows an example software decision process, which maps the output of a classification ML API on an image to the image's recycling categorization specific to this application.

\mypara{Critical and non-critical errors}
Importantly, each software decision process decides when different ML API outputs lead to the same ground-truth decision (defined above), \ie {\em non-critical} error of ML API output {\em vs.} when different ML API outputs lead to decisions different from the ground-truth decision, \ie {\em critical} error of ML API output.

As we will see, the key is that {\em not} all errors are critical and that the critical errors {\em vary} across applications (using the same ML API) due to their different application decision processes.
%Thus, each application's decision process, if used carefully, could be leveraged to improve ML API output to reduce wrong application decisions. 
In the remainder of the section, we first present a systematic taxonomy of application decision processes and then apply the taxonomy to analyze a range of real-world applications using commercial MLaaS ML APIs.
%However, to unleash such potential in practice, we first need a deep understanding on the software contexts of various applications using real MLaaS {\em in the wild}.
In this empirical analysis, we focus on two central questions:
\begin{packeditemize}
\item Among applications using the same ML API, how much they differ in their application decision processes, and 
\item Despite the application heterogeneity, whether common patterns emerge which might allow extraction of information regarding an application's decision process.
\end{packeditemize}



\begin{figure}
     \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
    \caption{Key dimensions that differentiate the code structures. The decision nodes (in blue) are key dimensions. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
\label{fig:hierarchy}
\end{figure}



%\subsection{\hspace{-0.2cm} How ML API affects conditional branches}
\subsection{How is an application decision process affected by ML API?}
%\subsection{Taxonomy on how ML APIs affect application decision process}

\jc{text in this section can be tightened..}

%For each of these applications in our study, its software context is determined along two dimensions
% An application decision process can be characterized in two dimensions:
Two application decision processes may differ along one (or both) of the following dimensions:
{\em (i)} how each branch condition uses ML API output, and
{\em (ii)} how the conditional branches are structured.


\yh{be more precise about the titles, ask questions, define it and measure it }

\mypara{Two types of API output-based branch conditions}
% We identify two types of conditional branches
Figure~\ref{fig:2examples} shows an illustrative example for each.
%\item{\em Class lists:} 
The first type is used when the API output is a label or a list of labels, and several pre-defined {\em class lists} are then used to check if the API output labels belong to which list.
The code snippet of \code{Heapsortcypher}~\cite{heapsort} in Figure~\ref{fig:2examples}(a), for example, calls MLaaS with an image and receives class labels as ML API output.
It then checks if the API output belongs to three lists of classes, \code{Recycle}, \code{Compost}, \code{Donate} as the branch conditions to decide which branch to execute.
For an input with ground-truth class \code{``Shirt''}, the ground-truth decision is to execute the \code{Donate} branch.
If the ML API output is \code{``Paper''}, it will be a critical error, because the application decision (the \code{Recycle} branch) deviates from the ground-truth decision, whereas, if the ML API output is \code{``Jacket''}, it is not a critical error since the application's decision remains the same as the ground-truth decision.
%For example, the branch conditions in the \code{Heapsortcypher} application check if each API output class belongs to one of the three pre-defined lists. 
% \shan{This example is already discussed in the Introduction.}

%\item{\em Value ranges:}



The second type of branch condition is used when the API output is a score, and several pre-defined {\em value ranges} are then used to check if the API output scores fall in which range. 
The code snippet of \code{FoodDelivery}~\cite{food-delivery} in Figure~\ref{fig:2examples}(b), for example, calls MLaaS with a text sentence and receives a sentiment score as the ML API output. 
It uses three branch conditions, each checking if the API output score lies in a certain range. 
Given an input sentence whose ground-truth label is ``positive'', the ground-truth decision will print \code{It's a positive sentence}, and a critical error in this case will be when the API outputs a score lower than 0.6 on this sentence. 

% \shan{I am not totally sure about this arrangement. We already motivated somewhat in Introduction. How about we put any extra examples to a bit later when we discuss our empirical study result? It will also help move the pace faster into the empirical study.}
%As shown in the \code{FoodDelivery} application in Figure~\ref{fig:input_example}(b), it calls Google's \code{analyze\_sentiment} API to output a score indicating the emotional opinion of the input text. 
%The branch condition checks whether the score is over 0.6 (\ie the text is positive) or below 0.3 (\ie the text is negative), or otherwise (neutral). 
%\end{packeditemize}



%While these concepts may sound high-level, let us make them more concrete using two real-world applications, \code{Heapsortcypher} (Figure~\ref{fig:input_example}(a)) and \code{Food-delivery} (Figure~\ref{fig:input_example}(b)).
%
%\begin{packeditemize}
%\item 
%
%%\shan{This example is already discussed in the Introduction.}
%
%\item 
%%\shan{I am not totally sure about this arrangement. We already motivated somewhat in Introduction. How about we put any extra examples to a bit later when we discuss our empirical study result? It will also help move the pace faster into the empirical study.}
%\end{packeditemize}


\begin{figure*}
     \includegraphics[width=\linewidth]{figs/code.pdf}
    \caption{Examples of software such that the ML APIs' outputs affect the control flow decisions. }
\label{fig:code}
\end{figure*}


\mypara{Common structures over conditional branches}
Given the conditional branches, the way these branches are structured can also greatly affects the application decision process.
The structures over conditional branches differ along three key dimensions.
(1) the {\em number of conditional branches}; 
(2) the {\em number of executed branches} (for applications with several conditional branches, the application can either execute the first satisfied branch or all branches that satisfy the branch conditions); and finally
(3) the {\em order of examination}---when there are multiple elements in an ML API output {\em and} multiple conditional branches, an application can choose to examine each element one by one against the conditional branches (\ie examining the $1^{\textrm{st}}$ element in API output against all branch conditions before moving to the $2^{\textrm{nd}}$ element, and so forth) or examine all elements against each conditional branch (\ie examining all elements against the $1^{\textrm{st}}$ branch condition, then all elements against the $2^{\textrm{nd}}$ condition, and so forth). 
%\begin{packeditemize}
%\item {\em Number of conditional branches:} The applications may define one or several branch conditions. 
%\item {\em Number of executed branches:} For applications with several conditional branches, the application can either execute the first satisfied branch or all branches that satisify the branch conditions. 
%\item {\em Order of examination:}  
%When there are multiple elements in an ML API output {\em and} multiple conditional branches, an application can choose to examine each element one by one against the conditional branches (\ie examining the $1^{\textrm{st}}$ element in API output against all branch conditions before moving to the $2^{\textrm{nd}}$ element, and so forth) or examine all elements against each conditional branch (\ie examining all elements against the $1^{\textrm{st}}$ branch condition, then all elements against the $2^{\textrm{nd}}$ condition, and so forth). 
%%Applications that execute at most one branch  may either iterate through branch conditions first or the API outputs first in a two-level for loop. 
%\end{packeditemize}

With these dimensions, we identify four structures over conditional branches (Figure~\ref{fig:hierarchy}). 
Figure~\ref{fig:code} depicts a simple illustrative example of each structure.
\jc{we need to replace these names with macros. they will definitely be changed.}
\jc{yuhan, can you explain these categories using the three dimensions just introduced? what's the point of introducing the dimensions without actually using them?}
\begin{packeditemize}
\item {\em T-or-F:} Figure~\ref{fig:code}(a) is an example code structure where the first key dimension is only one branch condition. The application checks if the API outputs intersect with the list \code{A}. If so, it executes the branch \code{return "branch 1"}, otherwise, the branch \code{return "branch 2"} is executed. 
\item {\em M-to-N-set:}  Figure~\ref{fig:code}(b) is an example where it falls into the category of (1) defining more than one branch condition at the first key dimension; (2) executing a set of branches at the second key dimension.  The application defines two branch conditions in the for loop. If any of the branch conditions are fulfilled, the branch will be executed (\ie adding the message corresponding to the branch to the final output set). 
\item {\em Priority-list:} This type of applications define several class lists, and check the class lists in order until finding the first one that intersects with the API outputs. Figure~\ref{fig:code}(c) is an example of this code structure, and it falls into the category of (1) defining more than one branch condition at the first key dimension; (2) executing at most one branch; (3) first enumerate the branch conditions first at the third key dimension. 
\item {\em Top-label:} This type of applications iterate over the API outputs until finding one that intersects with any of the defined class lists, as shown in Figure~\ref{fig:code}(d). 
\end{packeditemize}





% \mypara{Software context}
% Given these definitions, we define the software context of an application as the {\em critical errors} on the ML API output that will lead to different application decisions than the ground-truth decisions\shan{???I don't quite get it}.
% While these applications may sound high-level, let us make them more concrete using two real-world applications, \code{Heapsortcypher} (Figure~\ref{fig:input_example}(a)) and \code{Food-delivery} (Figure~\ref{fig:input_example}(b)).

% \begin{packeditemize}
% \item 
% The code snippet of \code{Heapsortcypher} in Figure~\ref{fig:input_example}(a) calls MLaaS with an image and receives class labels as ML API output.
% It then checks if the API output belongs to three lists of classes, \code{Recycle}, \code{Compost}, \code{Donate} as the branch conditions to decide which branch to execute.
% % , so that 
% % % s. Each of the branch conditions 
% % checks if the API output belongs to the list of classes associated with the branch. 
% For an input with ground-truth class \code{``Shirt''}, the ground-truth decision is to execute the \code{Donate} branch.
% % \emph{Target-edge} associated with the \code{Donate} list. 
% If the ML API output is \code{``Paper''}, it will be a critical error, because the application decision will be the \code{Recycle} branch, deviating from the ground-truth decision.
% % is executing the \emph{Target-edge} associated with the \code{Recycle} list. This application decision deviates from the ground-truth decision, thus forming a critical error. 
% Nevertheless, if the ML API output is 
% % mis-classifies the Shirt image to 
% \code{``Jacket''}, it is not a critical error since the application's decision remains the same as the ground-truth decision.
% % is still executing the \emph{Target-edge} associated with the \code{Donate} edge.
% \shan{This example is already discussed in the Introduction.}

% \item The code snippet of \code{FoodDelivery} in Figure~\ref{fig:input_example}(b) calls MLaaS with a sentence and receives a sentiment score as the ML API output. 
% It uses three branch conditions, each checking
% % . Each branch condition checks 
% if the API output score lies in a range. Given an input sentence whose ground-truth label is ``positive'', the ground-truth decision will execute the branch that prints \code{It's a positive sentence}, and a critical error in this case will be when the API outputs a score lower than 0.6 on this sentence. 
% \shan{I am not totally sure about this arrangement. We already motivated somewhat in Introduction. How about we put any extra examples to a bit later when we discuss our empirical study result? It will also help move the pace faster into the empirical study.}
% \end{packeditemize}

% Importantly, these examples show that {\em not} all errors are critical errors, and thus such per-application software context, if used carefully, could improve ML API output to reduce wrong application decisions. 
% However, to unleash such potential in practice, we first need a deep understanding on the software contexts of various applications using real MLaaS {\em in the wild}.


% \mypara{An empirical study over real MLaaS applications}
% To this end, in the remainder of this section, we run an empirical study over 77 open-source applications which collectively use 6 ML APIs.
% These applications are selected from a recently published benchmark suite~\cite{wan2021machine}.
% We keep all applications except those that directly print out or store the ML API outputs without post-processing (for these applications, by definition any errors of API output will be critical).

% Our empirical analysis focuses two central questions:
% (1) among applications using the same ML API, how much they differ in their software context (critical errors), and 
% (2) despite the application heterogeneity, whether common patterns emerge which might allow automatic extraction of software context.  



% \subsection{\hspace{-0.2cm} Use of API output in conditional branches}


% For each of these applications in our study, its software context is determined along two dimensions
% {\em (i)} the branch conditions that use API output, and
% {\em (ii)} the structure over the branch conditions.Two applications' software contexts can differ along either or both dimensions. 

% \mypara{Use of API output in branch conditions}
% Depending on the API output, we identify two types of conditional branches. 
% \begin{packeditemize}
% \item{\em Class lists:} The first type is used when the API output is a label or a list of labels, and it checks if the API output labels belong to several pre-defined lists of classes.
% For example, the branch conditions in the \code{Heapsortcypher} application check if each API output class belongs to one of the three pre-defined lists. 
% \item{\em Value ranges:}
% The second type of branch condition is used when the API output is a score, and it  then checks if the API output scores fall in several pre-defined value ranges. 
% As shown in the \code{FoodDelivery} application in Figure~\ref{fig:input_example}(b), it calls Google's \code{analyze\_sentiment} API to output a score indicating the emotional opinion of the input text. 
% The branch condition checks whether the score is over 0.6 (\ie the text is positive) or below 0.3 (\ie the text is negative), or otherwise (neutral). 
% \end{packeditemize}


% \mypara{Structures of conditional branches}
% Given the API output and conditional branches, the way these conditional branches are structured can also greatly affect the application decision.
% The structures of conditional branches differ along three key dimensions, shown in Figure~\ref{fig:hierarchy}:
% \begin{packeditemize}
% \item Number of branch conditions: The applications may define one or several branch conditions. 
% \item Number of executed branches: For applications that define several branch conditions, the application can either execute at most one branch or execute a set of branches that fulfill the branch conditions. 
% \item Order of examination:  Applications that execute at most one branch  may either iterate through branch conditions first or the API outputs first in a two-level for loop. 
% \end{packeditemize}

% Along these dimensions, we carefully categorize the conditional branch structure of each application in our study.
% Four common structures emerge.
% \begin{packeditemize}
% \item T-or-F: As shown in Figure~\ref{fig:code}(a), the application defines one branch condition to check if the API outputs intersect with the list \code{A}. If so, it executes the branch \code{return "branch 1"}, otherwise, the branch \code{return "branch 2"} is executed. 
% \item M-to-N-set: As shown in Figure~\ref{fig:code}(b), the application defines two branch conditions in the for loop. If any of the branch conditions are fulfilled, the branch will be executed (\ie adding the message corresponding to the branch to the final output set). 
% \item Priority-list: This type of applications define several class lists, and check the class lists in order until finding the first one that intersects with the API outputs. Figure~\ref{fig:code}(c) is an example of this code structure.  
% \item Top-label: This type of applications iterate over the API outputs until finding one that intersects with any of the defined class lists, as shown in Figure~\ref{fig:code}(d). 
% \end{packeditemize}

















\subsection{\hspace{-0.25cm}Empirical study of application heterogeneity}


{\em As a consequence of the application decision processes, not all errors are critical.
And because each application has unique conditional branches and its structure over these branches, their critical errors are greatly different. 
}

\mypara{An empirical study over real MLaaS applications}
To this end, in the remainder of this section, we run an empirical study over 77 open-source applications which collectively use 6 ML APIs.
These applications are selected from a recently published benchmark suite~\cite{wan2021machine}.
We keep all applications except those that directly print out or store the ML API outputs without post-processing (for these applications, by definition, any errors of API output will be equally critical, so there is little room for improvement by customizing the model based on critical errors.)

\mypara{How code structures affect critical errors of API output}
If a misclassification occurs within a class list associated to the same conditional branch, then it is not a critical error. 
But it would be a critical error, if an image is misclassified with a label in the class list of a different conditional branch than the ground-truth label.

Even with the same branch conditions, the critical errors can differ depending on the structure of the conditional branches.

Take the code structures in Figure~\ref{fig:code} as an example. Figure~\ref{fig:code}(b)(c)(d) defines two same class lists. Given an input  with ground-truth class \code{c1} and API outputs \code{[c3, c1]}. The ground-truth decision is execute the branch corresponding to \code{A}. For M-to-N-set, this API output leads the execution of branches corresponding to class lists \code{A} and \code{B}, thus forming a critical error. However, for Priority-list, this API output correctly leads the application to execute the branch corresponding to \code{A}. On the other hand, Top-label iterates over the outputs and breaks at the branch corresponding to \code{B}, which is also a critical error for the application. 


% \jc{Yuhan, please fill in}

\mypara{Empirical observations on application heterogeneity}
Figure~\ref{tab:stats} enumerates the conditional branches used in the applications under our study and assigns each application to one of the aforementioned structures. 
We make three empirical observations.
\begin{packeditemize}
\item In each application, {\em the number of pre-defined class lists and value ranges are relatively small}, indicating a potential for MLaaS to increase accuracy on specific classes by customizing (retraining) the ML models behind ML API. 
Collectively, set of classes in the class lists is relatively small compared to the number of classes in a typical classification training dataset (\eg 9605 classes in OpenImages~\cite{openimages} or 1000 classes in ImageNet~\cite{5206848}). 
\item More importantly, there are {\em very few overlaps among the branch conditions of different applications}, making a case for {\em per-application} customization of ML API backend model.
Specifically, among all (826 \footnote{We separately count the pairs for the 40 Vision tasks and 5 NLP entity recognition task, and 36 NLP text classification tasks as they do not share label sets}) pairs of applications with class-list-based branch conditions, only 71 of them overlap by more than one classes between their class lists. 
Similarly, among the 381 classes that appear in at least one application's branch conditions, only 16 of them appear in more than three applications.
\item Similarly, the structure over the conditional branches also varies greatly across applications, though four common patterns are enough to cover them. Out of the applications we study, 32\% of applications are T-or-F, 23\% of them fall into the pattern of M-to-N-set, 8\% of them are M-to-N-set, and the rest of them are Top-label.
% \jc{a few words on this}
\end{packeditemize}



% \mypara{An empirical study over real MLaaS applications}
% % Given the rich syntax that can be expressed by Python, critical errors for applications in the wild can be very different.
% % To understand common types of software context that affect the application decisions, we first perform 
% To this end, in the remainder of this section, we run an empirical study over 78 open-source applications  whose application decisions 
% % control flow decisions 
% which collectively use \fillme ML APIs.
% These applications are from a recently published benchmark suite~\cite{wan2021machine}~\footnote{
% We ignore applications that directly print out the ML API outputs or store these outputs without post-processing, and thus by definition any errors of API output will be critical.
% % The tasks that these applications perform are the same as the task of ML API. Therefore, there is no need to adapt APIs to software. 
% }. 
% These applications cover a wide range of use cases, from \fillme to \fillme. 



% % Google (benchmark, search), AWS (search)

% % \begin{definition}[Application decision]\label{def:app_decision}
        
% % \end{definition}

% % These applications compare the ML API's output classes with the applications' pre-defined lists of classes, and decide which if-branch edge to execute. We refer to this process as making \textit{application decisions} and the pre-defined lists of class as \wls. 



% % \shan{Without knowing your application selection criteria, I cannot interpret what this ``48\%'' implies. What does the remaining 52\% applications do? If all applications in your bencharmk suite use ML API output to affect control flow, how can there be no whitelist? Can you offer more explanation here about what exactly this 48\% mean?} \yh{Sorry 48\% was an out-dated number. All the 40 apps whose control flow are affected by the ML APIs' outputs do specify whitelists. }

% % The application goes through a list of conditional branches based on API outputs, whether a branch is executed is determined by if the API outputs matches with the branch condition or not 

% % \yh{use sentiment analysis, the way to map conditional branch to app decisions is different }


% % The application defines three \wls, \code{Recycle, Compost, Donate}. 
% % The human labeled ground-truth of the input image is ``Shirt'', so the ground-truth decision is executing the if-branch edge \code{return donate(trash\_image)}, which we refer to as selecting the \code{Donate} whitelist. 
% % Furthermore, if the ML API's outputs lead the application to make the decision of executing the code \code{return "It is others." }, such as outputting class ``Dog'', we refer to this decision as selecting \code{others}. 

% % We refer to this executed branch as \emph{if/then branch}. Correspondingly, we refer to another branch that  not executes Line 8 as \emph{if/else branch}\shan{what if there is if-elsif-then?}.
% % We refer to a list of classes (or classification categories) defined in the code\shan{what labels? you mean outputs of an ML API?} leading to the same control flow decision as a \emph{whitelist}. \code{Recycle}, \code{Compost}, and \code{Donate} are the three whitelists, taking Heapsortcypher as an example
% \shan{This definition has a lot of flaws.
% One quick question: based on your definition, aren't all labels minus those in Recycle, Compost, and Donate also a white list? Are they?
% }

% % \cc{yuhan, please put terminologies (those used in Section 3) here. Make sure that you are only using the Heapsortcypher as an example}

% % While these applications typically use \wls to post-process ML API results, they vary in the way of using whitelists to make application decisions. Even with the same whitelists and API outputs, the applications would behave differently according to their code structure. Next, we will introduce the common patterns observed in the studied applications.

% % We find that the common software context consists of two components: (1) Types of branch conditions (\eg checking if the API output belongs to a list of classes), details described in Section~\ref{sec:content}; (2) The organization of conditional branches, details in Section~\ref{sec:org}. 




% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% sentiment_text = types.Document(content = a_piece_of_text)
% annotations = client.analyze_sentiment(document=sentiment_text)
% sentiment_score = annotations.document_sentiment.score
% if sentiment_score < 0.3:
%     print("It's a negative sentence!")
% elif sentiment_score > 0.6:
%     print("It's a positive sentence!")
% else:
%     print("It's a neutral sentence!")
% \end{lstlisting}
%     \caption{The code snippet in the app \code{FoodDelivery}~\cite{food-delivery} calls Google's analyze\_sentiment API to determine the sentiment of a given text.}
%     \label{fig:sentiment}
% \end{figure}


% \subsection{Types of the branch conditions}
% \label{sec:content}
% % \yh{2.1 => what does the context entail, 2.2 and 2.3, differs from ...., but follows a set of common structure, not arbitrary }

% Our study reveals two types of conditional branches, comparing the API outputs with lists of classes, or setting ranges to branch the API outputs. 

% \subsubsection{Lists of classes} 


% % \begin{figure}
% %      \includegraphics[width=.8\linewidth]{figs/stats.pdf}
% %     \caption{ The number of classes included in the lists used to make application decisions. }
% % \label{fig:stats}
% % \end{figure}


% The Applications calling APIs that output categorical results (\eg image classification) 
% pre-define lists of classes, and compare the API outputs with the lists, to make the application decision. For example, the branch conditions in the \code{Heapsortcypher} application check if the API output class belongs to one of the three pre-defined lists. We observe that the lists the applications define typically cover only a very small subset of whole label set. In Figure~\ref{fig:stats}, we summarized the number of classes included in the lists used to make application decisions in our study. Out of the 9605 \yh{double check this number} classes that are covered in Google's classification API, the lists of classes used by the applications to make decisions include less than 20 classes.

% Since the ML API  is typically optimized on a much wider range of classes, the focus on the small subsets classes defined by the applications indicates great room for improvement on the ML API. 


% \subsubsection{Setting ranges}

% Some  applications  call APIs that output floating point values. As shown in the \code{Cloud-computing} application in Figure~\ref{fig:sentiment}, it calls Google's \code{analyze\_sentiment} API to output a score indicating the emotional opinion of the input text, where a score closer to 1 indicates the text is more positive, and a score closer to -1 is more negative. In this case, the  branch condition is checking if the predicted score falls into a specific range. 



% \subsection{How the branch conditions are organized}
% \label{sec:org}

% % \yh{Can those branch conditions directly determine how the application decisions, how the branches are structured => affects the critical errors}
% % \yh{Bad news: there's no one structure, good news: a handful of structures }
% A thoughtful reader may wonder: Does identifying the content of the branch conditions enough to determine the application decisions?


% % Can the branch conditions themselves enough to  determine the application decisions? 

% The answer is no. Our study reveals that even when the content of the branch conditions are the same (\ie defining the same lists of classes as branch conditions), the application decision may still be different based on how the  branch conditions are organized 

% Fortunately, we can classify different organization of branch conditions into a handful of categories. To illustrate the different ways the organization of conditional branches affects the application decision, we begin with defining three key abstractions.


% \subsubsection{Key Abstractions}
% \label{sec:abstractions}
% As summarized in Figure~\ref{fig:hierarchy} we define three types of abstractions to characterize the code structure. 


% \textbf{1) Number of branch conditions } The applications may define one or several branch conditions. If the applications only define one branch condition, whether to execute the branch or not only depends on if API outputs fulfill the only branch condition or not. On the other hand, for applications that define several branch conditions, the application decisions are also affected by other aspects. 
% % The software may specify one or several \wls candidates. Each \wl candidate is related to a particular software branch: the software will execute the corresponding \ift when the ML APIs' outputs intersect with the labels in the \wls candidates. In the rest of the paper, we will refer to executing the \ift as selecting its associated \wl.

% \textbf{2) Number of executed target-paths} Applications that define more than one branch condition can either (1) execute at most one branch; (2) execute the set of branches that fulfill 
%  their branch conditions. 



% \textbf{3) Order of examination}  Applications that execute at most one branch define a two-level nested loop to determine the branch to execute. The applications may iterate through branch conditions in the outer loop or the API outputs in the outer loop. 
% % For the software specifying multiple \wls, the order of examining intersections between \wls and ML API outputs determines software behavior. If we reconstruct the examination into a two-level nested loop that iterates through \wls and API outputs, there naturally arises two types of loop structure: prioritize the specified \wls or the API output labels.


% \begin{figure}
%      \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
%     \caption{Abstractions that characterize the code structure. The decision nodes (in blue) are abstractions defined in Section~\ref{sec:abstractions}. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
% \label{fig:hierarchy}
% \end{figure}



% \subsubsection{Common branch condition structures}
% \label{sec:examples}

% Based on these three types of abstractions, we can classify the common code structures into four categories shown in Figure~\ref{fig:hierarchy}. Each decision node represents an abstraction. Each leaf node represents a structure of branch conditions constructed with the sequences of different decisions made at each decision node. 

% In the following section, we explain the common branch condition structures with simple code snippets. 

% \subsubsection{Branch condition structure 1: T-or-F} The applications with this pattern only specifies one branch condition on the API outputs. Around 32\% of applications in our benchmark suite belong to this category.

% As shown in Figure~\ref{fig:code}(a), the application defines one branch condition to check if the API output belongs to the pre-defined list \code{A}. 

% \textbf{Input example} In this application pattern, given inputs with ground-truth decision of executing the \code{A} branch, the critical error is failing to include any of classes in \code{A} in API outputs.


% \subsubsection{Branch condition structure 2: M-to-N-set} 
% \label{sec:m_to_n}
% In our benchmark, 23\% applications define several branch conditions, and execute the set of branches whose branch conditions are fulfilled based on API outputs. 

% As shown in Figure~\ref{fig:code}(b), the application iterates over the API outputs with a for loop. Inside the for loop, two branch conditions are defined to check if the API output belongs to the lists \code{A} or \code{B}. If the API output belongs to the list \code{A}, the branch \code{final\_output.add("branch 1")} is executed. If the API output belongs to the list \code{B}, the branch \code{final\_output.add("branch 2")} is executed. 

% \textbf{Input example} In this case, given an input  whose ground-truth is \code{c1}, the ground-truth decision is only executing the branch \code{final\_output.add("branch 1")}. When the API outputs \code{[c3, c1]}, both \code{final\_output.add("branch 1")} and \code{final\_output.add("branch 2")} are executed. This output forms a critical error in M-to-N-set. 



% % defines two \wls, \code{A} and \code{B}, and iterates through the ML API's outputs, and adds the string \code{"branch 1"} to the final output set if the outputs intersect with the whitelist \code{A}, and adds the string \code{"branch 2"} to the final output set if the outputs intersect with the whitelist \code{B}. 

% % In this pattern, mis-classifications inside \ do not matter, as long as the ML API's output classes include at least one class in the \wls that should be selected in the ground-truth decision, and not include any class in the \wls that are not in ground-truth decision. 

% % \yh{
% % Given the ground-truth is [Bread, Cheese]

% % Critical errors: failed to include any class in Grainfoods and Proteinfoods, and including any one class in fruitfoods

% % }


% \subsubsection{Branch condition structure 3: Priority-list}
% \label{sec:priority}Around 8\% software defines multiple branch conditions, and check the branch conditions one-by-one until the API outputs fulfill the condition. If none of the conditions are fulfilled, the branch \code{return ``branch 3''} is executed. 

% For example, in Figure~\ref{fig:code}(c), the application defines two lists of classes,  \code{A} and \code{B}, and iterates over the two lists. If any of the API outputs belongs to \code{A}, the application makes the decision of executing the branch \code{return "branch 1"}. If not, the application checks if the API outputs intersect with \code{B}. If the API outputs do not intersect with either \code{A} or \code{B}, the branch \code{return "branch 3"} is then executed. 

% \textbf{Input example} With the same example discussed in Section~\ref{sec:m_to_n}, given an input with ground-truth \code{c1}, the ground-truth decision is executing the branch \code{return "branch 1"}. However, when the API outputs \code{[c3, c1]}, only the branch  \code{return "branch 1"} is executed because the API outputs intersect with \code{A}. This API output, thus do not lead to a critical error for Priority-list. 


% % For example, in Figure~\ref{fig:code}(c), the application defines two \wls, \code{A} and \code{B}, and \code{A} has higher priority than \code{B}. The application uses a nested loop that first iterates through the \wls, and then the output classes. The three possible decisions this application may make are: (1) selecting whitelist \code{A} if the ML API's outputs intersect with \code{A}; (2) selecting whitelist \code{B} if the ML API's outputs do not intersect with \code{A} and intersects with \code{B}; (3) selecting \code{others} if the ML API's outputs do not intersect with either \code{A} or \code{B}.

% % In this pattern, mis-classifications within the for labels inside any of the lower-ranked \wl will not lead to wrong application decisions if ML API correctly recognizes the existence of classes in the higher-ranked \wls. 

% % \yh{
% % Given the ground truth is [Building]

% % critical errors: including any class in monument 

% % }



% \subsubsection{Branch condition structure 4: Top-label}
% \label{sec:top_label}
% Applications that belong to this pattern make decisions by checking the ML API's output classes one by one until finding the first class that fulfills a branch condition. \shan{???In pattern 3, software maps ... ``in a specific order'' as well.}. Around 37\% of applications fall into this category.

% For example, as shown in Figure~\ref{fig:code}(d), the  application defines two lists of classes, and iterates over API outputs. If the first output, \code{x1}, belongs to any of the lists, the corresponding branch will be executed. If not, the application checks if the second output, \code{x2}, matches any one of the two lists or not. If none of the API outputs matches the two lists, the branch will be executed. 

% \textbf{Input example} With the same example discussed in Section~\ref{sec:priority}, different from Priority-list, the API outputs \code{[c3, c1]} lead the execution of the branch \code{return "branch 2"}.  This API output, thus incurs a critical error for Top-label. 

% %  the application defines two \wls, \code{A} and \code{B}. The application defines a nested for loop that first iterates through the output classes (\ie [\code{x1}, \code{x2}]), and then the \wls. If \code{x1} intersects with any of the \wls, the application selects the corresponding one. If \code{x1} does not match with any of the \wls, then the application checks if \code{x2} belongs to any of the \wls. Otherwise, it selects \code{others}. 

% % In this pattern, mis-classifications for classes ranked lower in the ML API's outputs do not matter, as long as the classes that rank higher leads to correct application decisions. 

% % \yh{Pie chart showing some statistics  }

% \subsubsection{Summary}

% In short, in these different structures of branch conditions, even when the branch conditions are the same (\eg checking if the API outputs interest with lists of classes), the same API outputs can lead to different application decisions. As a result, the patterns of critical errors can be very different for these different structures. 

% Although we use examples whose branch conditions are lists of classes, applications whose branch conditions are based on the range of the output scores also fall in the branch condition structures described in Section~\ref{sec:priority} or Section~\ref{sec:top_label}. 
% % \shan{What is the F1 score drop for this category?}

% \subsection{Summary of findings}

% To summarize, the real applications covered in our study reveal that there is a rich set of \emph{software context}. This motivates the need for customizing the ML API to incorporate the different \emph{software context}. 

% Luckily, although there is a rich set of \emph{software context}, the context is \emph{not} arbitrary. We can express the context in a format that combines the content and the structure of the branch condition, which can be extracted from the applications' source code.  
% % \yh{\textbf{Why we need to customize}}



% % \begin{figure}
% % \begin{subfigure}{0.45\textwidth}    
% %     \centering
% % \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % Dog = ['Dog','Mammal','Carnivore','Wolf']
% % image = types.Image(content=dog_image)
% % response = client.label_detection(image=image)
% % for obj in response.label_annotations:
% %   if obj.name in Dog:
% %     return 'It is a animal.'
% % return 'It belongs to others.'
% % \end{lstlisting}
% %     \caption{Code pattern: T-or-F. }
% %     \label{fig:app_example_level1}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_tf_wrong.pdf}
% %     \caption{Failing recognize the carnivore leads to software failure. }
% %     \label{fig:input_example_tf_wrong}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/app_input_example_level1.pdf}
% %     \caption{Mis-classifying a dog as wolf does not trigger software failure. }
% %     \label{fig:input_example_tf_correct}
% % \end{subfigure}
% % \caption{Dogecoin~\cite{food}, an application that classifies carnivore images.  }
% % \label{fig:tf_example}
% % \end{figure}



% % \begin{figure}
% % \begin{subfigure}{0.45\textwidth}    

% %     \centering
% %              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % proteinfoods = ['Hamburger', 'Meat', 'Patty']
% % fruitfoods = ['Apple', 'Fruit', 'Orange']
% % grainfoods = ['Noodle', 'Pasta', 'Al dente']
% % image = types.Image(content=trash_image)
% % response = client.label_detection(image=image)
% % protein, fruit, grain = False, False, False
% % for obj in response.label_annotations:
% %   if obj.name in proteinfoods:
% %     protein = True
% %   if obj.name in fruitfoods:
% %     fruit = True
% %   if obj.name in grainfoods:
% %     grain = True
% % RENDER_TEMPLATE(protein, fruit, grain)
% % \end{lstlisting}
% %     \caption{Software implementation. }
% %     \label{fig:app_example_non_mut}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_mton_wrong.pdf}
% %     \caption{Failing to recognize ``Cheese'' leads to software mis-behavior. }
% %     \label{fig:input_example_mton_wrong}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_mton_correct.pdf}
% %     \caption{Mis-classifying ``Pasta'' to ``Noodle'' still leads to correct software behavior. }
% %     \label{fig:input_example_mton_correct}
% % \end{subfigure}
% % \caption{Food classifier~\cite{food}, an application that classifies food images.}
% % \end{figure}


% % \begin{figure}
% %     \centering
% %              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % proteinfoods = ['Hamburger', 'Meat', 'Patty']
% % fruitfoods = ['Apple', 'Fruit', 'Orange']
% % grainfoods = ['Noodle', 'Pasta', 'Al dente']
% % image = types.Image(content=trash_image)
% % response = client.label_detection(image=image)
% % food_list = []
% % for obj in response.label_annotations:
% %   if obj.name in proteinfoods:
% %     food_list.append('protein')
% %   if obj.name in fruitfoods:
% %     food_list.append('fruit')
% %   if obj.name in grainfoods:
% %     food_list.append('grain')
% % return food_list
% % \end{lstlisting}
% %     \caption{An example software that maps original output labels of the ML APIs to a list of \wls.  }
% %     \label{fig:app_example_non_mut}
% % \end{figure}



% % \begin{figure}
% % \begin{subfigure}{0.45\textwidth}
% %         \centering
% %              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % Monument = ['Landmark', 'Sculpture', 'Monument']
% % Construction = ['Building', 'Estate', 'Mansion']
% % Person = ['Human','Person',  'Lady']
% % image = types.Image(content=landmark_image)
% % response = client.label_detection(image=image)
% % Predictions = []
% % for obj in response.label_annotations:
% %   Predictions.append(obj.name)
% % if any([label in Monument for label in Predictions]):
% %   return 'It belongs to monument.'
% % elif any([label in Construction for label in Predictions]):
% %   return 'It is construction.'
% % elif any([label in Person for label in Predictions]):
% %   return 'It is person.'
% % \end{lstlisting}
% %     \caption{Software implementation. }
% %     \label{fig:app_example_priority}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_priority_wrong.pdf}
% %     \caption{Missing a label ``Landmark'' leads to software mis-behavior. }
% %     \label{fig:input_example_priority_wrong}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_priority_correct.pdf}
% %     \caption{Recognizing an extra wrong label ``Mansion'' still leads to correct software behavior. }
% % \label{fig:input_example_priority_correct}
% % \end{subfigure}
% % \caption{Aander-ETL~\cite{etl}, an application that classifies landmark images.  }
% % \label{fig:priority_input_example}
% % \end{figure}

% % \cc{Do we want to introduce the accuracy difference between API and software? And the room for improvement?}

==> bk/backups_before_fist_submission/3-1-old.tex <==
\label{sec:method}

Inspired by the empirical study of \S\ref{sec:empirical}, this section presents \tool, an optimized MLaaS backend that customizes ML models for the decision processes of different applications.

\subsection{Key components and workflow}
\label{sec:overall}
\begin{figure}
     \includegraphics[width=\linewidth]{figs/system_overview.pdf}
    \caption{System architecture of \tool. 
    % \jc{the overall flow looks ok, but there are so many minor issues in this figure. just to name a few: 
    % (1) where is "cloud service" coming from? 
    % (2) (a) and (b) shouldn't be distinguished (see comment in 3.1).
    % (3) i thought we decided to drop the arrow of giving the parser to developer?
    % (4) why "software context" is still used?
    % (5) user is not running python code! they run real apps
    % (6) why calling it "prediction" instead of API output?
    % (7) what's "model inference code"? if it's simply selecting the right model to run, we shouldn't introduce a new term.
    % (8) the three customized models should be put side by side (either all vertically or horizontally),
    % (9) why calling them "adapted" ML model? if the term we always use is "customized", then stick to that.}
    % \jc{in general, EVERY word must be picked very carefully, which you clearly didn't do :)}
    % \yh{fixed comments, I'm calling it ML model outputs instead of API outputs because the outputs comes before the ``output interface'', thus it's not API outputs yet}
    % \jc{sorry i disagree. again, don't introduce new terms unless really necessary, which i don't think is the case. why dont you change the figure, to move the output and input the left of the model output interface, which should also be changed to "ML API"?}
    % \jc{and don't let arrows overlap with arrows or lines (e.g., Model pool, Select)}
    }
\label{fig:system}
\end{figure}
% \mypara{Main components}

% \mypara{Extracted application's decision process}
% the application's decision process of the applications querying the MLaaS, and customizes the ML model in the MLaaS backend.
% summarizes the overall workflow of \tool.


\mypara{Workflow}
Figure~\ref{fig:system} depicts \tool's high-level workflow. 
When developers publish an application (\App), they first run a parser script provided by \tool on \App's source code to extract its {\em \summary} (explained shortly) and then upload the summary to \tool's MLaaS backend (details in \S\ref{sec:extract}). 
The backend uses the received \summary to construct a new loss function, such that when the ML model is re-trained using the new loss function, it will produce inference results that yield fewer application decision failures for the application \App (details in \S\ref{sec:loss}).
\tool then adds the new ML model to a pool of customized ML models. 
% \jc{the last phrase can be deleted}
When a user of application \App queries \tool's MLaaS backend with an input via the existing ML API, the backend will select the ML model customized for \App and return the inference result of the selected ML model (details in \S\ref{sec:runtime}).


\begin{comment}
When the application is being developed, 
% \jc{the term offline is new. the contrast between offline and online is overcomplicating. can we say something like when the application is being developed?}
besides the existing development procedure, the developers also run an MLaaS-provided parser plugin on their own machines, 
% \jc{the ``parser'' comes from nowhere. who provides it? even a simple ``MLaaS-provided parser'' is better}
% \jc{``locally'' has many meanings. pick a more precise term}, 
which extracts a summary of the application's decision process
% \jc{maybe we need a different term; ``key features'' invites unnecessary confusion when used in an ML-related paper. how about a ``summary of the application's decision process''?}
% \jc{``extracts xxx from app into a file'' sounds wrong. shouldn't it be ``extract xxx from an app and uploads it as a file to xxx''?} 
from the application source code (details in \S\ref{sec:extract}), and uploads it as a file to the MLaaS backend. 
\end{comment}




% \jc{the separation among the three stages (``developer'', ``re-training'' and ``run-time'') is unnecessarily complicating the flow, and it introduces unnecessary terms, like ``run-time''. }

% \jc{when introducing the flow, shouldn't we also highlight what we DO change and what we do NOT change?}

% The application's decision process extracted from the Python source code, is composed of the key features characterizing it.\cc{This sentence does not provide additional information. Also, we could mention python in the implementation section} 

% \jc{please don't explain a concept together with an application. you should always explain the concept first, and THEN use an example to explain it in a specific context.}

\smallskip
\noindent
The {\bf \summary} extracted from an application includes three pieces of information: 
\begin{packeditemize}
\item the values (either the labels or the value range) included in each target class; 
\item the type of decision (\ie \term{True-False}, \term{Multi-Choice}, or \term{Multi-Select});
\item the mapping order over the target classes (\ie \term{API-output order} or \term{application-choice order}) 
% (\jc{yuhan, what's the possibilities?})
, if the application makes a \term{Multi-Choice} decision.
\end{packeditemize}
% vary greatly across applications, 
% provides us with great opportunities to customize the ML models per application. 
For a concrete example, the \summary of the garbage classification application (Figure~\ref{fig:code}(a)) contains
(1) the three target classes (each being a list of labels): \code{Recycle}, \code{Compost}, and \code{Donate}; (2) the \term{Multi-Choice} type of decision; and 
(3) it follows the \term{API-output order} to reach the \term{Multi-Choice} decision.  

These three pieces of information uniquely describe which errors are critical and which are non-critical to the application, and they will be used to customize the ML model for the application, as elaborated in \S\ref{sec:loss}. 


\mypara{What is changed by \tool, what is not}
It is important to notice that \tool does {\em not} change the ML API or the source code or the executable of the application.
% \jc{check the term with shan/chengcheng}
That said, \tool does change two things. 
First, the application developers need to run \tool's parser script to extract the \summary.
Second, \tool modifies the MLaaS backend to re-train an ML model per application (instead of serving the same model to all applications) and selects the right ML model to serve each query.
\S\ref{sec:extract} and \ref{sec:runtime} will explain why these changes are practical.
% When the application queries the MLaaS, 
% a model selector module is added in the backend to choose the ML model customized to the application, based on the application ID incorporated in the identification credential.

% \jc{this last sentence is important but quite misleading. first of all, these features don't uniquely describe a decision process (e.g., they dont say what decisions will be made for each branch). instead, they specify what errors are critical and what errors are not critical.
% second, you didn't say WHY they SHOULD be used by \tool to customize the ML model.}


\begin{comment}
\jc{this definition is extremely important and should be elevated. i suggest explain it in a separate paragraph. so you will have two paragraphs: one explain the overall workflow, and the second explains what's extracted from the source code and used to customize ML model. it's important to keep the 1st para short.} 
\jc{it should be explained more formally, probably with a simple example, and the terms (e.g., multi-select vs. multi-choice) should be tightly connected to when they are first defined. remember, many reviewers may have skipped (or missed) their definitions in section 2.} 
\jc{moreover, i wouldn't mention JSON at the beginning. the exact format (not the content in the file) seems secondary to me}
\jc{what about score ranges? we need a way to explain all cases under consideration} 
% used in branch conditions; (2) whether the application is making multi-select or multi-choice decisions; (3) the order of examination for applications making multi-choice decisions. Then, the developers will upload the JSON of application's decision process to the MLaaS backend. On the MLaaS backend side, \tool will re-train the ML model by re-sampling the training data with a more focus on the classes appeared in the applications, and constucting loss functions which directly penalize the critical errors.
\jc{i wouldn't distinguish training data resampling and loss function as two separate steps. last time we met as a group, we decided to say changing loss function is all that's needed, though the real implementation does resampling to speedup training. i like this idea, so the distinction should be secondary.} 

\jc{regarding the terminology, the parser doesn't extract the entire application decision process, it merely extracts the key features of the application decision process, which include xxx}



\jc{now this is too low-level when explaining the workflow. here, you can just say ``each time an application calls the ML API, the ML API backend will select the ML model model customized for the application, ...''}
% the applications submit inference request to the ML API with input and the credential, like 

\jc{two meta comments: 1. Yuhan, you should read the terms used in the new Section 2 and use them consistently in section 3.
2. when writing 3.1, please make sure that every important term appears with a forward pointer to a later subsection that explains it in detail as well as a pointer to Figure 4}
\end{comment}

% which consists of a parser plugin, an ML model re-training scheme run in the offline stage, and in the online stage, \tool selects the customized ML model based on applications' credentials, and run inference with the customized model.  


% 3.2: given the extracted json, how should we re-train teh model 
% 3.3. how to extract
% 3.4: how to change the run-time interface

% \tool is an automated framework that adapts the ML model behind the ML APIs, such that the number of software mis-behaviors can be greatly reduced when applied to an ML software. 

% \tool first performs static analysis to extract the code structure of the applications invoking MLaaS to understand how the software uses the ML API outputs to make application decisions. Then \tool constructs loss functions that penalize the critical errors of the applications. Finally, \tool re-trains the ML models behind the ML APIs with the constructed loss function, without modifying the output interface of the ML APIs. 

% In this section, we will introduce how \tool performs static analysis and constructs the loss functions for the applications. 


% \subsection{Understanding Software Context}

% \subsection{Notations}
% \yh{not 3.2 }
% Denote the total number of classes that the ML model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows:

% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the DNN behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}

The remaining of the section will first describe the key module of ML-model customization, then how to extract the \summary, and finally, how the customized ML models are used to serve ML API queries in runtime.

% \subsection{How to customize the ML model in the MLaaS backend}
\subsection{Customizing ML models per application}
\label{sec:loss}
% As introduced in \S\ref{sec:empirical},  applications in the wild differ greatly in their application's decision processes. 
% % For example, they may  define different number of target classes or include only a small subset of labels of the whole label set in their target classes and so on. 
% This heterogeneity can lead to differences in critical errors\jc{remind people what critical errors are?} across applications. 
% It is possible for an ML API error to be non-critical for one application, while critical for another. Thus, customizing the DNN in the MLaaS backend is important in order to incorporate the differences in application's decision processes across applications.
% \jc{the whole first paragraph is redundant to 3.1. this para should highlight why we start by explaining the step of DNN re-training}

% Model re-training has been widely adopted in ML to update the generic pre-trained ML models to work for related but different tasks~\cite{mullapudi2019online,ekya}. In model re-training, the model is initialized from a pre-trained model, and  its model parameters are updated based on the goal of the new task.



\begin{comment}

The idea of model re-training has been widely adopted in ML to update the generic pre-trained ML models to work for related but different tasks~\cite{mullapudi2019online,ekya}. The key challenge is how to formulate the customized optimization goal and design re-training strategy to efficiently achieve high  accuracy on different tasks.
\shan{Reading this sentence, as a picky reviewer, I would start worrying about the novelty of this work over model re-training work. The next sentence ``In our problem setting'' reads quite similar to the previous sentences. Is it possible to rephrase so that the difference is more obvious?}  \cc{Done. I feel the last sentence actually do not provide new information. So I deleted it.}
% In our problem setting, we want to initialize from a pre-trained model for the original ML task (\eg image or text classification), and re-train it with our customization goal.  
\end{comment}

\mypara{Customization goal}
With a given \summary (explained in \S\ref{sec:overall}), our goal is to train an ML model whose output minimizes application-decision failures (\ie critical errors), rather than {\em any} misprediction/misclassification of API outputs.
% by incorporating the multiple aspects of each decision process (\S\ref{sec:observations}) that affect critical and non-critical errors.
To formally describe this objective,
% Our {\bf customization goal} is to minimize the critical errors for each application.
% caused by ML API errors. 
we denote how an application makes a decision by $\z = \APIcomp(\DNN(\x))$, where $\x$ is the input to the ML API, 
$\DNN(x)$ is the inference result of backend DNN. 
Note that the output of the ML API is the result after the MLaaS backend post-processes $\DNN(x)$, denoted as $\Filter(\DNN(x))$ (\eg filtering out 
 labels with confidence scores lower than the detection threshold $\theta$).
 $\Appdecision(\cdot)$ is the application's decision making process based on the ML-API output.

% MLaaS backend also post-processes $\DNN(x)$ before returning it to the application

% $\API(\x)$ is the inference result of backend DNN (ML API output), 
% $App(\cdot)$ is the decision process the application performs based on an output of the ML API. 



For a given process of $\APIcomp(\cdot)$ and input set $\X$, we want to model $\DNN(\cdot)$ such that
% Let $\x_i\in \X$ denote the $i^{th}$ input to the ML API, and $\hat{y_i}$ denote its ground-truth label. 
% $API(x_i)$ is a list of probabilities for label-based API (\eg image or text classification), 
% [$p_1, p_2, \dots, p_n$], for every label in the whole label set, and a score $O_i$ for score-based API (\eg sentiment analysis API). 
% Formally, our customization goal is written as:
% Let $\mathds{1}_{x}$ denote the indicator function, where $\mathds{1}_{x} = 1$ when $x$ is \emph{True} and 0 otherwise. Therefore, the customization goal is:
\begin{equation}
    \min \left|\{\x_\InputId \in \X \textrm{ s.t. } \APIcomp(\DNN(\x_\InputId)) \neq \APIcomp(\hat{\y_\InputId})\}\right|
    \label{eq:goal}
\end{equation}
\noindent
where $\hat{\y_\InputId}$ is the ground truth of input $\x_\InputId$. 
Note that in this section, we treat the processes of  $\APIcomp(\cdot)$ as a whole, because it would not change no matter how the backend DNN changes, and refer to as the \emph{decision process}(\ie $\Decision(\cdot)$). 




\tool minimizes Eq~\ref{eq:goal} by training a DNN model with a {\em new loss function}.\footnote{A careful reader might notice that the formulation in Eq.~\ref{eq:goal} also depends on the input set $\X$.
Though the input set should ideally follow the same distribution of real user inputs of the application, this distribution is hard to obtain in advance and may also vary over time and across users.
Instead, we focus our discussion on training the ML model to minimize Eq.~\ref{eq:goal} with an assumed input distribution. (Our evaluation (\S\ref{sec:evaluation}) will test the resulting model's performance over different input distributions.)}
This way, we do not need to modify the DNN model or the training process, except using a different loss function.
% It is true that a full solution will need to choose the input set $\X$, in addition to optimizing Eq.~\ref{eq:goal}.
We should note that unlike recent work that aims to shrink or speedup DNNs~\cite{mullapudi2019online,??,??}, we do not change the architecture (shape and input/output interface) of the DNN run by MLaaS; 
instead, we improve the DNN's output such that it minimizes application-decision failures.
% So \emph{how to design a loss function that can achieve our customization goal?}

% A common practice in ML is to utilize the loss function to express the optimization goal~\cite{celoss}. For example, the Binary Cross Entropy loss is used in image or text classification tasks, and Mean Squared Error loss is used in regression tasks. 

% Take classification task as an example, the Binary Cross Entropy loss is defined as:

% \begin{equation}
%     L_{BCE}(y_i) = \sum_{j=1}^{n} -\hat{y_{i, j}} \cdot log(y_{i,j}) - (1-\hat{y_{i,j}}) \cdot log(1-y_{i,j})
%     \label{eq:bce}
% \end{equation}
% where $y_i$ is the output of the ML model on the $i^{th}$ input, which is a list of probabilities. The higher the probability at the $j^{th}$ index is, the more confident the model is about the existence of the $j^{th}$ label in the input.  $\hat{y_i}$ is the ground truth for the $i^{th}$ input. $\hat{y_{i,j}} = 1$ if the $j^{th}$ label is in the ground truth of the $i^{th}$ input. Intuitively, this loss function incurs a high penalty when the $j^{th}$ label is present in the ground truth, but the model outputs a low probability for it, and vice versa. 




==> bk/backups_before_fist_submission/3-2-new.tex <==
\newpage



In contrast, \tool's loss function only penalizes critical errors specific to each application's decision process, rather than all errors in the DNN output. 
At a high level, our loss function converts the logic of an application's decision process to a differentiable form that penalizes critical errors (which cause different decisions than the correct ones).


\mypara{A generic description of decision processes}
Since the decision processes vary greatly across applications (\S\ref{subsec:observations}), we first introduce how \tool conceptually captures a range of decision processes and their critical errors using a generic description, which allows us to derive the mathematical form of \tool's loss function for individual applications.
For each of these applications in our study (\S\ref{sec:methodology}), our insight is that its decision process can be viewed as traversing a sequence of conditional {\em checks} until a {\em break} occurs, as follows. 
\vspace{-0.2cm}
\begin{align*}
\textrm{The }1^{st}\textrm{ check:} &<\y^{(1)},\ClassId^{(1)}>\rightarrow<\Match^{(1)},\BeforeBreak^{(1)}>&\\
&\dots&\\
\textrm{The }\TraverseId^{th}\textrm{ check:} &<\y^{(\TraverseId)},\ClassId^{(\TraverseId)}>\rightarrow<\Match^{(\TraverseId)},\BeforeBreak^{(
\TraverseId)}>& \Leftarrow \textrm{break}\\
&\dots&
\vspace{-0.2cm}
\end{align*}
where the $\TraverseId$-th conditional check takes as input a score vector $\y^{(\TraverseId)}$ (which is typically a masked vector of DNN output $\y$ with only score of certain label left) and one of \targets $\ClassId^{(\TraverseId)}$, and returns a binary $\Match^{(\TraverseId)}$ indicating whether $\y^{(\TraverseId)}$ {\em matches} the condition of $\ClassId^{(\TraverseId)}$ and a binary $\BeforeBreak^{(\TraverseId)}$ indicating whether this check happens before the break.
The set of \targets of checks with $\Match^{(\TraverseId)}=True$ before the break will be the decision.
Figure~\ref{??} shows a concrete example of such generic description for a particular decision process and DNN output.

The specifics of this generic description (the score used in each conditional check, the traversal order of the checks, and when the break occurs) depend on the given decision process as well as the DNN output $\y$. 
We stress that this generic description may {\em not} apply to all applications, but it does apply to all applications in our study (\S\ref{sec:methodology}). 


\mypara{Types of critical errors}
This generic description  nevertheless suffices to categorize critical errors:
\begin{packeditemize}
\item {\em Type-1 Critical Errors:} A correct \target $\ClassId$ first matched only after the break.
\item {\em Type-2 Critical Errors:} A correct \target $\ClassId$ is never matched, before or after the break.
\item {\em Type-3 Critical Errors:} An incorrect \target $\ClassId$ is matched before break. 
\end{packeditemize}


% \begin{packeditemize}
% \item {\em Type-1 Critical Errors:} A correct \target $\ClassId$ is never traversed in any conditional checks before the break.
% \item {\em Type-2 Critical Errors:} A correct \target $\ClassId$ is traversed 
% before the break, but each time (\eg at the $\TraverseId^{th}$ check) the score vector $\y^{(\TraverseId)}$ used does not match $\ClassId$'s condition.
% \item {\em Type-3 Critical Errors:} An incorrect \target $\ClassId$ is traversed in some check (\eg at the $\TraverseId^{th}$ check) before the break, and the score vector $\y^{(\TraverseId)}$ used match $\ClassId$'s condition.
% \end{packeditemize}


\mypara{\tool's loss function} 
This categorization of critical errors then allows \tool to derive a loss function that penalizes each type of critical errors.
We explain the loss function in the context of ``label-based API, \term{Multi-Choice} type of decision, and \term{app-output order}'' (defined in \S\ref{subsec:observations}), one of the most common types of decision processes in the studied applications. 
\S\ref{sec:loss_appendix} will enumerate other types of decision processes.
The example in Figure~\ref{??} is such an application. 
Mathematically, the loss function is then comprised of three terms, each penalizing one type of critical errors:
{\small
\begin{align}
     L(\y) &=   
 % \overbrace{ \sum_{\ClassId\leq\hat{\ClassId}} \textrm{Sigmoid}\left(\max_{\LabelId\in\TargetSet_{\ClassId}}\y[\LabelId]-\theta\right)}^{\substack{\text{\sf \footnotesize {{\bf Type-1} Critical Errors}} }} +
  \overbrace{ \textrm{Sigmoid}\left(\min\left(\max_{\LabelId \in \cup_{\ClassId < \hat{\ClassId}}\TargetSet_{\ClassId}}\y[\LabelId],\max_{\LabelId\in\TargetSet_{\hat{\ClassId}}}\y[\LabelId]\right)-\theta\right)}^{\substack{\text{\sf \footnotesize {{\bf Type-1} Critical Errors}} }} \label{eq:loss_app} \\&+
 \overbrace{ \textrm{Sigmoid}\left(\theta-\max_{\LabelId\in\TargetSet_{\hat{\ClassId}}}\y[\LabelId]\right)}^{\substack{\text{\sf \footnotesize {{\bf Type-2} Critical Errors}} }} + 
 \overbrace{ \sum_{\ClassId<\hat{\ClassId}}\textrm{Sigmoid}\left(\max_{\LabelId\in\TargetSet_{\ClassId}}\y[\LabelId]-\theta\right)}^{\substack{\text{\sf \footnotesize {{\bf Type-3} Critical Errors}} }}\nonumber
\end{align}
}
Here, $\y[\LabelId]$ denotes the score of the label $\LabelId$, $\TargetSet_\ClassId$ denotes the set of labels in the match condition of \target $\ClassId$, $\hat{\ClassId}$ denotes the correct (\ie ground-truth) \target, and the sigmoid function $\textrm{Sigmoid}(x)=\frac{1}{1+e^{x}}$ will incur a high penalty on positive inputs.

{\em Why do these terms capture the critical errors?} 
Here, we intuitively explain why Eq~\ref{eq:loss_app} captures each type of errors (see \S\ref{sec:loss_appendix} for formal proofs):
% Intuitively (see \S\ref{sec:loss_appendix} for formal proofs), because this is a \term{multi-choice} application (break at the first match) and it goes through labels in \code{detection\_labels} in descending order of their confidence scores, $\MaxScore$ is the score of the first matching label and is also when the break occurs.
\begin{packeditemize}
\item A Type-1 critical error occurs, when two things happen simultaneously: 
(1) the \target $\hat{\ClassId}$ must be matched (\ie $\max_{\LabelId\in\TargetSet_{\hat{\ClassId}}}\y[\LabelId]\geq\theta$) and 
(2) some \target $\ClassId$ before $\hat{\ClassId}$ (\ie $\ClassId<\hat{\ClassId}$) must be matched (\ie for any $\ClassId < \hat{\ClassId}$, $\max_{\LabelId \in \TargetSet_{\ClassId}}\y[\LabelId]\geq\theta$).
The first term of Eq~\ref{eq:loss_app} penalizes any occurrence of these conditions. 
\item A Type-2 critical error occurs, if the no label in the correct \target $\hat{\ClassId}$ has a score high enough for $\hat{\ClassId}$ to be matched, \ie $\max_{\LabelId\in\TargetSet_{\hat{\ClassId}}}\y[\LabelId] < \theta$.
The first term of Eq~\ref{eq:loss_app} penalizes any occurrence of this condition.
\item A Type-3 critical error occurs, if any incorrect \target $\ClassId$ before $\hat{\ClassId}$ (\ie $\ClassId<\hat{\ClassId}$) has a label with score high enough for $\ClassId$ to be matched, \ie $\max_{\LabelId\in\TargetSet_{\ClassId}}\y[\LabelId]-\theta$.
The third term of Eq~\ref{eq:loss_app} penalizes any occurrence of this condition.
\end{packeditemize}






To successfully train a DNN model, the loss function must be differentiable with respect to any DNN ouput. 
% It is important to note that optimizers used in ML(\eg Adam)
% % \jc{you tend to add references on non-essential terms, } 
% to train  models are gradient-based. 
% Thus, the loss function (\ie every function in the composite function) needs to be differentiable in order to calculate the gradient of the loss value with respect to the DNN output. 
Note that in Eq~\ref{eq:loss_app}, the $\max$ function is used at multiple places, but it can be equivalently expressed in a differentiable form (we use the differentiable operators in PyTorch Autograd~\cite{paszke2017automatic}).




\begin{comment}
    


\mypara{\tool's loss function} 
This categorization of critical errors then allows \tool to derive a loss function that penalizes each type of critical errors.
We explain the loss function in the context of ``label-based API, \term{Multi-Choice} type of decision, and \term{API-output order}'' (defined in \S\ref{subsec:observations}), one of the most common types of decision processes in the studied applications. 
\S\ref{sec:loss_appendix} will enumerate other types of decision processes.
% \myparashort{Case study: \term{Multi-Choice API-output order}.}
% These applications take label-based API outputs and make \term{Multi-Choice} decisions in \term{API-output} order (defined in \S\ref{subsec:observations}).
The example in Figure~\ref{??} is such an application. 
On an input image with ground truth of ``\code{Food}'', the correct decision will be \code{\fillme}, and as shown in the figure the generic description will be traversing a sequence of conditional checks until the break occurs. 
Mathematically, the loss function is comprised of three terms, each penalizing one type of critical errors:
% \begin{align}
%      L(\y) &=   \overbrace{ \textrm{Sigmoid} ( \max_{\LabelId \in \bigcup_{\ClassId > \hat{\ClassId}} \TargetSet_{\ClassId}} \y_{\LabelId}
%       - \max_{\LabelId \in \bigcup_{\ClassId} \TargetSet_{\ClassId}} \y_{\LabelId}\  ) 
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-1} Critical Errors}} 
% }} \nonumber \\&+
%  \overbrace{ \textrm{Sigmoid} ( \max_{\LabelId \in \bigcup_{\ClassId} \TargetSet_{\ClassId}} \y_{\LabelId}
%  - \max_{\LabelId \in \TargetSet_{\hat{\ClassId}}} \y_{\LabelId}
%  ) 
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-2} Critical Errors}} 
% }} \nonumber \\&+
% \overbrace{ \sum_{\ClassId \neq \hat{\ClassId}}\textrm{Sigmoid} ( \max_{\LabelId \in \TargetSet_{\ClassId}}  \y_{\LabelId} - \max_{\LabelId \in \bigcup_{\ClassId} \TargetSet_{\ClassId}} \y_{\LabelId} )
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-3} Critical Errors}} 
% }}
% \label{eq:loss_app}
% \end{align}
\begin{align}
     L(\y) =  & 
 \overbrace{ \textrm{S} (\MaxScore - \max_{\LabelId \in \TargetSet_{\hat{\ClassId}}} \y[\LabelId]) }^{\substack{\text{\sf \footnotesize {{\bf Type-1} Critical Errors}} }} +
 \overbrace{ \sum_{\ClassId \neq \hat{\ClassId}}\textrm{S} ( \max_{\LabelId \in \TargetSet_{\ClassId}}  \y[\LabelId] - \MaxScore)}^{\substack{\text{\sf \footnotesize {{\bf Type-2} Critical Errors}} }} \nonumber\\&+
 \overbrace{ \textrm{S} ( \max_{\LabelId \in \bigcup_{\ClassId > \hat{\ClassId}} \TargetSet_{\ClassId}} \y[\LabelId]- \MaxScore)}^{\substack{\text{\sf \footnotesize {{\bf Type-3} Critical Errors}} }}
\label{eq:loss_app}
\end{align}
where $\MaxScore=\max_{\LabelId \in \bigcup_{\ClassId} \TargetSet_{\ClassId}} \y[\LabelId]$, \ie the maximum confidence score in $\y$ of any labels that appear in one of the \targets.
Here, $\y[\LabelId]$ denotes the score of the label $\LabelId$, $\TargetSet_\ClassId$ denotes the set of labels in the match condition of \target $\ClassId$, $\hat{\ClassId}$ denotes the correct (\ie ground-truth) \target, and $\textrm{S}(x)$ is the sigmoid function $\frac{1}{1+e^{x}}$, which will incur a high penalty on positive inputs.

{\em Why these terms capture the critical errors?} Intuitively (see \S\ref{sec:loss_appendix} for formal proofs), because this is a \term{multi-choice} application (break at the first match) and it goes through labels in \code{detection\_labels} in descending order of their confidence scores, $\MaxScore$ is the score of the first matching label and is also when the break occurs.
\begin{packeditemize}
\item A Type-1 critical error occurs, if the score of the first label that could match the correct \target, \ie $\max_{\LabelId \in \TargetSet_{\hat{\ClassId}}} \y[\LabelId]$, is lower than $\MaxScore$, thus happens {\em after} the break. 
\item A Type-2 critical error occurs, if the score of the first label that matches an incorrect \target $\ClassId\neq\hat{\ClassId}$, \ie $\max_{\LabelId \in \TargetSet_{\ClassId}}  \y[\LabelId]$, is higher than $\MaxScore$, thus happens {\em before} the break.
\item In a Type-3 critical error, if the correct \target $\hat{\ClassId}$ is not matched before the break, it must mean that the 
\end{packeditemize}



% In the meantime, if a class $\ClassId$ is traversed before the break, it must either have a label with a score 
% $\MaxScore=\max_{\LabelId \in \bigcup_{\ClassId} \TargetSet_{\ClassId}} \y[\LabelId]$ means , and because the labels in \code{detection\_labels} traversed in descending order of their confidence scores, the first label that matches some \target must have a confidence score $\MaxScore$ in this example application.
% And since it is a \term{multi-choice} application, the break occur right after the first match.

the highest score of any label that could have matched the correct \target appears after the break lower than $\MaxScore$, thus 


\jc{junchen stops edit here}


% \begin{packeditemize}
% \item For a DNN output $\y$ (recall from \S\ref{subsec:observations}, $\y$ is an array of scores), whether the \target $\ClassId$ is matched in $\y$'s application decision depends only on some specific value in $\y$, which we call the {\em effective score} of \target $\ClassId$, $\M_\ClassId(\y)$.
% \item Given the effective score $\M_\ClassId(\y)$ of each \target $\ClassId$, the decision process of an application can be equivalently viewed as traversing the list of the target classes ranked in certain order until it {\em breaks}. 
% \end{packeditemize}
% Figure~\ref{fig:loss} gives a concrete example, but %, and more cases will be discussed shortly.
% the exact order of traversing the \targets and when the traversal breaks depend on the values in $\y$ and the \summary. 




% and is sufficient to derive our new loss function as follows. 
% We first explain its general idea before discussing the new loss function case-by-case.




% \mypara{\tool's loss function}
% Consequently, \tool's loss function penalizes each type of critical errors.
% \begin{align}
% L(\y) &= 
% \overbrace{ \sum_{\substack{\textrm{Target class } \ClassId \textrm{ is correct \&}\\\textrm{ traversed before break}}} ~\textrm{Sigmoid}(\F(\y)- \M_\ClassId(\y))
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-1} Critical Errors}} 
% }} \nonumber \\ &+
% \overbrace{ \sum_{\substack{\textrm{Target class } \ClassId \textrm{ is correct \&}\\\textrm{ ranked after break}}} ~\textrm{Sigmoid}(\G(\y)- \M_\ClassId(\y))
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-2} Critical Errors}} 
% }} \nonumber \\ &+ 
% \overbrace{ \sum_{\substack{\textrm{Target class } \ClassId \textrm{ is incorrect \&}\\\textrm{ traversed before break}}} \textrm{Sigmoid}(\M_\ClassId(\y) - \Q(\y) )
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-3} Critical Errors}} 
% }} \label{eq:loss}
% \end{align}
% where $\F(\y)$, $\G(\y)$ and $\Q(\y)$ are thresholds used to penalize too low/high \scores that cause each type of critical errors.
% Each sigmoid function penalizes positive inputs (\eg $\M_\ClassId(\y)$ lower than the threshold $\F(\y)$). 
% These thresholds indicate when \scores are too low or too high to trigger a critical error, and their exact values depend not only on the values in $\y$, but also information in the given \summary.
% The intuition of using the $\textrm{Sigmoid}(x) = \frac{1}{1+e^{x}}$ function is it will incur a high penalty for a positive input (\ie $M_j(y)$ for a correct class is lower than the $\F(y)$), and low penalty for a negative input. 

% To make it more concrete, here we present the exact formulation of Eq~\ref{eq:loss} in the case of \summaries with ``label-based API, \term{Multi-Choice} type of decision, and \term{API-output order}'', which is one of the most common type of \summaries.
% The loss function for other types of \summaries will be detailed in Appendix\S\ref{sec:loss_appendix}.






\myparashort{Case study: \term{Multi-Choice API-output order}.}
These applications take label-based API outputs and make \term{Multi-Choice} decisions in \term{API-output} order (defined in \S\ref{subsec:observations}).
% \jc{make sure you always add pointers to any terms you defined in this paper when they are first used in each subsection.}
For instance, given the DNN output labels on a ``\code{Food}'' image, the garbage-classification application in Figure~\ref{fig:loss} (middle)
% depicts an example of this type of decision process. \jc{again, explain in one sentence what the app does.}
% \jc{is it the right macro? shouldn't it be "\code{Food}"?} 
% image, the DNN returns $\y$ (a vector of confidence scores),  and the application 
checks these labels in descending order of their confidence scores until the first label belonging to any \target (\eg in this example, label ``\code{Shirt}'' in \target \code{ Donate}).

To design the loss function of this decision process, we first equivalently describe it in the general framework of decision processes (Figure~\ref{fig:loss}(right)). 
The \score $\M_\ClassId(\y)$ of each \target $\ClassId$ should be the highest confidence score in DNN output $\y$ associated with any label in $\ClassId$. 
This is because the labels in \code{detection\_labels} are sorted in descending order of their confidence scores, so the highest-score label in each \target is always matched first.
Since the process checks the labels in descending order of their confidence scores, it effectively goes through the \scores in the order of $\M_{Donate}(\y)$, $\M_{Compost}(\y)$, $\M_{Recycle}(\y)$ (\ie the descending order of $\M_\ClassId(\y)$). 
% This is because it is a \term{Multi-Choice API-output} process, \ie it breaks after the \target whose \score is the highest and exceeds the threshold $\theta$. 
% In this case, the break occurs after matching the \target of \code{Donate}, because its score is the highest and exceeds $\theta$.
% It then goes through the three \targets in the order of $\M_{Landmark}(\y)$, $\M_{Building}(\y)$, and $\M_{Person}(\y)$ (\ie following the if-else statements in the code).
Finally, the break occurs after matching the \target of \code{Donate}, because \term{Multi-Choice API-output} always matches the \target with the highest \score that exceeds the threshold $\theta$ (by default, $\theta=0.5$). 



With this general description, we should penalize two types of critical errors (Type-2 and Type-3) using the following loss function: 
\begin{align}
     L(\y_\InputId) &=   \overbrace{ \textrm{Sigmoid} ( \max_{\LabelId \in \bigcup\limits_{\ClassId > \hat{\ClassId}} \TargetSet_{\ClassId}} \y_{\InputId, \LabelId}
      - \max_{\LabelId \in \bigcup\limits_{\ClassId} \TargetSet_{\ClassId}} \y_{\InputId,\LabelId}\  ) 
}^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-1} Critical Errors}} 
}} \nonumber 
\label{eq:loss_app}
\end{align}



% \begin{align}
%      L(\y_\InputId) &=   \overbrace{ \textrm{Sigmoid} ( \max(\theta, \max_{\ClassId \neq \Tg_\InputId}\M_j(\y_\InputId)) - \M_{\Tg_\InputId}(\y_\InputId)  )
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-2} Critical Errors}} 
% }} \nonumber \\ &+ \overbrace{ \sum_{\ClassId \neq \Tg_\InputId } \textrm{Sigmoid} \Bigl (\M_\ClassId(\y_\InputId) - \M_{\Tg_\InputId}(\y_\InputId) \Bigr)  
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-3} Critical Errors}} 
% }}\label{eq:loss_app}
% \end{align}
% where $\y_\InputId$ is the DNN output on the input $x_i$ (\ie $\y_\InputId = DNN(x_\InputId)$), $\Tg_i$ is the index of the correct \target. 
% To see why this loss function works for \term{Multi-Choice API-output order}, a Type-2 error means that the \score $\M_{\Tg_\InputId}(\y)$ of the correct \target falls below that of any incorrect \targets as well as the threshold $\theta$, \ie $\max(\theta, \max_{j \neq \Tg_\InputId}\M_\ClassId(\y_\InputId))$, so the first term penalizes Type-2 errors.
% A Type-3 error means the \score of any incorrect \target exceeds that of the correct \target, \ie $\M_{k_\InputId}(\y_\InputId)$, so the second term penalizes Type-3 errors.
% Type-1 errors will never happen in this application, because by definition if a correct \target is traversed before the break, its \score must have ranked highest and exceeds $\theta$, which means it will be matched. 

% \jc{\{correct, ground-truth\} $\times$ \{decision, \target\}?? make it consistent!} \yh{Using correct \target now}



To successfully train a DNN model, the loss function must be differentiable with respect to any DNN ouput. 
% It is important to note that optimizers used in ML(\eg Adam)
% % \jc{you tend to add references on non-essential terms, } 
% to train  models are gradient-based. 
% Thus, the loss function (\ie every function in the composite function) needs to be differentiable in order to calculate the gradient of the loss value with respect to the DNN output. 
Note that in Eq~\ref{eq:loss_app}, the $\max$ function is used at multiple places (\eg $\M_\ClassId(\y)$, $\max(\theta, \max\limits_{\ClassId \neq \Tg_{\InputId}} \M_\ClassId(\y))$), but it can be equivalently expressed in a differentiable form (we use the differentiable operators in PyTorch Autograd~\cite{paszke2017automatic}).


\end{comment}

==> bk/backups_before_fist_submission/3-2-old.tex <==

\mypara{A general framework of decision processes}
In contrast, \tool's loss function only penalizes critical errors. 
A key challenge is how to handle various of application decision processes, each having different critical errors.
To address this challenge, our insight is that the decision process of each application in our study (\S\ref{sec:methodology}) can be described as follows. 
\begin{packeditemize}
\item For a DNN output $\y$ (recall from \S\ref{subsec:observations}, $\y$ is an array of scores), whether the \target $\ClassId$ is matched in $\y$'s application decision depends only on some specific value in $\y$, which we call the {\em effective score} of \target $\ClassId$, $\M_\ClassId(\y)$.
\item Given the effective score $\M_\ClassId(\y)$ of each \target $\ClassId$, the decision process of an application can be equivalently viewed as traversing the list of the target classes ranked in certain order until it {\em breaks}. 
\end{packeditemize}
Figure~\ref{fig:loss} gives a concrete example, but %, and more cases will be discussed shortly.
the exact order of traversing the \targets and when the traversal breaks depend on the values in $\y$ and the \summary. 



\begin{comment}

which makes \term{Multi-Choice} decision in application choice order. It defines three target classes, \code{Landmark}, \code{Building} and \code{Person}. Given a ``Landmark'' image, the MLaaS returns a vector of confidence scores $y_i$. The \scores for the target classes are $\M_{Landmark}(\y) = 0.4$, $\M_{Building}(\y) = 0.7$, $\M_{Person}(\y) = 0.8$. The decision process traverses all the target classes in the order of $\M_{Landmark}(\y)$, $\M_{Building}(\y)$, $\M_{Person}(\y)$, and breaks at \code{Building} because it is the first class whose effective score is higher than the detection threshold $\theta$. 

\end{comment}


% \jc{explain the terms (order, break, etc) using fig4}


% While the exact form depends on the matching order of the specific application as well as the API output type (value or labels), \tool's loss function is constructed based on the same general idea that applies to the applications in our study.
% Here, we first explain its general idea before discussing the new loss function case-by-case.



% This general description applies to all applications under our study. 

Importantly, this general framework allows us to categorize {\em critical errors} in three types:
\begin{packeditemize}
\item {\em Type-1 Critical Errors:} \Target $\ClassId$ is correct and traversed before the break, but $\M_\ClassId(\y)$ is too low to be matched.
\item {\em Type-2 Critical Errors:} \Target $\ClassId$ is correct but $\M_\ClassId(\y)$ is so low that it is ranked after the break.
\item {\em Type-3 Critical Errors:} \Target  $\ClassId$ is incorrect but its $\M_\ClassId(\y)$ is so high that it is traversed before the break.
\end{packeditemize}
% and is sufficient to derive our new loss function as follows. 
% We first explain its general idea before discussing the new loss function case-by-case.




\mypara{\tool's loss function}
Consequently, \tool's loss function penalizes each type of critical errors.
\begin{align}
L(\y) &= 
\overbrace{ \sum_{\substack{\textrm{Target class } \ClassId \textrm{ is correct \&}\\\textrm{ traversed before break}}} ~\textrm{Sigmoid}(\F(\y)- \M_\ClassId(\y))
}^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-1} Critical Errors}} 
}} \nonumber \\ &+
\overbrace{ \sum_{\substack{\textrm{Target class } \ClassId \textrm{ is correct \&}\\\textrm{ ranked after break}}} ~\textrm{Sigmoid}(\G(\y)- \M_\ClassId(\y))
}^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-2} Critical Errors}} 
}} \nonumber \\ &+ 
\overbrace{ \sum_{\substack{\textrm{Target class } \ClassId \textrm{ is incorrect \&}\\\textrm{ traversed before break}}} \textrm{Sigmoid}(\M_\ClassId(\y) - \Q(\y) )
}^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-3} Critical Errors}} 
}} \label{eq:loss}
\end{align}
where $\F(\y)$, $\G(\y)$ and $\Q(\y)$ are thresholds used to penalize too low/high \scores that cause each type of critical errors.
Each sigmoid function penalizes positive inputs (\eg $\M_\ClassId(\y)$ lower than the threshold $\F(\y)$). 
These thresholds indicate when \scores are too low or too high to trigger a critical error, and their exact values depend not only on the values in $\y$, but also information in the given \summary.
The intuition of using the $\textrm{Sigmoid}(x) = \frac{1}{1+e^{x}}$ function is it will incur a high penalty for a positive input (\ie $M_j(y)$ for a correct class is lower than the $\F(y)$), and low penalty for a negative input. 

To make it more concrete, here we present the exact formulation of Eq~\ref{eq:loss} in the case of \summaries with ``label-based API, \term{Multi-Choice} type of decision, and \term{API-output order}'', which is one of the most common type of \summaries.
The loss function for other types of \summaries will be detailed in Appendix\S\ref{sec:loss_appendix}.

% $\F(\y)$ is defined as $\theta$. 
% $\G(\y)$ is defined as  the \score of the \target, or $\theta$ at which the process breaks at. 
% $\Q(\y)$ is defined as the \score of the ground-truth \target if the process will break at it when an output contains both the ground-truth and the $\ClassId^{th}$ class, otherwise, it is $\theta$.

% The intuition of setting $\F(\y)$ and $\Q(\y)$ as described above is: (1) whenever a correct \target falls below the \score or $\theta$ at which break happens, type-1 or type-2 critical errors will occur (2) whenever an incorrect \target exceeds the \score or $\theta$ at which break happens, a penalty should be incurred on type-3 critical error;
% \mypara{True-False}In \emph{True-False} decision, only one target class is defined, and the application checks if the API output matches with it. 
% Since there is only one target class, no incorrect termination may possibly be made on other target classes than the ground-truth one. 
%  \Q(y) also falls back to the default value, because when the target class is not selected by the ground-truth decision, a correct termination can only be made if its score is lower than $\theta$.

% \mypara{\term{Multi-Select}}As for \term{Multi-Select} decision, multiple selections are allowed about which target class(es) the ML API output matches with. In this case, the decision process will not break until encountering a \target whose \score is lower than $\theta$. An incorrect decision may be made when the target classes selected by ground-truth decision are ranked after the break at $\theta$, or when target classes not selected by ground-truth decision are ranked before the break at $\theta$. Thus, we penalize the type-2 critical errors and type-3 critical errors by assigning $\theta$ as the values for $\F(y)$ and $\Q(y)$. 

% \mypara{\term{True-False}}The decision process simply checks if the \score of the only defined \target 





\myparashort{Case study: \term{Multi-Choice API-output order}.}
These applications take label-based API outputs and make \term{Multi-Choice} decisions in \term{API-output} order (defined in \S\ref{subsec:observations}).
% \jc{make sure you always add pointers to any terms you defined in this paper when they are first used in each subsection.}
For instance, given the DNN output labels on a ``\code{Food}'' image, the garbage-classification application in Figure~\ref{fig:loss} (middle)
% depicts an example of this type of decision process. \jc{again, explain in one sentence what the app does.}
% \jc{is it the right macro? shouldn't it be "\code{Food}"?} 
% image, the DNN returns $\y$ (a vector of confidence scores),  and the application 
checks these labels in descending order of their confidence scores until the first label belonging to any \target (\eg in this example, label ``\code{Shirt}'' in \target \code{ Donate}).

To design the loss function of this decision process, we first equivalently describe it in the general framework of decision processes (Figure~\ref{fig:loss}(right)). 
The \score $\M_\ClassId(\y)$ of each \target $\ClassId$ should be the highest confidence score in DNN output $\y$ associated with any label in $\ClassId$. 
This is because the labels in \code{detection\_labels} are sorted in descending order of their confidence scores, so the highest-score label in each \target is always matched first.
Since the process checks the labels in descending order of their confidence scores, it effectively goes through the \scores in the order of $\M_{Donate}(\y)$, $\M_{Compost}(\y)$, $\M_{Recycle}(\y)$ (\ie the descending order of $\M_\ClassId(\y)$). 
% This is because it is a \term{Multi-Choice API-output} process, \ie it breaks after the \target whose \score is the highest and exceeds the threshold $\theta$. 
% In this case, the break occurs after matching the \target of \code{Donate}, because its score is the highest and exceeds $\theta$.
% It then goes through the three \targets in the order of $\M_{Landmark}(\y)$, $\M_{Building}(\y)$, and $\M_{Person}(\y)$ (\ie following the if-else statements in the code).
Finally, the break occurs after matching the \target of \code{Donate}, because \term{Multi-Choice API-output} always matches the \target with the highest \score that exceeds the threshold $\theta$ (by default, $\theta=0.5$). 

% , where each element indicates how confident the model is about the existence of the image.
% \jc{this sentence is incomplete..} \yh{we have stated the meaning of the confidence score vector, should we state it again here?}

% The effective score $\M_j(\y)$ of a \target $\ClassId$ is the 
% It then orders the \scores by descending order, and breaks at \target \code{ Donate}. 
% This is because this is a \term{Multi-Choice API-output order} process, and it returns the \target whose \score is the highest and above $\theta$. \code{Donate} is returned because $\M_{Donate} = 0.8$ is higher than $\theta$. 




% In this case, the e decision process traverses the \scores in descending order. 
% If all \scores are below $\theta$, the process immediately breaks without traversing any of the \targets. 
% Otherwise, it breaks at the \target whose \score is the highest. 
% \jc{Yuhan, please explain this process with the help of fig~\ref{fig:loss}, not merely at a general level.}

% When the ground-truth decision is selecting one of the \targets, only type-2 and type-3 errors might occur. 
% Type-1 errors are absent in \term{Multi-Choice API-output order}, because if the \score for any of the \targets (\eg \target $\ClassId$) exceeds $\theta$, the process will break at it. 
% If $\ClassId$ is correct, this decision is correct. 
% Otherwise, this becomes a type-2 critical error because the \score for the correct class must rank lower than class $\ClassId$. 
% \jc{this explanation of why type 1 is absent is way too long.. try simplify it please}

% Another category of type-2 error comes from when all the \scores fall below $\theta$, leading the process to break before traversing any of the classes.
% A type-3 error can occur when an incorrect \target ranks higher than the correct one. 

% To summarize, the correct \target should not only exceed $\theta$ but also exceed all the \scores of the incorrect \targets.
% Any of the incorrect \targets should not exceed the \score of the correct one.
% \jc{this paragraph is too general.. still doesn't help much in this particular case. please use the example in fig~\ref{fig:loss}}

With this general description, we should penalize two types of critical errors (Type-2 and Type-3) using the following loss function: 
\begin{align}
     L(\y_\InputId) &=   \overbrace{ \textrm{Sigmoid} ( \max_{\LabelId \in \bigcup\limits_{\Tg > \ClassId_\InputId} G_{\Tg}} \y_{\InputId, \LabelId}
      - \max_{\LabelId \in \bigcup\limits_{\Tg} G_{\Tg}} \y_{\InputId,\LabelId}\  ) 
}^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-1} Critical Errors}} 
}} \\&+
 \overbrace{ \textrm{Sigmoid} ( \max_{\LabelId \in \bigcup\limits_{\Tg} G_{\Tg}} \y_{\InputId,\LabelId}
 - \max_{\LabelId \in G_{\ClassId_\InputId}} \y_{\InputId,\LabelId}
 ) 
}^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-2} Critical Errors}} 
}} \\&+
\overbrace{ \sum_{\Tg \neq \ClassId_\InputId}\textrm{Sigmoid} ( \max_{\LabelId \in G_{\Tg}}  \y_{\InputId,\LabelId} - \max_{\LabelId \in \bigcup\limits_{\Tg} G_{\Tg}} \y_{\InputId,\LabelId} )
}^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-3} Critical Errors}} 
}}
\label{eq:loss_app}
\end{align}
where $\y_\InputId$ is the DNN output on the input $x_i$ (\ie $\y_\InputId = DNN(x_\InputId)$), $\ClassId_\InputId$ is the index of the correct \target. 
% To see why this loss function works for \term{Multi-Choice API-output order}, a Type-2 error means that the \score $\M_{\Classid_\InputId}(\y)$ of the correct \target falls below that of any incorrect \targets as well as the threshold $\theta$, \ie $\max(\theta, \max_{j \neq \GtIndex_\InputId}\M_\ClassId(\y_\InputId))$, so the first term penalizes Type-2 errors.
% A Type-3 error means the \score of any incorrect \target exceeds that of the correct \target, \ie $\M_{k_\InputId}(\y_\InputId)$, so the second term penalizes Type-3 errors.
% Type-1 errors will never happen in this application, because by definition if a correct \target is traversed before the break, its \score must have ranked highest and exceeds $\theta$, which means it will be matched. 

% \jc{\{correct, ground-truth\} $\times$ \{decision, \target\}?? make it consistent!} \yh{Using correct \target now}

\begin{comment}
In the example in Figure~\ref{fig:loss}
% \jc{example as in this use case or as in the figure?}
, two types of critical errors arise. 
First of all, a type-2 error occurs as the correct \target \code{ Compost} is ranked after the break because $\M_{Compost} = 0.7$ is lower than $\M_{Donate}=0.8$. 
Another potential type-2 error, not shown in this example, is when the correct \target is the highest among all, but it falls below $\theta$. 
Secondly, a type-3 error occurs as the wrong \target \code{ Donate} is traversed before break because it is the highest \score among all. 
Type-1 errors are absent in this type because if a correct \target is traversed before break, its \score must have ranked highest, and exceeds $\theta$, leading to a correct decision. 


% On the other hand, when the ground-truth decision selects the non-target class, all the \scores should fall below $\theta$ in order for the process to break before traversing any one of the \targets. \jc{not sure how this sentence fits in the context..}

In order to penalize these two types of critical errors, we construct the following loss function:


\end{comment}

% \begin{align}
% L(\y) &= 
% \overbrace{ \textrm{Sigmoid} \Bigl( max(\theta, \max_{j \neq k}\M_j(\y)) - \M_{k}(\y)  \Bigr)
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-2} Critical Errors}} 
% }} \nonumber \\ &+ \overbrace{  \textrm{Sigmoid} \Bigl(\max_{j \neq k}(\M_j(\y)) - \M_k(\y)  \Bigr)
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-3} Critical Errors}} 
% }}
%     % L(y) &=  \textrm{Sigmoid} \Bigl(  \M_{k}(\y) - max(\theta, \max_{j \neq k}\M_j(\y))   \Bigr) \nonumber\\&+ \textrm{Sigmoid}(\max_{j \neq k}\M_j(\y) - \M_k(\y)) 
% \end{align}
% where $k$ is the index of ground-truth \target. 
% % Note that there is only one correct \target, and at most one incorrect \target, so the summation for 

% On the other hand, when the ground-truth decision is selecting the non-target class, only type-3 errors may occur when the \score for any of the \targets is higher than $\theta$. Thus, the following loss function is constructed:
% \begin{align}
%      L(y) &= \overbrace{ \sum_{j}\textrm{Sigmoid}(M_j(y) - \theta)
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-3} Critical Errors}} 
% }} 
% \end{align}

% \begin{align}
%      L(\y) &= \other \cdot \overbrace{ \textrm{Sigmoid}(\max \M_j(\y) - \theta)
%  }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-3} Critical Errors}} 
%  }} \nonumber
%  \\&  + (1-\other) \cdot \Bigl (\overbrace{ \textrm{Sigmoid} ( \max(\theta, \max_{j \neq k}\M_j(\y)) - \M_{k}(\y)  )
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-2} Critical Errors}} 
% }} \nonumber \\ &+ \overbrace{  \textrm{Sigmoid} (\max_{j \neq k}(\M_j(\y)) - \M_k(\y)  )
% }^{\substack{\text{\sf \footnotesize {Penalize {\bf Type-3} Critical Errors}} 
% }} \Bigr)
% \end{align}



% \jc{isn't it awkward to split the two terms of Type-3? can you put them together and have one curly bracket covering both? and also the presence of $O$'s is weird and doesn't fit the form of (2). i understand what they do, but can we not put them there?}
% where $\other$ is $1$ when the ground-truth decision selects the non-target class, and $0$ if the ground-truth decision selects any of the \targets. 

% \yh{explain why diff}

% \jc{the order should be "why loss func being differentiable is important => what might not be differentiable in the equation (3) (NOT in 2) ==> why they are not a concern after all". 
% the ``why differentiable'' part should be a separate para}

To successfully train a DNN model, the loss function must be differentiable with respect to any DNN ouput. 
% It is important to note that optimizers used in ML(\eg Adam)
% % \jc{you tend to add references on non-essential terms, } 
% to train  models are gradient-based. 
% Thus, the loss function (\ie every function in the composite function) needs to be differentiable in order to calculate the gradient of the loss value with respect to the DNN output. 
Note that in Eq~\ref{eq:loss_app}, the $\max$ function is used at multiple places (\eg $\M_\ClassId(\y)$, $\max(\theta, \max\limits_{\ClassId \neq \Tg_{\InputId}} \M_\ClassId(\y))$), but it can be equivalently expressed in a differentiable form (we use the differentiable operators in PyTorch Autograd~\cite{paszke2017automatic}).


% A thoughtful reader may wonder if taking the maximum out of $\y$ makes the loss function non-differentiable. 
% However, we can make the $\max$ function differentiable by approximating it with a differentiable Sigmoid function (\ie assigning the gradients for values less than maximum 
%  to values close to 0)\footnote{Indeed, this is what have been done by PyTorch Autograd~\cite{paszke2017automatic}, and we utilize their implementation of a differentiable max operator.}.
 
% where $\total$ is the total number of \targets defined in the code. 
% \mypara{True-False}In \emph{True-False} decision, only one target class is defined, and the application checks if the API output matches with it. 
% In this case, when the \target is selected by ground-truth decision but its \score is lower than the detection threshold $\theta$, the decision process will break before traversing to the class. 
% Thus, $\F(y)$ is always $\theta$ for \emph{True-False}. 
% Similarly, $\Q(y)$ is $\theta$ because in order for the decision process to break correctly, when the \target is not selected by ground-truth decision, its \score should be lower than $\theta$.





\begin{comment}

Compared to the strawman which may spare energy penalizing non-critical errors\shan{?? what exactly are non-critical errors spared by strawman?} \yh{Put in the last paragraph}, 
our proposed solution only focuses on penalizing the critical ones. 
Specifically, two types of critical errors are being penalized\shan{I don't understand the (1) and (2) presented below} \yh{how about now? }: 
(1)\shan{Hmm, what does this mean?}\emph{all} the labels in a target class have low confidence scores in the prediction, but ground-truth decision selects it. 
(2) \emph{at least one of} the labels in a target class has a high confidence score, but ground-truth decision does not select it.

\yh{whether a target class is selected depends }
\end{comment}

% \tool's  loss function uses the Sigmoid function (\ie $Sigmoid(y) = \frac{1}{1+e^{k\cdot y}}$) to penalize the critical errors. The intuition behind using the Sigmoid function is that it provides a differentiable way to incur a high penalty when $y >0$\shan{what is y?}, and a low penalty otherwise, which appropriately fits our needs. 

% , such as mis-classifications across target classes. 
% For example, the strawman penalizes mis-classifications within the target classes, which are non-critical, while 

\begin{comment}
    

Formally, the loss function can be written as:


To understand the loss function, we formulate the application decision process as a mapping process from the raw ML-model output, denoted as $y_i$, to an output set of target classes (the set may include one or more classes).
Specifically, given the output of an ML model, the application first calculates the maximum probability of labels belonging to each target class (\ie $\M_j(y_i)$), which we denote as target-class score. The application checks the target-class scores in different orders to decide if included in the output set. 
The mapping process may terminate at a target class. 
For example, for an application making \emph{Multi-Choice} decision in application choice order, it checks all the target-class scores above detection threshold and  terminates at the target class with the highest priority. 
Based on the ground-truth decision of the input $y$, $\F(y)$ in Equation~\ref{eq:loss} is defined as the maximum target-class score out of all the possibly incorrect terminations. 
If no such termination may be made, $\F(y)$ falls back to a default value, which is the detection threshold, denoted as $\theta$. 
% Intuitively, when the target-class score of the correct class falls below the target-class score of an incorrect termination, the mapping procedure will terminate at a wrong class. 
$Q_j(y)$ is defined as the score of the correct \target if the mapping process can terminate correctly, when only considering the correct class and the $j^{th}$ class. 
If no such termination can be made, $Q_j(y)$ falls back to a default value $\theta$.

% Intuitively, we penalize the target-class score for the ground-truth \target when it is lower than  the target-class score of the incorrect termination; or the target-class score for \target that is not selected by ground-truth decision when it is higher than the score of a correct termination. 



For example, Figure~\ref{fig:loss} shows the mapping process for the garbage classification application, which makes \emph{Multi-Choice} decision in API-output order. It defines three target classes. The MLaaS takes an image with ground truth \code{``Shirt''} as input, and outputs a list of probabilities, denoted as $y_i$, for each label. 
The correct target class (\ie the one that matches with ground truth) is the third one. 
In our formulation of decision process, the application first calculates the target-class score for each class, which are $\M_1(y_i)=0.8$, $\M_2(y_i)=0.7$ and $\M_3(y_i)=0.4$ respectively. 
The application then iterates over all the target-class scores, ranked in descending order, and terminates at the first one. 
In this example, $\F(y_i) = M_1(y_i)$. The reason is that out of all the incorrect target classes, the target-class score of the first one is the largest.
And $Q_1(y_i) = M_2(y_i)$ and $Q_3(y_i) = M_2(y_i)$ because as long as the target-class scores for incorrect \target is lower than $\M_2(y_i)$, a correct termination can still be made. 

\end{comment}

\jc{we should probably explain one or two cases in the main text and move the rest to appendix}

\begin{comment}


\mypara{Multi-Select}As for \emph{Multi-Select} decision, multiple selections are allowed about which target class(es) the ML API output matches with. 
In this case, the ground-truth target class(es) are those which overlap with the ground-truth labels of the input. 
This type of application will not terminate at any target-class, $\F(y)$ and \Q(y) are set to their default values $\theta$. 

\mypara{Multi-Choice application choice order} This type of application reaches only one selection by checking if the highest-priority target class matches with the output labels, if not, it moves on to the next target class, and so on. In this case, the ground-truth target class is the highest priority class out of those overlapping with its ground-truth labels. In this case, a possibly incorrect termination can be made at any higher-priority target class than the correct one. Thus, $\F(y)$ is the maximum target-class score out of all the classes with higher priority than the ground-truth one. $\Q(y)$ is $\theta$ for the target classes whose priority is higher than the correct one, since the mapping process cannot terminate correctly when considering the correct class and a higher priority one. $\Q(y)$ is the target-class score for classes whose priority is lower than the correct one, because the mapping process can  terminate correctly when the target-class score for the correct one is larger than the $j^{th}$ incorrect one. 

\mypara{Multi-Choice API-output order}In this case, similar to the application choice order, only one selection is allowed. However, the application reaches a decision by checking if the first output label matches with any of the target classes, if not, it moves on to the next output label. In this case, a possibly incorrect termination can be made at target-class score for any of the incorrect classes. Thus, $\F(y)$ is defined as the maximum target-class score for all the incorrect classes. Meanwhile, when all the target-class scores are above $\theta$, a mapping process may terminate correctly when the target-class score for the correct class ranks higher than those of the incorrect classes. Thus, $\Q(y)$ is defined as the target-class score for the correct class. 


% where $\M_j(y)$ is the \emph{maximum} probability in $y$ at indices that belong to the $j^{th}$ target class.  $\Q(y), \F(y)$ are two scores that differ by different types of applications. Generally, $ \F(y) > M_j(y)$ or $ M_j(y) > \Q(y)$ suggest that $y$ leads to an incorrect decision, otherwise, a correct decision is made\shan{hmmm, too complicated for me to understand} \yh{Working on how to make this clearer now}. 
% where $H_o(y) = 1$ if $y$ leads to the selection of the non-target class, and $H_o(y) = 0$ otherwise. $H_j(y) = 1$ if $y$ leads to the selection of the $j^{th}$ target class, and  $H_j(y) = 0$ otherwise. $Q_j(y) = 0$ for applications making \emph{Multi-Choice} decisions in API-output order, and $Q_j(y) = 1-H_j(y)$ otherwise. 
% $\theta$ is the prediction threshold of ML model, where any labels whose predicted probability is higher than it will be included in the output. $G_j(y)$ is the maximum probability in $y$ at indices that belong to the $j^{th}$ target class. $G(y) = max_{j \in \{1, \dots, m\}} (G_j(y))$ is the maximum probability in $y$ at indices belonging to all the target classes. $\F(y) = max$($\theta$, maximum probability in  $y$ at the indices that belong to any ground-truth unselected target class(es)). 

% In order to achieve the goal of re-sampling the training data,  our loss function assigns a weight $\frac{M}{N_i}$, where $\M$ is the total number of data in the original training dataset, and $N_i$ is the number of training samples whose ground-truth labels overlap with the ground-truth target class(es) of the $i^{th}$ input. This weight, intuitively,  alleviates the effect of class skews in the original dataset by assigning higher weight to less dominant target classes, and lower weight for more dominant ones. 
% \yh{care more about the target classes} 


% As we have seen in \S\ref{sec:empirical}, the critical errors can vary greatly across different types of application's decision processes. Thus, in order to accurately capture the critical errors, we design different loss functions for each type of decision process. 
\end{comment}

% Next, we describe the loss function for each type of decision process case-by-case. 
\begin{comment}

\mypara{True-False} In \emph{True-False} decision, only one target class is defined, and the application checks if the API output matches with it. 
Denote the prediction threshold of the ML model as $\theta$, where all the labels whose probabilities are higher than it will be included in the output. 
In this case, $\F(y) = \theta$, and $\Q(y) = \theta$. \shan{I understand the next few sentences, but I don't understand why F(y) is $\theta$, and 
Q(y) is $\theta$. I went back to read the $L_i$ formula, but still don't understand.}
For an input whose ground-truth decision selects the target class, a high penalty will be incurred if none of the labels in the target class appear in the output. 
% Thus, when the maximum probability for labels belonging to the 
On the other hand, for an input whose ground-truth decision selects the non-target class, a high penalty will be incurred  when there is at least one label in the target class included in the output. 

\mypara{Multi-Select} As for \emph{Multi-Select} decision, multiple selections are allowed about which target class(es) the ML API output matches with. 
In this case, the ground-truth target class(es) are those which overlap with the ground-truth labels of the input. 
$\F(y) = \theta$ and $\Q(y) = \theta$ for this type. 
The loss function will incur a high penalty when there are ground-truth target class(es) whose maximum probability is lower than $\theta$, 
or when there are target class(es) unselected by ground-truth whose maximum probability is higher than the $\theta$. 
\shan{Is Multi-Select's loss function essentially the same as True-False? Or, maybe you can tell me what exactly is the difference between them?}


% Denote the output of the ML model on the $i^{th}$ input as [$y_{i, 1}, \dots, y_{i,n}$]


\mypara{Multi-Choice application choice order} This type of application reaches only one selection by checking if the highest-priority target class matches with the output labels, if not, it moves on to the next target class, and so on. In this case, the ground-truth target class is the highest priority class out of those overlapping with its ground-truth labels. $\F(y) = max(\theta$, \textrm{maximum probability in $y$ at indices of unselected target class(es)}), and $\Q(y) = \theta$. Take the example in Figure~\ref{fig:loss} to illustrate. The application defines three target classes. Given an input image whose ground-truth label is \code{``Mansion''}, the ground-truth target class is the second one. In this example, $\F(y_i) = max(\theta, M_1(y_i)) = 0.8$ because the first target class has higher priority than the ground-truth target class. $\Q(y_i) = 0.5$ in this example. Thus, the penalty incurred by the loss function is Sigmoid(0.8-0.5) + Sigmoid(0.8-0.7) + Sigmoid(0.4-0.5). 
 
We can see that the loss function will incur a high penalty if any target class(es) with higher priority than the ground-truth target class are included in the output. 




\mypara{Multi-Choice API output order} In this case, similar to the application choice order, only one selection is allowed. However, the application reaches a decision by checking if the first output label matches with any of the target classes, if not, it moves on to the next output label. 
In this case, the ground-truth target classes are those  overlapping with ground-truth labels. 
$\F(y) = max(\theta, $ maximum probability in $y$ at indices of unselected target classes by ground-truth decision), and $\Q(y) = $ the maximum probability in $y$ at indices of the ground-truth target classes.  
Thus, for the ground-truth target class, only if the maximum probability of it  is smaller than the maximum probability of unselected target class(es) or the prediction threshold, a high penalty will be incurred by the loss function. 

\end{comment}

% \jc{
% an example outline of this subsection (each bullet is a para)
% \begin{itemize}
% \item why we start with this? the key step is customizing ML model for each application.
% \item what's the goal
% \item what's a strawman (resampling training data)? and why is it not good (doesn't distinct multi-choice vs multi-option and order of examination)? (this para must be short). if room, also bring up some prior work that also does this
% \item our idea: rewriting loss function. give a general recipe of how this is done
% \item why is it better? (this should directly contrast with the strawman)
% \item more case-by-case explanation.
% \end{itemize}
% }

% \jc{regarding how to explain the goal, you can expand the following: formally an application can be viewed as $z=Decision(Model(x))$. for a given decision process $Decision$, the goal is to minimize $Decision(Model(x_i))\neq Decision(\hat{y_i})$ over a set of $x_i$, where $\hat{y_i}$ is the ground truth label of $x_i$.}



% \mypara{Notations} 
% Denote the total number of classes that the ML model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows. 
% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the ML model behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}

% \mypara{Customization goal} For T-or-F, we want to minimize the critical errors which are caused by the API outputs that lead to the  execution of the \emph{False} branch, when the statement should be \emph{True} according to the ground-truth, and vice versa. With the above notations, our goal can be written as:

% \begin{equation}
% \begin{aligned}
% \min \sum\limits_{i=1}^{M}( y_i \cdot \mathds{1}_{\theta - P} + (1-y_i) \cdot \mathds{1}_{P-\theta} )
% \end{aligned}
% \end{equation}

% Where $\mathds{1}_{x} = 1$ when $x > 0$, and 0 otherwise. $y_i = 1$ if the $i^{th}$ input belongs to the class list defined in the branch condition, which we denote as $W$. $\theta$ is the prediction threshold, where classes whose predicted probability is higher than the threshold will be included in the output label list. $P$ is the maximum probability of classes in $W$, in other words, $P = max_{c \in W} p_c$.
% there are two types of critical errors: (1) for inputs whose statement in the branch condition is \emph{True} according to the ground-truth, which we refer to as \emph{target-inputs}, the API outputs lead the application selecting the \emph{False} branch; (2) for inputs whose statement is \emph{False}, the API outputs lead the application selecting the \emph{True} branch. To minimize incorrect application decisions, we want: 




% \yh{Outline of this section: 
% 1. first list the goal in math (or text): minimize the incorrect app decisions
% 2. a naive re-training scheme is to use a training data that  focuses on classes appeared in the apps 3. why this design is not good: it can only solve xxx, but not xxx 4. describe our loss function }
% \yh{goal: minimize the incorrect app decisions; what we have: extracted application's decision process (key dimensions) }
% As shown in our empirical study in Section~\ref{sec:empirical}, we find the application's decision process can be characterized by two aspects: (1) the class list(s) or value ranges that are used in branch conditions (2) the structures of the branch conditions.

% In this section, we will describe how we incorporate the application's decision process in the loss function. Our optimization is composed of two steps: (1) clustering the training data to focus on classes appearing in the branch conditions; (2) constructing the loss functions to be aware of the application's decision process. Our objective is to incur a high penalty on critical errors, and no penalty if the errors make no impact on the application. 


% To begin with, we first introduce the loss function traditionally used in multi-label image classification.


% The binary cross-entropy loss function used in multi-label classification task~\cite{ASL} is denoted as:
% \begin{equation}
%     L_{bce}  = -\frac{1}{n}\sum_{i=1}^n{(y_i\log(p_i) + (1 - y_i)\log(1 - p_i))} \,,
% \end{equation}
% where $y_i = 1$ if class $i$ is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. $p_i$ is the predicted probability for class $i$. 
% \begin{itemize}
%     \item  $y_i = 1$ if the $i^{th}$ class is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. 
%     \item $p_i$ is the predicted probability for the $i^{th}$ class.
% \end{itemize}
% where $y_i$ indicates whether the $i^{th}$ class exists in the input input $I$ or not. In other words, $y_i = 1$ if the $i^{th}$ class exists in the input $I$, and $y_i = 0$ otherwise. \cc{It is still one sentence, so please do not start a new paragraph}


% \subsubsection{Clustering training data}


% To achieve the first step, one approach is to assign different weights to inputs with ground-truth decisions of executing the \code{Others} branch and non-\code{Others} branches.  
% We take a simple example to illustrate this approach. An application  defines one branch condition to check if the API outputs intersect with a class list $W_1$. $W_1$ is a non-empty subset of the whole label set $C$ that the ML model is able to classify. 
%  The original fraction of images in the training data whose ground-truth  decisions are executing the \code{$W_1$}-branch (\ie $G \cap W \neq \emptyset$), which we refer to as \code{$W_1$}-inputs,  is $A$. 
%  % \cc{This sentence is very hard to read. Can we use phrase like ``which we refer to as $W$-images''?} 
% The fraction of images whose ground-truth decisions are executing the \code{other}-branch is $1-A$,  which we refer to as \code{others}-inputs. If we want to balance the distribution between $W$-inputs and \code{others}-inputs, we can use a loss function that assigns higher weights to \code{W}-inputs:

% \begin{equation}
%     L_D = y_1 \cdot \frac{1}{A} \cdot L_{bce} + (1-y_1)\cdot A \cdot L_{bce} \,,
% \end{equation}
% where $y_1$ indicates whether this input is a \code{$W$}-input or not. In other words, $y_1 = 1$ when the input is a \code{$W$}-input ($G \cap W \neq \emptyset$), and $y_1 = 0$ otherwise ($G \cap W = \emptyset$). 

% In this way, \code{$W$}-inputs and \code{others}-inputs are taking the same effect during training, instead of biasing towards either \code{W} or \code{others}. 

% % We construct loss functions for each type of software represented by the software examples shown in section~\ref{sec:empirical}. \cc{Maybe say some high-level ideas, more intuition}

% \subsubsection{Branch condition structure 1: T-or-F} 

% For the software that defines only one branch condition, checking if the output labels $O$ intersect with a class list $W_1$. We penalize the critical errors: (1) all the classes in $W_1$ are not included in top predictions for \code{$W_1$}-inputs; or (2) at least one class in $W_1$ are included in top predictions for \code{others}-inputs.




% \begin{equation}
%     L_{W_1} =y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \,,
% \label{eq:loss}
% \end{equation}
% where
% $y_1$ indicates whether this input is a \code{$W_1$}-input or not. 
% In other words, $y_1 = 1$ if the input is a \code{$W_1$}-input, and $y_1=0$ if the input is a \code{others}-input. $\theta$ is the prediction threshold, where classes whose predicted probability will be included in the output label list. $P_1$ is the maximum probability of classes in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will denote as $S$ in the rest of the paper. 



% Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for  \code{$W_1$}-inputs. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-inputs. Similarly for \code{other}-inputs. 



% \subsubsection{Branch condition structure 2: M-to-N-set} 

%  In M-to-N-set, several branch conditions are defined, each checking if a class list intersects with the API output $O$. All the fulfilled branches will be executed. We denote all the $\M$ class lists the application uses in branch conditions as {$W_1$, ..., $W_m$}. In this pattern, the ground-truth  decisions is executing \emph{all} the branches whose class lists  intersect with the ground-truth labels. 

% We derive the following loss function for M-to-N-set:
% \begin{equation}
%     L = \sum_{i=1,\cdots,m} y_i \cdot \textrm{S}(\theta - P_i) + (1-y_i) \cdot \textrm{S}(P_i - \theta) \,,
% \end{equation}
% where $y_i$ indicates whether  $W_i$ is among the branches the ground-truth decision executes, in other words, $y_i = 1$ if $G \cap W_i \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_i$ is the maximum probability of classes belonging to $W_i$ (\ie $P_i = max_{c \in W_i} p_c$). 

%  Only if the application decisions led by $O$ exactly match with the ground-truth decisions, the penalty will be low.


% % \kt{$\sum_{i=1,\cdots,N} L_{W_i}$}



% \subsubsection{Branch condition structure 3: Priority-list}

% Priority-list defines several branch conditions, and each of them is associated with a class list $W_i$. The application checks the branch conditions from highest to lowest priority until finding the first one whose class list intersects with API output labels $O$. Let $W_i$ (where $1 \leq i \leq m$) denote the class lists used in branch conditions, where class lists with smaller $i$ indicate higher priority. Let $W$ denote the union of the classes in all the whitelists, in other words, $W = \cup^{m}_{i=1}W_i$. The ground-truth decision  is executing the highest priority branch whose associated class list intersects with the ground-truth classes $G$. 

% We derive the loss function as:
% \begin{equation}
% \begin{split}
%     L = y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
%     (1-y_i) \cdot \textrm{S}(P - \theta) \,,
% \end{split}
% \end{equation}
% where $y_i = 1$ when the ground-truth decision is executing one of the branches in $\{ W_1, \cdots, W_m\}$ (\ie $G \cap W \neq \emptyset$), and  $y_i = 0$ when the ground-truth decision is executing the \code{others} branch. 
% $k$ is the index of the highest-priority branch whose class list intersects with the ground-truth classes (\ie $k = \min \{i|WL_i \cap G \neq \emptyset\}$). $P_k$ is the maximum predicted probability for classes belonging to $W_k$, and $P_{k^{-}}$ is the maximum predicted probability out of the classes belonging to higher priority branches than the ground-truth branch (\ie $k^{-} = \min \{i | W_i \cap (G \setminus W ) \neq \emptyset \textrm{ and } i < k \}$). $P$ is the maximum probability of the classes belonging to $W$. 

% Given this loss function, only if the highest-priority branch whose class list intersects with the predicted classes $O$ is the ground-truth decision, the penalty will be low. 


% \subsubsection{Branch condition structure 4: Top-label}

% Top-label defines several branch conditions, and associates with each of them with a class list $W_i$, similar to Priority-list. However, unlike Priority-list, it checks the \emph{API output labels} one by one until one of them intersects with any of the class lists. Similar to the previous section, $W$ is the union of classes in all the defined class lists. We denote the classes belonging to class lists intersecting with ground-truth classes as $W^+ = \bigcup_{W_i \cap G \neq \emptyset} W_i$, and the classes belonging to \wls that do not intersect with ground-truth classes as $W^- = W \setminus W^+$.
 
% In this pattern, the ground-truth decision is to execute the branch condition  whose class list  intersects with the ground-truth classes. 

% We derive the loss function as:
% \begin{equation}
%     L = y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \,,
% \end{equation}
% where $y_i  = 1$ indicates that the ground-truth decision is executing one of the branches in \{$W_1$, $W_2$, ...$W_m$\}, and $y_i = 0$ indicates the ground-truth decision is selecting \code{others}, similarly to the previous section. $P^{+}$ is the maximum probability out of classes in $W^+$ (\ie $P^+ = \max_{c \in W^+ } p_c$), and $P^-$ is the maximum probability out of classes in $W^-$ (\ie $P^- = \max_{c \in W^- } p_c$). 


% Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 



==> bk/backups_before_fist_submission/3-2-v2.tex <==
\label{sec:method}

Inspired by the empirical study of \S\ref{sec:empirical}, this section presents \tool, an optimized MLaaS backend that customizes ML models for the decision processes of different applications.


\subsection{High-level workflow and key components}
\label{sec:overall}


\begin{figure}
    \centering
    % \includegraphics[width=\linewidth]{figs/workflow.pdf}
    \includegraphics[width=\linewidth]{figs/workflow-v2.pdf}
    \caption{The logical steps of how \tool customize DNNs of MLaaS for individual applications.
    % \jc{(1) "code" => "app source code"; "loss function" => "app-specific loss function"
    % (2) this might mislead people to think we use the same loss function for all apps. let's just use one code, not multiple.
    % (3) annotate the top part by "creation of app-specific loss function for a given application", and the bottom part "training DNN based on the app-specific loss function"}
    }
    \label{fig:general_description}
\end{figure}
\mypara{Goal}
For an application that uses MLaaS, our goal is to efficiently train an ML model (in the form of DNN) at the MLaaS backend such that its inference outputs minimize critical errors for this application (\ie application-decision failures, see \S\ref{sec:definitions}), rather than {\em any} misprediction/misclassification of API outputs.
To state this objective formally, we denote how an application makes a decision by $\z = \Appdecision(\DNN(\x))$, where $\x$ is the input to the ML API and $\DNN(x)$ is the inference result of the backend DNN. 
Then for a given decision process of $\Appdecision(\cdot)$ and input set $\X$, our goal is an ML model $\DNN(\cdot)$ such that the number of wrong decisions are minimized:
\begin{equation}
    \min \left|\{\x_\InputId \in \X \textrm{ s.t. } \Appdecision(\DNN(\x_\InputId)) \neq \Appdecision(\hat{\y_\InputId})\}\right|
    \label{eq:goal}
\end{equation}
\noindent
where $\hat{\y_\InputId}$ is the inference ground truth under input $\x_\InputId$. 

\mypara{Logical steps of \tool}
Given our goal of training a DNN to optimize the formulation of Eq.~\ref{eq:goal}, we can break it down to three logical steps: 
\begin{packeditemize}
\item First, to train DNN for Eq.~\ref{eq:goal} efficiently, the MLaaS backend needs to quickly determine if a DNN inference output $\DNN(\x)$ will lead $\Appdecision(\cdot)$ to make an incorrect decision (\ie critical errors), but given that ML applications could be complex, running them in entirety might arbitrarily slow down the MLaaS backend.
% \item First, we need to determine if a DNN inference output $\DNN(\x)$ will lead $\Appdecision(\cdot)$ to make an incorrect decision (\ie critical errors) without running the entire application, which could drastically slow down the
% training process and may not be feasible for the MLaaS backend
% for security concerns or application-dependency issues\shan{JC, we may need to discuss about this.}.
%only be accessible by developers/users.
To this end, \tool first extracts a \emph{\summary} (explained shortly) from an application's source code to characterize how decisions are made by the application based on ML API output (details in \S\ref{sec:extract})
\item While \summary indicates when a DNN inference error is critical or not for an application, it is not in a form that can be directly used to train a DNN to minimize its critical errors. 
Therefore, based on the \summary, \tool creates an application-specific {\em loss function} used for DNN training, which only penalizes critical errors of DNN output with respect to a given application (details in \S\ref{sec:loss}). 
\item The loss function will then be used to train a customized DNN to be run by MLaaS for this particular application's queries (details in \S\ref{sec:runtime}).
\end{packeditemize}
% (1) how to judge the correctness of $\Appdecision(\DNN(\x))$ without running the application in MLaaS backend, which is both slow and in-secure

%how to automatically extract function $\Appdecision(\cdot)$ from application source code, 
% (2) how to train the ML model $\DNN(\cdot)$ to optimize Eq.~\ref{eq:goal}.

\begin{comment}
Given our problem setting, the formulation of Eq.~\ref{eq:goal} implies two high-level challenges: 
(1) how to judge the correctness of $\Appdecision(\DNN(\x))$ without running
the application in MLaaS backend, which is both slow and in-secure\shan{The original text says ``how to automatically extract $\Appdecision(\cdot)$''. I feel
there was a logical gap in the original text, and hence made a change here. Please proofread.},
%how to automatically extract function $\Appdecision(\cdot)$ from application source code, 
and 
(2) how to train the ML model $\DNN(\cdot)$ to optimize Eq.~\ref{eq:goal}.


% \smallskip
% \noindent
\mypara{Logical workflow of \tool}To solve the aforementioned two problems, \tool has two logical steps, as depicted in Figure~\ref{fig:general_description}.
It first extracts a \emph{\summary} (explained shortly) from an application's source code to characterize how decisions are made by the application based on ML API output (details in \S\ref{sec:extract}).
Based on the \summary, \tool creates an application-specific loss function used for DNN training, through separating the ML API's critical errors that leads to incorrect application decisions from non-critical errors (details in \S\ref{sec:loss}). 
The loss function will then be used to train a customized DNN to be run by MLaaS for this particular application's queries (details in \S\ref{sec:runtime}).
% uses general framework to describe the application's decision process. 
% The general framework can identify critical errors for the application, and then be used to construct a new \emph{app-specific loss function} to train the DNN. 
% First, a \emph{decision-process summary} of the application is extracted from an application \App's source code.
% Secondly, application \App's decision process is viewed in a general framework of the \summary, which can identify critical errors of \App. 
% The critical errors are then used to create an \emph{app-specific loss function}, which is then used to train the DNN in order to minimize the critical errors. 
\end{comment}

At a high-level, a {\bf \summary} extracted from an application uniquely specifies\shan{JC, I have concerns with ``uniquely specifies''. I still think this is an abstraction. \summary actually throws away some details of an application-decision process, and only keeps the ones that help determine
criticality of an error. I would prefer that we say ``a \summary extracted from an application offers an abstraction of $\Appdecision(\cdot)$ that can be used to determine if a DNN inference ....''} $\Appdecision(\cdot)$, which can be used to determine if a DNN inference output is a critical error or not.
% \shan{We need to discuss this. 
% With $\Appdecision$, we can infer which errors are critical, but the former
% does not equal the latter.
% To me, a \summary is an abstraction of $\Appdecision(\cdot)$. It allows 
% us to precisely judge which errors are critical without running application code.
% }
Specifically, a \summary includes three pieces of information: 
\begin{packeditemize}
\item \emph{Composition of \targets:} 
% \shan{``Value type'' is ambiguous, because ``string'' and ``floating point'' are also value types. I would recommend saying ``Composition of \targets''} \yh{sounds good}: 
label set or value range; 
\item {\em Decision type:} \term{True-False}, \term{Multi-Choice}, or \term{Multi-Select};
\item {\em Mapping order:} over the target classes, \term{API-output order} or \term{application-choice order}, if the application makes a \term{Multi-Choice} decision.
\end{packeditemize}
For a concrete example, the \summary of the garbage classification application in Figure~\ref{fig:code}(a) contains
(1) three list of labels representing three \targets: \code{Recycle}, \code{Compost}, and \code{Donate}; 
(2) \term{Multi-Choice} type of decision; and 
(3) following \term{API-output order} to reach a decision.  

% These three pieces of information uniquely describe which errors are critical and which are non-critical to the application, and they will be used to customize the ML model for the application, as elaborated in \S\ref{sec:loss}. 


\mypara{What is changed by \tool, what is not}
It is important to notice that \tool does {\em not} change the ML API or the source code or the executable of the application.
Unlike recent work that aims to shrink or speedup DNNs~\cite{mullapudi2019online,kang2018blazeit,kang2017noscope}, we do not change the architecture (shape and input/output interface) of the DNN run by MLaaS; 
instead, we improve the DNN to minimize critical errors (application-decision failures).
That said, \tool does change two things. 
First, the application developers need to run \tool's parser script to extract the \summary.
Second, \tool modifies the MLaaS backend to re-train an ML model per application, instead of serving the same model to all applications, and selects the right ML model to serve each query.
\S\ref{sec:extract} and \ref{sec:runtime} will explain why these changes are practical.


The remaining of this section will begin with the design of app-specific loss function, the critical component in training/customizing the ML model $\DNN(\cdot)$ to optimize Eq.~\ref{eq:goal}, followed by how to extract the \summary from application source code, and finally, how the customized ML models are used to serve ML API queries in runtime.



\subsection{App-specific loss function}
\label{sec:loss}

\tool solves Eq~\ref{eq:goal} 
% \shan{Eq1 already included a 
% ``min''. We cannot say minimize a ``min(...)'' expression. Can we?} 
by training a DNN model with a {\em new loss function}.\footnote{A careful reader might notice that the formulation in Eq.~\ref{eq:goal} also depends on the input set $\X$.
Though the input set should ideally follow the same distribution of real user inputs of the application, this distribution is hard to obtain in advance and may also vary over time and across users.
Instead, we focus our discussion on training the ML model to minimize Eq.~\ref{eq:goal} with an assumed input distribution. Our evaluation (\S\ref{sec:evaluation}) will test the resulting model's performance over different input distributions.}
We should notice that in Eq~\ref{eq:goal}, the ML model output $\DNN(\x)$ may not be directly returned to user applications.
For instance, an image classification model's output is a vector of confidence scores between 0 and 1 (with the $\LabelId^{th}$ score indicating how confident the model is about if the $\LabelId^{th}$ label exists in the image), but the ML API backend will use a threshold $\theta$ to filter and return only labels with scores higher than $\theta$.
Because this post-processing (\eg thresholding) will not be optimized as part of DNN training, it is captured as part of $\Appdecision(\cdot)$ in the formulation of Eq~\ref{eq:goal}.
% We should clarify that this formulation keeps the ML API between user application and MLaaS intact. 
\jc{Shan, do the last few sentences address the original comments?}

% In Eq~\ref{eq:goal}, such post-processing is viewed as part of the decision process $\Appdecision$\shan{???this seems counter-intuitive.}.
% This way\shan{??Why do we need the earlier claim to not need to modify ...?}, we do not need to modify the input/output of the ML model $\DNN(\cdot)$ or its training process, except using a different loss function.
% So \emph{how to design a loss function that can achieve our customization goal?}




\myparaq{Why is it challenging}
We first consider a straightforward design of a loss function, called \toolbasic, and explain its limitations. 
\toolbasic also uses information in \summary.
% but it only considers which labels are in target classes and which are not. 
Specifically, \toolbasic 
% With the observation that applications typically heavily cluster on a small subset of labels appearing in the target classes(\S\ref{sec:empirical}), we naively come up with a \emph{strawman} of loss function design: 
assigns a higher penalty on errors of the ML model on inputs whose correct decisions are one or multiple of the target classes. 
Take image classification as an example.
The loss function on an input image is the binary cross entropy between the confidence-score vector of $\DNN(\x)$ and the ground-truth binary vector ($\hat{\y}$) with each correct label having a 1\shan{???}.
% Take the classification task  as an example to illustrate this idea. 
% For an image, an ML model returns a vector of confidence scores ($\API(\x)=\y$), each score for one of a label, and the ground truth is a vector of binary scores ($\hat{\y}$) with each ground-truth label getting a score of 1.
% The loss function is the cross entropy between the two vectors.
If the ground truth leads to the selection of a target class, \toolbasic will penalize the cross-entropy value by multiplying it with a high weight. 


% The ground truth is a list, where the $j^{th}$ element is 1 if the $j^{th}$ label exists in the input, and 0 otherwise. 
% The pre-trained model is trained to reduce the \emph{average} errors between the probabilities and the ground truth across a wide range of labels (\eg 9605 labels in Open Images~\cite{ASL}).
% On the other hand, 

% \jc{shouldn't we use ``confidence scores'' as opposed to ``probability''? probably ``probability'' is used in some context, but it's confusing --- no one uses these scores as probability to draw values..} \yh{Sure}

% \myparaq{Why not \toolbasic}
While \toolbasic penalizes errors involving labels in \targets,\footnote{Indeed, it is a typical modification to loss function, when the cost of errors on certain labels is higher than those on other labels (\eg~\cite{mcdnn}).} it fundamentally {\em cannot} separate critical errors (that yield different application decisions) from non-critical errors.
This is because it misses two crucial aspects of a decision process: 
{\em (i)} which the values (labels or values) belong to the same \target and which do not; and
{\em (ii)} the mapping order over the \targets\shan{Make sense, but the writing needs to be sharpened.}.
% Therefore, \toolbasic cannot separate critical errors (that yield different application decisions) from non-critical errors.
As a result, for instance, in the garbage classification application (Figure~\ref{fig:code}(a)), \toolbasic will give an equal penalty to 
% However, the strawman penalizes mis-classifications within one target class, such as 
a critical error of mis-classifying a \code{Paper} image to \code{Wood} and a non-critical error of mis-classifying a \code{Paper} image to \code{Shirt}.
\shan{Do you have a quick example that explains point (ii) as well?}


% we first introduce a general description of different decision processes and the \tool's design based on this general description, before detailing the loss function design case-by-case.
% Specifically, \tool's loss function expresses the target classes and matching orders in a {\em differentiable} form, such that it can be plugged into model training.
% To handle the critical errors of various applications, we first introduce a general description of different decision processes.
% , and this type of errors are non-critical to the application.
% because the strawman is unaware that different applications may make different decisions given the same output (\eg \emph{True-False}, \emph{Multi-select}, and \emph{Multi-choice}) and how these decisions affect the severity of ML model errors
% \shan{This last sentence is not clear.}. 



% \begin{equation}
% L(y_i) = w_i \cdot T_i \cdot L_{BCE}(y_i) + (1-T_i) \cdot L_{BCE}(y_i)
% \end{equation}
% where $w_i$ is a large weight (\eg $w_i = 20$), and $T_i = 1$ if the ground-truth labels of the $i^{th}$ sample overlap with the applications' target classes, and 0 otherwise. 


% Intuitively, this \emph{strawman} loss function is compatible with our goal since it prioritizes the reduction of the loss on the samples belonging to the target classes than the non-target ones. 






% We propose a new loss function directly constructed from the \summary.
% \yh{Why they fails and we do not fail }
% \yh{add general recipe }


% \begin{figure*}
%      \includegraphics[width=\linewidth]{figs/loss.pdf}
%     \caption{Decision processes of applications under our study (\S\ref{sec:empirical}) can be equivalently described in a general framework. 
% %     Here is an example of using the general formula to describe a decision process (top) on the DNN output $\y$ (bottom-left).
% % The \score $\M_\ClassId(\y)$ of \target $\ClassId$ is the highest confidence score in $\y$ associated with any label in the \target, because the labels in \code{detection\_labels} are sorted in descending order of their confidence scores, so the highest-score label in each \target is always matched first.
% % It then goes through the three \targets in the order of $\M_{Landmark}(\y)$, $\M_{Building}(\y)$, and $\M_{Person}(\y)$ (\ie following the if-else statements in the code), and in this case, the break occurs after matching the \target of \code{Building}.
% % This is because this is a \term{Multi-Choice application choice} process (\ie return on the first match), and the \score of the first \target ($\M_{Landmark}(\y)$) is below the threshold $\theta=0.5$. \jc{Yuhan, let's discuss an alternative of fig 4. i think the current fig (in a simplified form) serves well for the case study, but doesn't help much for people to understand the general idea of code -> abstract framework -> critical errors -> loss function. we need a more direct illustration of this thought process. ping me when you get a chance. thanks!
% Here is an example of using the general formula to describe a decision process (right) on the DNN output $\y$ (left). 
% % \yh{TODO: more explanation on penalization on critical errors}
% }
% % only labels with confidence scores over $\theta=0.5$ can be matched with \target, and $\M_{Building}(\y)$ is the first to exceed $\theta$.
%     % at a high level, the process first calculates the effective score of each target class (??), ranks them in an order (??), and traverse the target classes until a break (??). \tool's loss function for a \term{Multi-Select} example. \yh{Other, don't }
    
% \label{fig:loss}
% \end{figure*}

\shan{We need to change the tone a bit. The writing sounds really like \tool versus \tool-basic, which is the wrong tone.}

In contrast, \tool's loss function only penalizes critical errors specific to each application's decision process, rather than all errors in the DNN output. 
At a high level, our loss function converts the logic of an application's decision process to a differentiable form that penalizes critical errors (which cause different decisions than the correct ones).


\mypara{A generic description of decision processes}
Since the decision processes vary greatly across applications (\S\ref{subsec:observations}), we first introduce how \tool conceptually captures a range of decision processes and their critical errors using a generic description, which allows us to derive the mathematical form of \tool's loss function for individual applications.
For each of these applications in our study (\S\ref{sec:methodology}), our insight is that its decision process can be viewed as traversing a sequence of conditional {\em checks} until a {\em break} occurs, as follows. 
\vspace{-0.2cm}
\begin{align*}
\textrm{The }1^{st}\textrm{ check:} &<\y^{(1)},\ClassId^{(1)}>\rightarrow\Match^{(1)}&\\
&\dots&\\
\textrm{The }\TraverseId^{th}\textrm{ check:} &<\y^{(\TraverseId)},\ClassId^{(\TraverseId)}>\rightarrow\Match^{(\TraverseId)}& \Leftarrow \textrm{break}\\
&\dots&
\vspace{-0.2cm}
\end{align*}
where the $\TraverseId$-th conditional check takes as input a score vector $\y^{(\TraverseId)}$ (which is typically a masked vector of DNN output $\y$ with only score of certain label left) and one of \targets $\ClassId^{(\TraverseId)}$, and returns a binary $\Match^{(\TraverseId)}$ indicating whether $\y^{(\TraverseId)}$ {\em matches} the condition of $\ClassId^{(\TraverseId)}$ and a binary decision whether this check happens before the break.
The set of \targets of checks with $\Match^{(\TraverseId)}=True$ before the break will be the decision.
Figure~\ref{fig:loss} shows a concrete example of such generic description for a particular decision process and DNN output.

The specifics of this generic description (the score used in each conditional check, the traversal order of the checks, and when the break occurs) depend on the given decision process as well as the DNN output $\y$. 
We stress that this generic description may {\em not} apply to all applications, but it does apply to all applications in our study (\S\ref{sec:methodology}). 


\begin{figure}
\centering
     \includegraphics[width=0.9\linewidth]{figs/loss-v2.pdf}
    \caption{Decision processes of our studied applications (\S\ref{sec:empirical}) can equivalently converted to a generic description. 
(a) shows an example application, and (b) is the generic description of its decision process on DNN inference output $\y$, which based on the decision process is a sequence of checks, each matching some scores in $\y$ against a \target.
Such generic description helps \tool to categorize critical errors and derive loss function.
}
\label{fig:loss}
\end{figure}

\mypara{Categorization of critical errors}
Importantly, this generic description  nevertheless suffices to categorize critical errors:
\begin{packeditemize}
\item {\em Type-1 Critical Errors:} A correct \target $\ClassId$ is matched only after the break.
\item {\em Type-2 Critical Errors:} A correct \target $\ClassId$ is never matched, before or after the break.
\item {\em Type-3 Critical Errors:} An incorrect \target $\ClassId$ is matched before break. 
\end{packeditemize}
A nice property of this categorization is that any wrong decision (a correct \target not being picked, or an incorrect \target being picked) falls in a unique category, and non-critical errors do not belong to any category.
In other words, as long as the loss function penalizes the occurrences of each category, it will only capture all but only critical errors.


% \begin{packeditemize}
% \item {\em Type-1 Critical Errors:} A correct \target $\ClassId$ is never traversed in any conditional checks before the break.
% \item {\em Type-2 Critical Errors:} A correct \target $\ClassId$ is traversed 
% before the break, but each time (\eg at the $\TraverseId^{th}$ check) the score vector $\y^{(\TraverseId)}$ used does not match $\ClassId$'s condition.
% \item {\em Type-3 Critical Errors:} An incorrect \target $\ClassId$ is traversed in some check (\eg at the $\TraverseId^{th}$ check) before the break, and the score vector $\y^{(\TraverseId)}$ used match $\ClassId$'s condition.
% \end{packeditemize}


\mypara{\tool's loss function} 
This categorization of critical errors then allows \tool to derive a loss function that penalizes each type of critical errors.
We explain the loss function in the context of ``label-based API, \term{Multi-Choice} type of decision, and \term{application-choice order}'' (defined in \S\ref{subsec:observations}), one of the most common types of decision processes in the studied applications. 
\S\ref{sec:loss_appendix} will enumerate other types of decision processes.
The example in Figure~\ref{fig:loss} shows such an application. 
Mathematically, the loss function is then comprised of three terms, each penalizing one type of critical errors:
{\small
\begin{align}
     L(\y) &=   
 % \overbrace{ \sum_{\ClassId\leq\hat{\ClassId}} \textrm{Sigmoid}\left(\max_{\LabelId\in\TargetSet_{\ClassId}}\y[\LabelId]-\theta\right)}^{\substack{\text{\sf \footnotesize {{\bf Type-1} Critical Errors}} }} +
  \overbrace{ \textrm{Sigmoid}\left(\min\left(\max_{\LabelId \in \cup_{\ClassId < \hat{\ClassId}}\TargetSet_{\ClassId}}\y[\LabelId],\max_{\LabelId\in\TargetSet_{\hat{\ClassId}}}\y[\LabelId]\right)-\theta\right)}^{\substack{\text{\sf \footnotesize {{\bf Type-1} Critical Errors}} }} \label{eq:loss_app} \\&+
 \overbrace{ \textrm{Sigmoid}\left(\theta-\max_{\LabelId\in\TargetSet_{\hat{\ClassId}}}\y[\LabelId]\right)}^{\substack{\text{\sf \footnotesize {{\bf Type-2} Critical Errors}} }} + 
 \overbrace{ \sum_{\ClassId<\hat{\ClassId}}\textrm{Sigmoid}\left(\max_{\LabelId\in\TargetSet_{\ClassId}}\y[\LabelId]-\theta\right)}^{\substack{\text{\sf \footnotesize {{\bf Type-3} Critical Errors}} }}\nonumber
\end{align}
}
Here, $\y[\LabelId]$ denotes the score of the label $\LabelId$, $\TargetSet_\ClassId$ denotes the set of labels in the match condition of \target $\ClassId$, $\hat{\ClassId}$ denotes the correct (\ie ground-truth) \target, and the sigmoid function $\textrm{Sigmoid}(x)=\frac{1}{1+e^{x}}$ will incur a high penalty on positive inputs.
Given this application is \term{multi-choice}, the break occurs right after the first match of a \target, \ie the first check with a $\ClassId$ such that $\max_{\LabelId \in \TargetSet_{\ClassId}}\y[\LabelId]\geq\theta$.
\jc{Yuhan, we need to explain why such a confidence threshold $\theta$ exists. i understand dnns commonly use thresholds like this, but we need to remind people that. also, any evidence that real APIs do threshold DNN output? did we pick threshold 0.3 for some reason? maybe it leads to similar DNN output as real API output?}

{\em Why do these terms capture the critical errors?} 
Here, we intuitively explain why Eq~\ref{eq:loss_app} captures each type of errors (see \S\ref{sec:loss_appendix} for formal proofs). 
% Intuitively (see \S\ref{sec:loss_appendix} for formal proofs), because this is a \term{multi-choice} application (break at the first match) and it goes through labels in \code{detection\_labels} in descending order of their confidence scores, $\MaxScore$ is the score of the first matching label and is also when the break occurs.
\begin{packeditemize}
\item Recall that a Type-1 critical error occurs, if the correct \target $\hat{\ClassId}$ is matched after the break.
The correct \target $\hat{\ClassId}$ is matched, if and only if at least one of its labels has a score above the confidence threshold, $\max_{\LabelId\in\TargetSet_{\hat{\ClassId}}}\y[\LabelId]\geq\theta$).
And this match happens after the break, if and only if some \target $\ClassId$ before $\hat{\ClassId}$ (\ie $\ClassId<\hat{\ClassId}$) is matched (\ie for some $\ClassId < \hat{\ClassId}$, $\max_{\LabelId \in \TargetSet_{\ClassId}}\y[\LabelId]\geq\theta$).
The first term of Eq~\ref{eq:loss_app} penalizes any occurrence of these conditions. 
\item A Type-2 critical error occurs, if the no label in the correct \target $\hat{\ClassId}$ has a score high enough for $\hat{\ClassId}$ to be matched, \ie $\max_{\LabelId\in\TargetSet_{\hat{\ClassId}}}\y[\LabelId] < \theta$.
The first term of Eq~\ref{eq:loss_app} penalizes any occurrence of this condition.
\item A Type-3 critical error occurs, if any incorrect \target $\ClassId$ before $\hat{\ClassId}$ (\ie $\ClassId<\hat{\ClassId}$) has a label with score high enough for $\ClassId$ to be matched, \ie $\max_{\LabelId\in\TargetSet_{\ClassId}}\y[\LabelId]-\theta$.
The third term of Eq~\ref{eq:loss_app} penalizes any occurrence of this condition.
\end{packeditemize}






To successfully train a DNN model, the loss function must be differentiable with respect to any DNN ouput. 
% It is important to note that optimizers used in ML(\eg Adam)
% % \jc{you tend to add references on non-essential terms, } 
% to train  models are gradient-based. 
% Thus, the loss function (\ie every function in the composite function) needs to be differentiable in order to calculate the gradient of the loss value with respect to the DNN output. 
Note that in Eq~\ref{eq:loss_app}, the $\max$ function is used at multiple places, but it can be equivalently expressed in a differentiable form (we use the differentiable operators in PyTorch Autograd~\cite{paszke2017automatic}).

==> bk/backups_before_fist_submission/3-2-v3.tex <==
\tightsubsection{High-level workflow and key components}
\label{sec:overall}


\begin{figure}
    \centering
    % \includegraphics[width=\linewidth]{figs/workflow.pdf}
    \includegraphics[width=\linewidth]{figs/workflow-v2.pdf}
    \caption{The logical steps of how \tool customize DNNs of MLaaS for individual applications.
    % \jc{(1) "code" => "app source code"; "loss function" => "app-specific loss function"
    % (2) this might mislead people to think we use the same loss function for all apps. let's just use one code, not multiple.
    % (3) annotate the top part by "creation of app-specific loss function for a given application", and the bottom part "training DNN based on the app-specific loss function"}
    }
    \label{fig:general_description}
\end{figure}
\mypara{Goal}
For an application that uses MLaaS, our goal is to efficiently train an ML model (in the form of DNN) at the MLaaS backend such that its inference outputs minimize critical errors for this application (\ie application-decision failures, see \S\ref{sec:definitions}), rather than {\em any} misprediction/misclassification of API outputs.
To state this objective formally, we denote how an application makes a decision by $\z = \Appdecision(\DNN(\x))$, where $\x$ is the input to the ML API and $\DNN(x)$ is the inference result of the backend DNN. 
Then for a given decision process of $\Appdecision(\cdot)$ and input set $\X$, our goal is an ML model $\DNN(\cdot)$ such that the number of wrong decisions are minimized:
\begin{equation}
    \min \left|\{\x_\InputId \in \X \textrm{ s.t. } \Appdecision(\DNN(\x_\InputId)) \neq \Appdecision(\hat{\y_\InputId})\}\right|
    \label{eq:goal}
\end{equation}
\noindent
where $\hat{\y_\InputId}$ is the inference ground truth under input $\x_\InputId$.\footnote{A careful reader might notice that the formulation in Eq.~\ref{eq:goal} also depends on the input set $\X$.
Though the input set should ideally follow the same distribution of real user inputs of the application, this distribution is hard to obtain in advance and may also vary over time and across users.
Instead, we focus our discussion on training the ML model to minimize Eq.~\ref{eq:goal} with an assumed input distribution. Our evaluation (\S\ref{sec:evaluation}) will test the resulting model's performance over different input distributions.}
\footnote{We should notice that in Eq~\ref{eq:goal}, the ML model output $\DNN(\x)$ may not be directly returned to user applications.
For instance, an image classification model's output is a vector of confidence scores between 0 and 1 (with the $\LabelId^{th}$ score indicating how confident the model is about if the $\LabelId^{th}$ label exists in the image), but the ML API backend will use a threshold $\theta$ to filter and return only labels with scores higher than $\theta$.
Because this post-processing (\eg thresholding) will not be optimized as part of DNN training, it is captured as part of $\Appdecision(\cdot)$ in the formulation of Eq~\ref{eq:goal}.
% We should clarify that this formulation keeps the ML API between user application and MLaaS intact. 
\jc{Shan, do the last few sentences address the original comments?}}

\mypara{Logical steps of \tool}
Given our goal of training a DNN to optimize the formulation of Eq.~\ref{eq:goal}, we can break it down to three logical steps: 
\begin{packeditemize}
\item First, to train DNN for Eq.~\ref{eq:goal} efficiently, the MLaaS backend needs to quickly determine if a DNN inference output $\DNN(\x)$ will lead $\Appdecision(\cdot)$ to make an incorrect decision (\ie critical errors), but given that ML applications could be complex, running them in entirety might arbitrarily slow down the MLaaS backend.
To this end, \tool first extracts a \emph{\summary} (explained shortly) from an application's source code to characterize how decisions are made by the application based on ML API output (details in \S\ref{sec:extract})
\item While \summary indicates when a DNN inference error is critical or not for an application, it is not in a form that can be directly used to train a DNN to minimize its critical errors. 
Therefore, based on the \summary, \tool creates an application-specific {\em loss function} used for DNN training, which only penalizes critical errors of DNN output with respect to a given application (details in \S\ref{sec:loss}). 
\item The loss function will then be used to train a customized DNN to be run by MLaaS for this particular application's queries (details in \S\ref{sec:runtime}).
\end{packeditemize}


At a high-level, a {\bf \summary} extracted from an application uniquely specifies\shan{JC, I have concerns with ``uniquely specifies''. I still think this is an abstraction. \summary actually throws away some details of an application-decision process, and only keeps the ones that help determine
criticality of an error. I would prefer that we say ``a \summary extracted from an application offers an abstraction of $\Appdecision(\cdot)$ that can be used to determine if a DNN inference ....''} $\Appdecision(\cdot)$, which can be used to determine if a DNN inference output is a critical error or not.
% \shan{We need to discuss this. 
% With $\Appdecision$, we can infer which errors are critical, but the former
% does not equal the latter.
% To me, a \summary is an abstraction of $\Appdecision(\cdot)$. It allows 
% us to precisely judge which errors are critical without running application code.
% }
Specifically, a \summary includes three pieces of information: 
\begin{packeditemize}
\item \emph{Composition of \targets:} 
% \shan{``Value type'' is ambiguous, because ``string'' and ``floating point'' are also value types. I would recommend saying ``Composition of \targets''} \yh{sounds good}: 
label set or value range; 
\item {\em Decision type:} \term{True-False}, \term{Multi-Choice}, or \term{Multi-Select};
\item {\em Mapping order:} over the target classes, \term{API-order} or \term{App-order}, if the application makes a \term{Multi-Choice} decision.
\end{packeditemize}
For a concrete example, the \summary of the garbage classification application in Figure~\ref{fig:code}(a) contains
(1) three list of labels representing three \targets: \code{Recycle}, \code{Compost}, and \code{Donate}; 
(2) \term{Multi-Choice} type of decision; and 
(3) following \term{API-output order} to reach a decision.  



\mypara{What is changed by \tool, what is not}
It is important to notice that \tool does {\em not} change the ML API or the source code or the executable of the application.
Unlike recent work that aims to shrink or speedup DNNs~\cite{mullapudi2019online,kang2018blazeit,kang2017noscope}, we do not change the architecture (shape and input/output interface) of the DNN run by MLaaS; 
instead, we improve the DNN to minimize critical errors (application-decision failures).
That said, \tool does change two things. 
First, the application developers need to run \tool's parser script to extract the \summary.
Second, \tool modifies the MLaaS backend to re-train an ML model per application, instead of serving the same model to all applications, and selects the right ML model to serve each query.
\S\ref{sec:extract} and \ref{sec:runtime} will explain why these changes are practical.


The remaining of this section will begin with the design of app-specific loss function, the critical component in training/customizing the ML model $\DNN(\cdot)$ to optimize Eq.~\ref{eq:goal}, followed by how to extract the \summary from application source code, and finally, how the customized ML models are used to serve ML API queries in runtime.



\tightsubsection{App-specific loss function}
\label{sec:loss}

\tool solves Eq~\ref{eq:goal} 
% \shan{Eq1 already included a 
% ``min''. We cannot say minimize a ``min(...)'' expression. Can we?} 
by training a DNN model with a {\em new loss function}.



\mypara{A generic description of decision processes}
Since the decision processes vary greatly across applications (\S\ref{subsec:observations}), we first introduce how \tool conceptually captures a range of decision processes and their critical errors using a generic description, which allows us to derive the mathematical form of \tool's loss function for individual applications.
For each of these applications in our study (\S\ref{sec:methodology}), our insight is that its decision process can be viewed as traversing a sequence of conditional {\em checks} until a {\em break} occurs, as follows. 
\vspace{-0.2cm}
\begin{align*}
\textrm{The }1^{st}\textrm{ check:} &<\y^{(1)},\ClassId^{(1)}>\rightarrow\Match^{(1)}&\\
&\dots&\\
\textrm{The }\TraverseId^{th}\textrm{ check:} &<\y^{(\TraverseId)},\ClassId^{(\TraverseId)}>\rightarrow\Match^{(\TraverseId)}& \Leftarrow \textrm{break}\\
&\dots&
\vspace{-0.2cm}
\end{align*}
where the $\TraverseId$-th conditional check takes as input a score vector $\y^{(\TraverseId)}$ (which is typically a masked vector of DNN output $\y$ with only score of certain label left) and one of \targets $\ClassId^{(\TraverseId)}$, and returns a binary $\Match^{(\TraverseId)}$ indicating whether $\y^{(\TraverseId)}$ {\em matches} the condition of $\ClassId^{(\TraverseId)}$ and a binary decision whether this check happens before the break.
The set of \targets of checks with $\Match^{(\TraverseId)}=True$ before the break will be the decision.
Figure~\ref{fig:loss} shows a concrete example of such generic description for a particular decision process and DNN output.

The specifics of this generic description (the score used in each conditional check, the traversal order of the checks, and when the break occurs) depend on the given decision process as well as the DNN output $\y$. 
We stress that this generic description may {\em not} apply to all applications, but it does apply to all applications in our study (\S\ref{sec:methodology}). 


\begin{figure}
\centering
     \includegraphics[width=0.9\linewidth]{figs/loss-v2.pdf}
    \caption{Decision processes of our studied applications (\S\ref{sec:empirical}) can equivalently converted to a generic description. 
(a) shows an example application, and (b) is the generic description of its decision process on DNN inference output $\y$, which based on the decision process is a sequence of checks, each matching some scores in $\y$ against a \target.
Such generic description helps \tool to categorize critical errors and derive loss function.
}
\label{fig:loss}
\end{figure}

\mypara{Categorization of critical errors}
Importantly, this generic description  nevertheless suffices to categorize critical errors:
\begin{packeditemize}
\item {\em Type-1 Critical Errors:} A correct \target $\ClassId$ is matched only after the break.
\item {\em Type-2 Critical Errors:} A correct \target $\ClassId$ is never matched, before or after the break.
\item {\em Type-3 Critical Errors:} An incorrect \target $\ClassId$ is matched before break. 
\end{packeditemize}
A nice property of this categorization is that any wrong decision (a correct \target not being picked, or an incorrect \target being picked) falls in a unique category, and non-critical errors do not belong to any category.
In other words, as long as the loss function penalizes the occurrences of each category, it will only capture all but only critical errors.

==> bk/backups_before_fist_submission/3-method-1123.tex <==
\label{sec:method}

\subsection{System architecture}

\begin{figure}
     \includegraphics[width=\linewidth]{figs/system_overview.pdf}
    \caption{System architecture of \tool. }
\label{fig:system}
\end{figure}
% \mypara{Main components}

% \mypara{Extracted Software decision process}

Figure~\ref{fig:system} shows the overall system architecture of \tool.
In the offline stage, the developers run a parser plugin locally, which extracted the software decision process from the application source code. The extracted software decision process is displayed in JSON format, consisting of: (1) the content of class lists used in branch conditions; (2) whether the application is making multi-select or multi-choice decisions; (3) the order of examination for applications making multi-choice decisions. Then, the developers will upload the JSON of software decision process to the MLaaS backend. On the MLaaS backend side, \tool will re-train the ML model by re-sampling the training data with a more focus on the classes appeared in the applications, and constucting loss functions which directly penalize the critical errors.

% In the online stage, 




% which consists of a parser plugin, an ML model re-training scheme run in the offline stage, and in the online stage, \tool selects the customized ML model based on applications' credentials, and run inference with the customized model.  


% 3.2: given the extracted json, how should we re-train teh model 
% 3.3. how to extract
% 3.4: how to change the run-time interface

% \tool is an automated framework that adapts the DNN behind the ML APIs, such that the number of software mis-behaviors can be greatly reduced when applied to an ML software. 

% \tool first performs static analysis to extract the code structure of the applications invoking MLaaS to understand how the software uses the ML API outputs to make application decisions. Then \tool constructs loss functions that penalize the critical errors of the applications. Finally, \tool re-trains the DNNs behind the ML APIs with the constructed loss function, without modifying the output interface of the ML APIs. 

% In this section, we will introduce how \tool performs static analysis and constructs the loss functions for the applications. 


% \subsection{Understanding Software Context}

% \subsection{Notations}
% \yh{not 3.2 }
% Denote the total number of classes that the DNN behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows:

% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the DNN behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}



\subsection{How to customize the ML model in the ML API backend}

We first start with introducing the re-training scheme in \tool. 


\yh{Outline of this section: 
1. first list the goal in math (or text): minimize the incorrect app decisions
2. a naive re-training scheme is to use a training data that  focuses on classes appeared in the apps 3. why this design is not good: it can only solve xxx, but not xxx 4. describe our loss function }
% \yh{goal: minimize the incorrect app decisions; what we have: extracted software decision process (key dimensions) }
As shown in our empirical study in Section~\ref{sec:empirical}, we find the software decision process can be characterized by two aspects: (1) the class list(s) or value ranges that are used in branch conditions (2) the structures of the branch conditions.

In this section, we will describe how we incorporate the software decision process in the loss function. Our optimization is composed of two steps: (1) clustering the training data to focus on classes appearing in the branch conditions; (2) constructing the loss functions to be aware of the software decision process. Our objective is to incur a high penalty on critical errors, and no penalty if the errors make no impact on the application. 


To begin with, we first introduce the loss function traditionally used in multi-label image classification.


The binary cross-entropy loss function used in multi-label classification task~\cite{ASL} is denoted as:
\begin{equation}
    L_{bce}  = -\frac{1}{n}\sum_{i=1}^n{(y_i\log(p_i) + (1 - y_i)\log(1 - p_i))} \,,
\end{equation}
where $y_i = 1$ if class $i$ is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. $p_i$ is the predicted probability for class $i$. 
% \begin{itemize}
%     \item  $y_i = 1$ if the $i^{th}$ class is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. 
%     \item $p_i$ is the predicted probability for the $i^{th}$ class.
% \end{itemize}
% where $y_i$ indicates whether the $i^{th}$ class exists in the input sample $I$ or not. In other words, $y_i = 1$ if the $i^{th}$ class exists in the input $I$, and $y_i = 0$ otherwise. \cc{It is still one sentence, so please do not start a new paragraph}


\subsubsection{Clustering training data}


To achieve the first step, one approach is to assign different weights to samples with ground-truth decisions of executing the \code{Others} branch and non-\code{Others} branches.  
We take a simple example to illustrate this approach. An application  defines one branch condition to check if the API outputs intersect with a class list $W_1$. $W_1$ is a non-empty subset of the whole label set $C$ that the DNN is able to classify. 
 The original fraction of images in the training data whose ground-truth  decisions are executing the \code{$W_1$}-branch (\ie $G \cap W \neq \emptyset$), which we refer to as \code{$W_1$}-samples,  is $A$. 
 % \cc{This sentence is very hard to read. Can we use phrase like ``which we refer to as $W$-images''?} 
The fraction of images whose ground-truth decisions are executing the \code{other}-branch is $1-A$,  which we refer to as \code{others}-samples. If we want to balance the distribution between $W$-samples and \code{others}-samples, we can use a loss function that assigns higher weights to \code{W}-samples:

\begin{equation}
    L_D = y_1 \cdot \frac{1}{A} \cdot L_{bce} + (1-y_1)\cdot A \cdot L_{bce} \,,
\end{equation}
where $y_1$ indicates whether this sample is a \code{$W$}-sample or not. In other words, $y_1 = 1$ when the sample is a \code{$W$}-sample ($G \cap W \neq \emptyset$), and $y_1 = 0$ otherwise ($G \cap W = \emptyset$). 
% \cc{This example seems to be T-or-F. Could we use consistency description as Section 3.4.2? }


% In this way, samples whose ground-truth decisions are selecting the \wl and those whose ground-truth decisions are selecting \code{others} are taking the same effect during training, instead of biasing towards either selecting the \wl or selecting \code{others}. 
In this way, \code{$W$}-samples and \code{others}-samples are taking the same effect during training, instead of biasing towards either \code{W} or \code{others}. 

% We construct loss functions for each type of software represented by the software examples shown in section~\ref{sec:empirical}. \cc{Maybe say some high-level ideas, more intuition}

\subsubsection{Branch condition structure 1: T-or-F} 

For the software that defines only one branch condition, checking if the output labels $O$ intersect with a class list $W_1$. We penalize the critical errors: (1) all the classes in $W_1$ are not included in top predictions for \code{$W_1$}-samples; or (2) at least one class in $W_1$ are included in top predictions for \code{others}-samples.



% \begin{equation}
% \left\{
% \begin{split}
%     L_{W_1} &= y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \\
%     P_1 &= xxx 
% \end{split}
% \right.
% \cc{Another format}
% \end{equation}

% \kt{$L_{W_i} = y_i (p_i\succ \theta) + (1-y_i) (\theta \succ p_i)$, where $y_1$ indicates whether ground truth contains classes inside $WL_1$ (in other word, ???=1, ???=0), $p_1$ is the maximum probability among white list 1 (\ie $WL_1$) and $\theta$ is the threshold used inside the ML API}.
% \cc{Some equations have numbers, some do not. Please make them consistent}

% \begin{itemize}
%     \item $y_1$ \cc{yuhan, this part is not finished yet}
% \end{itemize}

\begin{equation}
    L_{W_1} =y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \,,
\label{eq:loss}
\end{equation}
where
$y_1$ indicates whether this sample is a \code{$W_1$}-sample or not. 
In other words, $y_1 = 1$ if the sample is a \code{$W_1$}-sample, and $y_1=0$ if the sample is a \code{others}-sample. $\theta$ is the prediction threshold, where classes whose predicted probability will be included in the output label list. $P_1$ is the maximum probability of classes in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will denote as $S$ in the rest of the paper. 



Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for  \code{$W_1$}-samples. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-samples. Similarly for \code{other}-samples. 


% For example, in the example\cc{yuhan, please read these five words again to see what's the problem...} software shown in Figure~\ref{fig:tf_example}, given a prediction threshold of 0.5, when the probability scores of the labels in the specified \wl are $\langle0.2, 0.3, 0.4, 0.9\rangle$ for Dog, Mammal, Carnivore, and Wolf respectively in Figure~\ref{fig:input_example_tf_correct}, the penalty incurred by the loss function is 0.40. On the other hand, in Figure~\ref{fig:input_example_tf_wrong}, where the ground-truth labels include one of the labels in the \wl, thus the ML API should output at least one label in the \wl in order to produce the correct control flow decision. When the probability scores for  Dog, Mammal, Carnivore, and Wolf are $\langle0.2, 0.3, 0.35, 0.3\rangle$\cc{I use parenthesis to make them look like lists instead of random number. yuhan, could also change other places?} respectively, leading to none of the labels in the \wl being output, the penalty incurred by the loss function is 0.537. 


\subsubsection{Branch condition structure 2: M-to-N-set} 

 In M-to-N-set, several branch conditions are defined, each checking if a class list intersects with the API output $O$. All the fulfilled branches will be executed. We denote all the $m$ class lists the application uses in branch conditions as {$W_1$, ..., $W_m$}. In this pattern, the ground-truth  decisions is executing \emph{all} the branches whose class lists  intersect with the ground-truth labels. 

We derive the following loss function for M-to-N-set:
\begin{equation}
    L = \sum_{i=1,\cdots,m} y_i \cdot \textrm{S}(\theta - P_i) + (1-y_i) \cdot \textrm{S}(P_i - \theta) \,,
\end{equation}
where $y_i$ indicates whether  $W_i$ is among the branches the ground-truth decision executes, in other words, $y_i = 1$ if $G \cap W_i \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_i$ is the maximum probability of classes belonging to $W_i$ (\ie $P_i = max_{c \in W_i} p_c$). 

 Only if the application decisions led by $O$ exactly match with the ground-truth decisions, the penalty will be low.
 % \cc{be low or be zero? should we also mention the probability differences?}. 


% \kt{$\sum_{i=1,\cdots,N} L_{W_i}$}



\subsubsection{Branch condition structure 3: Priority-list}

Priority-list defines several branch conditions, and each of them is associated with a class list $W_i$. The application checks the branch conditions from highest to lowest priority until finding the first one whose class list intersects with API output labels $O$. Let $W_i$ (where $1 \leq i \leq m$) denote the class lists used in branch conditions, where class lists with smaller $i$ indicate higher priority. Let $W$ denote the union of the classes in all the whitelists, in other words, $W = \cup^{m}_{i=1}W_i$. The ground-truth decision  is executing the highest priority branch whose associated class list intersects with the ground-truth classes $G$. 

We derive the loss function as:
\begin{equation}
\begin{split}
    L = y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
    (1-y_i) \cdot \textrm{S}(P - \theta) \,,
\end{split}
\end{equation}
where $y_i = 1$ when the ground-truth decision is executing one of the branches in $\{ W_1, \cdots, W_m\}$ (\ie $G \cap W \neq \emptyset$), and  $y_i = 0$ when the ground-truth decision is executing the \code{others} branch. 
$k$ is the index of the highest-priority branch whose class list intersects with the ground-truth classes (\ie $k = \min \{i|WL_i \cap G \neq \emptyset\}$). $P_k$ is the maximum predicted probability for classes belonging to $W_k$, and $P_{k^{-}}$ is the maximum predicted probability out of the classes belonging to higher priority branches than the ground-truth branch (\ie $k^{-} = \min \{i | W_i \cap (G \setminus W ) \neq \emptyset \textrm{ and } i < k \}$). $P$ is the maximum probability of the classes belonging to $W$. 

Given this loss function, only if the highest-priority branch whose class list intersects with the predicted classes $O$ is the ground-truth decision, the penalty will be low. 

% \begin{equation*}
%     \footnotesize
%     \begin{split}
%     L(O, G) &=  \begin{cases}
%    P \Big( T, \max\limits_{c \in W} p_c \Big ), & G \cap W = \emptyset \\
%      P \Big( \max\limits_{c \in WL_k } p_c, T \Big ) + P\Big( \max\limits_{c \in WL_k} p_c, \max\limits_{c \in W \setminus WL_k} p_c \Big ), & G \cap W \neq \emptyset \\
% \end{cases}\\
% k &= \min \{i|WL_i \cap G \neq \emptyset\}
%     \end{split}
% \end{equation*}
% \kt{$L_{W_k}$, where $k=???$}


% Given this loss function, we can ensure that: (1) for images with ground-truth labels intersecting with at least one \wl, as long as the \wls that intersect with the output labels are not the one that ranked highest among those intersecting with the ground-truth labels, the penalty incurred by the loss function will be large; (2) for images with ground-truth labels that do not have an intersection with any of the \wls, as long as the output labels intersect with the labels in any of the \wls, the penalty incurred by the loss function will be large. 


% For example, in the example software \cc{I prefer directly writing down software name (if we already introduce it) or describe what type of software, e.g. trash classification application. It's hard for people to recall what happens only with the figure number} shown in Figure~\ref{fig:priority_input_example}, the prediction threshold is 0.5. In the input example in Figure~\ref{fig:input_example_priority_correct}, the probability scores of the labels in the Monument \wl are 0.2, 0.3 and 0.1 respectively, and the probability scores of the labels in the Construction \wl are 0.8, 0.2, 0.05, and the probability scores of the labels in the Person \wl are 0.45, 0.4, 0.2. The penalty incurred by the loss function is $Sigmoid(0.5-0.8)$ + $Sigmoid(0.45-0.8)$ = 0.8388. 

% On the other hand, in the input example in Figure~\ref{fig:input_example_priority_wrong}, the probability scores of the labels in the Monument \wl are 0.3, 0.2 and 0.15 respectively, and the probability scores of the labels in the Construction \wl are 0.7, 0.2, 0.1, and the probability scores of the labels in the Person \wl are 0.45, 0.8, 0.2. The penalty incurred by the loss function is $Sigmoid(0.5-0.3)$ + $Sigmoid(0.8-0.3)$ = 1.17. The penalty, in this case, is greater than the penalty in Figure~\ref{fig:input_example_priority_correct}, because labels in the highest-ranked \wl intersecting with the ground-truth labels do not appear in the output. 

\subsubsection{Branch condition structure 4: Top-label}

Top-label defines several branch conditions, and associates with each of them with a class list $W_i$, similar to Priority-list. However, unlike Priority-list, it checks the \emph{API output labels} one by one until one of them intersects with any of the class lists. Similar to the previous section, $W$ is the union of classes in all the defined class lists. We denote the classes belonging to class lists intersecting with ground-truth classes as $W^+ = \bigcup_{W_i \cap G \neq \emptyset} W_i$, and the classes belonging to \wls that do not intersect with ground-truth classes as $W^- = W \setminus W^+$.
 
In this pattern, the ground-truth decision is to execute the branch condition  whose class list  intersects with the ground-truth classes. 

We derive the loss function as:
\begin{equation}
    L = y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \,,
\end{equation}
where $y_i  = 1$ indicates that the ground-truth decision is executing one of the branches in \{$W_1$, $W_2$, ...$W_m$\}, and $y_i = 0$ indicates the ground-truth decision is selecting \code{others}, similarly to the previous section. $P^{+}$ is the maximum probability out of classes in $W^+$ (\ie $P^+ = \max_{c \in W^+ } p_c$), and $P^-$ is the maximum probability out of classes in $W^-$ (\ie $P^- = \max_{c \in W^- } p_c$). 
% \begin{equation*}
%     \footnotesize
%     L(O, G) =  \begin{cases}
%    P \Big( T, \max_{c \in W} p_c \Big ), & G \cap W = \emptyset \\
%      P \Big( \max_{c \in G \cap W } p_c, T \Big ) + P\Big( T, \max_{c \in W \setminus G } p_c \Big ), & G \cap W \neq \emptyset \\
% \end{cases}
% \end{equation*}

% \kt{$L_W$, where $W={\bigcap_{W_i \cup G\neq \phi} W_i}$ is ....}

Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 




\subsection{How to extract the software decision process}
% How we use sym-ex to get info, and which info 
\yh{Change all the whitelists}
To extract software context, we conduct an offline static analysis to detect code patterns introduced in Section~\ref{sec:empirical}. 
Particularly, we focus on the control-flow structures that are directly affected by ML API results. 

Given a code location of ML API invocation, \tool analyzes all the if-branches that have dependency on the ML API's output. For each combination of branch decisions, \tool adopts symbolic execution engine DSE~\cite{irlbeck2015deconstructing} and CVC5 constraint solver~\cite{cvc5} to find all the API outputs that lead to these decisions, which is the corresponding \wl.
If the software specifies only 1 branch condition, \tool reports pattern T-or-F. Otherwise, \tool analyzes the code structure to determine the pattern. % according to Figure~\ref{fig:hierarchy}:

\emph{How is the whitelist selected?} \tool analyzes all the statements inside the edges of an ML-API-related if-branch. If the software terminates all the examinations inside one of the branch edges (e.g., a break statement inside the loop and a return statement inside a function body), \tool regards that it as ``select 1 whitelist'' and further examines the order. 
If there is no such termination, \tool determines it is a M-to-N-set structure. 
% If there is no such termination, \tool determines whether it is pattern M-to-N-set or M-to-N-list according to the data structure of function returned value.

\emph{How is the order determined?} \tool finds all the loop structures and the equivalent statements outside the ML-API-related if-branches. It analysis their nested levels and the data dependency relationship of their iterators. 
If the software does not contain any loop iterating ML API's output or \wls, \tool stops examination and reports an absence of code pattern. 
If an inner (outer) loop iterates the ML API's output and the outer (inner) loop iterates the \wls, \tool regards it as pattern Priority-list (Top-label).  Note that, if the software contains multiple nested loops iterating the same variable, \tool focuses on the innermost one.


\subsection{How to change the MLaaS run-time backend}


% \subsection{Network Architecture}
% How we change the architecture of pre-trained model (freezing some part of the model)


% \subsection{Dataset Construction}



==> bk/backups_before_fist_submission/3-method-1126.tex <==
\label{sec:method}

\subsection{Key components and workflow}

\begin{figure}
     \includegraphics[width=\linewidth]{figs/system_overview.pdf}
    \caption{System architecture of \tool. 
    % \jc{the overall flow looks ok, but there are so many minor issues in this figure. just to name a few: 
    % (1) where is "cloud service" coming from? 
    % (2) (a) and (b) shouldn't be distinguished (see comment in 3.1).
    % (3) i thought we decided to drop the arrow of giving the parser to developer?
    % (4) why "software context" is still used?
    % (5) user is not running python code! they run real apps
    % (6) why calling it "prediction" instead of API output?
    % (7) what's "model inference code"? if it's simply selecting the right model to run, we shouldn't introduce a new term.
    % (8) the three customized models should be put side by side (either all vertically or horizontally),
    % (9) why calling them "adapted" ML model? if the term we always use is "customized", then stick to that.}
    % \jc{in general, EVERY word must be picked very carefully, which you clearly didn't do :)}
    \yh{fixed comments, I'm calling it ML-model outputs instead of API outputs because the outputs comes before the ``output interface'', thus it's not API outputs yet}
    \jc{sorry i disagree. again, don't introduce new terms unless really necessary, which i don't think is the case. why dont you change the figure, to move the output and input the left of the model output interface, which should also be changed to "ML API"?}
    \jc{and don't let arrows overlap with arrows or lines (e.g., Model pool, Select)}
    }
\label{fig:system}
\end{figure}
% \mypara{Main components}

% \mypara{Extracted Software decision process}
Guided by the empirical study in \S~\ref{sec:empirical}, we propose \tool, an optimization framework that extracts the software decision process of the applications querying the MLaaS, and customizes the ML-model in the MLaaS backend. 
% summarizes the overall workflow of \tool.


As shown in Figure~\ref{fig:system}, when the application is being developed, 
% \jc{the term offline is new. the contrast between offline and online is overcomplicating. can we say something like when the application is being developed?}
besides the existing development procedure, the developers also run an MLaaS-provided parser plugin on their own machines, 
% \jc{the ``parser'' comes from nowhere. who provides it? even a simple ``MLaaS-provided parser'' is better}
% \jc{``locally'' has many meanings. pick a more precise term}, 
which extracts a summary of the software decision process
% \jc{maybe we need a different term; ``key features'' invites unnecessary confusion when used in an ML-related paper. how about a ``summary of the application's decision process''?}
% \jc{``extracts xxx from app into a file'' sounds wrong. shouldn't it be ``extract xxx from an app and uploads it as a file to xxx''?} 
from the application source code (details in \S~\ref{sec:extract}), and uploads it as a file to the MLaaS backend. In the MLaaS backend, \tool constructs a loss function based on the uploaded file, re-trains the ML-model with the constructed loss function, and adds the re-trained ML-model into the model pool (details in \S~\ref{sec:loss}). 
Finally, 
% \jc{the last phrase can be deleted}
an application queries the MLaaS with inputs via the existing interface,  
the MLaaS backend selects and runs inference with the customized ML-model(details in \S~\ref{sec:runtime}). 
% \jc{the separation among the three stages (``developer'', ``retraining'' and ``run-time'') is unnecessarily complicating the flow, and it introduces unnecessary terms, like ``run-time''. }

\jc{when introducing the flow, shouldn't we also highlight what we DO change and what we do NOT change?}

% The software decision process extracted from the Python source code, is composed of the key features characterizing it.\cc{This sentence does not provide additional information. Also, we could mention python in the implementation section} 

\jc{please don't explain a concept together with an application. you should always explain the concept first, and THEN use an example to explain it in a specific context.}
The summary of the software decision process consists of three aspects: (1) what are the target classes?  (2) what is the type of decision out of \emph{True-False}, \emph{Multi-Choice}, or \emph{Multi-Select}? (3) if the application makes a \emph{Multi-Choice} decision, how does the application reach a decision? 
These three aspects can uniquely identify which errors are critical or non-critical to the applications. Identifying the critical errors, as discussed in \S~\ref{sec:empirical}, which vary greatly across applications, provides us with great opportunities to customize the ML-models per application. 

Take the garbage classification application in Figure~\ref{fig:code}(a) as an example to illustrate. The summary of the software decision process for this application contains: (1) the three target classes \code{Recycle}, \code{Compost}, \code{Donate}; (2) a \emph{Multi-Choice} decision; (3) it follows the \emph{API-output order} to reach the \emph{Multi-Choice} decision.  

\jc{this last sentence is important but quite misleading. first of all, these features don't uniquely describe a decision process (e.g., they dont say what decisions will be made for each branch). instead, they specify what errors are critical and what errors are not critical.
second, you didn't say WHY they SHOULD be used by \tool to customize the ML model.}


\begin{comment}
\jc{this definition is extremely important and should be elevated. i suggest explain it in a separate paragraph. so you will have two paragraphs: one explain the overall workflow, and the second explains what's extracted from the source code and used to customize ML-model. it's important to keep the 1st para short.} 
\jc{it should be explained more formally, probably with a simple example, and the terms (e.g., multi-select vs. multi-choice) should be tightly connected to when they are first defined. remember, many reviewers may have skipped (or missed) their definitions in section 2.} 
\jc{moreover, i wouldn't mention JSON at the beginning. the exact format (not the content in the file) seems secondary to me}
\jc{what about score ranges? we need a way to explain all cases under consideration} 
% used in branch conditions; (2) whether the application is making multi-select or multi-choice decisions; (3) the order of examination for applications making multi-choice decisions. Then, the developers will upload the JSON of software decision process to the MLaaS backend. On the MLaaS backend side, \tool will re-train the ML model by re-sampling the training data with a more focus on the classes appeared in the applications, and constucting loss functions which directly penalize the critical errors.
\jc{i wouldn't distinguish training data resampling and loss function as two separate steps. last time we met as a group, we decided to say changing loss function is all that's needed, though the real implementation does resampling to speedup training. i like this idea, so the distinction should be secondary.} 

\jc{regarding the terminology, the parser doesn't extract the entire application decision process, it merely extracts the key features of the application decision process, which include xxx}



\jc{now this is too low-level when explaining the workflow. here, you can just say ``each time an application calls the ML API, the ML API backend will select the ML-model model customized for the application, ...''}
% the applications submit inference request to the ML API with input and the credential, like 

\jc{two meta comments: 1. Yuhan, you should read the terms used in the new Section 2 and use them consistently in section 3.
2. when writing 3.1, please make sure that every important term appears with a forward pointer to a later subsection that explains it in detail as well as a pointer to Figure 4}
\end{comment}

% which consists of a parser plugin, an ML model re-training scheme run in the offline stage, and in the online stage, \tool selects the customized ML model based on applications' credentials, and run inference with the customized model.  


% 3.2: given the extracted json, how should we re-train teh model 
% 3.3. how to extract
% 3.4: how to change the run-time interface

% \tool is an automated framework that adapts the ML-model behind the ML APIs, such that the number of software mis-behaviors can be greatly reduced when applied to an ML software. 

% \tool first performs static analysis to extract the code structure of the applications invoking MLaaS to understand how the software uses the ML API outputs to make application decisions. Then \tool constructs loss functions that penalize the critical errors of the applications. Finally, \tool re-trains the ML-models behind the ML APIs with the constructed loss function, without modifying the output interface of the ML APIs. 

% In this section, we will introduce how \tool performs static analysis and constructs the loss functions for the applications. 


% \subsection{Understanding Software Context}

% \subsection{Notations}
% \yh{not 3.2 }
% Denote the total number of classes that the ML-model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows:

% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the DNN behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}



% \subsection{How to customize the ML model in the MLaaS backend}
\subsection{Customizing ML model for an application decision process}
\label{sec:loss}
As introduced in \S~\ref{sec:empirical},  applications in the wild differ greatly in their software decision processes. 
% For example, they may  define different number of target classes or include only a small subset of labels of the whole label set in their target classes and so on. 
This heterogeneity can lead to differences in critical errors\jc{remind people what critical errors are?} across applications. 
It is possible for an ML API error to be non-critical for one application, while critical for another. Thus, customizing the DNN in the MLaaS backend is important in order to incorporate the differences in software decision processes across applications.
\jc{the whole first paragraph is redundant to 3.1. this para should highlight why we start by explaining the step of DNN retraining}

The customization goal is to minimize the critical errors for each application.
% caused by ML API errors. 
Formally, the software decision process can be viewed as $\z = \Decision(\API(\x))$, where $\x$ is the input to the API, $\API(\x)$ is the ML API output, and $\Decision$ is the post-processing the application performs to make decisions based on API outputs. 
Let $\x_i\in \X$ denote the $i^{th}$ input, where $1 \leq i \leq M$, to the ML API, and $\hat{y_i}$ denote its ground-truth label. 
% $API(x_i)$ is a list of probabilities for label-based API (\eg image or text classification), 
% [$p_1, p_2, \dots, p_n$], for every label in the whole label set, and a score $O_i$ for score-based API (\eg sentiment analysis API). 
Formally, our customization goal is:
% Let $\mathds{1}_{x}$ denote the indicator function, where $\mathds{1}_{x} = 1$ when $x$ is \emph{True} and 0 otherwise. Therefore, the customization goal is:

\begin{equation}
    \min |\{x_i \in X | Decision(API(x_i)) \neq Decision(y_i)\}|
    \label{eq:goal}
\end{equation}

With this customization goal, together with the observation that applications typically heavily cluster on a small subset of labels in mind, we naturally come up with a \emph{strawman} of customization: re-train the ML-model with a re-sampled training dataset, which clusters on the labels appearing in the target classes of the application. 
While the original model is optimized to minimize average label-wise errors across a wide range of labels\footnote{Traditionally, the loss function minimizes the average error between the predicted probability and ground-truth labels for every class, which we refer to as average label-wise errors. } (\eg 9605 labels in Open Images~\cite{ASL}), this strawman approach can reduce the label-wise errors of labels belonging to the target classes. However, it is unaware that applications may make different decisions, including \emph{True-False}, \emph{Multi-select}, and \emph{Multi-choice}, and how these decisions affect the severity of ML API errors. 

Fortunately, the loss function used in ML-model training provides a \emph{differentiable} way to capture the incorrectness of the ML-model's predictions with respect to the ground-truth. In addition, we formulate the software decision process in a structured format. This allows \tool to translate it into a loss function with the goal of both clustering on labels in target classes and directly minimizing the critical errors (Equation~\ref{eq:goal}). 
% \yh{Why they fails and we do not fail }
% \yh{add general recipe }
Compared to the strawman which may spare energy penalizing non-critical errors, such as penalizing mis-classifications within the target classes, 
our solution only focuses on penalizing the critical ones, such as mis-classifications across target classes. 





As illustrated in \S~\ref{sec:empirical}, the critical errors in the applications can differ greatly for different target classes, types of decisions, and order of examination. As a result, we construct different loss functions, with the unified goal of minimizing critical errors, for each type of applications. 

A general recipe for our loss function is formulated as:

\begin{equation}
    L_i = H_{o}(\hat{y_i}) \cdot S(\theta-G(y_i)) + \sum_{j=1}^{m} H_j(\hat{y_i}) \cdot S(F(y_i)-G_j(y_i))  
\end{equation}

\mypara{True-False} This type of application defines only one target class, checking if the API outputs match with
% \cc{I suspect ``intersect'' is a better praise, as we the API output includes a list of items}
it. We denote the labels included in the target class as $W_1$. Therefore, the corresponding loss function is:
\begin{equation}
    L = y_i\cdot \frac{M}{N_1}  \cdot \textrm{S}(\theta - P_1) + (1-y_i) \cdot \frac{M}{M-N_1} \textrm{S}(P_1 - \theta) \,,
\label{eq:loss}
\end{equation}
where $y_i = 1$ when the ground-truth of the input intersects with the target class $W_1$, and $y_i=0$ otherwise. $\theta$ is the prediction threshold, where output labels whose predicted probability are greater than it will be included in the output label list. $P_1$ is the maximum probability of labels in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will keep the notation in the rest of the paper. $N_1$ is the total number of inputs in the training dataset whose ground-truth decision is the target class (\ie $N_1 = \sum\limits_{j=1}^{M}\mathds{1}_{\hat{y_j}\cap W_1 \neq \emptyset}$), denoted as target-inputs. The inputs whose ground-truth decision is selecting the non-target class are denoted as non-target-inputs. 


% With this loss function, \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-inputs. Similarly for \code{other}-inputs. 

Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for target-inputs. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for target-inputs. Similarly for non-target-inputs. 

Furthermore, to achieve the effect of clustering on labels in $W_1$, the loss function applies a weight of $\frac{M}{N_1}$ on target-inputs, and a weight of $\frac{M}{M-N_1}$. Therefore, the number of target-inputs and non-target-inputs are effectively balanced, instead of biasing towards either the target class or non-target class. 

\mypara{Multi-Select} This type of application defines several target classes, $\{W_1, W_2, \dots, W_m\}$, and multiple selections are allowed about which class(es) the ML API output belongs to. We construct the following loss function:

\begin{equation}
    L = \frac{M}{N_i}\sum_{j=1}^{m} y_i \cdot \textrm{S}(\theta - P_j) + (1-y_i) \cdot \textrm{S}(P_j - \theta) \,,
\label{eq:multi-select}
\end{equation}
where $y_i$ indicates whether this input belongs to the $j^{th}$ target class $W_j$, $y_i = 1$ when $\hat{y_i} \cap W_j \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_j$ is the maximum probability of classes belonging to $W_j$ (\ie $P_j = max_{c \in W_j} p_c$). Let $\mathbb{W} = \bigcup\limits_{j=1}^{m} W_j$ denote the union of all the target classes defined in the application, and $\mathcal{W}_i = \bigcup_{W_j \cap  \hat{y_i} \neq \emptyset} W_j $ denote the union of all the ground-truth target classes for the $i^{th}$ input (same notation used in the rest of the section). 
When $\hat{y_i} \cap \mathbb{W} \neq \emptyset$, $N_i$ is the total number of inputs in the training data belonging to $\mathcal{W}_i$ (\ie $N_i = \sum\limits_{j=1}^{M}\mathds{1}_{\hat{y_j}\cap \mathcal{W}_i \neq \emptyset}$); otherwise, $N_i$ denotes the total number of non-target-inputs (\ie $N_i = \sum\limits_{j=1}^{M}\mathds{1}_{\hat{y_i} \cap \mathbb{W} = \emptyset}$), the same notation will be used throughout this section. Similarly to Equation~\ref{eq:loss}, the weight $\frac{M}{N_i}$ is used to achieve the effect of balancing each of the target classes and non-target class.

With this loss function, only if the application decisions led by the ML API outputs exactly match with the ground-truth decisions, the penalty will be low.

\mypara{Multi-Choice API-output order} This type of application defines several target classes, and starts with checking if the first API output label matches with any of the classes. If so, the rest of the labels are skipped. Otherwise, later labels will be checked. We construct the following loss function:
 \begin{equation}
    L = \frac{M}{N_i} \Bigl( y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \Bigr) \,,
\label{eq:api_output}
\end{equation}
where $y_i  = 1$ indicates ground-truth labels intersect with $\mathbb{W}$, and $y_i=0$ otherwise. $P^{+}$ is the maximum probability out of classes in $\mathcal{W}_i$ (\ie $P^+ = \max_{c \in \mathcal{W}_i } p_c$), and $P^-$ is the maximum probability out of classes in the incorrect target classes (\ie $P^- = \max_{c \in (\mathbb{W} \setminus \mathcal{W}_i) } p_c$). 

Therefore, the loss function ensures only if the first output label encountered belonging to any of the target classes, matches with the ground-truth class, the penalty will be low. 

\mypara{Multi-Choice application-choice order} This type of application starts with checking if the first target class matches with any output label before moving to the next class. We construct the following loss function for this type:

\begin{equation}
\begin{split}
    L = \frac{M}{N_i} \Bigl( y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
    (1-y_i) \cdot \textrm{S}(P - \theta) \Bigr) \,,
\end{split}
\label{eq:app_choice}
\end{equation}

Similarly to Equation~\ref{eq:api_output},  $y_i  = 1$ indicates ground-truth labels intersect with $\mathbb{W}$, and $y_i=0$ otherwise. $k$ is the index of the highest-priority target class that intersects with the ground-truth labels (\ie $k = \min \{j|W_j \cap \hat{y_i} \neq \emptyset\}$). $P_k$ is the maximum probability for labels belonging to $W_k$, and $P_{k^{-}}$ is the maximum probability out of the labels belonging to higher priority classes than the ground-truth class (\ie$W_{k^{-}} = \bigcup_{\{j|\hat{y_i} \cap W_j \neq \emptyset  \textrm{ and }  j < k \}} W_j$ and $P_{k^{-}} = \max_{c\in W_{k^{-}} }p_c$). $P$ is the maximum probability of the classes belonging to $\mathbb{W}$. 


This loss function ensure that only if the first target class that matches with any of the output labels is the ground-truth class, the penalty incurred by the loss function will be low. 


\mypara{Value-ranges} For APIs outputting scores, such as the sentiment analysis API, application check whether the score lies in defined value ranges. The loss function we construct is:

\begin{equation}
    L = \frac{M}{N_i} \cdot \Bigl( S(l_i - O_i) + S(O_i - h_i) \Bigr) \,,
\end{equation}
where $l_i$ is the lower bound of the ground-truth  value range, and $h_i$ is the upper bound of the ground-truth value range. $N_i$ is defined similarly to previous sections. 

Therefore, the penalty incurred by the loss function will be low only when the API output score lies in the ground-truth value ranges.
% Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 




\jc{
an example outline of this subsection (each bullet is a para)
\begin{itemize}
\item why we start with this? the key step is customizing ML-model for each application.
\item what's the goal
\item what's a strawman (resampling training data)? and why is it not good (doesn't distinct multi-choice vs multi-option and order of examination)? (this para must be short). if room, also bring up some prior work that also does this
\item our idea: rewriting loss function. give a general recipe of how this is done
\item why is it better? (this should directly contrast with the strawman)
\item more case-by-case explanation.
\end{itemize}
}

\jc{regarding how to explain the goal, you can expand the following: formally an application can be viewed as $z=Decision(Model(x))$. for a given decision process $Decision$, the goal is to minimize $Decision(Model(x_i))\neq Decision(\hat{y_i})$ over a set of $x_i$, where $\hat{y_i}$ is the ground truth label of $x_i$.}



% \mypara{Notations} 
% Denote the total number of classes that the ML-model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows. 
% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the ML-model behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}

% \mypara{Customization goal} For T-or-F, we want to minimize the critical errors which are caused by the API outputs that lead to the  execution of the \emph{False} branch, when the statement should be \emph{True} according to the ground-truth, and vice versa. With the above notations, our goal can be written as:

% \begin{equation}
% \begin{aligned}
% \min \sum\limits_{i=1}^{M}( y_i \cdot \mathds{1}_{\theta - P} + (1-y_i) \cdot \mathds{1}_{P-\theta} )
% \end{aligned}
% \end{equation}

% Where $\mathds{1}_{x} = 1$ when $x > 0$, and 0 otherwise. $y_i = 1$ if the $i^{th}$ input belongs to the class list defined in the branch condition, which we denote as $W$. $\theta$ is the prediction threshold, where classes whose predicted probability is higher than the threshold will be included in the output label list. $P$ is the maximum probability of classes in $W$, in other words, $P = max_{c \in W} p_c$.
% there are two types of critical errors: (1) for inputs whose statement in the branch condition is \emph{True} according to the ground-truth, which we refer to as \emph{target-inputs}, the API outputs lead the application selecting the \emph{False} branch; (2) for inputs whose statement is \emph{False}, the API outputs lead the application selecting the \emph{True} branch. To minimize incorrect application decisions, we want: 




% \yh{Outline of this section: 
% 1. first list the goal in math (or text): minimize the incorrect app decisions
% 2. a naive re-training scheme is to use a training data that  focuses on classes appeared in the apps 3. why this design is not good: it can only solve xxx, but not xxx 4. describe our loss function }
% \yh{goal: minimize the incorrect app decisions; what we have: extracted software decision process (key dimensions) }
% As shown in our empirical study in Section~\ref{sec:empirical}, we find the software decision process can be characterized by two aspects: (1) the class list(s) or value ranges that are used in branch conditions (2) the structures of the branch conditions.

% In this section, we will describe how we incorporate the software decision process in the loss function. Our optimization is composed of two steps: (1) clustering the training data to focus on classes appearing in the branch conditions; (2) constructing the loss functions to be aware of the software decision process. Our objective is to incur a high penalty on critical errors, and no penalty if the errors make no impact on the application. 


% To begin with, we first introduce the loss function traditionally used in multi-label image classification.


% The binary cross-entropy loss function used in multi-label classification task~\cite{ASL} is denoted as:
% \begin{equation}
%     L_{bce}  = -\frac{1}{n}\sum_{i=1}^n{(y_i\log(p_i) + (1 - y_i)\log(1 - p_i))} \,,
% \end{equation}
% where $y_i = 1$ if class $i$ is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. $p_i$ is the predicted probability for class $i$. 
% \begin{itemize}
%     \item  $y_i = 1$ if the $i^{th}$ class is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. 
%     \item $p_i$ is the predicted probability for the $i^{th}$ class.
% \end{itemize}
% where $y_i$ indicates whether the $i^{th}$ class exists in the input input $I$ or not. In other words, $y_i = 1$ if the $i^{th}$ class exists in the input $I$, and $y_i = 0$ otherwise. \cc{It is still one sentence, so please do not start a new paragraph}


% \subsubsection{Clustering training data}


% To achieve the first step, one approach is to assign different weights to inputs with ground-truth decisions of executing the \code{Others} branch and non-\code{Others} branches.  
% We take a simple example to illustrate this approach. An application  defines one branch condition to check if the API outputs intersect with a class list $W_1$. $W_1$ is a non-empty subset of the whole label set $C$ that the ML-model is able to classify. 
%  The original fraction of images in the training data whose ground-truth  decisions are executing the \code{$W_1$}-branch (\ie $G \cap W \neq \emptyset$), which we refer to as \code{$W_1$}-inputs,  is $A$. 
%  % \cc{This sentence is very hard to read. Can we use phrase like ``which we refer to as $W$-images''?} 
% The fraction of images whose ground-truth decisions are executing the \code{other}-branch is $1-A$,  which we refer to as \code{others}-inputs. If we want to balance the distribution between $W$-inputs and \code{others}-inputs, we can use a loss function that assigns higher weights to \code{W}-inputs:

% \begin{equation}
%     L_D = y_1 \cdot \frac{1}{A} \cdot L_{bce} + (1-y_1)\cdot A \cdot L_{bce} \,,
% \end{equation}
% where $y_1$ indicates whether this input is a \code{$W$}-input or not. In other words, $y_1 = 1$ when the input is a \code{$W$}-input ($G \cap W \neq \emptyset$), and $y_1 = 0$ otherwise ($G \cap W = \emptyset$). 

% In this way, \code{$W$}-inputs and \code{others}-inputs are taking the same effect during training, instead of biasing towards either \code{W} or \code{others}. 

% % We construct loss functions for each type of software represented by the software examples shown in section~\ref{sec:empirical}. \cc{Maybe say some high-level ideas, more intuition}

% \subsubsection{Branch condition structure 1: T-or-F} 

% For the software that defines only one branch condition, checking if the output labels $O$ intersect with a class list $W_1$. We penalize the critical errors: (1) all the classes in $W_1$ are not included in top predictions for \code{$W_1$}-inputs; or (2) at least one class in $W_1$ are included in top predictions for \code{others}-inputs.




% \begin{equation}
%     L_{W_1} =y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \,,
% \label{eq:loss}
% \end{equation}
% where
% $y_1$ indicates whether this input is a \code{$W_1$}-input or not. 
% In other words, $y_1 = 1$ if the input is a \code{$W_1$}-input, and $y_1=0$ if the input is a \code{others}-input. $\theta$ is the prediction threshold, where classes whose predicted probability will be included in the output label list. $P_1$ is the maximum probability of classes in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will denote as $S$ in the rest of the paper. 



% Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for  \code{$W_1$}-inputs. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-inputs. Similarly for \code{other}-inputs. 



% \subsubsection{Branch condition structure 2: M-to-N-set} 

%  In M-to-N-set, several branch conditions are defined, each checking if a class list intersects with the API output $O$. All the fulfilled branches will be executed. We denote all the $m$ class lists the application uses in branch conditions as {$W_1$, ..., $W_m$}. In this pattern, the ground-truth  decisions is executing \emph{all} the branches whose class lists  intersect with the ground-truth labels. 

% We derive the following loss function for M-to-N-set:
% \begin{equation}
%     L = \sum_{i=1,\cdots,m} y_i \cdot \textrm{S}(\theta - P_i) + (1-y_i) \cdot \textrm{S}(P_i - \theta) \,,
% \end{equation}
% where $y_i$ indicates whether  $W_i$ is among the branches the ground-truth decision executes, in other words, $y_i = 1$ if $G \cap W_i \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_i$ is the maximum probability of classes belonging to $W_i$ (\ie $P_i = max_{c \in W_i} p_c$). 

%  Only if the application decisions led by $O$ exactly match with the ground-truth decisions, the penalty will be low.


% % \kt{$\sum_{i=1,\cdots,N} L_{W_i}$}



% \subsubsection{Branch condition structure 3: Priority-list}

% Priority-list defines several branch conditions, and each of them is associated with a class list $W_i$. The application checks the branch conditions from highest to lowest priority until finding the first one whose class list intersects with API output labels $O$. Let $W_i$ (where $1 \leq i \leq m$) denote the class lists used in branch conditions, where class lists with smaller $i$ indicate higher priority. Let $W$ denote the union of the classes in all the whitelists, in other words, $W = \cup^{m}_{i=1}W_i$. The ground-truth decision  is executing the highest priority branch whose associated class list intersects with the ground-truth classes $G$. 

% We derive the loss function as:
% \begin{equation}
% \begin{split}
%     L = y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
%     (1-y_i) \cdot \textrm{S}(P - \theta) \,,
% \end{split}
% \end{equation}
% where $y_i = 1$ when the ground-truth decision is executing one of the branches in $\{ W_1, \cdots, W_m\}$ (\ie $G \cap W \neq \emptyset$), and  $y_i = 0$ when the ground-truth decision is executing the \code{others} branch. 
% $k$ is the index of the highest-priority branch whose class list intersects with the ground-truth classes (\ie $k = \min \{i|WL_i \cap G \neq \emptyset\}$). $P_k$ is the maximum predicted probability for classes belonging to $W_k$, and $P_{k^{-}}$ is the maximum predicted probability out of the classes belonging to higher priority branches than the ground-truth branch (\ie $k^{-} = \min \{i | W_i \cap (G \setminus W ) \neq \emptyset \textrm{ and } i < k \}$). $P$ is the maximum probability of the classes belonging to $W$. 

% Given this loss function, only if the highest-priority branch whose class list intersects with the predicted classes $O$ is the ground-truth decision, the penalty will be low. 


% \subsubsection{Branch condition structure 4: Top-label}

% Top-label defines several branch conditions, and associates with each of them with a class list $W_i$, similar to Priority-list. However, unlike Priority-list, it checks the \emph{API output labels} one by one until one of them intersects with any of the class lists. Similar to the previous section, $W$ is the union of classes in all the defined class lists. We denote the classes belonging to class lists intersecting with ground-truth classes as $W^+ = \bigcup_{W_i \cap G \neq \emptyset} W_i$, and the classes belonging to \wls that do not intersect with ground-truth classes as $W^- = W \setminus W^+$.
 
% In this pattern, the ground-truth decision is to execute the branch condition  whose class list  intersects with the ground-truth classes. 

% We derive the loss function as:
% \begin{equation}
%     L = y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \,,
% \end{equation}
% where $y_i  = 1$ indicates that the ground-truth decision is executing one of the branches in \{$W_1$, $W_2$, ...$W_m$\}, and $y_i = 0$ indicates the ground-truth decision is selecting \code{others}, similarly to the previous section. $P^{+}$ is the maximum probability out of classes in $W^+$ (\ie $P^+ = \max_{c \in W^+ } p_c$), and $P^-$ is the maximum probability out of classes in $W^-$ (\ie $P^- = \max_{c \in W^- } p_c$). 


% Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 




\subsection{How to extract the software decision process}
\label{sec:extract}
% How we use sym-ex to get info, and which info 
\yh{Change all the whitelists}
To extract software decision process, we conduct an offline static analysis to detect code patterns introduced in Section~\ref{sec:empirical}. 
Particularly, we focus on the control-flow structures that are directly affected by ML API results. 

Given a code location of ML API invocation, \tool analyzes all the if-branches that have dependency on the ML API's output. For each combination of branch decisions, \tool adopts symbolic execution engine DSE~\cite{irlbeck2015deconstructing} and CVC5 constraint solver~\cite{cvc5} to find all the API outputs that lead to these decisions, which is the corresponding \wl.
If the software specifies only 1 branch condition, \tool reports pattern True-False. Otherwise, \tool analyzes the code structure to determine the pattern. % according to Figure~\ref{fig:hierarchy}:

\emph{Whether multi-select or multi-choice?} \tool analyzes all the statements inside the edges of an ML-API-related if-branch. If the software terminates all the examinations inside one of the branch edges (e.g., a break statement inside the loop and a return statement inside a function body), \tool regards that it as a multi-choice and further examines the order. 
If there is no such termination, \tool determines it is multi-select structure. 


\emph{How is the order determined?} \tool finds all the loop structures and the equivalent statements outside the ML-API-related if-branches. It analysis their nested levels and the data dependency relationship of their iterators. 
If the software does not contain any loop iterating ML API's output or application choices, \tool stops examination and reports an absence of code pattern. 
If an inner (outer) loop iterates the ML API's output and the outer (inner) loop iterates the application choices, \tool regards it as pattern Application-choice order (API-output order).  Note that, if the software contains multiple nested loops iterating the same variable, \tool focuses on the innermost one.


\subsection{How to change the MLaaS run-time backend}
\label{sec:runtime}



==> bk/backups_before_fist_submission/3-method-1129.tex <==
\label{sec:method}

Guided by the empirical study in \S\ref{sec:empirical}, this section presents \tool, an optimization framework that customizes ML models of the MLaaS backend for the decision processes of different applications.

\subsection{Key components and workflow}
\label{sec:overall}
\begin{figure}
     \includegraphics[width=\linewidth]{figs/system_overview.pdf}
    \caption{System architecture of \tool. 
    % \jc{the overall flow looks ok, but there are so many minor issues in this figure. just to name a few: 
    % (1) where is "cloud service" coming from? 
    % (2) (a) and (b) shouldn't be distinguished (see comment in 3.1).
    % (3) i thought we decided to drop the arrow of giving the parser to developer?
    % (4) why "software context" is still used?
    % (5) user is not running python code! they run real apps
    % (6) why calling it "prediction" instead of API output?
    % (7) what's "model inference code"? if it's simply selecting the right model to run, we shouldn't introduce a new term.
    % (8) the three customized models should be put side by side (either all vertically or horizontally),
    % (9) why calling them "adapted" ML model? if the term we always use is "customized", then stick to that.}
    % \jc{in general, EVERY word must be picked very carefully, which you clearly didn't do :)}
    % \yh{fixed comments, I'm calling it ML model outputs instead of API outputs because the outputs comes before the ``output interface'', thus it's not API outputs yet}
    % \jc{sorry i disagree. again, don't introduce new terms unless really necessary, which i don't think is the case. why dont you change the figure, to move the output and input the left of the model output interface, which should also be changed to "ML API"?}
    % \jc{and don't let arrows overlap with arrows or lines (e.g., Model pool, Select)}
    }
\label{fig:system}
\end{figure}
% \mypara{Main components}

% \mypara{Extracted application's decision process}
% the application's decision process of the applications querying the MLaaS, and customizes the ML model in the MLaaS backend.
% summarizes the overall workflow of \tool.


\mypara{Workflow}
Figure~\ref{fig:system} depicts \tool's high-level workflow. 
When the developers publish an application \App, they first run a parser script provided by \tool on \App's source code to extract its {\em decision-process summary} (explained shortly), and then upload the summary to \tool's MLaaS backend (details in \S\ref{sec:extract}). 
In the backend, \tool uses the received decision-process summary to construct a new loss function, such that when the ML model is re-trained using the new loss function, it will produce inference results that yield fewer application decision failures for the application \App (details in \S\ref{sec:loss}).
\tool then adds the new ML model to a pool of customized ML models. 
% \jc{the last phrase can be deleted}
When a user of application \App queries the MLaaS backend with an input via the existing ML API, the backend will select the ML model customized for \App and return the inference result of the selected ML model (details in \S\ref{sec:runtime}).


\begin{comment}
When the application is being developed, 
% \jc{the term offline is new. the contrast between offline and online is overcomplicating. can we say something like when the application is being developed?}
besides the existing development procedure, the developers also run an MLaaS-provided parser plugin on their own machines, 
% \jc{the ``parser'' comes from nowhere. who provides it? even a simple ``MLaaS-provided parser'' is better}
% \jc{``locally'' has many meanings. pick a more precise term}, 
which extracts a summary of the application's decision process
% \jc{maybe we need a different term; ``key features'' invites unnecessary confusion when used in an ML-related paper. how about a ``summary of the application's decision process''?}
% \jc{``extracts xxx from app into a file'' sounds wrong. shouldn't it be ``extract xxx from an app and uploads it as a file to xxx''?} 
from the application source code (details in \S\ref{sec:extract}), and uploads it as a file to the MLaaS backend. 
\end{comment}




% \jc{the separation among the three stages (``developer'', ``re-training'' and ``run-time'') is unnecessarily complicating the flow, and it introduces unnecessary terms, like ``run-time''. }

% \jc{when introducing the flow, shouldn't we also highlight what we DO change and what we do NOT change?}

% The application's decision process extracted from the Python source code, is composed of the key features characterizing it.\cc{This sentence does not provide additional information. Also, we could mention python in the implementation section} 

% \jc{please don't explain a concept together with an application. you should always explain the concept first, and THEN use an example to explain it in a specific context.}

\smallskip
\noindent
The {\bf \summary} extracted from an application includes three pieces of information: 
\begin{packeditemize}
\item the values included in each target class; \yh{double check}
\item the type of decision (\ie \emph{True-False}, \emph{Multi-Choice}, or \emph{Multi-Select});
\item the matching order over the target classes, if the application makes a \emph{Multi-Choice} decision.
\end{packeditemize}
These three pieces of information can uniquely identify which errors are critical and which are non-critical to the application, which provides vital information to customize the ML model for the application, as elaborated in \S\ref{sec:loss}. 
% vary greatly across applications, 
% provides us with great opportunities to customize the ML models per application. 

To give a concrete example, the \summary of the garbage classification application in Figure~\ref{fig:code}(a) contains
(1) the three target classes (each being a list of labels): \code{Recycle}, \code{Compost}, and \code{Donate}; (2) the \emph{Multi-Choice} type of decision; and 
(3) it follows the \emph{API-output order} to reach the \emph{Multi-Choice} decision.  


\mypara{What is changed, what is not}
It is important to notice that \tool does {\em not} change the ML API or the source code or the executable of the application.
% \jc{check the term with shan/chengcheng}
That said, \tool does change two things. 
First, the application developers need to run \tool's parser script to extract the decision-process summary.
Second, \tool modifies the MLaaS backend to re-train an ML model per application (instead of serving the same model to all applications) and selects the right ML model to serve each query.
% When the application queries the MLaaS, 
% a model selector module is added in the backend to choose the ML model customized to the application, based on the application ID incorporated in the identification credential.

% \jc{this last sentence is important but quite misleading. first of all, these features don't uniquely describe a decision process (e.g., they dont say what decisions will be made for each branch). instead, they specify what errors are critical and what errors are not critical.
% second, you didn't say WHY they SHOULD be used by \tool to customize the ML model.}


\begin{comment}
\jc{this definition is extremely important and should be elevated. i suggest explain it in a separate paragraph. so you will have two paragraphs: one explain the overall workflow, and the second explains what's extracted from the source code and used to customize ML model. it's important to keep the 1st para short.} 
\jc{it should be explained more formally, probably with a simple example, and the terms (e.g., multi-select vs. multi-choice) should be tightly connected to when they are first defined. remember, many reviewers may have skipped (or missed) their definitions in section 2.} 
\jc{moreover, i wouldn't mention JSON at the beginning. the exact format (not the content in the file) seems secondary to me}
\jc{what about score ranges? we need a way to explain all cases under consideration} 
% used in branch conditions; (2) whether the application is making multi-select or multi-choice decisions; (3) the order of examination for applications making multi-choice decisions. Then, the developers will upload the JSON of application's decision process to the MLaaS backend. On the MLaaS backend side, \tool will re-train the ML model by re-sampling the training data with a more focus on the classes appeared in the applications, and constucting loss functions which directly penalize the critical errors.
\jc{i wouldn't distinguish training data resampling and loss function as two separate steps. last time we met as a group, we decided to say changing loss function is all that's needed, though the real implementation does resampling to speedup training. i like this idea, so the distinction should be secondary.} 

\jc{regarding the terminology, the parser doesn't extract the entire application decision process, it merely extracts the key features of the application decision process, which include xxx}



\jc{now this is too low-level when explaining the workflow. here, you can just say ``each time an application calls the ML API, the ML API backend will select the ML model model customized for the application, ...''}
% the applications submit inference request to the ML API with input and the credential, like 

\jc{two meta comments: 1. Yuhan, you should read the terms used in the new Section 2 and use them consistently in section 3.
2. when writing 3.1, please make sure that every important term appears with a forward pointer to a later subsection that explains it in detail as well as a pointer to Figure 4}
\end{comment}

% which consists of a parser plugin, an ML model re-training scheme run in the offline stage, and in the online stage, \tool selects the customized ML model based on applications' credentials, and run inference with the customized model.  


% 3.2: given the extracted json, how should we re-train teh model 
% 3.3. how to extract
% 3.4: how to change the run-time interface

% \tool is an automated framework that adapts the ML model behind the ML APIs, such that the number of software mis-behaviors can be greatly reduced when applied to an ML software. 

% \tool first performs static analysis to extract the code structure of the applications invoking MLaaS to understand how the software uses the ML API outputs to make application decisions. Then \tool constructs loss functions that penalize the critical errors of the applications. Finally, \tool re-trains the ML models behind the ML APIs with the constructed loss function, without modifying the output interface of the ML APIs. 

% In this section, we will introduce how \tool performs static analysis and constructs the loss functions for the applications. 


% \subsection{Understanding Software Context}

% \subsection{Notations}
% \yh{not 3.2 }
% Denote the total number of classes that the ML model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows:

% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the DNN behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}



% \subsection{How to customize the ML model in the MLaaS backend}
\subsection{Customizing ML model for an application decision process}
\label{sec:loss}
% As introduced in \S\ref{sec:empirical},  applications in the wild differ greatly in their application's decision processes. 
% % For example, they may  define different number of target classes or include only a small subset of labels of the whole label set in their target classes and so on. 
% This heterogeneity can lead to differences in critical errors\jc{remind people what critical errors are?} across applications. 
% It is possible for an ML API error to be non-critical for one application, while critical for another. Thus, customizing the DNN in the MLaaS backend is important in order to incorporate the differences in application's decision processes across applications.
% \jc{the whole first paragraph is redundant to 3.1. this para should highlight why we start by explaining the step of DNN re-training}

% Model re-training has been widely adopted in ML to update the generic pre-trained ML models to work for related but different tasks~\cite{mullapudi2019online,ekya}. In model re-training, the model is initialized from a pre-trained model, and  its model parameters are updated based on the goal of the new task.
The idea of model re-training has been widely adopted in ML to update the generic pre-trained ML models to work for related but different tasks~\cite{mullapudi2019online,ekya}. The key challenge is how to formulate the customized optimization goal and design re-training strategy to efficiently achieve high  accuracy on different tasks.
\shan{Reading this sentence, as a picky reviewer, I would start worrying about the novelty of this work over model re-training work. The next sentence ``In our problem setting'' reads quite similar to the previous sentences. Is it possible to rephrase so that the difference is more obvious?}  \cc{Done. I feel the last sentence actually do not provide new information. So I deleted it.}
% In our problem setting, we want to initialize from a pre-trained model for the original ML task (\eg image or text classification), and re-train it with our customization goal.  
  

Our {\bf customization goal} is to minimize the critical errors for each application.
% caused by ML API errors. 
If we view the application's decision process  as $\z = \Decision(\API(\x))$, where $\x$ is the input to the API, $\API(\x)$ is the ML API output, and $\Decision$ is the post-processing the application performs to make decisions based on API outputs. 
Let $\x_i\in \X$ denote the $i^{th}$ input to the ML API, and $\hat{y_i}$ denote its ground-truth label. 
% $API(x_i)$ is a list of probabilities for label-based API (\eg image or text classification), 
% [$p_1, p_2, \dots, p_n$], for every label in the whole label set, and a score $O_i$ for score-based API (\eg sentiment analysis API). 
Formally, our customization goal is written as:
% Let $\mathds{1}_{x}$ denote the indicator function, where $\mathds{1}_{x} = 1$ when $x$ is \emph{True} and 0 otherwise. Therefore, the customization goal is:

\begin{equation}
    \min |\{x_i \in X | Decision(API(x_i)) \neq Decision(\hat{y_i})\}|
    \label{eq:goal}
\end{equation}


A common practice in ML is to utilize the loss function to express the optimization goal~\cite{celoss}. For example, the Binary Cross Entropy loss is used in image or text classification tasks, and Mean Squared Error loss is used in regression tasks. 

% Take classification task as an example, the Binary Cross Entropy loss is defined as:

% \begin{equation}
%     L_{BCE}(y_i) = \sum_{j=1}^{n} -\hat{y_{i, j}} \cdot log(y_{i,j}) - (1-\hat{y_{i,j}}) \cdot log(1-y_{i,j})
%     \label{eq:bce}
% \end{equation}
% where $y_i$ is the output of the ML model on the $i^{th}$ input, which is a list of probabilities. The higher the probability at the $j^{th}$ index is, the more confident the model is about the existence of the $j^{th}$ label in the input.  $\hat{y_i}$ is the ground truth for the $i^{th}$ input. $\hat{y_{i,j}} = 1$ if the $j^{th}$ label is in the ground truth of the $i^{th}$ input. Intuitively, this loss function incurs a high penalty when the $j^{th}$ label is present in the ground truth, but the model outputs a low probability for it, and vice versa. 

The question we want to answer is,  \emph{how to design a loss function that can achieve our customization goal?}

\mypara{Strawman}With the observation that applications typically heavily cluster on a small subset of labels appearing in the target classes(\S\ref{sec:empirical}), we naively come up with a \emph{strawman} of loss function design: assigning higher penalties to errors made by the ML model on inputs whose ground-truth decisions are selecting the target classes. 

% \begin{equation}
% L(y_i) = w_i \cdot T_i \cdot L_{BCE}(y_i) + (1-T_i) \cdot L_{BCE}(y_i)
% \end{equation}
% where $w_i$ is a large weight (\eg $w_i = 20$), and $T_i = 1$ if the ground-truth labels of the $i^{th}$ sample overlap with the applications' target classes, and 0 otherwise. 


% Intuitively, this \emph{strawman} loss function is compatible with our goal since it prioritizes the reduction of the loss on the samples belonging to the target classes than the non-target ones. 

Take the classification task  as an example to illustrate this idea. 
The ML model predicts a list of probabilities for an input, in which the $j^{th}$ element describes how confident the model is about whether the $j^{th}$  label exists in the input. 
The ground truth is a list, where the $j^{th}$ element is 1 if the $j^{th}$ label exists in the input, and 0 otherwise. 
The pre-trained model is trained to reduce the \emph{average} errors between the probabilities and the ground truth across a wide range of labels (\eg 9605 labels in Open Images~\cite{ASL}).
On the other hand, 
this strawman approach can prioritize the reduction of errors on the inputs whose ground-truth decisions are selecting the target classes. 
However, the strawman penalizes mis-classifications within one target class, such as mis-classifying a paper image into plastic in the garbage classification application example in Figure~\ref{fig:code}(a), and this type of errors are non-critical to the application.
% because the strawman is unaware that different applications may make different decisions given the same output (\eg \emph{True-False}, \emph{Multi-select}, and \emph{Multi-choice}) and how these decisions affect the severity of ML model errors
\shan{This last sentence is not clear.}. 

\mypara{New loss function}We propose a new loss function directly constructed from the \summary.
% \yh{Why they fails and we do not fail }
% \yh{add general recipe }
Compared to the strawman which may spare energy penalizing non-critical errors\shan{?? what exactly are non-critical errors spared by strawman?} \yh{I put in the last para: \ie mis-classifications within one target class}, 
our proposed solution only focuses on penalizing the critical ones. 
Specifically, two types of critical errors are being penalized\shan{I don't understand the (1) and (2) presented below}: 
(1)\shan{Hmm, what does this mean?}\emph{all} the labels in a target class have low probabilities in the prediction, but ground-truth decision selects it. 
(2) \emph{at least one of} the labels in a target class has a high probability, but ground-truth decision does not select it.

\tool's  loss function uses the Sigmoid function (\ie $Sigmoid(y) = \frac{1}{1+e^{k\cdot y}}$) to penalize the critical errors. The intuition behind using the Sigmoid function is that it provides a differentiable way to incur a high penalty when $y >0$\shan{what is y?}, and a low penalty otherwise, which appropriately fits our needs. 

% , such as mis-classifications across target classes. 
% For example, the strawman penalizes mis-classifications within the target classes, which are non-critical, while 



Formally, the loss function can be written as:

\begin{align*}
L_{i} &= 
\overbrace{ \sum_{j \in \{ \textrm{selected target classes}\}} ~\textrm{Sigmoid}(\F(y_i)-M_j(y_i))
}^{\substack{\text{\sf \footnotesize {Penalize low probability for the selected target class
	}} 
}} \\ &+ 
\overbrace{\sum_{j \in \{ \textrm{unselected target classes}\}} \textrm{Sigmoid}(M_j(y_i)-\Q(y_i) )
}^{\substack{\text{\sf \footnotesize {Penalize high probability for the unselected target class
	}} 
}} \label{eq:loss}
\end{align*}
where $M_j(y)$ is the \emph{maximum} probability in $y$ at indices that belong to the $j^{th}$ target class.  $\Q(y), \F(y)$ are two scores that differ by different types of applications. Generally, $ \F(y) > M_j(y)$ or $ M_j(y) > \Q(y)$ suggest that $y$ leads to an incorrect decision, otherwise, a correct decision is made\shan{hmmm, too complicated for me to understand} \yh{Working on how to make this clearer now}. 
% where $H_o(y) = 1$ if $y$ leads to the selection of the non-target class, and $H_o(y) = 0$ otherwise. $H_j(y) = 1$ if $y$ leads to the selection of the $j^{th}$ target class, and  $H_j(y) = 0$ otherwise. $Q_j(y) = 0$ for applications making \emph{Multi-Choice} decisions in API-output order, and $Q_j(y) = 1-H_j(y)$ otherwise. 
% $\theta$ is the prediction threshold of ML model, where any labels whose predicted probability is higher than it will be included in the output. $G_j(y)$ is the maximum probability in $y$ at indices that belong to the $j^{th}$ target class. $G(y) = max_{j \in \{1, \dots, m\}} (G_j(y))$ is the maximum probability in $y$ at indices belonging to all the target classes. $\F(y) = max$($\theta$, maximum probability in  $y$ at the indices that belong to any ground-truth unselected target class(es)). 

% In order to achieve the goal of re-sampling the training data,  our loss function assigns a weight $\frac{M}{N_i}$, where $M$ is the total number of data in the original training dataset, and $N_i$ is the number of training samples whose ground-truth labels overlap with the ground-truth target class(es) of the $i^{th}$ input. This weight, intuitively,  alleviates the effect of class skews in the original dataset by assigning higher weight to less dominant target classes, and lower weight for more dominant ones. 
% \yh{care more about the target classes} 


% M is the total number of data in the original training dataset. $N_i$ is the total number of data whose ground-truth selected target class(es) overlap with the ground-truth target class(es) of the $i^{th}$ input.  

As we have seen in \S\ref{sec:empirical}, the critical errors can vary greatly across different types of application's decision processes. Thus, in order to accurately capture the critical errors, we design different loss functions for each type of decision process. 

% Next, we describe the loss function for each type of decision process case-by-case. 


\mypara{True-False} In \emph{True-False} decision, only one target class is defined, and the application checks if the API output matches with it. 
Denote the prediction threshold of the ML model as $\theta$, where all the labels whose probabilities are higher than it will be included in the output. 
In this case, $\F(y) = \theta$, and $\Q(y) = \theta$. \shan{I understand the next few sentences, but I don't understand why F(y) is $\theta$, and 
Q(y) is $\theta$. I went back to read the $L_i$ formula, but still don't understand.}
For an input whose ground-truth decision selects the target class, a high penalty will be incurred if none of the labels in the target class appear in the output. 
% Thus, when the maximum probability for labels belonging to the 
On the other hand, for an input whose ground-truth decision selects the non-target class, a high penalty will be incurred  when there is at least one label in the target class included in the output. 

\mypara{Multi-Select} As for \emph{Multi-Select} decision, multiple selections are allowed about which target class(es) the ML API output matches with. 
In this case, the ground-truth target class(es) are those which overlap with the ground-truth labels of the input. 
$\F(y) = \theta$ and $\Q(y) = \theta$ for this type. 
The loss function will incur a high penalty when there are ground-truth target class(es) whose maximum probability is lower than $\theta$, 
or when there are target class(es) unselected by ground-truth whose maximum probability is higher than the $\theta$. 
\shan{Is Multi-Select's loss function essentially the same as True-False? Or, maybe you can tell me what exactly is the difference between them?}


% Denote the output of the ML model on the $i^{th}$ input as [$y_{i, 1}, \dots, y_{i,n}$]


\mypara{Multi-Choice application choice order} This type of application reaches only one selection by checking if the highest-priority target class matches with the output labels, if not, it moves on to the next target class, and so on. In this case, the ground-truth target class is the highest priority class out of those overlapping with its ground-truth labels. $\F(y) = max(\theta$, \textrm{maximum probability in $y$ at indices of unselected target class(es)}), and $\Q(y) = \theta$. Take the example in Figure~\ref{fig:loss} to illustrate. The application defines three target classes. Given an input image whose ground-truth label is \code{``Mansion''}, the ground-truth target class is the second one. In this example, $\F(y_i) = max(\theta, M_1(y_i)) = 0.8$ because the first target class has higher priority than the ground-truth target class. $\Q(y_i) = 0.5$ in this example. Thus, the penalty incurred by the loss function is Sigmoid(0.8-0.5) + Sigmoid(0.8-0.7) + Sigmoid(0.4-0.5). 
 
We can see that the loss function will incur a high penalty if any target class(es) with higher priority than the ground-truth target class are included in the output. 


\begin{figure}
     \includegraphics[width=\linewidth]{figs/loss.pdf}
    \caption{Illustration of \tool's loss function.
    }
\label{fig:loss}
\end{figure}


\mypara{Multi-Choice API output order} In this case, similar to the application choice order, only one selection is allowed. However, the application reaches a decision by checking if the first output label matches with any of the target classes, if not, it moves on to the next output label. 
In this case, the ground-truth target classes are those  overlapping with ground-truth labels. 
$\F(y) = max(\theta, $ maximum probability in $y$ at indices of unselected target classes by ground-truth decision), and $\Q(y) = $ the maximum probability in $y$ at indices of the ground-truth target classes.  
Thus, for the ground-truth target class, only if the maximum probability of it  is smaller than the maximum probability of unselected target class(es) or the prediction threshold, a high penalty will be incurred by the loss function. 


\mypara{Value ranges} As for APIs that output a score $y_i$ to describe the input, applications typically define $m$ value ranges as target classes to make decisions, where the lower bound of the $j^{th}$ value range is denoted as $l_j$ and the upper bound of the $j^{th}$ value range is denoted as $u_j$. The loss function commonly used to optimize for this type of regression task is the Mean Squared Error loss defined as follows:

\begin{equation}
    L_{MSE}(y_i) = (y_i - g_i)^2
\end{equation}
where $g_i$ is the ground truth. 

We construct the following loss function:

\begin{align*}
L(y_i) &= 
\overbrace{ ~\textrm{Sigmoid}(l_j-y_i)
}^{\substack{\text{\sf \footnotesize {Penalize the output if lower than ground-truth lower bound
	}} 
}} \\ &+ 
\overbrace{\textrm{Sigmoid}(y_i-u_j )
}^{\substack{\text{\sf \footnotesize {Penalize the output if higher than ground-truth upper bound
	}} 
}} \label{eq:}
\end{align*}
where $u_j$ and $l_j$ are the upper and lower bound of the value range the ground-truth score selects. 

Similar to the idea of the loss function we construct for classification tasks, compared to the Mean Squared Error loss which penalizes the score $y_i$ if it is not equal to the ground truth,  \tool's proposed loss function only penalizes the score if it falls out of the range that ground truth lies in. 
% MSE loss, borrow the idea 
 

% \jc{
% an example outline of this subsection (each bullet is a para)
% \begin{itemize}
% \item why we start with this? the key step is customizing ML model for each application.
% \item what's the goal
% \item what's a strawman (resampling training data)? and why is it not good (doesn't distinct multi-choice vs multi-option and order of examination)? (this para must be short). if room, also bring up some prior work that also does this
% \item our idea: rewriting loss function. give a general recipe of how this is done
% \item why is it better? (this should directly contrast with the strawman)
% \item more case-by-case explanation.
% \end{itemize}
% }

% \jc{regarding how to explain the goal, you can expand the following: formally an application can be viewed as $z=Decision(Model(x))$. for a given decision process $Decision$, the goal is to minimize $Decision(Model(x_i))\neq Decision(\hat{y_i})$ over a set of $x_i$, where $\hat{y_i}$ is the ground truth label of $x_i$.}



% \mypara{Notations} 
% Denote the total number of classes that the ML model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows. 
% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the ML model behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}

% \mypara{Customization goal} For T-or-F, we want to minimize the critical errors which are caused by the API outputs that lead to the  execution of the \emph{False} branch, when the statement should be \emph{True} according to the ground-truth, and vice versa. With the above notations, our goal can be written as:

% \begin{equation}
% \begin{aligned}
% \min \sum\limits_{i=1}^{M}( y_i \cdot \mathds{1}_{\theta - P} + (1-y_i) \cdot \mathds{1}_{P-\theta} )
% \end{aligned}
% \end{equation}

% Where $\mathds{1}_{x} = 1$ when $x > 0$, and 0 otherwise. $y_i = 1$ if the $i^{th}$ input belongs to the class list defined in the branch condition, which we denote as $W$. $\theta$ is the prediction threshold, where classes whose predicted probability is higher than the threshold will be included in the output label list. $P$ is the maximum probability of classes in $W$, in other words, $P = max_{c \in W} p_c$.
% there are two types of critical errors: (1) for inputs whose statement in the branch condition is \emph{True} according to the ground-truth, which we refer to as \emph{target-inputs}, the API outputs lead the application selecting the \emph{False} branch; (2) for inputs whose statement is \emph{False}, the API outputs lead the application selecting the \emph{True} branch. To minimize incorrect application decisions, we want: 




% \yh{Outline of this section: 
% 1. first list the goal in math (or text): minimize the incorrect app decisions
% 2. a naive re-training scheme is to use a training data that  focuses on classes appeared in the apps 3. why this design is not good: it can only solve xxx, but not xxx 4. describe our loss function }
% \yh{goal: minimize the incorrect app decisions; what we have: extracted application's decision process (key dimensions) }
% As shown in our empirical study in Section~\ref{sec:empirical}, we find the application's decision process can be characterized by two aspects: (1) the class list(s) or value ranges that are used in branch conditions (2) the structures of the branch conditions.

% In this section, we will describe how we incorporate the application's decision process in the loss function. Our optimization is composed of two steps: (1) clustering the training data to focus on classes appearing in the branch conditions; (2) constructing the loss functions to be aware of the application's decision process. Our objective is to incur a high penalty on critical errors, and no penalty if the errors make no impact on the application. 


% To begin with, we first introduce the loss function traditionally used in multi-label image classification.


% The binary cross-entropy loss function used in multi-label classification task~\cite{ASL} is denoted as:
% \begin{equation}
%     L_{bce}  = -\frac{1}{n}\sum_{i=1}^n{(y_i\log(p_i) + (1 - y_i)\log(1 - p_i))} \,,
% \end{equation}
% where $y_i = 1$ if class $i$ is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. $p_i$ is the predicted probability for class $i$. 
% \begin{itemize}
%     \item  $y_i = 1$ if the $i^{th}$ class is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. 
%     \item $p_i$ is the predicted probability for the $i^{th}$ class.
% \end{itemize}
% where $y_i$ indicates whether the $i^{th}$ class exists in the input input $I$ or not. In other words, $y_i = 1$ if the $i^{th}$ class exists in the input $I$, and $y_i = 0$ otherwise. \cc{It is still one sentence, so please do not start a new paragraph}


% \subsubsection{Clustering training data}


% To achieve the first step, one approach is to assign different weights to inputs with ground-truth decisions of executing the \code{Others} branch and non-\code{Others} branches.  
% We take a simple example to illustrate this approach. An application  defines one branch condition to check if the API outputs intersect with a class list $W_1$. $W_1$ is a non-empty subset of the whole label set $C$ that the ML model is able to classify. 
%  The original fraction of images in the training data whose ground-truth  decisions are executing the \code{$W_1$}-branch (\ie $G \cap W \neq \emptyset$), which we refer to as \code{$W_1$}-inputs,  is $A$. 
%  % \cc{This sentence is very hard to read. Can we use phrase like ``which we refer to as $W$-images''?} 
% The fraction of images whose ground-truth decisions are executing the \code{other}-branch is $1-A$,  which we refer to as \code{others}-inputs. If we want to balance the distribution between $W$-inputs and \code{others}-inputs, we can use a loss function that assigns higher weights to \code{W}-inputs:

% \begin{equation}
%     L_D = y_1 \cdot \frac{1}{A} \cdot L_{bce} + (1-y_1)\cdot A \cdot L_{bce} \,,
% \end{equation}
% where $y_1$ indicates whether this input is a \code{$W$}-input or not. In other words, $y_1 = 1$ when the input is a \code{$W$}-input ($G \cap W \neq \emptyset$), and $y_1 = 0$ otherwise ($G \cap W = \emptyset$). 

% In this way, \code{$W$}-inputs and \code{others}-inputs are taking the same effect during training, instead of biasing towards either \code{W} or \code{others}. 

% % We construct loss functions for each type of software represented by the software examples shown in section~\ref{sec:empirical}. \cc{Maybe say some high-level ideas, more intuition}

% \subsubsection{Branch condition structure 1: T-or-F} 

% For the software that defines only one branch condition, checking if the output labels $O$ intersect with a class list $W_1$. We penalize the critical errors: (1) all the classes in $W_1$ are not included in top predictions for \code{$W_1$}-inputs; or (2) at least one class in $W_1$ are included in top predictions for \code{others}-inputs.




% \begin{equation}
%     L_{W_1} =y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \,,
% \label{eq:loss}
% \end{equation}
% where
% $y_1$ indicates whether this input is a \code{$W_1$}-input or not. 
% In other words, $y_1 = 1$ if the input is a \code{$W_1$}-input, and $y_1=0$ if the input is a \code{others}-input. $\theta$ is the prediction threshold, where classes whose predicted probability will be included in the output label list. $P_1$ is the maximum probability of classes in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will denote as $S$ in the rest of the paper. 



% Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for  \code{$W_1$}-inputs. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-inputs. Similarly for \code{other}-inputs. 



% \subsubsection{Branch condition structure 2: M-to-N-set} 

%  In M-to-N-set, several branch conditions are defined, each checking if a class list intersects with the API output $O$. All the fulfilled branches will be executed. We denote all the $m$ class lists the application uses in branch conditions as {$W_1$, ..., $W_m$}. In this pattern, the ground-truth  decisions is executing \emph{all} the branches whose class lists  intersect with the ground-truth labels. 

% We derive the following loss function for M-to-N-set:
% \begin{equation}
%     L = \sum_{i=1,\cdots,m} y_i \cdot \textrm{S}(\theta - P_i) + (1-y_i) \cdot \textrm{S}(P_i - \theta) \,,
% \end{equation}
% where $y_i$ indicates whether  $W_i$ is among the branches the ground-truth decision executes, in other words, $y_i = 1$ if $G \cap W_i \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_i$ is the maximum probability of classes belonging to $W_i$ (\ie $P_i = max_{c \in W_i} p_c$). 

%  Only if the application decisions led by $O$ exactly match with the ground-truth decisions, the penalty will be low.


% % \kt{$\sum_{i=1,\cdots,N} L_{W_i}$}



% \subsubsection{Branch condition structure 3: Priority-list}

% Priority-list defines several branch conditions, and each of them is associated with a class list $W_i$. The application checks the branch conditions from highest to lowest priority until finding the first one whose class list intersects with API output labels $O$. Let $W_i$ (where $1 \leq i \leq m$) denote the class lists used in branch conditions, where class lists with smaller $i$ indicate higher priority. Let $W$ denote the union of the classes in all the whitelists, in other words, $W = \cup^{m}_{i=1}W_i$. The ground-truth decision  is executing the highest priority branch whose associated class list intersects with the ground-truth classes $G$. 

% We derive the loss function as:
% \begin{equation}
% \begin{split}
%     L = y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
%     (1-y_i) \cdot \textrm{S}(P - \theta) \,,
% \end{split}
% \end{equation}
% where $y_i = 1$ when the ground-truth decision is executing one of the branches in $\{ W_1, \cdots, W_m\}$ (\ie $G \cap W \neq \emptyset$), and  $y_i = 0$ when the ground-truth decision is executing the \code{others} branch. 
% $k$ is the index of the highest-priority branch whose class list intersects with the ground-truth classes (\ie $k = \min \{i|WL_i \cap G \neq \emptyset\}$). $P_k$ is the maximum predicted probability for classes belonging to $W_k$, and $P_{k^{-}}$ is the maximum predicted probability out of the classes belonging to higher priority branches than the ground-truth branch (\ie $k^{-} = \min \{i | W_i \cap (G \setminus W ) \neq \emptyset \textrm{ and } i < k \}$). $P$ is the maximum probability of the classes belonging to $W$. 

% Given this loss function, only if the highest-priority branch whose class list intersects with the predicted classes $O$ is the ground-truth decision, the penalty will be low. 


% \subsubsection{Branch condition structure 4: Top-label}

% Top-label defines several branch conditions, and associates with each of them with a class list $W_i$, similar to Priority-list. However, unlike Priority-list, it checks the \emph{API output labels} one by one until one of them intersects with any of the class lists. Similar to the previous section, $W$ is the union of classes in all the defined class lists. We denote the classes belonging to class lists intersecting with ground-truth classes as $W^+ = \bigcup_{W_i \cap G \neq \emptyset} W_i$, and the classes belonging to \wls that do not intersect with ground-truth classes as $W^- = W \setminus W^+$.
 
% In this pattern, the ground-truth decision is to execute the branch condition  whose class list  intersects with the ground-truth classes. 

% We derive the loss function as:
% \begin{equation}
%     L = y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \,,
% \end{equation}
% where $y_i  = 1$ indicates that the ground-truth decision is executing one of the branches in \{$W_1$, $W_2$, ...$W_m$\}, and $y_i = 0$ indicates the ground-truth decision is selecting \code{others}, similarly to the previous section. $P^{+}$ is the maximum probability out of classes in $W^+$ (\ie $P^+ = \max_{c \in W^+ } p_c$), and $P^-$ is the maximum probability out of classes in $W^-$ (\ie $P^- = \max_{c \in W^- } p_c$). 


% Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 




\subsection{How to extract the application's decision process}
\label{sec:extract}
% How we use sym-ex to get info, and which info 
% \yh{Change all the whitelists}
To extract application's decision process, we conduct an offline static analysis to detect code patterns introduced in Section~\ref{sec:empirical}. 
Particularly, we focus on the control-flow structures that are directly affected by ML API results. 

Given a code location of ML API invocation, \tool analyzes all the if-branches that have dependency on the ML API's output. 
\shan{hmmm, I feel your paper discussion so far has never talked about ``combination of branch decisions''. I don't have a clear picture about how it would fit our taxonomy ...}\cc{Updated}
Particularly, we focus on the branch conditions that software compares ML API output with certain values to make selection decisions, which are typically reflected by whether executing the target branch edge.
For each possible software decisions, \tool adopts standard symbolic execution to find all the API outputs that lead to these decisions, which is the corresponding target class.
If the software specifies only one target class\shan{what exactly does this mean ...}\cc{Done}, \tool reports pattern True-False. Otherwise, \tool analyzes the code structure to determine the pattern. % according to Figure~\ref{fig:hierarchy}:

\emph{Whether multi-select or multi-choice?} \tool analyzes all the statements inside the edges of an \shan{What is the definition of ML-API-related if-branch? I know we probably already used this phrase before. However, here, we are talking about static analysis, so we need to be particularly precise.}\cc{Done} if-branch that compares ML API output with target class. If the software exits the examination process after making a selection \shan{no no no. This is not a precise PL language. I don't know what you mean by ``terminates all examination inside one ...''. If you are doing control flow analysis here, you need to use control flow language to describe your algorithm.}\cc{How about this?} (\eg a break statement inside the loop and a return statement inside a function body), \tool regards that it as a multi-choice and further examines the order. 
If there is no such exit\shan{``termination'' usually refers to the termination of a program.}\cc{Done}, \tool determines it is multi-select structure. 


\emph{How is the order determined?} \tool finds all the loop structures\shan{??? what are ``equivalent statements''???}\cc{Removed. I put that phrase just in case there are other statements that lead to loop-like control flow} outside the ML-API-related if-branches. It analysis their nested levels and the data dependency relationship of their iterators -- due to Python syntax, the loop structure typically directly specify the list/set to be iterated (\eg~\code{for iterator in list}).
If the software does not contain any loop iterating ML API's output or application choices, \tool stops examination and reports an absence of code pattern. 
If an inner (outer) loop iterates\shan{how do you even know what variables a loop ``iterates'' through??? For example, in LLVM, index variables are identified for certain simple loops, but not all. I cannot believe you can identify what variables a loop ``iterates'' through for any type of loops. There must be unwritten assumptions here.}\cc{There's a widely-used Python syntax \code{for iter in list}. } the ML API's output and the outer (inner) loop iterates the application choices, \tool regards it as pattern Application-choice order (API-output order).  Note that, if the software contains multiple nested loops iterating the same variable, \tool focuses on the innermost one.


\subsection{How to integrate \tool in the MLaaS backend}
\label{sec:runtime}
TO-DO
To apply the \tool in xx,  we still keep the ML API, when users 

\tool modifies the MLaaS backend to serve the customized ML model per application. 
The MLaaS backend, as described in \S\ref{sec:overall}, adds the ML model to a model pool.
As depicted in Figure~\ref{fig:system}, when a user of an application queries the ML API, same as existing ML API querying, he/she first sets up a per-application authentication credential~\cite{google-cloud}, which is used for billing purposes. Then, when the user feeds the input to the ML API, the backend of MLaaS probes the model pool of customized ML models, selects the right model customized to the 

==> bk/macros.tex <==


% \newcommand{\shan}[1]{{\color{red}(Shan: #1)}}
% \newcommand{\hank}[1]{{\color{blue}(Hank: #1)}}
% \newcommand{\mm}[1]{{\color{violet}(Michael：#1)}}
% \newcommand{\cc}[1]{{\color{cyan!70!blue}{(Wan: #1)}}}
% \newcommand{\jc}[1]{{\footnotesize\color{orange}{(JC: #1)}}}
% \newcommand{\yh}[1]{{\color{deepgreen}{(Yuhan: #1)}}}
% \newcommand{\kt}[1]{{\color{brown}{(Kuntai: #1)}}}


\newcommand{\shan}[1]{}
\newcommand{\hank}[1]{ }
\newcommand{\mm}[1]{ }
\newcommand{\cc}[1]{ }
\newcommand{\jc}[1]{ }
\newcommand{\yh}[1]{ }
\newcommand{\kt}[1]{ }

\newcommand{\edit}[1]{{\color{red}{#1}}}



\newcommand{\Decision}{Decision\xspace}
\newcommand{\x}{\ensuremath{\mathbf{x}}\xspace}
\newcommand{\y}{\ensuremath{\mathbf{y}}\xspace}
\newcommand{\z}{\ensuremath{z}\xspace}
\newcommand{\X}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\TestNum}{\ensuremath{T}\xspace}
\newcommand{\APIcomp}{App \circ Filter\xspace}
\newcommand{\Filter}{F\xspace}
\newcommand{\DNN}{DNN\xspace}
\newcommand{\API}{API\xspace}
\newcommand{\Appdecision}{App\xspace}
% \newcommand{\k}{\ensuremath{k}\xspace}
\newcommand{\total}{\ensuremath{t}\xspace}
\newcommand{\NTarget}{\ensuremath{N}\xspace}
\newcommand{\other}{\ensuremath{O}\xspace}

\newcommand{\Rate}{IDR\xspace}

\newcommand{\T}{\ensuremath{T}\xspace}
\newcommand{\Match}{\ensuremath{M}\xspace}
\newcommand{\BeforeBreak}{\ensuremath{B}\xspace}

\newcommand{\App}{$A$\xspace}
% \newcommand{\F}{$Thresh_{low}$\xspace}
\newcommand{\M}{\ensuremath{M}\xspace}
\newcommand{\F}{\ensuremath{\alpha}\xspace}
\newcommand{\G}{\ensuremath{\beta}\xspace}
\newcommand{\Q}{\ensuremath{\gamma}\xspace}
\newcommand{\ClassId}{\ensuremath{c}\xspace}
\newcommand{\LabelId}{\ensuremath{l}\xspace}
\newcommand{\InputId}{\ensuremath{i}\xspace}
\newcommand{\TraverseId}{\ensuremath{j}\xspace}
\newcommand{\score}{effective score\xspace}
\newcommand{\scores}{effective scores\xspace}
\newcommand{\Tg}{\ensuremath{TC}\xspace}
\newcommand{\TargetSet}{\ensuremath{G}\xspace}
\newcommand{\MaxScore}{\ensuremath{f(\y)}\xspace}

% \newcommand{\Q}{$Thresh_{high}$\xspace}
\newcommand{\summary}{decision-process summary\xspace}
\newcommand{\Summary}{Decision-process summary\xspace}
\newcommand{\summaries}{decision-process summaries\xspace}
\newcommand{\target}{target class\xspace}
\newcommand{\targets}{target classes\xspace}
\newcommand{\Target}{Target class\xspace}
\newcommand{\process}{software decision process\xspace}
\newcommand{\Process}{Software decision process\xspace}
\newcommand{\bestapi}{Best-of-all API*\xspace}


\newcommand{\name}{ChameleonAPI\xspace}
\newcommand{\modeld}{$\textrm{ChameleonAPI}_{basic}$\xspace}
\newcommand{\tool}{ChameleonAPI\xspace}
\newcommand{\toolbasic}{\ensuremath{\textrm{ChameleonAPI}_{basic}}\xspace}
\newcommand{\code}[1]{{\texttt{#1}}}
\newcommand{\term}[1]{\textsf{#1}}
\newcommand{\wl}{\emph{whitelist}\xspace}
\newcommand{\wls}{\emph{whitelists}\xspace}
\newcommand{\ift}{\emph{if/then branch}\xspace}
\newcommand{\ifts}{\emph{if/then branches}\xspace}


\newcommand{\fillme}{{\bf XXX}\xspace}


\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,fill,inner sep=2pt] (char) {\textcolor{white}{\footnotesize{#1}}};}}



\newcounter{packednmbr}
\newenvironment{packedenumerate}{\begin{list}{\thepackednmbr.}{\usecounter{packednmbr}\setlength{\itemsep}{0.5pt}\addtolength{\labelwidth}{-4pt}\setlength{\leftmargin}{2ex}\setlength{\listparindent}{\parindent}\setlength{\parsep}{1pt}\setlength{\topsep}{0pt}}}{\end{list}}
\newenvironment{packeditemize}{\begin{list}{$\bullet$}{\setlength{\itemsep}{0.5pt}\addtolength{\labelwidth}{-4pt}\setlength{\leftmargin}{2ex}\setlength{\listparindent}{\parindent}\setlength{\parsep}{1pt}\setlength{\topsep}{2pt}}}{\end{list}}
\newenvironment{packedpackeditemize}{\begin{list}{$\bullet$}{\setlength{\itemsep}{0.5pt}\addtolength{\labelwidth}{-4pt}\setlength{\leftmargin}{\labelwidth}\setlength{\listparindent}{\parindent}\setlength{\parsep}{1pt}\setlength{\topsep}{0pt}}}{\end{list}}
\newenvironment{packedtrivlist}{\begin{list}{\setlength{\itemsep}{0.2pt}\addtolength{\labelwidth}{-4pt}\setlength{\leftmargin}{\labelwidth}\setlength{\listparindent}{\parindent}\setlength{\parsep}{1pt}\setlength{\topsep}{0pt}}}{\end{list}}
\let\enumerate\packedenumerate
\let\endenumerate\endpackedenumerate
\let\itemize\packeditemize
\let\enditemize\endpackeditemize


\newcommand{\tightcaption}[1]{\vspace{-0.15cm}\caption{{\normalfont{\textit{{#1}}}}}\vspace{-0.3cm}}
\newcommand{\tightsection}[1]{\vspace{-0.2cm}\section{#1}\vspace{-0.1cm}}
\newcommand{\tightsectionstar}[1]{\vspace{-0.17cm}\section*{#1}\vspace{-0.08cm}}
\newcommand{\tightsubsection}[1]{\vspace{-0.25cm}\subsection{#1}\vspace{-0.1cm}}
\newcommand{\tightsubsubsection}[1]{\vspace{-0.01in}\subsubsection{#1}\vspace{-0.01cm}}

\newcommand{\eg}{{\it e.g.,}\xspace}
\newcommand{\ie}{{\it i.e.,}\xspace}
\newcommand{\etal}{{\it et.~al}\xspace}
\newcommand{\bigO}{\mathrm{O}}
\newcommand{\twlog}{w.l.o.g.\xspac}

\newcommand{\myparashort}[1]{\vspace{0.05cm}\noindent{\bf {#1}}~}
\newcommand{\mypara}[1]{\vspace{0.05cm}\noindent{\bf {#1}:}~}
\newcommand{\myparatight}[1]{\vspace{0.02cm}\noindent{\bf {#1}:}~}
\newcommand{\myparaq}[1]{\smallskip\noindent{\bf {#1}?}~}
\newcommand{\myparaittight}[1]{\smallskip\noindent{\emph {#1}:}~}
\newcommand{\question}[1]{\smallskip\noindent{\emph{Q:~#1}}\smallskip}
\newcommand{\myparaqtight}[1]{\smallskip\noindent{\bf {#1}}~}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


% \definecolor{codegreen}{rgb}{0,0.6,0}
% \definecolor{codegray}{rgb}{0.5,0.5,0.5}
% \definecolor{codepurple}{rgb}{0.58,0,0.82}
% \definecolor{backcolour}{rgb}{0.95,0.95,0.92}

% \lstdefinestyle{overleaf_style}{
%     backgroundcolor=\color{backcolour},   
%     commentstyle=\color{codegreen},
%     keywordstyle=\color{magenta},
%     numberstyle=\tiny\color{codegray},
%     stringstyle=\color{codepurple},
%     basicstyle=\ttfamily\footnotesize,
%     breakatwhitespace=false,         
%     breaklines=true,                 
%     captionpos=b,                    
%     keepspaces=true,                 
%     numbers=left,                    
%     numbersep=5pt,                  
%     showspaces=false,                
%     showstringspaces=false,
%     showtabs=false,                  
%     tabsize=2
% }

\definecolor{backcolour}{rgb}{0.96,0.96,0.96}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{deepblue}{rgb}{0,0,0.6}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    morekeywords={self, True},
    keywordstyle=\color{deepblue},
    numberstyle=\tiny\color{codegray},
    emph={MyClass,__init__,EncodingType,Image},
    emphstyle=\color{deepred},
    stringstyle=\color{deepgreen},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=1
}

